Oxygen Abundances in Nearby FGK Stars and the Galactic Chemical Evolution of the Local Disk and Halo

Atmospheric parameters and oxygen abundances of 825 nearby FGK stars are derived using high-quality spectra and a non-LTE analysis of the 777 nm O I triplet lines. We assign a kinematic probability for the stars to be thin-disk (P1), thick-disk (P2), and halo (P3) members. We confirm previous findings of enhanced [O/Fe] in thick-disk (P2>0.5) relative to thin-disk (P1>0.5) stars with [Fe/H]<-0.2, as well as a "knee" that connects the mean [O/Fe]-[Fe/H] trend of thick-disk stars with that of thin-disk members at [Fe/H]>-0.2. Nevertheless, we find that the kinematic membership criterion fails at separating perfectly the stars in the [O/Fe]-[Fe/H] plane, even when a very restrictive kinematic separation is employed. Stars with "intermediate" kinematics (P1<0.7, P2<0.7) do not all populate the region of the [O/Fe]-[Fe/H] plane intermediate between the mean thin-disk and thick-disk trends, but their distribution is not necessarily bimodal. Halo stars (P3>0.5) show a large star-to-star scatter in [O/Fe]-[Fe/H], but most of it is due to stars with Galactocentric rotational velocity V<-200 km/s; halo stars with V>-200 km/s follow an [O/Fe]-[Fe/H] relation with almost no star-to-star scatter. Early mergers with satellite galaxies explain most of our observations, but the significant fraction of disk stars with "ambiguous" kinematics and abundances suggests that scattering by molecular clouds and radial migration have both played an important role in determining the kinematic and chemical properties of solar neighborhood stars.

==> t2_complete.tex <==
  HD 32071 &   8.93 &        \nodata &$   8.3\pm  0.5$&$ -24.0\pm  2.5$&$ -25.0\pm  2.5$&$  56.0\pm  2.5$&  0.77 &  0.22 &  0.00 \\
  HD 59490 &   8.68 &        \nodata &$  91.0\pm  0.5$&$ -83.0\pm  2.5$&$ -49.0\pm  2.5$&$ -17.0\pm  2.5$&  0.70 &  0.30 &  0.00 \\
  HD 67163 &   8.05 &        \nodata &$  65.3\pm  0.5$&$ -16.0\pm  2.5$&$ -64.0\pm  2.5$&$  -4.0\pm  2.5$&  0.70 &  0.30 &  0.00 \\
  HD 82960 &   8.53 &        \nodata &$  46.0\pm  0.5$&$  28.0\pm  2.5$&$ -58.0\pm  2.5$&$   5.0\pm  2.5$&  0.80 &  0.19 &  0.00 \\
 HD 130047 &   8.56 &        \nodata &$  15.9\pm  0.5$&$  41.0\pm  2.5$&$ -63.0\pm  2.5$&$ -21.0\pm  2.5$&  0.57 &  0.43 &  0.00 \\
 HD 144070 &   4.84 &   $43.0\pm4.2$ &$ -32.6\pm  1.1$&$ -30.0\pm  2.5$&$  -6.0\pm  2.5$&$ -14.0\pm  2.5$&  0.99 &  0.01 &  0.00 \\
 HD 170058 &   8.42 &        \nodata &$ -21.2\pm  0.5$&$   3.0\pm  2.5$&$ -49.0\pm  2.5$&$ -28.0\pm  2.5$&  0.86 &  0.14 &  0.00 \\
 HD 171029 &   8.24 &        \nodata &$ -37.8\pm  0.5$&$ -22.0\pm  2.5$&$ -65.0\pm  2.5$&$  -7.0\pm  2.5$&  0.65 &  0.34 &  0.00 \\
 HD 183490 &   8.22 &        \nodata &$ -66.1\pm  0.7$&$  -5.0\pm  2.5$&$ -71.0\pm  2.5$&$   0.0\pm  2.5$&  0.50 &  0.49 &  0.00 \\
 HD 213746 &   8.55 &        \nodata &$ -59.1\pm  1.9$&$  -2.0\pm  2.5$&$ -71.0\pm  2.5$&$ -15.0\pm  2.5$&  0.45 &  0.54 &  0.01 \\
 HD 223723 &   8.60 &        \nodata &$   4.3\pm  0.5$&$ -85.0\pm  2.5$&$ -35.0\pm  2.5$&$ -26.0\pm  2.5$&  0.83 &  0.17 &  0.00 \\
   HIP 171 &   5.74 & $82.17\pm2.23$ &$ -36.9\pm  0.5$&$  -8.0\pm  0.7$&$ -73.1\pm  1.7$&$ -31.1\pm  2.0$&  0.23 &  0.76 &  0.01 \\
   HIP 348 &   8.62 & $17.43\pm0.90$ &$  18.1\pm  0.5$&$ -94.0\pm  6.1$&$ -12.1\pm  1.6$&$ -12.2\pm  0.4$&  0.94 &  0.06 &  0.00 \\
   HIP 394 &   6.11 & $25.52\pm3.28$ &$   4.6\pm  0.5$&$-124.8\pm 19.4$&$ -51.3\pm  8.7$&$ -10.9\pm  1.5$&  0.27 &  0.71 &  0.02 \\
   HIP 475 &   8.22 & $19.01\pm0.82$ &$ -28.4\pm  0.5$&$   6.8\pm  0.4$&$ -31.4\pm  0.6$&$ -36.7\pm  2.0$&  0.93 &  0.07 &  0.00 \\
   HIP 493 &   7.45 & $26.93\pm0.56$ &$ -45.6\pm  0.5$&$  45.8\pm  1.1$&$ -34.2\pm  0.4$&$  17.0\pm  0.6$&  0.95 &  0.05 &  0.00 \\
   HIP 522 &   5.70 & $38.89\pm0.37$ &$   5.3\pm  0.5$&$ -57.4\pm  1.0$&$ -37.5\pm  0.6$&$ -15.3\pm  0.5$&  0.93 &  0.07 &  0.00 \\
   HIP 530 &   8.35 &  $9.38\pm0.71$ &$ -31.8\pm  0.5$&$ -28.2\pm  4.5$&$ -48.5\pm  2.4$&$   2.8\pm  0.9$&  0.92 &  0.08 &  0.00 \\
   HIP 544 &   6.10 & $73.15\pm0.56$ &$  -6.9\pm  0.5$&$ -15.0\pm  0.2$&$ -21.6\pm  0.4$&$ -10.1\pm  0.3$&  0.99 &  0.01 &  0.00 \\
   HIP 656 &   8.15 &  $9.14\pm0.98$ &$ -42.5\pm  0.5$&$  -5.8\pm  2.5$&$ -55.7\pm  1.9$&$ -29.0\pm  3.6$&  0.74 &  0.25 &  0.00 \\
   HIP 768 &   7.94 & $14.68\pm0.85$ &$ -31.0\pm  0.5$&$ -80.8\pm  8.4$&$ -58.5\pm  3.5$&$  15.0\pm  0.7$&  0.50 &  0.49 &  0.01 \\
   HIP 950 &   5.24 & $47.00\pm0.27$ &$  -1.6\pm  0.5$&$ -20.8\pm  0.3$&$   2.2\pm  0.1$&$  -2.7\pm  0.5$&  0.99 &  0.01 &  0.00 \\
   HIP 996 &   8.20 & $18.58\pm0.84$ &$ -48.6\pm  0.5$&$ -30.9\pm  2.3$&$ -61.8\pm  1.5$&$  20.4\pm  0.7$&  0.64 &  0.35 &  0.00 \\
  HIP 1105 &   8.07 &  $9.86\pm0.66$ &$   9.5\pm  0.5$&$ -39.3\pm  3.1$&$ -10.8\pm  1.8$&$  -0.4\pm  0.4$&  0.99 &  0.01 &  0.00 \\
  HIP 1128 &   8.37 & $23.50\pm1.02$ &$ -23.4\pm  8.5$&$ -54.3\pm  2.7$&$ -79.3\pm  4.5$&$  -0.6\pm  8.2$&  0.14 &  0.84 &  0.01 \\
  HIP 1297 &   8.92 & $14.98\pm0.86$ &$ -19.3\pm  0.8$&$ -50.0\pm  3.7$&$ -25.1\pm  0.9$&$  39.0\pm  2.0$&  0.91 &  0.09 &  0.00 \\
  HIP 1411 &   9.06 & $14.82\pm0.97$ &$ -50.9\pm  2.2$&$  77.7\pm  4.6$&$ -24.4\pm  2.2$&$   1.2\pm  1.9$&  0.95 &  0.05 &  0.00 \\
  HIP 1499 &   6.45 & $43.02\pm0.51$ &$ -10.5\pm  0.5$&$ -31.6\pm  0.6$&$ -39.0\pm  0.7$&$  -1.3\pm  0.5$&  0.96 &  0.04 &  0.00 \\
  HIP 1599 &   4.23 & $116.46\pm0.16 &$   9.1\pm  0.5$&$ -72.1\pm  0.5$&$  -3.7\pm  0.2$&$ -44.3\pm  0.4$&  0.88 &  0.12 &  0.00 \\
  HIP 1813 &   7.58 & $24.83\pm0.46$ &$ -31.1\pm  2.8$&$  -7.2\pm  1.1$&$ -63.0\pm  2.5$&$ -16.4\pm  2.2$&  0.68 &  0.31 &  0.00 \\
  HIP 2021 &   2.80 & $134.07\pm0.11 &$  22.4\pm  0.5$&$ -60.9\pm  0.3$&$ -46.4\pm  0.3$&$ -31.0\pm  0.3$&  0.75 &  0.24 &  0.00 \\
  HIP 2131 &   8.92 & $14.02\pm1.02$ &$ -26.3\pm  0.5$&$ -32.5\pm  3.4$&$ -47.5\pm  1.9$&$  34.0\pm  2.4$&  0.80 &  0.20 &  0.00 \\
  HIP 2453 &   7.37 & $24.89\pm0.45$ &$  12.5\pm  0.5$&$ -56.9\pm  1.4$&$ -17.2\pm  0.9$&$ -17.3\pm  0.5$&  0.97 &  0.03 &  0.00 \\
  HIP 2711 &   5.57 & $39.24\pm0.34$ &$  36.2\pm  0.6$&$ -15.9\pm  0.4$&$ -22.6\pm  0.3$&$ -36.5\pm  0.5$&  0.96 &  0.04 &  0.00 \\
  HIP 2712 &   7.38 & $22.12\pm0.61$ &$ -12.6\pm  0.5$&$ -72.4\pm  3.2$&$ -53.7\pm  1.8$&$  10.3\pm  0.3$&  0.71 &  0.29 &  0.00 \\
  HIP 2760 &   7.38 & $21.47\pm1.24$ &$ -65.5\pm  0.5$&$  27.1\pm  0.4$&$ -64.2\pm  0.6$&$ -12.3\pm  1.1$&  0.64 &  0.35 &  0.00 \\
  HIP 2894 &   8.66 & $17.50\pm1.18$ &$   4.9\pm  0.5$&$ -15.1\pm  0.9$&$  -5.1\pm  0.8$&$  -7.0\pm  0.5$&  0.99 &  0.01 &  0.00 \\
  HIP 2909 &   8.18 & $17.00\pm0.81$ &$  26.2\pm  0.5$&$  28.6\pm  2.0$&$ -65.1\pm  4.8$&$ -30.1\pm  0.6$&  0.44 &  0.55 &  0.01 \\
  HIP 2981 &   7.53 & $22.05\pm0.72$ &$  31.5\pm  2.0$&$ -33.5\pm  1.3$&$   9.2\pm  1.8$&$ -28.1\pm  1.1$&  0.98 &  0.02 &  0.00 \\
  HIP 3014 &   8.38 & $10.62\pm0.71$ &$   6.8\pm  0.5$&$ -14.4\pm  1.2$&$ -11.0\pm  1.5$&$ -12.9\pm  0.9$&  0.99 &  0.01 &  0.00 \\
  HIP 3026 &   9.14 &  $9.51\pm1.11$ &$ -50.2\pm  1.0$&$ 135.9\pm 18.8$&$-236.6\pm 31.9$&$ -40.5\pm 12.7$&  0.00 &  0.00 &  1.00 \\
  HIP 3086 &   7.34 & $20.25\pm0.66$ &$ -27.9\pm  0.5$&$-168.8\pm  7.0$&$ -54.7\pm  1.7$&$  48.5\pm  1.1$&  0.00 &  0.81 &  0.19 \\
  HIP 3093 &   5.88 & $90.42\pm0.32$ &$ -33.5\pm  0.5$&$  40.3\pm  0.3$&$ -19.9\pm  0.3$&$   8.8\pm  0.3$&  0.98 &  0.02 &  0.00 \\
  HIP 3132 &   6.40 & $30.07\pm0.28$ &$ -34.7\pm  0.5$&$  34.0\pm  0.4$&$ -22.1\pm  0.4$&$   0.3\pm  0.3$&  0.98 &  0.02 &  0.00 \\
  HIP 3185 &   6.14 & $34.62\pm0.45$ &$ -48.2\pm  0.5$&$ -47.5\pm  1.0$&$ -90.3\pm  1.8$&$  41.6\pm  0.5$&  0.01 &  0.96 &  0.03 \\
  HIP 3206 &   7.36 & $57.71\pm0.80$ &$ -63.9\pm  0.5$&$  18.3\pm  0.3$&$ -82.8\pm  0.7$&$ -27.1\pm  0.9$&  0.08 &  0.91 &  0.01 \\
  HIP 3272 &   7.84 & $17.11\pm0.68$ &$  -1.3\pm  0.5$&$ -13.2\pm  0.8$&$ -22.3\pm  1.3$&$ -12.0\pm  0.8$&  0.99 &  0.01 &  0.00 \\
  HIP 3441 &   9.36 &  $9.28\pm1.22$ &$-108.3\pm  1.0$&$  79.2\pm  7.1$&$ -71.4\pm  4.4$&$  79.3\pm  2.7$&  0.00 &  0.91 &  0.09 \\
  HIP 3765 &   5.74 & $134.14\pm0.51 &$ -10.8\pm  0.5$&$  -1.0\pm  0.1$&$ -47.9\pm  0.4$&$ -12.8\pm  0.4$&  0.92 &  0.08 &  0.00 \\
  HIP 3821 &   3.44 & $167.98\pm0.48 &$   8.2\pm  0.5$&$ -29.4\pm  0.3$&$ -10.8\pm  0.4$&$ -16.7\pm  0.1$&  0.99 &  0.01 &  0.00 \\
  HIP 4039 &   9.77 &  $6.55\pm1.06$ &$  -5.3\pm  1.0$&$-126.1\pm 21.0$&$ -97.8\pm 15.2$&$  39.4\pm  6.6$&  0.00 &  0.86 &  0.14 \\
  HIP 4127 &   6.78 & $23.94\pm0.55$ &$ -73.9\pm  0.6$&$  50.4\pm  0.6$&$ -43.8\pm  0.7$&$  37.9\pm  0.4$&  0.76 &  0.24 &  0.00 \\
  HIP 4148 &   7.16 & $70.56\pm0.61$ &$ -13.3\pm  0.5$&$ -36.2\pm  0.4$&$ -20.2\pm  0.2$&$  13.4\pm  0.5$&  0.98 &  0.02 &  0.00 \\
  HIP 4151 &   4.80 & $53.35\pm0.33$ &$  20.8\pm  0.5$&$  -6.5\pm  0.3$&$  21.1\pm  0.4$&$  14.3\pm  0.2$&  0.99 &  0.01 &  0.00 \\
  HIP 4195 &   8.67 & $18.06\pm0.76$ &$  14.1\pm  1.6$&$  -1.2\pm  0.4$&$ -79.6\pm  5.6$&$ -17.3\pm  1.6$&  0.18 &  0.81 &  0.01 \\
  HIP 4457 &   7.94 & $12.99\pm0.75$ &$ -19.9\pm  7.4$&$  25.4\pm  3.9$&$   2.0\pm  5.6$&$  18.6\pm  3.6$&  0.99 &  0.01 &  0.00 \\
  HIP 4544 &   9.72 &  $9.23\pm1.03$ &$-112.2\pm  1.0$&$ -43.5\pm 12.9$&$-138.7\pm  6.2$&$ -81.6\pm  6.3$&  0.00 &  0.43 &  0.57 \\
  HIP 4909 &   8.55 & $17.72\pm1.11$ &$  -3.5\pm  0.5$&$  -2.2\pm  0.4$&$   2.3\pm  0.3$&$   4.7\pm  0.5$&  0.99 &  0.01 &  0.00 \\
  HIP 5016 &   6.83 & $15.73\pm0.51$ &$ -39.1\pm  0.6$&$  56.2\pm  1.6$&$ -11.8\pm  1.0$&$ -14.6\pm  0.9$&  0.98 &  0.02 &  0.00 \\
  HIP 5106 &   8.25 & $19.57\pm0.92$ &$ -28.8\pm  0.5$&$ -34.8\pm  2.8$&$ -58.1\pm  1.9$&$ -40.0\pm  2.2$&  0.46 &  0.53 &  0.01 \\
  HIP 5122 &   8.74 &  $9.91\pm0.71$ &$   8.9\pm  1.0$&$-103.2\pm  7.4$&$ -78.2\pm  6.4$&$  41.6\pm  2.8$&  0.01 &  0.94 &  0.05 \\
  HIP 5134 &   8.95 &  $6.97\pm1.34$ &$  -3.1\pm  0.5$&$  13.8\pm  1.1$&$   7.3\pm  0.7$&$   1.7\pm  0.5$&  0.99 &  0.01 &  0.00 \\
  HIP 5163 &   9.43 & $10.84\pm1.29$ &$  26.1\pm  1.0$&$ -31.0\pm  2.4$&$ -64.6\pm  7.9$&$ -46.0\pm  2.6$&  0.21 &  0.78 &  0.01 \\
  HIP 5315 &   6.46 & $20.63\pm0.45$ &$ -94.7\pm  0.5$&$  49.9\pm  0.8$&$-122.9\pm  3.4$&$  38.2\pm  1.8$&  0.00 &  0.88 &  0.12 \\
  HIP 5336 &   5.16 & $132.38\pm0.82 &$ -98.3\pm  0.5$&$ -42.5\pm  0.5$&$-157.8\pm  0.5$&$ -35.2\pm  0.2$&  0.00 &  0.47 &  0.53 \\
  HIP 5441 &   8.42 & $11.34\pm0.69$ &$  31.3\pm  0.5$&$ -11.9\pm  0.7$&$  18.1\pm  0.6$&$ -29.1\pm  1.6$&  0.98 &  0.02 &  0.00 \\
  HIP 5531 &   6.55 & $18.30\pm0.53$ &$ -10.5\pm  0.5$&$ -48.9\pm  2.1$&$ -47.9\pm  1.6$&$  10.6\pm  0.5$&  0.88 &  0.11 &  0.00 \\
  HIP 5682 &   7.41 & $17.26\pm0.72$ &$ -21.1\pm  0.5$&$  41.8\pm  1.9$&$  -6.4\pm  0.6$&$ -11.6\pm  1.4$&  0.99 &  0.01 &  0.00 \\
  HIP 5775 &  10.00 &  $6.15\pm1.95$ &$  81.8\pm  1.0$&$ -69.7\pm 14.1$&$-102.9\pm 29.0$&$ -81.6\pm  1.1$&  0.00 &  0.78 &  0.22 \\
  HIP 5862 &   4.96 & $66.16\pm0.24$ &$  11.7\pm  0.5$&$ -44.4\pm  0.4$&$ -21.5\pm  0.2$&$ -10.7\pm  0.5$&  0.98 &  0.02 &  0.00 \\
  HIP 6159 &   8.90 & $15.35\pm1.17$ &$  -6.7\pm  1.0$&$ 138.2\pm 11.4$&$ -73.2\pm  5.9$&$ -47.2\pm  4.5$&  0.00 &  0.89 &  0.11 \\
  HIP 6407 &   8.55 & $17.49\pm0.97$ &$   5.7\pm  0.5$&$   8.4\pm  0.8$&$ -37.5\pm  2.7$&$ -26.0\pm  1.5$&  0.94 &  0.05 &  0.00 \\
  HIP 6607 &   8.30 & $25.06\pm0.94$ &$  84.3\pm  0.5$&$ -25.5\pm  0.9$&$ -85.9\pm  3.9$&$ -75.2\pm  0.6$&  0.00 &  0.93 &  0.07 \\
  HIP 6711 &   5.96 & $23.97\pm0.45$ &$  31.2\pm  0.5$&$ -34.5\pm  0.6$&$   6.1\pm  0.6$&$ -18.4\pm  0.3$&  0.99 &  0.01 &  0.00 \\
  HIP 6762 &   7.94 & $34.07\pm1.00$ &$  13.1\pm  1.4$&$ -13.7\pm  0.6$&$ -59.1\pm  1.9$&$ -28.7\pm  1.3$&  0.66 &  0.33 &  0.00 \\
  HIP 6975 &   7.62 & $20.68\pm0.82$ &$ -50.8\pm  0.5$&$  39.4\pm  0.7$&$ -28.3\pm  0.3$&$  21.6\pm  0.6$&  0.97 &  0.03 &  0.00 \\
  HIP 6978 &   7.95 & $24.91\pm0.77$ &$  11.3\pm  0.5$&$ -42.7\pm  1.6$&$ -20.3\pm  1.3$&$   1.1\pm  0.4$&  0.98 &  0.02 &  0.00 \\
  HIP 7221 &   8.40 & $19.97\pm0.82$ &$ -20.4\pm  0.5$&$ -29.0\pm  2.2$&$ -47.2\pm  1.7$&$  15.0\pm  0.6$&  0.91 &  0.09 &  0.00 \\
  HIP 7245 &   8.35 & $19.10\pm1.06$ &$  21.4\pm  0.5$&$ -46.5\pm  1.9$&$ -22.8\pm  2.0$&$ -15.2\pm  0.4$&  0.98 &  0.02 &  0.00 \\
  HIP 7312 &   8.90 &  $7.47\pm1.25$ &$  29.8\pm  0.5$&$  14.6\pm  3.8$&$ -30.3\pm  5.5$&$ -52.9\pm  3.9$&  0.79 &  0.21 &  0.00 \\
  HIP 7357 &   6.92 & $27.03\pm0.60$ &$ -22.7\pm  0.5$&$   3.4\pm  0.3$&$ -63.5\pm  1.9$&$   3.6\pm  0.7$&  0.72 &  0.28 &  0.00 \\
  HIP 7513 &   4.09 & $74.12\pm0.19$ &$ -28.9\pm  0.5$&$  28.9\pm  0.3$&$ -22.7\pm  0.3$&$ -14.1\pm  0.3$&  0.98 &  0.02 &  0.00 \\
  HIP 7612 &   8.18 & $13.52\pm0.78$ &$  27.5\pm  0.5$&$-100.2\pm  6.7$&$ -45.9\pm  5.0$&$   9.4\pm  1.9$&  0.66 &  0.33 &  0.01 \\
 HIP 7751B &   5.96 & $127.84\pm2.19 &$  20.2\pm  0.5$&$  -5.5\pm  0.1$&$ -16.0\pm  0.3$&$ -15.7\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 7751A &   5.81 & $127.84\pm2.19 &$  21.5\pm  0.5$&$  -5.2\pm  0.1$&$ -16.6\pm  0.3$&$ -16.8\pm  0.4$&  0.99 &  0.01 &  0.00 \\
  HIP 7885 &   8.67 & $14.55\pm0.83$ &$  32.0\pm  0.5$&$ -10.5\pm  0.6$&$ -65.5\pm  4.2$&$ -19.8\pm  1.0$&  0.58 &  0.41 &  0.00 \\
  HIP 7902 &   7.70 & $26.84\pm0.78$ &$  17.4\pm  0.5$&$-111.9\pm  3.5$&$ -62.8\pm  2.7$&$ -20.3\pm  0.8$&  0.13 &  0.84 &  0.03 \\
  HIP 7918 &   4.95 & $78.50\pm0.54$ &$   3.0\pm  0.5$&$ -37.5\pm  0.5$&$ -31.1\pm  0.5$&$  -1.8\pm  0.2$&  0.97 &  0.03 &  0.00 \\
  HIP 7961 &   7.46 & $20.99\pm0.73$ &$  -8.5\pm  0.8$&$ -96.6\pm  4.8$&$ -76.2\pm  3.7$&$  33.5\pm  1.4$&  0.02 &  0.94 &  0.04 \\
  HIP 7978 &   5.54 & $57.36\pm0.25$ &$  28.0\pm  1.0$&$  -1.1\pm  0.2$&$ -26.8\pm  0.5$&$ -18.2\pm  0.9$&  0.98 &  0.02 &  0.00 \\
  HIP 7981 &   5.24 & $132.76\pm0.50 &$ -34.2\pm  0.5$&$  34.9\pm  0.3$&$ -25.1\pm  0.3$&$   2.9\pm  0.4$&  0.98 &  0.02 &  0.00 \\
  HIP 8102 &   3.49 & $273.96\pm0.17 &$ -17.1\pm  0.5$&$  18.9\pm  0.1$&$  29.4\pm  0.1$&$  13.3\pm  0.5$&  0.98 &  0.02 &  0.00 \\
  HIP 8121 &   8.11 & $17.58\pm0.74$ &$   3.5\pm  0.6$&$  60.3\pm  3.9$&$ -57.8\pm  3.6$&$ -16.4\pm  1.0$&  0.65 &  0.34 &  0.00 \\
  HIP 8362 &   5.63 & $99.33\pm0.53$ &$   2.5\pm  0.5$&$ -24.5\pm  0.4$&$ -16.5\pm  0.4$&$  -5.4\pm  0.1$&  0.99 &  0.01 &  0.00 \\
  HIP 8433 &   5.78 & $35.90\pm0.34$ &$ -24.3\pm  0.5$&$  25.4\pm  0.4$&$  18.0\pm  0.7$&$  39.6\pm  0.6$&  0.96 &  0.04 &  0.00 \\
  HIP 8476 &   8.14 & $17.72\pm0.87$ &$  30.6\pm  0.5$&$ -26.9\pm  0.6$&$  -2.5\pm  1.4$&$ -33.7\pm  1.3$&  0.98 &  0.02 &  0.00 \\
  HIP 8507 &   8.91 & $17.61\pm0.98$ &$  -9.9\pm  0.5$&$  -6.8\pm  0.8$&$  -3.1\pm  0.3$&$  12.3\pm  0.5$&  0.99 &  0.01 &  0.00 \\
  HIP 8674 &   8.95 & $19.03\pm1.36$ &$  40.6\pm  0.5$&$  19.1\pm  2.4$&$ -93.5\pm  7.1$&$ -49.6\pm  1.0$&  0.00 &  0.96 &  0.04 \\
  HIP 8720 &  10.89 & $11.31\pm1.44$ &$  -3.7\pm  1.0$&$  80.4\pm 15.0$&$ -65.0\pm 12.2$&$ -49.6\pm 10.1$&  0.06 &  0.92 &  0.03 \\
  HIP 8841 &   9.23 & $12.62\pm1.01$ &$  22.6\pm  0.5$&$   1.9\pm  1.0$&$ -63.6\pm  6.3$&$ -27.9\pm  0.8$&  0.56 &  0.44 &  0.00 \\
  HIP 8859 &   6.78 & $24.12\pm0.64$ &$ -17.1\pm  0.5$&$  58.5\pm  2.0$&$ -22.3\pm  0.7$&$ -30.0\pm  1.8$&  0.94 &  0.05 &  0.00 \\
  HIP 9080 &  10.54 & $12.28\pm2.36$ &$ -14.2\pm  1.0$&$ -93.0\pm 15.1$&$ -90.9\pm 12.7$&$  45.3\pm  5.3$&  0.00 &  0.93 &  0.07 \\
  HIP 9349 &   7.99 & $23.40\pm0.86$ &$  19.1\pm  0.5$&$ -11.7\pm  0.3$&$  -9.3\pm  0.5$&$ -16.2\pm  0.5$&  0.99 &  0.01 &  0.00 \\
  HIP 9519 &   8.20 & $19.61\pm0.97$ &$   4.2\pm  0.5$&$  -6.9\pm  0.4$&$  -5.4\pm  0.4$&$  -2.3\pm  0.4$&  0.99 &  0.01 &  0.00 \\
  HIP 9643 &   8.92 & $16.63\pm1.27$ &$   1.1\pm  0.5$&$  -2.7\pm  0.5$&$  -7.6\pm  0.9$&$  -3.3\pm  0.6$&  0.99 &  0.01 &  0.00 \\
  HIP 9884 &   2.01 & $49.56\pm0.25$ &$ -14.6\pm  1.4$&$  -0.1\pm  0.9$&$ -27.0\pm  0.8$&$   3.4\pm  0.8$&  0.98 &  0.02 &  0.00 \\
 HIP 10138 &   6.12 & $92.74\pm0.32$ &$  56.7\pm  0.5$&$ -97.6\pm  0.7$&$ -75.3\pm  0.4$&$ -29.7\pm  0.5$&  0.03 &  0.93 &  0.03 \\
 HIP 10212 &   5.63 & $24.56\pm0.30$ &$ -18.9\pm  0.5$&$  40.3\pm  1.2$&$  -3.5\pm  0.2$&$  -7.6\pm  0.9$&  0.99 &  0.01 &  0.00 \\
 HIP 10303 &   7.74 & $20.89\pm7.39$ &$  -5.8\pm  0.7$&$ -47.0\pm  2.5$&$ -65.0\pm  2.5$&$  24.0\pm  2.5$&  0.45 &  0.54 &  0.01 \\
 HIP 10322 &   7.00 & $24.40\pm0.62$ &$ -31.0\pm  0.5$&$ -22.5\pm  1.5$&$ -66.8\pm  1.5$&$ -21.8\pm  0.8$&  0.50 &  0.49 &  0.00 \\
 HIP 10449 &   9.08 & $15.87\pm1.23$ &$  27.9\pm  1.0$&$-205.9\pm 15.8$&$-201.4\pm 17.1$&$  58.4\pm  6.8$&  0.00 &  0.00 &  1.00 \\
 HIP 10644 &   4.86 & $92.73\pm0.39$ &$  -7.7\pm  0.5$&$ -34.2\pm  0.5$&$ -49.2\pm  0.5$&$  11.9\pm  0.2$&  0.89 &  0.10 &  0.00 \\
 HIP 10652 &   9.04 & $15.93\pm1.19$ &$ -20.5\pm  1.0$&$-100.6\pm 10.5$&$ -91.8\pm  7.7$&$  82.9\pm  6.5$&  0.00 &  0.76 &  0.24 \\
 HIP 10710 &   8.93 & $15.92\pm1.15$ &$  23.8\pm  0.5$&$ -32.6\pm  1.5$&$ -15.1\pm  2.2$&$ -12.7\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 10711 &   8.85 & $12.56\pm1.22$ &$  49.6\pm  1.0$&$ -92.1\pm  7.3$&$ -61.5\pm 11.8$&$ -51.0\pm  4.4$&  0.05 &  0.92 &  0.03 \\
 HIP 10798 &   6.35 & $78.93\pm0.35$ &$   7.2\pm  0.5$&$ -11.0\pm  0.2$&$  26.8\pm  0.3$&$  -9.8\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 11072 &   5.19 & $45.53\pm0.82$ &$  15.3\pm  2.3$&$ -18.4\pm  0.8$&$ -16.3\pm  0.5$&$  -7.3\pm  2.2$&  0.99 &  0.01 &  0.00 \\
 HIP 11237 &   8.44 & $12.76\pm1.16$ &$  32.5\pm  0.5$&$ -62.0\pm  4.4$&$ -22.6\pm  4.2$&$   3.0\pm  2.4$&  0.97 &  0.03 &  0.00 \\
 HIP 11309 &   7.36 & $14.80\pm0.60$ &$  -8.7\pm  0.5$&$  63.4\pm  3.5$&$ -39.5\pm  2.3$&$ -62.3\pm  4.2$&  0.25 &  0.73 &  0.02 \\
 HIP 11505 &   7.78 & $17.87\pm0.81$ &$ -62.3\pm  0.5$&$  16.4\pm  1.4$&$ -71.7\pm  1.4$&$  26.7\pm  1.4$&  0.31 &  0.68 &  0.01 \\
 HIP 11584 &   8.02 & $10.86\pm0.75$ &$  -6.0\pm  0.5$&$ -24.0\pm  3.3$&$ -47.0\pm  5.4$&$   8.1\pm  0.7$&  0.93 &  0.07 &  0.00 \\
 HIP 11728 &   8.03 & $25.11\pm0.88$ &$   4.6\pm  0.5$&$ -25.0\pm  1.1$&$  -9.0\pm  0.6$&$  17.1\pm  0.9$&  0.99 &  0.01 &  0.00 \\
 HIP 11915 &   8.61 & $17.45\pm1.07$ &$  14.1\pm  0.5$&$ -49.9\pm  3.1$&$ -33.7\pm  2.2$&$  11.3\pm  1.7$&  0.96 &  0.04 &  0.00 \\
 HIP 11923 &   7.75 & $20.05\pm0.86$ &$   9.8\pm  1.2$&$ -73.5\pm  3.5$&$ -65.4\pm  3.7$&$  19.5\pm  1.1$&  0.33 &  0.66 &  0.01 \\
 HIP 12262 &   7.50 & $12.05\pm0.62$ &$ -20.7\pm  0.5$&$   9.2\pm  0.5$&$ -17.1\pm  0.4$&$ -25.4\pm  1.4$&  0.98 &  0.02 &  0.00 \\
 HIP 12294 &  10.48 &  $5.82\pm2.18$ &$  50.6\pm  1.0$&$-195.5\pm 52.8$&$-154.5\pm 52.4$&$  65.1\pm 33.5$&  0.00 &  0.01 &  0.99 \\
 HIP 12306 &   7.36 & $29.17\pm0.81$ &$-100.1\pm  0.5$&$ 136.3\pm  2.4$&$ -31.1\pm  0.6$&$ -40.9\pm  3.5$&  0.19 &  0.77 &  0.04 \\
 HIP 12381 &   7.97 & $14.06\pm1.07$ &$  49.5\pm  0.7$&$  14.6\pm  3.9$&$ -68.4\pm  6.9$&$ -56.7\pm  1.5$&  0.06 &  0.92 &  0.02 \\
 HIP 12444 &   5.78 & $45.96\pm0.41$ &$  -1.0\pm  4.1$&$  14.1\pm  2.1$&$   3.3\pm  0.2$&$  -7.5\pm  3.5$&  0.99 &  0.01 &  0.00 \\
 HIP 12579 &   9.16 & $14.00\pm1.25$ &$ -12.5\pm  1.0$&$ -12.1\pm  2.0$&$ -60.1\pm  4.7$&$ -74.5\pm  6.9$&  0.02 &  0.95 &  0.03 \\
 HIP 12777 &   4.11 & $89.87\pm0.22$ &$  24.3\pm  0.5$&$ -30.5\pm  0.4$&$   1.2\pm  0.3$&$  -0.9\pm  0.1$&  0.99 &  0.01 &  0.00 \\
 HIP 13336 &   8.65 & $17.12\pm1.21$ &$  16.5\pm  1.0$&$-110.5\pm 12.8$&$-126.9\pm 18.0$&$ -12.8\pm  1.6$&  0.00 &  0.76 &  0.24 \\
 HIP 13366 &   8.38 & $16.39\pm1.07$ &$   6.4\pm  0.5$&$  36.3\pm  3.8$&$-105.1\pm  9.7$&$ -81.2\pm  7.1$&  0.00 &  0.83 &  0.17 \\
 HIP 13402 &   6.04 & $96.60\pm0.40$ &$  17.5\pm  0.5$&$ -15.0\pm  0.3$&$ -21.8\pm  0.2$&$  -8.7\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 14023 &   8.12 & $32.14\pm1.18$ &$  70.9\pm  0.5$&$-101.8\pm  2.3$&$ -81.3\pm  4.1$&$ -11.6\pm  1.7$&  0.02 &  0.94 &  0.03 \\
 HIP 14086 &   5.88 & $31.06\pm0.36$ &$  38.0\pm  0.5$&$   9.9\pm  0.6$&$ -82.1\pm  1.5$&$ -16.9\pm  0.6$&  0.13 &  0.86 &  0.01 \\
 HIP 14241 &   8.09 & $28.54\pm0.97$ &$ -20.5\pm  0.5$&$   5.1\pm  0.5$&$ -69.1\pm  3.0$&$  26.4\pm  0.6$&  0.40 &  0.59 &  0.01 \\
 HIP 14286 &   6.64 & $41.27\pm0.58$ &$  -2.2\pm  0.5$&$ -69.6\pm  1.4$&$ -78.5\pm  1.5$&$ -27.6\pm  0.6$&  0.06 &  0.92 &  0.02 \\
 HIP 14594 &   8.06 & $24.92\pm0.91$ &$-139.3\pm  0.5$&$ 156.0\pm  1.8$&$-123.1\pm  3.4$&$ -67.5\pm  5.7$&  0.00 &  0.25 &  0.75 \\
 HIP 14614 &   7.84 & $22.71\pm0.71$ &$ -27.5\pm  0.5$&$  25.0\pm  0.4$&$ -41.7\pm  1.5$&$  -1.1\pm  0.8$&  0.95 &  0.05 &  0.00 \\
 HIP 14632 &   4.05 & $94.87\pm0.23$ &$  49.4\pm  0.5$&$ -75.7\pm  0.5$&$ -15.7\pm  0.4$&$  21.4\pm  0.2$&  0.95 &  0.05 &  0.00 \\
 HIP 14668 &   3.80 & $28.93\pm0.21$ &$  29.2\pm  0.5$&$ -42.8\pm  0.6$&$ -15.4\pm  0.7$&$ -11.0\pm  0.2$&  0.98 &  0.02 &  0.00 \\
 HIP 14721 &   8.70 & $17.35\pm0.97$ &$ -27.7\pm  0.5$&$   1.7\pm  1.5$&$ -47.3\pm  3.1$&$  27.1\pm  0.9$&  0.88 &  0.12 &  0.00 \\
 HIP 14879 &   3.85 & $70.24\pm0.45$ &$ -19.4\pm  0.6$&$ -37.4\pm  0.5$&$  17.3\pm  0.2$&$  31.3\pm  0.5$&  0.97 &  0.03 &  0.00 \\
 HIP 15126 &  10.19 & $12.88\pm1.85$ &$  88.1\pm  1.0$&$-155.1\pm 12.4$&$ -57.3\pm  7.7$&$  28.7\pm 12.1$&  0.02 &  0.89 &  0.09 \\
 HIP 15206 &   8.03 & $10.27\pm0.76$ &$  45.1\pm  0.5$&$ -78.6\pm  4.7$&$ -55.4\pm  6.5$&$  13.7\pm  4.5$&  0.61 &  0.38 &  0.01 \\
 HIP 15249 &   8.76 & $14.85\pm0.93$ &$ -70.9\pm  1.0$&$  55.8\pm  0.8$&$ -81.9\pm  5.2$&$  19.0\pm  1.8$&  0.07 &  0.91 &  0.02 \\
 HIP 15330 &   5.53 & $83.28\pm0.20$ &$  12.1\pm  0.5$&$ -70.6\pm  0.5$&$ -46.9\pm  0.4$&$  16.1\pm  0.4$&  0.81 &  0.19 &  0.00 \\
 HIP 15371 &   5.24 & $83.11\pm0.19$ &$  11.6\pm  0.5$&$ -70.1\pm  0.5$&$ -46.3\pm  0.4$&$  16.4\pm  0.4$&  0.82 &  0.18 &  0.00 \\
 HIP 15383 &   5.40 & $14.89\pm0.84$ &$  31.7\pm  3.0$&$ -54.9\pm  3.0$&$ -69.6\pm  4.5$&$  11.7\pm  3.1$&  0.37 &  0.63 &  0.01 \\
 HIP 15394 &   7.41 & $12.19\pm1.15$ &$   5.7\pm  1.0$&$  18.7\pm  2.0$&$ -57.8\pm  4.3$&$ -54.5\pm  3.9$&  0.23 &  0.76 &  0.01 \\
 HIP 15405 &   8.78 &  $8.20\pm0.96$ &$  17.8\pm  1.0$&$-146.9\pm 15.8$&$-100.6\pm 13.2$&$ -47.2\pm  6.0$&  0.00 &  0.71 &  0.29 \\
 HIP 15457 &   4.84 & $109.41\pm0.27 &$  18.7\pm  0.5$&$ -21.5\pm  0.4$&$  -4.3\pm  0.0$&$  -4.5\pm  0.3$&  0.99 &  0.01 &  0.00 \\
 HIP 15510 &   4.26 & $165.47\pm0.19 &$  87.2\pm  0.5$&$ -78.8\pm  0.2$&$ -92.9\pm  0.3$&$ -28.7\pm  0.4$&  0.00 &  0.95 &  0.04 \\
 HIP 15565 &   7.34 & $14.65\pm0.69$ &$  48.0\pm  0.5$&$ -61.4\pm  1.6$&$ -19.1\pm  1.6$&$  -3.2\pm  1.7$&  0.98 &  0.02 &  0.00 \\
 HIP 15940 &   7.97 & $15.05\pm0.67$ &$  49.6\pm  1.4$&$  50.7\pm  4.6$&$ -42.0\pm  1.8$&$ -86.7\pm  3.0$&  0.01 &  0.93 &  0.05 \\
 HIP 16072 &  10.73 &  $9.45\pm2.33$ &$ -13.3\pm  1.0$&$ -41.8\pm 16.9$&$-284.7\pm 88.2$&$ -56.4\pm 19.3$&  0.00 &  0.00 &  1.00 \\
 HIP 16169 &   8.24 & $21.38\pm0.88$ &$  63.7\pm  0.8$&$ -56.6\pm  1.0$&$ -90.9\pm  4.4$&$ -19.2\pm  1.6$&  0.02 &  0.96 &  0.03 \\
 HIP 16467 &   8.56 & $16.45\pm1.45$ &$  10.0\pm  0.5$&$ -50.0\pm  2.5$&$ -63.3\pm  4.0$&$  17.8\pm  1.2$&  0.55 &  0.45 &  0.00 \\
 HIP 16537 &   3.73 & $310.94\pm0.16 &$  16.0\pm  0.5$&$  -3.3\pm  0.3$&$   7.1\pm  0.1$&$ -20.4\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 16723 &   7.48 & $16.73\pm0.78$ &$  42.8\pm  0.5$&$ -30.4\pm  0.5$&$  -8.5\pm  0.6$&$ -30.6\pm  0.4$&  0.98 &  0.02 &  0.00 \\
 HIP 16738 &   8.23 &  $8.92\pm0.91$ &$  60.0\pm  1.0$&$-101.1\pm  9.8$&$ -67.9\pm 13.5$&$  30.3\pm 12.1$&  0.07 &  0.90 &  0.03 \\
 HIP 16818 &   8.20 & $16.49\pm0.79$ &$  -8.5\pm  0.5$&$  -0.2\pm  0.5$&$ -16.5\pm  0.7$&$  13.4\pm  0.8$&  0.99 &  0.01 &  0.00 \\
 HIP 16852 &   4.29 & $71.62\pm0.54$ &$  27.8\pm  0.5$&$   1.4\pm  0.4$&$ -15.3\pm  0.2$&$ -41.8\pm  0.4$&  0.95 &  0.05 &  0.00 \\
 HIP 17022 &   6.74 & $24.78\pm1.15$ &$ -40.5\pm  1.2$&$  49.5\pm  1.6$&$  -8.4\pm  1.0$&$ -36.9\pm  3.5$&  0.96 &  0.04 &  0.00 \\
 HIP 17147 &   6.69 & $39.12\pm0.56$ &$ 120.3\pm  0.5$&$-109.8\pm  0.6$&$ -85.8\pm  1.5$&$ -45.0\pm  0.9$&  0.00 &  0.92 &  0.08 \\
 HIP 17231 &   8.20 & $10.95\pm0.97$ &$ -58.7\pm  0.5$&$  63.9\pm  1.6$&$  -6.7\pm  2.6$&$  14.9\pm  1.2$&  0.98 &  0.02 &  0.00 \\
 HIP 17378 &   3.53 & $110.61\pm0.22 &$  -6.2\pm  0.9$&$ -13.4\pm  0.6$&$  26.9\pm  0.3$&$  12.9\pm  0.7$&  0.98 &  0.02 &  0.00 \\
 HIP 17409 &   7.48 & $23.08\pm0.65$ &$  31.3\pm  0.5$&$ -68.3\pm  1.6$&$ -66.7\pm  3.1$&$  -1.1\pm  0.3$&  0.41 &  0.59 &  0.01 \\
 HIP 17420 &   7.10 & $71.69\pm0.67$ &$  25.3\pm  0.5$&$ -30.5\pm  0.4$&$ -14.9\pm  0.2$&$  -4.5\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 17655 &   8.31 & $16.34\pm0.82$ &$ -56.0\pm  0.5$&$  59.7\pm  0.8$&$  -3.0\pm  1.5$&$   9.5\pm  0.4$&  0.98 &  0.02 &  0.00 \\
 HIP 17666 &   8.17 & $45.65\pm2.63$ &$  50.5\pm  0.8$&$ -95.3\pm  2.8$&$-114.8\pm  7.4$&$ -76.4\pm  3.7$&  0.00 &  0.63 &  0.37 \\
 HIP 18235 &   6.70 & $15.57\pm0.57$ &$ 100.5\pm  0.5$&$ -26.9\pm  1.3$&$-163.2\pm  6.3$&$ -27.1\pm  2.5$&  0.00 &  0.43 &  0.57 \\
 HIP 18261 &   7.97 & $21.63\pm0.86$ &$  15.6\pm  0.5$&$  -2.5\pm  0.6$&$ -23.6\pm  1.3$&$ -18.3\pm  0.5$&  0.98 &  0.02 &  0.00 \\
 HIP 18347 &   8.84 & $16.56\pm1.19$ &$  17.2\pm  0.5$&$ -31.0\pm  1.3$&$ -56.2\pm  4.6$&$   7.3\pm  1.3$&  0.82 &  0.17 &  0.00 \\
 HIP 18366 &   6.79 & $26.38\pm0.54$ &$ -33.3\pm  0.5$&$  44.2\pm  0.7$&$   9.1\pm  1.0$&$   2.0\pm  0.1$&  0.99 &  0.01 &  0.00 \\
 HIP 18413 &   6.54 & $45.49\pm0.62$ &$ -20.0\pm  2.4$&$  34.7\pm  2.0$&$  15.1\pm  1.5$&$  -7.8\pm  0.3$&  0.99 &  0.01 &  0.00 \\
 HIP 18606 &   5.83 & $21.53\pm0.41$ &$  37.5\pm  1.8$&$  -3.6\pm  1.5$&$ -27.8\pm  0.8$&$ -44.9\pm  1.4$&  0.90 &  0.10 &  0.00 \\
 HIP 19631 &   8.15 & $13.32\pm0.92$ &$ -65.3\pm  0.5$&$  49.7\pm  1.0$&$ -23.6\pm  0.3$&$  66.9\pm  4.7$&  0.42 &  0.57 &  0.01 \\
 HIP 19696 &   9.13 & $10.05\pm1.48$ &$  -6.3\pm  0.7$&$ -11.0\pm  2.5$&$ -54.5\pm  7.6$&$  33.4\pm  4.6$&  0.72 &  0.28 &  0.00 \\
 HIP 19786 &   8.04 & $23.29\pm1.25$ &$  37.8\pm  0.5$&$ -41.6\pm  0.7$&$ -18.1\pm  1.1$&$  -0.9\pm  1.2$&  0.99 &  0.01 &  0.00 \\
 HIP 19849 &   4.42 & $200.62\pm0.23 &$ -43.0\pm  0.5$&$  97.7\pm  0.5$&$ -12.3\pm  0.2$&$ -41.4\pm  0.4$&  0.77 &  0.23 &  0.01 \\
 HIP 19911 &   7.51 & $32.64\pm2.65$ &$ -16.4\pm  0.8$&$  21.8\pm  0.8$&$   5.7\pm  0.6$&$  -5.9\pm  0.8$&  0.99 &  0.01 &  0.00 \\
 HIP 20094 &   8.36 & $23.26\pm1.27$ &$ -40.9\pm  1.0$&$  41.9\pm  1.0$&$ -44.5\pm  1.8$&$ -63.5\pm  3.8$&  0.24 &  0.75 &  0.02 \\
 HIP 20298 &   9.74 &  $8.27\pm1.49$ &$  36.6\pm  1.0$&$-104.2\pm 13.1$&$-137.9\pm 28.2$&$  74.5\pm 14.2$&  0.00 &  0.30 &  0.70 \\
 HIP 20366 &   8.71 & $15.45\pm1.49$ &$  -2.8\pm  5.5$&$   6.1\pm  4.9$&$   2.9\pm  0.5$&$  -6.3\pm  2.5$&  0.99 &  0.01 &  0.00 \\
 HIP 20753 &   7.68 & $13.54\pm0.72$ &$  47.3\pm  0.5$&$ -70.9\pm  1.9$&$ -56.0\pm  5.1$&$ -12.6\pm  0.6$&  0.66 &  0.34 &  0.00 \\
 HIP 20754 &   8.13 & $10.98\pm0.83$ &$  10.9\pm  0.5$&$ -12.0\pm  0.5$&$  10.2\pm  0.7$&$ -41.0\pm  4.7$&  0.96 &  0.04 &  0.00 \\
 HIP 20984 &   8.98 & $11.90\pm1.33$ &$  44.8\pm  5.9$&$ -31.2\pm  4.8$&$-100.7\pm 11.2$&$  12.1\pm  5.6$&  0.01 &  0.97 &  0.03 \\
 HIP 21227 &   9.04 &  $9.18\pm2.27$ &$  65.7\pm  1.0$&$-103.2\pm  8.2$&$ -76.3\pm 19.5$&$  10.7\pm  2.7$&  0.05 &  0.92 &  0.03 \\
 HIP 21306 &   9.65 & $12.13\pm2.08$ &$ -83.0\pm  1.0$&$ 110.0\pm  5.3$&$ -97.2\pm 15.8$&$ -30.9\pm  9.8$&  0.00 &  0.91 &  0.09 \\
 HIP 21703 &   8.93 & $17.27\pm0.90$ &$ -19.7\pm  1.0$&$  13.1\pm  1.0$&$ -67.5\pm  4.4$&$  33.7\pm  1.8$&  0.35 &  0.64 &  0.01 \\
 HIP 21847 &   6.00 & $31.38\pm0.62$ &$  46.6\pm  0.5$&$ -55.4\pm  0.6$&$ -20.5\pm  0.9$&$  13.1\pm  0.5$&  0.98 &  0.02 &  0.00 \\
 HIP 21921 &   8.28 & $27.29\pm1.10$ &$ -59.8\pm  0.5$&$  41.2\pm  0.4$&$ -64.1\pm  1.1$&$  41.9\pm  2.1$&  0.25 &  0.73 &  0.01 \\
 HIP 22020 &   9.01 & $10.62\pm1.47$ &$  28.1\pm  1.0$&$ -81.5\pm  7.4$&$ -90.6\pm 13.4$&$ -60.4\pm  8.2$&  0.00 &  0.92 &  0.08 \\
 HIP 22060 &   9.95 &  $9.13\pm2.10$ &$ 172.1\pm  1.0$&$-194.3\pm  6.9$&$ -71.5\pm 21.9$&$  45.2\pm 21.1$&  0.00 &  0.57 &  0.43 \\
 HIP 22263 &   5.50 & $75.32\pm0.36$ &$  21.6\pm  0.5$&$ -23.8\pm  0.4$&$  -8.5\pm  0.2$&$  -2.8\pm  0.3$&  0.99 &  0.01 &  0.00 \\
 HIP 22336 &   5.78 & $37.85\pm0.35$ &$  77.0\pm  0.5$&$ -52.1\pm  0.5$&$ -72.8\pm  1.1$&$ -21.0\pm  0.5$&  0.23 &  0.76 &  0.01 \\
 HIP 22349 &   6.96 & $33.58\pm0.84$ &$  51.7\pm  4.1$&$ -45.1\pm  3.9$&$ -62.4\pm  1.9$&$ -25.9\pm  1.2$&  0.52 &  0.48 &  0.01 \\
 HIP 22449 &   3.19 & $123.94\pm0.17 &$  23.7\pm  0.5$&$ -25.3\pm  0.5$&$ -14.7\pm  0.1$&$   4.5\pm  0.2$&  0.99 &  0.01 &  0.00 \\
 HIP 22489 &   9.00 &        \nodata &$ -34.1\pm  0.5$&$  -1.2\pm 25.2$&$ -49.6\pm 27.0$&$ -26.0\pm 16.6$&  0.86 &  0.14 &  0.00 \\
 HIP 22528 &   9.54 & $11.62\pm0.97$ &$ -33.9\pm  0.5$&$  -8.8\pm  3.3$&$ -23.2\pm  0.5$&$-110.2\pm  9.6$&  0.00 &  0.87 &  0.13 \\
 HIP 22596 &   6.98 & $33.13\pm0.88$ &$  28.9\pm  0.5$&$ -59.9\pm  1.2$&$ -80.1\pm  3.0$&$  -9.3\pm  0.4$&  0.11 &  0.88 &  0.02 \\
 HIP 23080 &   8.19 & $29.42\pm0.73$ &$  38.6\pm  0.5$&$ -56.9\pm  0.9$&$ -72.4\pm  2.9$&$  48.3\pm  1.9$&  0.05 &  0.93 &  0.02 \\
 HIP 23311 &   6.23 & $114.84\pm0.50 &$  21.1\pm  0.8$&$   5.4\pm  0.7$&$ -54.6\pm  0.5$&$ -10.6\pm  0.4$&  0.86 &  0.13 &  0.00 \\
 HIP 23693 &   4.71 & $85.87\pm0.18$ &$  -0.9\pm  0.5$&$  -6.1\pm  0.1$&$   2.6\pm  0.4$&$  -1.4\pm  0.3$&  0.99 &  0.01 &  0.00 \\
 HIP 23835 &   4.92 & $64.79\pm0.33$ &$  20.3\pm  0.5$&$ -25.8\pm  0.5$&$ -23.7\pm  0.3$&$  28.5\pm  0.5$&  0.97 &  0.03 &  0.00 \\
 HIP 23884 &   7.60 & $27.48\pm0.72$ &$ -62.9\pm  0.5$&$  64.4\pm  0.5$&$  -5.0\pm  0.1$&$  -6.6\pm  0.6$&  0.98 &  0.02 &  0.00 \\
 HIP 23922 &   9.28 & $11.76\pm1.20$ &$-111.7\pm  0.5$&$  36.2\pm  8.4$&$-139.4\pm 12.1$&$-124.2\pm 14.3$&  0.00 &  0.07 &  0.93 \\
 HIP 23941 &   5.12 & $39.28\pm0.27$ &$  10.1\pm  0.5$&$ -10.3\pm  0.4$&$  -6.3\pm  0.2$&$   1.9\pm  0.3$&  0.99 &  0.01 &  0.00 \\
 HIP 24030 &   9.68 &  $8.66\pm1.77$ &$ -15.7\pm  1.0$&$  10.3\pm  1.2$&$ -93.7\pm 15.6$&$  89.8\pm 13.7$&  0.00 &  0.85 &  0.15 \\
 HIP 24037 &   8.48 & $22.26\pm1.15$ &$  64.1\pm  0.5$&$ -18.7\pm  1.9$&$ -56.2\pm  1.7$&$ -59.4\pm  1.8$&  0.18 &  0.81 &  0.02 \\
 HIP 24660 &   8.54 & $18.79\pm0.74$ &$  43.5\pm  0.5$&$ -37.4\pm  0.5$&$ -23.6\pm  1.1$&$ -17.7\pm  0.5$&  0.98 &  0.02 &  0.00 \\
 HIP 24813 &   4.70 & $79.17\pm0.28$ &$  66.5\pm  0.5$&$ -75.7\pm  0.5$&$ -35.2\pm  0.6$&$   4.4\pm  0.1$&  0.92 &  0.08 &  0.00 \\
 HIP 25052 &   7.70 & $21.06\pm0.88$ &$  10.6\pm  0.5$&$ -35.9\pm  1.4$&$ -69.2\pm  3.7$&$  18.2\pm  0.9$&  0.42 &  0.57 &  0.01 \\
 HIP 25361 &   9.76 & $10.24\pm1.65$ &$ -19.2\pm  1.0$&$   9.9\pm  1.8$&$ -97.5\pm 15.4$&$  12.1\pm  2.0$&  0.01 &  0.97 &  0.02 \\
 HIP 25528 &   7.21 & $10.25\pm0.77$ &$ -80.9\pm  0.5$&$ 130.5\pm  7.0$&$ -39.9\pm  8.2$&$  15.4\pm  1.8$&  0.40 &  0.58 &  0.02 \\
 HIP 25586 &   8.67 & $17.07\pm0.98$ &$ -22.3\pm  0.5$&$  26.6\pm  0.6$&$   0.5\pm  0.3$&$ -36.0\pm  2.9$&  0.97 &  0.03 &  0.00 \\
 HIP 25670 &   8.28 & $20.58\pm0.92$ &$  -9.7\pm  0.5$&$  19.8\pm  0.8$&$   6.0\pm  0.3$&$ -17.1\pm  1.1$&  0.99 &  0.01 &  0.00 \\
 HIP 25840 &   6.91 & $22.45\pm0.61$ &$  22.8\pm  0.5$&$  19.9\pm  1.4$&$ -70.6\pm  2.1$&$  -6.9\pm  0.2$&  0.48 &  0.51 &  0.01 \\
 HIP 25860 &   8.64 & $20.07\pm1.15$ &$  48.1\pm  1.0$&$ -24.5\pm  1.9$&$ -79.7\pm  5.2$&$ -66.9\pm  4.2$&  0.00 &  0.96 &  0.04 \\
 HIP 25973 &   6.47 & $23.42\pm0.48$ &$  33.0\pm  0.5$&$ -52.3\pm  0.9$&$ -32.7\pm  1.7$&$   3.5\pm  0.2$&  0.96 &  0.04 &  0.00 \\
 HIP 26100 &   7.31 & $16.06\pm0.74$ &$ -16.3\pm  0.5$&$  18.2\pm  0.5$&$   3.9\pm  0.2$&$ -13.0\pm  1.0$&  0.99 &  0.01 &  0.00 \\
 HIP 26129 &   9.10 & $14.65\pm1.34$ &$  10.7\pm  0.5$&$ -11.4\pm  0.5$&$   5.7\pm  0.9$&$  -5.6\pm  0.6$&  0.99 &  0.01 &  0.00 \\
 HIP 26326 &   7.99 & $16.87\pm0.86$ &$  -3.2\pm  0.6$&$   2.5\pm  0.6$&$ -11.7\pm  0.9$&$  -8.8\pm  0.8$&  0.99 &  0.01 &  0.00 \\
 HIP 26437 &   7.76 & $19.75\pm0.61$ &$ -62.6\pm  0.5$&$  13.0\pm  1.2$&$ -60.3\pm  0.8$&$ -44.8\pm  0.8$&  0.37 &  0.62 &  0.01 \\
 HIP 26452 &   9.53 & $12.69\pm1.56$ &$ -37.7\pm  1.0$&$  -6.9\pm  4.3$&$-101.4\pm  9.5$&$  40.5\pm  6.2$&  0.00 &  0.96 &  0.04 \\
 HIP 26534 &   7.59 & $17.12\pm0.70$ &$  71.5\pm  0.5$&$ -31.0\pm  1.1$&$ -74.0\pm  1.7$&$ -14.4\pm  0.8$&  0.31 &  0.68 &  0.01 \\
 HIP 26617 &  10.34 &  $8.79\pm2.67$ &$ 127.2\pm  1.0$&$ -60.0\pm 16.2$&$-228.9\pm 53.7$&$  26.7\pm 16.5$&  0.00 &  0.00 &  1.00 \\
 HIP 26779 &   6.22 & $81.45\pm0.54$ &$   0.9\pm  0.5$&$ -13.4\pm  0.5$&$ -23.1\pm  0.3$&$ -14.5\pm  0.2$&  0.98 &  0.02 &  0.00 \\
 HIP 26807 &   7.68 & $27.63\pm0.95$ &$ -42.7\pm  0.5$&$  49.7\pm  0.6$&$ -28.3\pm  1.5$&$  -1.0\pm  0.3$&  0.97 &  0.03 &  0.00 \\
 HIP 26828 &   7.89 & $12.91\pm0.83$ &$  30.9\pm 35.8$&$ -26.7\pm 35.6$&$ -82.8\pm  7.1$&$  36.1\pm  4.0$&  0.04 &  0.94 &  0.02 \\
 HIP 27072 &   3.59 & $112.02\pm0.18 &$  -9.5\pm  0.5$&$  18.2\pm  0.3$&$   4.5\pm  0.3$&$ -11.8\pm  0.2$&  0.99 &  0.01 &  0.00 \\
 HIP 27128 &   8.24 & $15.49\pm0.78$ &$ 183.7\pm  0.5$&$-174.1\pm  4.1$&$ -75.7\pm  3.1$&$ -75.4\pm  0.4$&  0.00 &  0.49 &  0.51 \\
 HIP 27207 &   7.36 & $45.76\pm0.76$ &$ -29.7\pm  0.5$&$  22.2\pm  0.5$&$ -70.4\pm  1.4$&$  12.7\pm  0.3$&  0.46 &  0.53 &  0.01 \\
 HIP 27878 &   7.76 & $18.68\pm0.81$ &$  49.9\pm  3.1$&$ -29.1\pm  3.2$&$ -66.3\pm  3.1$&$ -40.3\pm  2.0$&  0.26 &  0.73 &  0.01 \\
 HIP 27913 &   4.40 & $115.43\pm0.27 &$ -13.9\pm  0.5$&$  14.1\pm  0.5$&$   2.0\pm  0.1$&$  -7.2\pm  0.1$&  0.99 &  0.01 &  0.00 \\
 HIP 28066 &   6.60 & $37.59\pm0.63$ &$   0.1\pm  0.5$&$  18.5\pm  0.7$&$ -78.2\pm  2.2$&$  11.1\pm  0.3$&  0.23 &  0.76 &  0.01 \\
 HIP 28103 &   3.71 & $67.21\pm0.25$ &$  -1.7\pm  0.5$&$  -5.7\pm  0.4$&$   8.7\pm  0.3$&$   1.8\pm  0.2$&  0.99 &  0.01 &  0.00 \\
 HIP 28145 &   8.60 & $17.25\pm1.12$ &$ -69.9\pm  2.0$&$  70.3\pm  2.0$&$ -17.2\pm  1.0$&$  12.8\pm  1.4$&  0.97 &  0.03 &  0.00 \\
 HIP 28159 &   8.21 & $15.38\pm0.82$ &$ -26.2\pm  1.7$&$  44.8\pm  2.3$&$ -74.8\pm  6.8$&$ -12.0\pm  1.3$&  0.26 &  0.73 &  0.01 \\
 HIP 28336 &   8.98 & $16.20\pm1.24$ &$  90.7\pm  0.5$&$-104.9\pm  3.8$&$ -35.1\pm  2.2$&$  11.4\pm  3.6$&  0.78 &  0.21 &  0.00 \\
 HIP 28671 &   9.31 & $16.81\pm2.04$ &$-190.7\pm  1.0$&$ 235.1\pm  8.1$&$-239.5\pm 46.0$&$  91.9\pm 14.5$&  0.00 &  0.00 &  1.00 \\
 HIP 29001 &   7.35 & $28.31\pm0.81$ &$  49.1\pm  0.5$&$ -43.3\pm  0.5$&$ -31.0\pm  0.8$&$   3.6\pm  0.3$&  0.97 &  0.03 &  0.00 \\
 HIP 29074 &   8.03 & $23.37\pm0.90$ &$  34.3\pm  0.6$&$ -33.1\pm  0.6$&$ -22.3\pm  1.0$&$  -2.7\pm  0.3$&  0.98 &  0.02 &  0.00 \\
 HIP 29248 &   8.49 & $21.01\pm1.12$ &$   6.1\pm  4.0$&$   7.6\pm  4.0$&$ -64.4\pm  4.1$&$  15.6\pm  1.0$&  0.65 &  0.35 &  0.00 \\
 HIP 29269 &   8.92 & $11.13\pm1.32$ &$ -32.0\pm  1.0$&$-105.0\pm 18.0$&$ -90.7\pm 10.0$&$ -81.9\pm  9.9$&  0.00 &  0.76 &  0.24 \\
 HIP 29271 &   5.08 & $98.06\pm0.14$ &$  35.6\pm  0.5$&$  18.9\pm  0.1$&$ -30.2\pm  0.4$&$ -11.7\pm  0.2$&  0.98 &  0.02 &  0.00 \\
 HIP 29432 &   6.86 & $42.55\pm0.55$ &$ -53.7\pm  0.5$&$  62.1\pm  0.5$&$ -11.9\pm  0.7$&$  11.0\pm  0.2$&  0.98 &  0.02 &  0.00 \\
 HIP 29650 &   5.20 & $48.04\pm0.34$ &$  34.3\pm  0.5$&$ -31.5\pm  0.5$&$ -18.2\pm  0.2$&$ -16.6\pm  0.3$&  0.98 &  0.02 &  0.00 \\
 HIP 29716 &   5.64 & $26.89\pm0.31$ &$ -39.6\pm  0.5$&$  49.3\pm  0.6$&$   4.1\pm  0.5$&$ -34.6\pm  1.1$&  0.96 &  0.04 &  0.00 \\
 HIP 30545 &   5.87 & $29.79\pm0.46$ &$  46.9\pm  0.5$&$ -17.4\pm  0.8$&$ -65.7\pm  1.3$&$  12.4\pm  0.6$&  0.62 &  0.38 &  0.00 \\
 HIP 30990 &   8.43 & $13.66\pm1.12$ &$  61.8\pm  0.5$&$ -87.4\pm  3.0$&$ -63.1\pm  7.2$&$  38.6\pm  1.3$&  0.13 &  0.85 &  0.02 \\
 HIP 31083 &   7.14 & $36.00\pm0.61$ &$  21.5\pm  1.7$&$ -22.2\pm  1.5$&$  -2.6\pm  0.8$&$ -13.5\pm  0.3$&  0.99 &  0.01 &  0.00 \\
 HIP 31188 &   8.62 & $16.79\pm0.91$ &$   3.3\pm  1.0$&$   9.0\pm  1.1$&$ -31.2\pm  1.8$&$  64.4\pm  3.8$&  0.51 &  0.48 &  0.01 \\
 HIP 31419 &   8.94 & $13.81\pm0.78$ &$  47.2\pm  0.5$&$   2.3\pm  1.7$&$ -65.7\pm  1.9$&$  22.8\pm  2.7$&  0.55 &  0.44 &  0.00 \\
 HIP 32650 &   7.92 & $18.82\pm1.00$ &$ -87.0\pm  0.5$&$ 107.7\pm  2.4$&$ -29.1\pm  5.3$&$ -57.5\pm  4.1$&  0.20 &  0.77 &  0.03 \\
 HIP 32673 &   8.07 & $22.94\pm1.63$ &$  41.3\pm 10.7$&$ -46.9\pm 10.3$&$  -1.7\pm  0.6$&$ -14.1\pm  3.2$&  0.99 &  0.01 &  0.00 \\
 HIP 32851 &   5.76 & $33.69\pm0.42$ &$ -12.2\pm  0.7$&$  24.0\pm  0.7$&$ -14.2\pm  0.6$&$  -9.2\pm  0.3$&  0.99 &  0.01 &  0.00 \\
 HIP 33287 &   8.01 & $25.98\pm1.86$ &$  30.8\pm  0.5$&$ -18.6\pm  1.4$&$ -60.5\pm  7.4$&$  28.1\pm  2.3$&  0.63 &  0.37 &  0.00 \\
 HIP 33382 &   7.40 & $31.99\pm0.68$ &$  -8.4\pm  0.5$&$  47.7\pm  1.2$&$ -61.6\pm  1.8$&$ -41.5\pm  1.1$&  0.30 &  0.69 &  0.01 \\
 HIP 33608 &   8.64 & $16.14\pm1.02$ &$  36.9\pm  0.5$&$ -30.1\pm  0.5$&$ -23.1\pm  0.5$&$  -6.3\pm  0.7$&  0.98 &  0.02 &  0.00 \\
 HIP 34017 &   5.93 & $52.27\pm0.41$ &$  24.3\pm  0.5$&$ -17.8\pm  0.5$&$ -77.5\pm  1.2$&$  -9.1\pm  0.3$&  0.26 &  0.73 &  0.01 \\
 HIP 34164 &   8.45 & $11.29\pm1.92$ &$  28.0\pm  1.1$&$  19.0\pm  7.4$&$ -84.6\pm 12.0$&$ -37.2\pm  6.7$&  0.03 &  0.95 &  0.02 \\
 HIP 34511 &   8.00 & $21.64\pm0.79$ &$  42.6\pm  0.5$&$ -34.4\pm  0.5$&$ -56.0\pm  2.0$&$ -46.5\pm  2.6$&  0.39 &  0.60 &  0.01 \\
 HIP 34521 &   7.84 & $10.09\pm0.73$ &$  13.5\pm  0.5$&$  -9.7\pm  0.6$&$ -34.8\pm  3.4$&$   1.0\pm  0.7$&  0.97 &  0.03 &  0.00 \\
 HIP 34608 &   6.43 & $21.82\pm0.40$ &$  -2.1\pm  1.1$&$   6.0\pm  1.0$&$ -80.1\pm  3.1$&$ -75.7\pm  2.8$&  0.00 &  0.94 &  0.05 \\
 HIP 34642 &   8.86 & $11.04\pm1.23$ &$ -29.5\pm  1.0$&$ -23.0\pm  5.7$&$ -93.1\pm  9.7$&$ -63.1\pm  6.0$&  0.00 &  0.94 &  0.05 \\
 HIP 34653 &   9.09 & $12.94\pm1.10$ &$ -30.4\pm  1.0$&$  61.8\pm  3.1$&$ -98.9\pm  9.5$&$  -0.4\pm  0.9$&  0.01 &  0.96 &  0.03 \\
 HIP 34710 &   7.15 & $16.26\pm0.68$ &$  70.8\pm  0.5$&$ -32.8\pm  1.0$&$ -66.8\pm  1.0$&$  -3.3\pm  0.3$&  0.58 &  0.41 &  0.00 \\
 HIP 35148 &   7.88 & $16.83\pm0.92$ &$  42.0\pm  0.9$&$  11.9\pm  1.9$&$ -61.9\pm  1.6$&$  42.3\pm  2.6$&  0.37 &  0.62 &  0.01 \\
 HIP 35185 &   8.42 & $18.70\pm0.85$ &$  21.7\pm  0.5$&$ -16.2\pm  0.5$&$ -17.1\pm  0.5$&$  -6.0\pm  0.6$&  0.99 &  0.01 &  0.00 \\
 HIP 35214 &   9.11 & $13.61\pm1.23$ &$  26.1\pm  0.5$&$ -22.3\pm  0.5$&$   4.2\pm  0.5$&$  13.4\pm  0.6$&  0.99 &  0.01 &  0.00 \\
 HIP 35599 &   8.96 & $10.82\pm1.14$ &$  36.4\pm  1.0$&$-103.9\pm  8.6$&$ -81.5\pm 11.0$&$ -18.4\pm  4.0$&  0.02 &  0.94 &  0.04 \\
 HIP 35989 &   9.16 & $21.42\pm1.71$ &$   7.6\pm  1.2$&$ -48.5\pm  3.2$&$ -47.0\pm  3.4$&$ -71.9\pm  5.5$&  0.07 &  0.90 &  0.03 \\
 HIP 36210 &   6.72 & $44.10\pm0.36$ &$   4.3\pm  0.5$&$ -11.7\pm  0.2$&$   4.8\pm  0.5$&$ -28.0\pm  0.3$&  0.98 &  0.02 &  0.00 \\
 HIP 36439 &   5.37 & $49.41\pm0.36$ &$ -27.6\pm  0.5$&$  26.0\pm  0.4$&$ -15.3\pm  0.2$&$  -4.5\pm  0.3$&  0.99 &  0.01 &  0.00 \\
 HIP 36481 &   7.07 & $24.41\pm0.66$ &$  59.9\pm  0.5$&$ -44.9\pm  0.6$&$ -44.7\pm  1.2$&$  18.3\pm  0.3$&  0.90 &  0.10 &  0.00 \\
 HIP 36515 &   6.64 & $45.84\pm0.37$ &$   9.2\pm  0.5$&$ -11.3\pm  0.2$&$  -4.7\pm  0.5$&$  -6.9\pm  0.1$&  0.99 &  0.01 &  0.00 \\
 HIP 36849 &   8.92 & $12.37\pm1.23$ &$ -33.8\pm  0.5$&$  58.0\pm  3.0$&$ -91.0\pm 10.6$&$ -52.8\pm  4.3$&  0.00 &  0.95 &  0.05 \\
 HIP 36874 &   7.36 & $25.58\pm0.65$ &$-135.8\pm  0.5$&$ 140.5\pm  0.8$&$ -36.2\pm  2.7$&$ -48.2\pm  0.3$&  0.07 &  0.87 &  0.07 \\
 HIP 37171 &   8.41 & $19.93\pm1.02$ &$  88.3\pm  0.5$&$ -79.3\pm  2.2$&$ -58.1\pm  1.2$&$  -0.4\pm  0.3$&  0.58 &  0.42 &  0.01 \\
 HIP 37233 &   7.57 & $18.57\pm0.64$ &$  51.3\pm  0.5$&$   4.8\pm  2.2$&$ -71.8\pm  1.9$&$  43.2\pm  1.9$&  0.14 &  0.85 &  0.01 \\
 HIP 37279 &   0.37 & $284.56\pm1.26 &$  -4.2\pm  0.5$&$   5.5\pm  0.4$&$  -8.3\pm  0.3$&$ -18.8\pm  0.1$&  0.99 &  0.01 &  0.00 \\
 HIP 37316 &   8.71 & $11.37\pm1.16$ &$ -87.4\pm  0.5$&$  73.6\pm  0.7$&$ -40.2\pm  3.5$&$ -39.6\pm  0.6$&  0.67 &  0.32 &  0.00 \\
 HIP 37349 &   7.18 & $70.37\pm0.64$ &$ -18.6\pm  0.5$&$  25.6\pm  0.4$&$  -2.2\pm  0.4$&$  -7.6\pm  0.1$&  0.99 &  0.01 &  0.00 \\
 HIP 37419 &   8.68 & $19.16\pm0.88$ &$  -9.1\pm  6.9$&$  96.3\pm  6.0$&$ -42.6\pm  6.7$&$  37.5\pm  2.1$&  0.47 &  0.52 &  0.01 \\
 HIP 37789 &   6.75 & $28.90\pm0.68$ &$  -5.6\pm  0.5$&$  -5.3\pm  0.6$&$-108.6\pm  3.5$&$ -23.1\pm  0.7$&  0.00 &  0.96 &  0.04 \\
 HIP 37826 &   1.14 & $96.54\pm0.27$ &$   3.5\pm  0.5$&$ -16.4\pm  0.5$&$   4.7\pm  0.1$&$ -25.8\pm  0.3$&  0.99 &  0.01 &  0.00 \\
 HIP 37853 &   5.36 & $65.75\pm0.51$ &$ 103.3\pm  0.7$&$-146.2\pm  1.0$&$ -58.7\pm  0.7$&$  38.9\pm  0.4$&  0.01 &  0.90 &  0.09 \\
 HIP 37971 &   8.51 & $18.16\pm1.00$ &$  12.6\pm  0.5$&$ -12.7\pm  0.5$&$  -7.5\pm  0.3$&$  -1.1\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 38072 &   9.22 & $13.21\pm1.02$ &$  58.8\pm  0.5$&$ -47.9\pm  2.0$&$ -41.5\pm  1.1$&$ -17.8\pm  1.5$&  0.92 &  0.08 &  0.00 \\
 HIP 38172 &   7.10 & $23.21\pm0.47$ &$ -11.1\pm  0.5$&$  -1.0\pm  0.6$&$   4.8\pm  0.2$&$ -27.6\pm  0.9$&  0.99 &  0.01 &  0.00 \\
 HIP 38228 &   6.89 & $45.45\pm0.53$ &$ -16.5\pm  0.5$&$  14.3\pm  0.4$&$   2.5\pm  0.1$&$  -7.9\pm  0.2$&  0.99 &  0.01 &  0.00 \\
 HIP 38325 &   6.02 & $33.78\pm0.39$ &$   1.5\pm  0.5$&$  -1.4\pm  0.4$&$   8.8\pm  0.2$&$  -3.6\pm  0.3$&  0.99 &  0.01 &  0.00 \\
 HIP 38613 &   8.95 & $12.41\pm1.04$ &$  61.9\pm  0.5$&$ -95.3\pm  3.7$&$ -66.1\pm  6.5$&$ -19.9\pm  4.5$&  0.17 &  0.81 &  0.02 \\
 HIP 38625 &   7.43 & $49.78\pm1.85$ &$ 102.7\pm  0.8$&$ -82.6\pm  0.7$&$ -65.4\pm  0.5$&$   1.4\pm  0.8$&  0.34 &  0.65 &  0.01 \\
 HIP 38769 &   8.81 & $11.56\pm0.98$ &$   6.8\pm  0.5$&$  14.9\pm  2.0$&$ -70.9\pm  6.7$&$  62.5\pm  5.5$&  0.03 &  0.95 &  0.03 \\
 HIP 39072 &   8.66 & $15.55\pm1.04$ &$  63.6\pm 25.4$&$ -65.4\pm 21.5$&$  -4.3\pm  3.8$&$  17.5\pm 13.1$&  0.98 &  0.02 &  0.00 \\
 HIP 39157 &   7.00 & $59.64\pm0.56$ &$  14.5\pm  0.5$&$ -13.0\pm  0.4$&$ -89.0\pm  1.1$&$ -30.0\pm  0.5$&  0.03 &  0.95 &  0.02 \\
 HIP 39417 &   8.26 & $18.21\pm1.07$ &$  44.3\pm  0.5$&$ -13.4\pm  1.3$&$ -65.1\pm  2.4$&$ -28.4\pm  2.6$&  0.50 &  0.50 &  0.01 \\
 HIP 39506 &   7.26 & $34.01\pm0.63$ &$ -54.7\pm  1.7$&$  61.0\pm  1.5$&$  22.4\pm  0.9$&$  13.6\pm  1.3$&  0.97 &  0.03 &  0.00 \\
 HIP 39616 &   8.17 & $17.58\pm0.71$ &$   4.9\pm  0.5$&$ -64.1\pm  3.1$&$ -40.6\pm  2.2$&$ -41.9\pm  2.3$&  0.69 &  0.31 &  0.00 \\
 HIP 39780 &   5.29 & $42.94\pm0.30$ &$ -36.2\pm  0.5$&$  33.1\pm  0.4$&$   4.2\pm  0.2$&$ -16.1\pm  0.2$&  0.99 &  0.01 &  0.00 \\
 HIP 39822 &   8.20 & $21.45\pm0.81$ &$  36.2\pm  0.5$&$-104.7\pm  3.5$&$ -56.1\pm  3.3$&$ -12.1\pm  1.4$&  0.36 &  0.62 &  0.01 \\
 HIP 39893 &   9.63 & $10.00\pm2.09$ &$ -42.9\pm  0.5$&$  58.2\pm  4.7$&$-131.3\pm 30.5$&$ -63.6\pm  9.5$&  0.00 &  0.67 &  0.33 \\
 HIP 40001 &   6.61 & $21.37\pm0.53$ &$ -57.5\pm  1.9$&$  75.1\pm  2.1$&$ -58.6\pm  3.1$&$   3.1\pm  1.9$&  0.59 &  0.40 &  0.01 \\
 HIP 40023 &   5.72 & $24.18\pm0.35$ &$ -45.0\pm  1.0$&$  39.8\pm  0.9$&$ -51.7\pm  2.0$&$ -52.6\pm  1.1$&  0.35 &  0.64 &  0.01 \\
 HIP 40118 &   6.83 & $45.90\pm0.55$ &$  29.6\pm  0.5$&$ -47.9\pm  0.6$&$ -60.6\pm  1.1$&$ -39.4\pm  1.1$&  0.35 &  0.64 &  0.01 \\
 HIP 40613 &   7.72 & $20.50\pm0.95$ &$ 112.9\pm  0.5$&$ -38.1\pm  2.1$&$-144.5\pm  3.7$&$ -43.2\pm  4.3$&  0.00 &  0.66 &  0.34 \\
 HIP 40674 &   9.34 & $14.14\pm1.06$ &$  -1.3\pm  0.5$&$  -5.1\pm  0.8$&$ -88.9\pm  7.9$&$   0.3\pm  0.6$&  0.06 &  0.92 &  0.01 \\
 HIP 40693 &   5.97 & $80.04\pm0.35$ &$  29.8\pm  0.5$&$  28.9\pm  0.5$&$ -60.9\pm  0.5$&$ -10.1\pm  0.2$&  0.73 &  0.27 &  0.00 \\
 HIP 40765 &   7.43 & $28.20\pm0.63$ &$  31.1\pm  0.5$&$ -23.4\pm  0.4$&$ -17.8\pm  0.4$&$  12.1\pm  0.2$&  0.99 &  0.01 &  0.00 \\
 HIP 40843 &   5.14 & $54.73\pm0.32$ &$  32.6\pm  0.5$&$ -24.1\pm  0.4$&$ -38.5\pm  0.5$&$   7.1\pm  0.3$&  0.96 &  0.04 &  0.00 \\
 HIP 40848 &   8.38 & $31.84\pm0.86$ &$ -11.7\pm  2.3$&$ -54.5\pm  2.4$&$ -59.1\pm  2.0$&$ -30.4\pm  1.4$&  0.50 &  0.49 &  0.01 \\
 HIP 41484 &   6.34 & $44.94\pm0.46$ &$ -32.6\pm  0.5$&$  20.3\pm  0.4$&$ -38.2\pm  0.7$&$ -22.6\pm  0.3$&  0.95 &  0.05 &  0.00 \\
 HIP 41832 &   8.13 & $22.08\pm1.14$ &$ -23.2\pm  0.5$&$   6.6\pm  0.7$&$ -24.9\pm  1.0$&$ -21.6\pm  0.6$&  0.98 &  0.02 &  0.00 \\
 HIP 41926 &   6.38 & $81.91\pm0.46$ &$  14.4\pm  0.5$&$ -75.0\pm  0.6$&$   6.5\pm  0.5$&$ -24.6\pm  0.2$&  0.96 &  0.04 &  0.00 \\
 HIP 42343 &   7.03 & $22.18\pm0.53$ &$  13.3\pm  0.5$&$ -25.2\pm  0.8$&$ -10.9\pm  0.4$&$ -28.0\pm  1.3$&  0.98 &  0.02 &  0.00 \\
 HIP 42438 &   5.63 & $69.66\pm0.37$ &$ -12.8\pm  0.5$&$  10.1\pm  0.4$&$   0.5\pm  0.2$&$ -10.0\pm  0.3$&  0.99 &  0.01 &  0.00 \\
 HIP 42575 &   8.02 & $25.05\pm0.90$ &$  35.0\pm  0.5$&$ -76.7\pm  2.2$&$ -57.7\pm  2.8$&$ -14.5\pm  1.5$&  0.56 &  0.44 &  0.01 \\
 HIP 42612 &   8.48 & $11.83\pm1.11$ &$  85.1\pm  0.5$&$ -86.7\pm  3.2$&$ -59.4\pm  0.4$&$ -22.3\pm  5.0$&  0.37 &  0.62 &  0.01 \\
 HIP 42734 &   7.42 & $21.49\pm0.66$ &$  54.0\pm  0.5$&$ -35.4\pm  0.5$&$ -70.6\pm  2.8$&$  28.6\pm  0.4$&  0.28 &  0.71 &  0.01 \\
 HIP 42808 &   6.56 & $89.76\pm0.37$ &$  12.5\pm  0.5$&$ -25.9\pm  0.2$&$  -7.9\pm  0.5$&$  -0.9\pm  0.0$&  0.99 &  0.01 &  0.00 \\
 HIP 43393 &   9.18 & $17.86\pm1.16$ &$  29.1\pm  3.0$&$  24.8\pm  3.6$&$-106.5\pm  7.1$&$ -88.2\pm  8.0$&  0.00 &  0.78 &  0.22 \\
 HIP 43587 &   5.95 & $81.03\pm0.75$ &$  27.8\pm  0.5$&$ -37.5\pm  0.4$&$ -18.3\pm  0.2$&$  -7.8\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 43595 &  10.78 &  $7.87\pm2.47$ &$  49.9\pm  1.0$&$ -81.4\pm 15.0$&$-153.0\pm 46.3$&$-101.8\pm 44.2$&  0.00 &  0.06 &  0.94 \\
 HIP 43618 &   8.64 & $16.64\pm1.00$ &$   2.0\pm  0.5$&$  50.6\pm  4.2$&$ -69.2\pm  5.6$&$  -2.4\pm  0.5$&  0.43 &  0.56 &  0.01 \\
 HIP 43727 &   7.83 & $15.98\pm1.14$ &$  28.9\pm  0.5$&$ -29.3\pm  0.6$&$ -64.7\pm  3.6$&$ -23.7\pm  2.6$&  0.53 &  0.46 &  0.00 \\
 HIP 43861 &   8.17 & $22.47\pm0.98$ &$  32.1\pm  0.5$&$ -39.1\pm  1.3$&$ -50.9\pm  4.0$&$  -3.5\pm  2.0$&  0.88 &  0.12 &  0.00 \\
 HIP 43904 &   7.32 & $22.17\pm0.67$ &$  33.7\pm  0.5$&$ -25.0\pm  0.4$&$ -12.3\pm  0.4$&$  20.4\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 43981 &   7.84 & $16.17\pm0.66$ &$  -4.8\pm  0.5$&$ -10.3\pm  0.9$&$  -0.6\pm  0.2$&$ -19.1\pm  0.9$&  0.99 &  0.01 &  0.00 \\
 HIP 44075 &   5.82 & $47.54\pm0.31$ &$ 120.0\pm  0.9$&$ -48.4\pm  0.4$&$ -90.9\pm  0.8$&$  69.8\pm  0.7$&  0.00 &  0.92 &  0.08 \\
 HIP 44212 &   7.80 & $21.60\pm0.94$ &$   8.1\pm  0.5$&$  26.8\pm  1.5$&$ -28.5\pm  1.1$&$  -1.9\pm  0.3$&  0.98 &  0.02 &  0.00 \\
 HIP 44324 &   7.95 & $22.72\pm0.79$ &$   4.0\pm  0.6$&$ -17.7\pm  0.8$&$ -24.6\pm  1.1$&$  -8.6\pm  0.6$&  0.98 &  0.02 &  0.00 \\
 HIP 44347 &   9.55 & $11.54\pm1.61$ &$ -57.4\pm  1.0$&$ 107.2\pm  8.0$&$ -69.6\pm  9.2$&$  24.1\pm  7.7$&  0.06 &  0.91 &  0.03 \\
 HIP 44441 &   7.03 & $19.90\pm0.65$ &$  72.5\pm  0.5$&$-120.3\pm  2.9$&$  -9.4\pm  0.2$&$ -27.6\pm  3.2$&  0.76 &  0.24 &  0.01 \\
 HIP 44858 &   8.26 & $21.24\pm1.29$ &$  29.5\pm  0.5$&$ -31.9\pm  0.8$&$   8.4\pm  1.1$&$  13.3\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 44860 &   7.29 & $26.90\pm0.62$ &$  66.5\pm  0.5$&$ -68.8\pm  1.4$&$ -73.7\pm  0.7$&$ -64.0\pm  2.9$&  0.01 &  0.95 &  0.05 \\
 HIP 44927 &   7.98 & $10.64\pm0.65$ &$  69.4\pm  0.5$&$ -59.9\pm  3.3$&$ -61.7\pm  0.5$&$ -18.5\pm  4.2$&  0.53 &  0.46 &  0.01 \\
 HIP 44997 &   8.35 & $19.12\pm0.74$ &$ -12.3\pm  0.5$&$ -23.6\pm  1.8$&$  11.1\pm  0.4$&$ -37.6\pm  1.7$&  0.97 &  0.03 &  0.00 \\
 HIP 45333 &   5.17 & $51.10\pm0.32$ &$  -8.6\pm  8.0$&$   4.6\pm  5.5$&$  -5.7\pm  2.7$&$  -5.5\pm  5.2$&  0.99 &  0.01 &  0.00 \\
 HIP 45699 &   6.64 & $24.60\pm0.58$ &$ -14.7\pm  0.5$&$  -0.4\pm  0.5$&$ -17.3\pm  0.9$&$ -34.0\pm  1.0$&  0.97 &  0.03 &  0.00 \\
 HIP 45718 &   8.83 & $15.05\pm1.10$ &$  11.3\pm  0.5$&$ -48.7\pm  3.3$&$ -34.7\pm  3.0$&$ -18.0\pm  2.1$&  0.95 &  0.05 &  0.00 \\
 HIP 45947 &   8.33 &  $8.47\pm1.15$ &$  26.6\pm  1.0$&$ -26.4\pm  1.5$&$-109.8\pm 14.4$&$ -67.8\pm 12.3$&  0.00 &  0.88 &  0.12 \\
 HIP 46066 &   8.93 & $16.31\pm1.17$ &$   4.5\pm  0.5$&$ -27.2\pm  1.8$&$ -19.8\pm  1.6$&$  -7.7\pm  0.9$&  0.99 &  0.01 &  0.00 \\
 HIP 46453 &   7.71 & $12.34\pm0.76$ &$  16.8\pm  0.5$&$ -24.4\pm  1.3$&$ -55.8\pm  4.3$&$ -37.7\pm  4.3$&  0.60 &  0.40 &  0.00 \\
 HIP 46853 &   3.17 & $74.19\pm0.14$ &$  14.6\pm  0.5$&$ -56.8\pm  0.6$&$ -34.7\pm  0.4$&$ -24.8\pm  0.5$&  0.92 &  0.08 &  0.00 \\
 HIP 47080 &   5.41 & $87.96\pm0.32$ &$  14.8\pm  0.5$&$ -36.8\pm  0.4$&$ -17.8\pm  0.2$&$ -15.4\pm  0.4$&  0.98 &  0.02 &  0.00 \\
 HIP 47173 &   6.89 &  $4.42\pm0.51$ &$  -6.6\pm  0.5$&$  -4.7\pm  1.3$&$ -11.1\pm  1.9$&$ -16.7\pm  1.7$&  0.99 &  0.01 &  0.00 \\
 HIP 47292 &   7.75 & $18.23\pm0.81$ &$  17.8\pm  0.5$&$ -35.3\pm  1.6$&$ -30.9\pm  1.3$&$ -30.9\pm  2.5$&  0.94 &  0.06 &  0.00 \\
 HIP 47588 &   8.56 & $14.13\pm0.88$ &$  19.0\pm  3.0$&$ -16.5\pm  1.3$&$ -64.9\pm  4.6$&$ -67.4\pm  6.3$&  0.03 &  0.94 &  0.03 \\
 HIP 48113 &   5.09 & $54.44\pm0.28$ &$   4.8\pm  0.5$&$  11.9\pm  0.4$&$  -5.6\pm  0.1$&$  17.1\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 48152 &   8.32 & $13.74\pm0.78$ &$ -14.5\pm  0.5$&$ 225.4\pm 18.7$&$-238.4\pm 20.9$&$  -6.8\pm  0.6$&  0.00 &  0.00 &  1.00 \\
 HIP 48209 &   9.67 & $13.10\pm1.20$ &$ -35.2\pm  1.0$&$-130.8\pm 31.1$&$-129.9\pm 23.6$&$ -93.7\pm 14.3$&  0.00 &  0.13 &  0.87 \\
 HIP 48468 &   6.29 & $18.57\pm0.45$ &$  59.7\pm 10.4$&$ -82.7\pm  3.5$&$ -54.7\pm  9.6$&$  -8.0\pm  3.9$&  0.62 &  0.37 &  0.01 \\
 HIP 48701 &   8.14 & $22.12\pm1.94$ &$  31.0\pm  1.4$&$ -47.3\pm  3.2$&$  -6.4\pm  0.5$&$   2.0\pm  2.6$&  0.99 &  0.01 &  0.00 \\
 HIP 48833 &   5.14 & $35.53\pm0.71$ &$  -9.9\pm  1.1$&$  -6.0\pm  0.7$&$  -5.7\pm  0.1$&$ -17.3\pm  0.9$&  0.99 &  0.01 &  0.00 \\
 HIP 49070 &   7.60 & $19.64\pm0.56$ &$ -73.6\pm  0.5$&$  77.6\pm  1.5$&$ -21.6\pm  0.3$&$ -27.9\pm  1.3$&  0.92 &  0.08 &  0.00 \\
 HIP 49130 &   7.97 & $27.81\pm0.71$ &$  20.4\pm  0.8$&$ -39.4\pm  1.1$&$ -73.2\pm  2.8$&$  19.2\pm  0.6$&  0.28 &  0.71 &  0.01 \\
 HIP 49246 &   7.49 & $12.82\pm0.76$ &$ -11.8\pm  0.5$&$ -44.0\pm  3.5$&$ -57.3\pm  3.7$&$ -29.8\pm  1.5$&  0.61 &  0.38 &  0.00 \\
 HIP 49572 &   9.30 & $12.00\pm1.16$ &$   0.9\pm  0.5$&$ -20.3\pm  1.8$&$ -55.9\pm  5.0$&$ -26.3\pm  2.4$&  0.75 &  0.25 &  0.00 \\
 HIP 49615 &   7.74 & $21.25\pm0.62$ &$  23.2\pm  0.5$&$ -91.0\pm  4.8$&$ -14.2\pm  0.4$&$ -24.3\pm  2.2$&  0.92 &  0.08 &  0.00 \\
 HIP 49621 &   8.68 & $18.58\pm1.12$ &$ -14.6\pm  0.5$&$ -34.0\pm  2.9$&$ -22.3\pm  1.6$&$ -43.6\pm  2.2$&  0.92 &  0.08 &  0.00 \\
 HIP 49668 &   7.27 & $26.62\pm0.74$ &$  14.7\pm  0.5$&$  10.3\pm  0.5$&$ -45.5\pm  1.3$&$ -47.0\pm  2.0$&  0.69 &  0.31 &  0.00 \\
 HIP 49756 &   7.54 & $28.62\pm0.71$ &$ -18.3\pm  0.5$&$ -21.1\pm  1.0$&$   4.3\pm  0.4$&$ -34.0\pm  0.8$&  0.98 &  0.02 &  0.00 \\
 HIP 49988 &   7.89 & $15.02\pm0.81$ &$  60.8\pm  1.3$&$ -42.8\pm  1.2$&$-100.9\pm  6.0$&$   1.3\pm  3.7$&  0.01 &  0.97 &  0.03 \\
 HIP 50005 &  10.22 & $11.98\pm1.97$ &$  60.1\pm  1.0$&$  90.8\pm 17.0$&$-104.5\pm  9.9$&$  34.0\pm  1.3$&  0.00 &  0.92 &  0.08 \\
 HIP 50319 &   5.97 & $32.08\pm0.80$ &$ -35.6\pm  0.5$&$  -7.2\pm  0.7$&$   9.5\pm  0.2$&$ -44.5\pm  0.6$&  0.95 &  0.05 &  0.00 \\
 HIP 50355 &   7.57 & $25.74\pm0.79$ &$ -14.3\pm  0.5$&$  44.5\pm  1.5$&$ -38.7\pm  1.7$&$  -1.6\pm  0.6$&  0.95 &  0.05 &  0.00 \\
 HIP 50671 &   7.18 & $30.55\pm0.58$ &$  82.6\pm  0.5$&$ -70.7\pm  1.7$&$ -47.3\pm  0.7$&$  57.0\pm  0.4$&  0.21 &  0.77 &  0.02 \\
 HIP 50965 &   9.76 &  $9.14\pm1.37$ &$  19.8\pm  1.0$&$ -61.4\pm  8.3$&$ -93.2\pm 11.6$&$ -91.8\pm 15.3$&  0.00 &  0.79 &  0.21 \\
 HIP 51128 &   8.32 & $20.98\pm0.72$ &$ -20.0\pm  0.9$&$  20.2\pm  0.7$&$  -7.1\pm  0.3$&$  -9.5\pm  0.8$&  0.99 &  0.01 &  0.00 \\
 HIP 51248 &   6.45 & $43.65\pm0.43$ &$  -7.1\pm  0.5$&$  21.2\pm  0.4$&$ -94.1\pm  1.7$&$  22.7\pm  0.7$&  0.02 &  0.96 &  0.02 \\
 HIP 51406 &   7.80 &  $9.00\pm0.61$ &$   5.6\pm  0.5$&$ -13.9\pm  1.2$&$ -13.5\pm  1.3$&$  -4.5\pm  1.0$&  0.99 &  0.01 &  0.00 \\
 HIP 51459 &   4.83 & $78.25\pm0.28$ &$   8.5\pm  0.5$&$ -13.6\pm  0.3$&$  -2.0\pm  0.1$&$   1.8\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 51477 &   8.70 & $11.14\pm0.89$ &$ 102.9\pm  1.0$&$  65.4\pm  7.7$&$-178.6\pm  9.4$&$ -85.6\pm 14.2$&  0.00 &  0.02 &  0.98 \\
 HIP 51784 &   6.68 & $28.69\pm0.53$ &$  -4.7\pm  0.5$&$  14.6\pm  0.5$&$ -15.8\pm  0.7$&$ -17.0\pm  0.6$&  0.99 &  0.01 &  0.00 \\
 HIP 51933 &   5.69 & $39.88\pm0.37$ &$  -6.3\pm  0.5$&$  68.5\pm  1.1$&$ -34.6\pm  0.8$&$ -35.7\pm  0.6$&  0.82 &  0.17 &  0.00 \\
 HIP 51993 &   8.58 &  $8.83\pm0.83$ &$  40.7\pm  0.5$&$ -79.1\pm  7.1$&$ -56.2\pm  5.5$&$  -8.8\pm  5.2$&  0.61 &  0.39 &  0.01 \\
 HIP 52015 &   8.38 & $11.02\pm0.75$ &$  43.7\pm  0.5$&$  13.9\pm  2.9$&$ -62.7\pm  4.3$&$  31.9\pm  0.6$&  0.52 &  0.48 &  0.00 \\
 HIP 52040 &   9.19 & $15.49\pm1.21$ &$  21.2\pm  0.5$&$ -33.0\pm  1.9$&$ -22.2\pm  2.4$&$  11.2\pm  0.7$&  0.98 &  0.02 &  0.00 \\
 HIP 52137 &   8.64 & $19.00\pm1.09$ &$ -21.8\pm  0.5$&$  19.9\pm  0.6$&$ -11.9\pm  0.4$&$  -9.8\pm  0.6$&  0.99 &  0.01 &  0.00 \\
 HIP 52153 &   8.36 & $14.24\pm0.95$ &$  36.2\pm  0.5$&$ -34.5\pm  1.5$&$ -62.9\pm  3.7$&$   3.8\pm  2.0$&  0.69 &  0.31 &  0.00 \\
 HIP 52325 &   8.99 & $16.21\pm1.31$ &$  52.6\pm  0.5$&$ -68.4\pm  7.2$&$ -56.4\pm  1.1$&$   6.4\pm  1.9$&  0.69 &  0.31 &  0.00 \\
 HIP 52673 &   9.55 & $14.07\pm1.29$ &$  74.7\pm  1.0$&$  42.0\pm  3.9$&$-104.3\pm  3.9$&$ -46.9\pm  8.1$&  0.00 &  0.94 &  0.06 \\
 HIP 52761 &   9.18 & $13.65\pm1.33$ &$  -5.0\pm  0.5$&$  -6.3\pm  0.9$&$  -4.0\pm  0.7$&$  -9.8\pm  0.7$&  0.99 &  0.01 &  0.00 \\
 HIP 52771 &  10.23 & $10.45\pm1.42$ &$  83.0\pm  1.8$&$ 152.0\pm 31.1$&$-344.5\pm 54.8$&$  96.3\pm  4.1$&  0.00 &  0.00 &  1.00 \\
 HIP 52990 &   7.53 & $19.60\pm0.60$ &$  42.7\pm  1.3$&$ -47.0\pm  2.0$&$ -63.4\pm  1.7$&$ -16.3\pm  2.2$&  0.57 &  0.42 &  0.00 \\
 HIP 53049 &   7.85 & $20.42\pm0.85$ &$   6.6\pm  0.5$&$  14.4\pm  1.0$&$ -45.9\pm  2.4$&$ -13.5\pm  1.1$&  0.93 &  0.07 &  0.00 \\
 HIP 53229 &   3.82 & $34.38\pm0.21$ &$  14.8\pm  0.8$&$  16.5\pm  0.7$&$ -36.2\pm  0.8$&$  21.4\pm  0.7$&  0.96 &  0.04 &  0.00 \\
 HIP 53535 &   8.35 & $11.90\pm0.91$ &$ -90.1\pm  0.5$&$  48.4\pm  0.4$&$ -75.8\pm  3.1$&$ -43.9\pm  1.9$&  0.05 &  0.93 &  0.02 \\
 HIP 53537 &   7.94 & $20.32\pm0.66$ &$   9.9\pm  0.5$&$ -14.7\pm  0.6$&$ -59.2\pm  2.9$&$ -12.9\pm  1.2$&  0.78 &  0.22 &  0.00 \\
 HIP 53721 &   5.05 & $71.11\pm0.25$ &$  11.1\pm  0.5$&$ -24.0\pm  0.3$&$  -2.5\pm  0.0$&$   0.5\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 53725 &   8.22 & $19.70\pm0.96$ &$  35.3\pm  0.5$&$ -16.9\pm  0.5$&$ -67.0\pm  2.6$&$  -2.1\pm  1.7$&  0.62 &  0.38 &  0.00 \\
 HIP 53898 &   8.18 & $23.24\pm0.74$ &$  14.0\pm  0.6$&$ -40.2\pm  1.6$&$ -23.1\pm  0.9$&$  -6.4\pm  1.0$&  0.98 &  0.02 &  0.00 \\
 HIP 54196 &   7.63 & $18.03\pm0.60$ &$   0.6\pm  0.5$&$ -91.7\pm  5.5$&$ -52.4\pm  3.2$&$ -46.0\pm  2.8$&  0.18 &  0.79 &  0.02 \\
 HIP 54239 &   9.06 & $14.09\pm1.21$ &$  18.0\pm  0.5$&$ -21.2\pm  1.3$&$   8.4\pm  0.9$&$  10.8\pm  0.7$&  0.99 &  0.01 &  0.00 \\
 HIP 54582 &   6.81 & $31.09\pm0.46$ &$ -16.6\pm  0.5$&$ -17.8\pm  0.5$&$ -18.8\pm  0.8$&$ -41.2\pm  0.8$&  0.95 &  0.05 &  0.00 \\
 HIP 54728 &   8.15 & $20.27\pm0.91$ &$ -19.5\pm  0.5$&$  35.3\pm  1.6$&$  -8.4\pm  1.0$&$ -25.5\pm  0.6$&  0.98 &  0.02 &  0.00 \\
HIP 55288A &   7.08 & $20.78\pm1.52$ &$  19.5\pm  2.0$&$ -32.8\pm  2.7$&$ -61.2\pm  4.6$&$ -23.9\pm  3.9$&  0.62 &  0.38 &  0.00 \\
HIP 55288B &   7.90 & $20.78\pm1.52$ &$  16.9\pm  2.0$&$ -32.6\pm  2.7$&$ -59.7\pm  4.6$&$ -25.9\pm  3.9$&  0.64 &  0.36 &  0.00 \\
 HIP 55459 &   7.66 & $24.96\pm0.66$ &$   6.9\pm  0.5$&$   2.5\pm  0.3$&$   9.7\pm  0.3$&$   5.7\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 55592 &   9.96 &  $8.35\pm1.58$ &$  98.7\pm  0.5$&$-105.8\pm 14.5$&$-244.2\pm 39.3$&$   7.1\pm 15.3$&  0.00 &  0.00 &  1.00 \\
 HIP 55666 &   6.95 & $20.10\pm0.60$ &$ -29.3\pm  0.5$&$  -5.4\pm  0.3$&$  -3.0\pm  1.0$&$ -40.4\pm  0.9$&  0.97 &  0.03 &  0.00 \\
 HIP 55761 &   7.87 & $22.95\pm0.64$ &$  10.2\pm  0.5$&$ -23.3\pm  0.8$&$  20.8\pm  0.8$&$  -0.8\pm  0.6$&  0.99 &  0.01 &  0.00 \\
 HIP 56148 &   5.96 & $18.72\pm0.35$ &$ -32.7\pm  0.5$&$  -6.1\pm  0.8$&$  11.4\pm  0.6$&$ -39.3\pm  0.6$&  0.97 &  0.03 &  0.00 \\
 HIP 56186 &   7.18 & $25.03\pm0.55$ &$  29.8\pm  0.5$&$ -79.1\pm  2.5$&$  11.2\pm  0.5$&$   6.6\pm  0.9$&  0.97 &  0.03 &  0.00 \\
 HIP 56290 &   5.48 & $35.73\pm0.54$ &$ -47.9\pm  0.5$&$  22.2\pm  0.2$&$ -29.8\pm  0.3$&$ -32.7\pm  0.4$&  0.95 &  0.05 &  0.00 \\
 HIP 56423 &   7.30 & $22.94\pm0.43$ &$ -30.8\pm  0.5$&$  12.3\pm  0.3$&$ -53.3\pm  1.1$&$  -1.4\pm  0.7$&  0.89 &  0.11 &  0.00 \\
 HIP 56452 &   5.96 & $104.61\pm0.37 &$ -22.3\pm  0.5$&$ -47.6\pm  0.3$&$  19.9\pm  0.4$&$  12.1\pm  0.3$&  0.98 &  0.02 &  0.00 \\
 HIP 56948 &   8.67 & $15.68\pm0.67$ &$   5.5\pm  0.5$&$ -37.7\pm  1.9$&$ -13.8\pm  0.9$&$  -6.6\pm  0.7$&  0.99 &  0.01 &  0.00 \\
 HIP 56960 &   7.42 & $25.52\pm0.71$ &$  -5.8\pm  8.0$&$  -2.5\pm  0.5$&$   0.8\pm  5.1$&$  -6.7\pm  6.2$&  0.99 &  0.01 &  0.00 \\
 HIP 56997 &   5.32 & $104.04\pm0.26 &$  -5.9\pm  0.5$&$   7.9\pm  0.2$&$ -15.9\pm  0.1$&$  -4.1\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 57080 &   7.08 & $21.37\pm0.51$ &$ -51.1\pm  0.5$&$  21.9\pm  0.7$&$  -5.2\pm  1.0$&$ -54.4\pm  0.5$&  0.88 &  0.11 &  0.00 \\
 HIP 57117 &   8.10 &  $7.15\pm0.73$ &$ -27.4\pm  0.5$&$ -11.3\pm  2.6$&$ -29.3\pm  3.3$&$ -29.3\pm  0.7$&  0.96 &  0.04 &  0.00 \\
 HIP 57300 &   8.29 & $13.89\pm1.30$ &$  -8.1\pm  0.8$&$  36.2\pm  4.4$&$ -37.9\pm  4.8$&$  -4.7\pm  0.9$&  0.96 &  0.04 &  0.00 \\
 HIP 57349 &   8.06 & $20.29\pm0.70$ &$  27.8\pm  1.0$&$-114.5\pm  4.8$&$-118.8\pm  5.7$&$  11.7\pm  1.1$&  0.00 &  0.82 &  0.18 \\
 HIP 57443 &   4.89 & $108.45\pm0.22 &$  16.8\pm  0.5$&$ -59.8\pm  0.5$&$ -38.6\pm  0.5$&$   5.2\pm  0.2$&  0.93 &  0.07 &  0.00 \\
 HIP 57450 &   9.91 & $12.85\pm1.33$ &$  64.3\pm  0.5$&$-231.0\pm 23.4$&$-275.3\pm 33.1$&$  53.2\pm  0.7$&  0.00 &  0.00 &  1.00 \\
 HIP 57532 &   8.75 & $17.71\pm0.78$ &$ -92.7\pm  1.1$&$  92.5\pm  2.5$&$ -50.3\pm  0.8$&$ -29.0\pm  1.7$&  0.47 &  0.52 &  0.01 \\
 HIP 57617 &   7.99 & $14.44\pm0.79$ &$ -43.5\pm  0.5$&$ -16.1\pm  1.6$&$  -2.9\pm  1.0$&$ -48.6\pm  0.7$&  0.93 &  0.06 &  0.00 \\
 HIP 57757 &   3.61 & $91.50\pm0.22$ &$   4.1\pm  0.5$&$  40.3\pm  0.3$&$   3.6\pm  0.3$&$   6.5\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 57939 &   6.45 & $109.99\pm0.41 &$ -99.0\pm  0.5$&$ 280.0\pm  1.8$&$-158.3\pm  1.1$&$ -14.0\pm  0.8$&  0.00 &  0.00 &  1.00 \\
 HIP 58171 &   9.22 & $14.08\pm1.33$ &$ -11.0\pm  0.5$&$  -3.6\pm  0.6$&$  13.5\pm  1.2$&$  -7.0\pm  0.6$&  0.99 &  0.01 &  0.00 \\
 HIP 58201 &   9.11 & $12.75\pm1.07$ &$  -2.4\pm  0.5$&$ -16.3\pm  1.5$&$  -8.9\pm  0.8$&$  -6.4\pm  0.6$&  0.99 &  0.01 &  0.00 \\
 HIP 58229 &   9.98 &  $5.84\pm1.38$ &$ 168.0\pm  5.0$&$ -76.6\pm 24.0$&$-206.4\pm 17.9$&$  50.1\pm 12.6$&  0.00 &  0.01 &  0.99 \\
 HIP 58331 &   6.59 & $17.50\pm0.46$ &$  12.2\pm  0.5$&$ -27.6\pm  1.4$&$ -16.7\pm  0.5$&$   6.8\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 58576 &   5.55 & $78.35\pm0.31$ &$   0.0\pm  0.5$&$  21.3\pm  0.2$&$ -15.2\pm  0.3$&$ -16.2\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 58843 &   9.22 & $14.24\pm1.33$ &$   9.8\pm  0.5$&$  98.8\pm  7.8$&$-128.6\pm  9.8$&$ -57.1\pm  5.2$&  0.00 &  0.61 &  0.39 \\
 HIP 59021 &   6.48 & $19.36\pm0.75$ &$  30.0\pm  3.0$&$  10.6\pm  1.0$&$ -50.2\pm  2.8$&$ -29.3\pm  2.7$&  0.83 &  0.17 &  0.00 \\
 HIP 59233 &   9.48 & $12.59\pm1.61$ &$ -10.3\pm  0.5$&$-191.2\pm 48.4$&$ -78.0\pm 20.1$&$ -42.5\pm  8.2$&  0.00 &  0.58 &  0.42 \\
 HIP 59253 &   8.50 & $18.53\pm0.91$ &$   0.4\pm  1.4$&$ -28.8\pm  1.7$&$ -18.3\pm  1.1$&$  -4.5\pm  1.4$&  0.99 &  0.01 &  0.00 \\
 HIP 59532 &   7.43 & $28.69\pm0.46$ &$  14.1\pm  0.5$&$-115.3\pm  3.6$&$  -4.6\pm  0.3$&$  31.2\pm  0.7$&  0.78 &  0.22 &  0.01 \\
 HIP 59589 &   7.56 & $29.02\pm0.69$ &$ -25.0\pm  0.5$&$  47.7\pm  1.4$&$ -69.3\pm  2.2$&$ -50.4\pm  0.9$&  0.07 &  0.91 &  0.02 \\
 HIP 59735 &   8.28 & $18.60\pm1.05$ &$  40.1\pm  0.5$&$  -9.5\pm  0.4$&$   2.3\pm  0.3$&$  39.2\pm  0.5$&  0.97 &  0.03 &  0.00 \\
 HIP 59750 &   6.11 & $44.74\pm0.81$ &$   4.0\pm  5.0$&$  53.1\pm  1.6$&$ -71.3\pm  3.3$&$ -62.0\pm  4.2$&  0.02 &  0.95 &  0.03 \\
 HIP 60019 &   7.50 & $14.76\pm0.55$ &$  -8.2\pm  0.5$&$   2.0\pm  0.3$&$ -16.9\pm  1.3$&$ -22.7\pm  1.1$&  0.98 &  0.02 &  0.00 \\
 HIP 60268 &   8.25 & $24.48\pm0.61$ &$ -82.9\pm  0.5$&$  -2.9\pm  1.1$&$-104.0\pm  2.2$&$ -46.0\pm  0.8$&  0.00 &  0.95 &  0.05 \\
 HIP 60314 &   8.80 & $15.26\pm0.96$ &$   5.7\pm  0.5$&$ -26.4\pm  2.2$&$ -44.7\pm  4.0$&$   3.8\pm  0.5$&  0.94 &  0.06 &  0.00 \\
 HIP 60331 &   8.07 & $23.58\pm0.50$ &$ -98.7\pm  0.5$&$ -49.1\pm  2.6$&$ -79.2\pm  0.7$&$-105.7\pm  1.1$&  0.00 &  0.76 &  0.24 \\
 HIP 60366 &   8.47 & $18.34\pm0.82$ &$  -6.8\pm  0.5$&$   1.5\pm  0.3$&$   1.6\pm  0.3$&$  -6.9\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 60588 &   7.36 & $23.63\pm0.58$ &$ -49.3\pm  0.5$&$  42.7\pm  0.8$&$  -8.0\pm  0.5$&$ -37.3\pm  0.4$&  0.96 &  0.04 &  0.00 \\
 HIP 60719 &   8.04 &  $5.73\pm0.67$ &$   9.0\pm  1.1$&$-137.2\pm 32.3$&$-111.3\pm 25.2$&$ -18.3\pm  6.3$&  0.00 &  0.77 &  0.23 \\
 HIP 60956 &   9.03 & $20.56\pm0.99$ &$   2.1\pm  0.8$&$  -3.4\pm  0.3$&$-142.0\pm  8.3$&$ -75.4\pm  4.6$&  0.00 &  0.49 &  0.51 \\
 HIP 61044 &   7.93 & $20.29\pm0.64$ &$ -11.2\pm  0.5$&$ -21.8\pm  0.9$&$ -63.3\pm  2.2$&$   2.8\pm  0.7$&  0.71 &  0.29 &  0.00 \\
 HIP 61157 &   7.38 & $12.05\pm0.42$ &$  -3.2\pm  0.5$&$  28.6\pm  1.6$&$   1.3\pm  0.4$&$   9.5\pm  0.8$&  0.99 &  0.01 &  0.00 \\
 HIP 61264 &   8.14 & $11.30\pm0.76$ &$  23.8\pm  0.5$&$ -30.6\pm  2.0$&$ -28.0\pm  2.8$&$  26.3\pm  0.6$&  0.96 &  0.04 &  0.00 \\
 HIP 61272 &   8.41 & $19.16\pm0.89$ &$   2.4\pm  0.5$&$   0.1\pm  0.4$&$   1.8\pm  0.3$&$   2.3\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 61293 &   7.43 & $20.42\pm0.47$ &$ -77.6\pm  0.5$&$  51.8\pm  0.6$&$ -40.1\pm  0.3$&$ -47.2\pm  0.4$&  0.66 &  0.33 &  0.00 \\
 HIP 61317 &   4.26 & $118.49\pm0.20 &$   6.3\pm  0.5$&$ -30.7\pm  0.2$&$  -3.5\pm  0.1$&$   1.3\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 62039 &   7.84 & $23.43\pm0.79$ &$  35.1\pm  1.0$&$ -13.7\pm  0.9$&$ -69.9\pm  2.2$&$   7.9\pm  1.2$&  0.51 &  0.48 &  0.00 \\
 HIP 62077 &   9.54 &  $9.32\pm1.13$ &$  15.4\pm  1.0$&$  79.8\pm 12.4$&$ -90.8\pm 13.8$&$  23.7\pm  1.6$&  0.01 &  0.96 &  0.04 \\
 HIP 62162 &   7.61 & $15.95\pm0.74$ &$ -19.5\pm  2.8$&$  -1.9\pm  0.4$&$ -69.4\pm  5.4$&$ -25.8\pm  2.8$&  0.40 &  0.59 &  0.01 \\
 HIP 62175 &   8.01 & $21.62\pm0.61$ &$  -9.4\pm  0.5$&$ -38.5\pm  1.5$&$ -24.0\pm  0.8$&$ -12.4\pm  0.5$&  0.98 &  0.02 &  0.00 \\
 HIP 62198 &   9.06 & $12.66\pm1.18$ &$ -17.0\pm  1.0$&$ -80.2\pm  8.2$&$ -66.2\pm  7.4$&$ -23.4\pm  1.2$&  0.23 &  0.75 &  0.01 \\
 HIP 62240 &   9.46 &  $9.09\pm1.09$ &$ -35.2\pm  0.5$&$  51.5\pm  8.3$&$ -73.8\pm 12.2$&$ -75.9\pm  6.2$&  0.00 &  0.94 &  0.06 \\
 HIP 62307 &   8.49 &  $8.83\pm0.82$ &$  11.4\pm  0.5$&$  39.2\pm  4.4$&$ -28.9\pm  3.0$&$  -7.8\pm  2.2$&  0.97 &  0.02 &  0.00 \\
 HIP 62507 &   8.79 & $11.59\pm0.96$ &$ -43.7\pm  0.5$&$ -81.0\pm  9.0$&$ -84.2\pm  9.6$&$ -45.2\pm  0.5$&  0.01 &  0.95 &  0.04 \\
 HIP 62527 &   7.35 & $26.25\pm0.47$ &$ -21.4\pm  0.5$&$ -85.5\pm  2.3$&$ -51.3\pm  1.0$&$ -28.9\pm  0.5$&  0.51 &  0.48 &  0.01 \\
 HIP 62607 &   8.15 & $30.71\pm0.74$ &$   2.3\pm  0.5$&$  39.5\pm  1.2$&$ -84.2\pm  2.5$&$ -42.4\pm  1.4$&  0.02 &  0.96 &  0.02 \\
 HIP 62661 &   7.61 & $18.46\pm0.73$ &$  -5.1\pm  2.5$&$ -91.7\pm  4.5$&$ -50.3\pm  3.2$&$   1.7\pm  1.4$&  0.66 &  0.33 &  0.00 \\
 HIP 62816 &   8.49 & $19.18\pm0.77$ &$ -11.6\pm  0.5$&$ -32.7\pm  1.8$&$ -16.8\pm  0.8$&$ -13.5\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 62882 &   8.34 & $10.50\pm1.26$ &$ 150.9\pm  1.4$&$ 269.3\pm 23.1$&$-205.3\pm 12.8$&$-111.4\pm 24.0$&  0.00 &  0.00 &  1.00 \\
 HIP 63330 &   7.23 & $17.65\pm0.54$ &$ -41.8\pm  0.5$&$  51.5\pm  2.7$&$ -43.2\pm  2.2$&$ -48.3\pm  0.6$&  0.58 &  0.41 &  0.01 \\
 HIP 63354 &   8.14 & $18.74\pm0.86$ &$ -24.8\pm  0.8$&$ -28.8\pm  1.2$&$  12.4\pm  0.4$&$ -15.6\pm  0.8$&  0.99 &  0.01 &  0.00 \\
 HIP 63405 &   7.19 & $13.06\pm0.57$ &$  -7.0\pm  0.8$&$   7.0\pm  0.7$&$   2.1\pm  0.3$&$  -7.2\pm  0.8$&  0.99 &  0.01 &  0.00 \\
 HIP 63881 &   8.79 & $14.11\pm0.97$ &$  17.0\pm  0.5$&$  32.4\pm  2.3$&$ -70.7\pm  5.1$&$   3.1\pm  1.1$&  0.46 &  0.54 &  0.01 \\
 HIP 64103 &   9.67 & $13.69\pm1.34$ &$ -56.5\pm  0.5$&$ -80.9\pm  6.8$&$ -48.6\pm  6.7$&$ -52.8\pm  0.5$&  0.20 &  0.78 &  0.02 \\
 HIP 64150 &   6.80 & $38.27\pm0.54$ &$  22.6\pm  0.5$&$  57.2\pm  1.2$&$ -64.8\pm  1.4$&$ -11.0\pm  0.9$&  0.51 &  0.49 &  0.01 \\
 HIP 64241 &   4.32 & $56.10\pm0.89$ &$ -12.0\pm  2.2$&$ -31.5\pm 12.3$&$  -9.0\pm  4.3$&$  -8.1\pm  2.6$&  0.99 &  0.01 &  0.00 \\
 HIP 64254 &   9.03 & $14.90\pm1.17$ &$   1.0\pm  0.5$&$  11.6\pm  1.4$&$   0.3\pm  0.3$&$  -1.0\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 64344 &   9.17 & $12.99\pm0.97$ &$ -15.7\pm  0.5$&$  -5.5\pm  0.5$&$  -8.9\pm  1.0$&$ -16.4\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 64394 &   4.26 & $109.54\pm0.17 &$   5.0\pm  0.5$&$ -50.2\pm  0.3$&$  11.5\pm  0.1$&$   7.3\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 64407 &   5.04 & $29.49\pm0.29$ &$ -12.5\pm  0.5$&$  23.1\pm  0.8$&$ -12.5\pm  0.6$&$ -40.6\pm  0.9$&  0.96 &  0.04 &  0.00 \\
 HIP 64426 &   7.31 & $25.87\pm0.76$ &$  49.2\pm  0.5$&$ -82.9\pm  5.2$&$ -69.4\pm  3.8$&$  57.4\pm  0.7$&  0.01 &  0.94 &  0.04 \\
 HIP 64497 &   8.91 & $14.68\pm1.08$ &$ -13.5\pm  0.5$&$ -40.6\pm  2.9$&$ -18.6\pm  2.1$&$  -6.9\pm  0.5$&  0.98 &  0.02 &  0.00 \\
 HIP 64583 &   4.91 & $54.95\pm0.30$ &$ -63.7\pm  0.5$&$ -55.0\pm  0.4$&$  37.8\pm  0.4$&$ -15.3\pm  0.1$&  0.95 &  0.05 &  0.00 \\
 HIP 64698 &   8.45 & $18.48\pm1.10$ &$  -7.5\pm  1.2$&$ -59.6\pm  3.5$&$ -75.8\pm  4.8$&$  -8.1\pm  1.1$&  0.19 &  0.80 &  0.01 \\
 HIP 64792 &   5.21 & $56.95\pm0.26$ &$ -27.4\pm  0.5$&$ -38.6\pm  0.5$&$   1.5\pm  0.1$&$ -18.2\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 64794 &   8.39 & $18.40\pm1.07$ &$  37.0\pm  0.5$&$  53.9\pm  3.2$&$ -36.3\pm  2.2$&$  20.0\pm  1.2$&  0.93 &  0.07 &  0.00 \\
 HIP 64797 &   6.53 & $90.32\pm0.74$ &$   3.8\pm  7.8$&$  35.6\pm  1.5$&$   8.0\pm  0.7$&$  -2.0\pm  7.6$&  0.99 &  0.01 &  0.00 \\
 HIP 64924 &   4.74 & $116.89\pm0.22 &$  -8.2\pm  0.5$&$ -23.6\pm  0.3$&$ -47.1\pm  0.4$&$ -31.7\pm  0.4$&  0.84 &  0.16 &  0.00 \\
 HIP 65049 &   8.01 & $20.80\pm0.87$ &$  -3.3\pm  0.5$&$ -67.8\pm  3.3$&$ -70.5\pm  3.4$&$  10.6\pm  0.8$&  0.28 &  0.71 &  0.01 \\
 HIP 65449 &   9.53 &  $7.69\pm0.85$ &$ -21.6\pm  1.0$&$-150.9\pm 21.0$&$ -61.0\pm  6.4$&$ -44.4\pm  3.9$&  0.01 &  0.88 &  0.11 \\
 HIP 65641 &   8.43 & $19.49\pm0.96$ &$  -0.0\pm  0.5$&$   6.4\pm  0.4$&$  23.4\pm  1.4$&$  -7.4\pm  0.6$&  0.99 &  0.01 &  0.00 \\
 HIP 65708 &   7.43 & $22.69\pm0.66$ &$  -4.9\pm  2.8$&$  78.8\pm  3.5$&$ -34.9\pm  1.7$&$ -52.6\pm  3.1$&  0.46 &  0.53 &  0.01 \\
 HIP 65971 &   8.08 & $22.24\pm0.62$ &$  -2.0\pm  1.2$&$  -9.4\pm  0.4$&$  -4.3\pm  0.6$&$  -2.2\pm  1.0$&  0.99 &  0.01 &  0.00 \\
 HIP 65982 &   7.34 & $32.57\pm2.01$ &$ -52.9\pm  0.5$&$-138.1\pm  6.4$&$ -30.1\pm  2.5$&$  -6.6\pm  2.2$&  0.51 &  0.47 &  0.02 \\
 HIP 66051 &   7.98 & $16.28\pm0.72$ &$ -28.8\pm  0.5$&$  68.6\pm  3.8$&$ -54.9\pm  2.7$&$ -19.9\pm  0.7$&  0.65 &  0.35 &  0.00 \\
 HIP 66464 &   8.41 & $14.97\pm0.80$ &$  18.7\pm  0.5$&$   7.2\pm  0.5$&$ -30.9\pm  2.3$&$  29.2\pm  0.9$&  0.96 &  0.04 &  0.00 \\
 HIP 66514 &   7.77 & $21.74\pm0.80$ &$ -22.8\pm  4.0$&$ -18.5\pm  0.9$&$ -62.0\pm  3.0$&$  -6.2\pm  3.9$&  0.74 &  0.26 &  0.00 \\
 HIP 66860 &   6.16 & $27.44\pm0.36$ &$ -10.1\pm  4.1$&$ -44.5\pm  1.8$&$ -49.4\pm  1.5$&$  -1.6\pm  3.8$&  0.89 &  0.11 &  0.00 \\
 HIP 66974 &   6.94 & $18.89\pm0.70$ &$   5.0\pm  2.2$&$ -66.1\pm  3.9$&$ -57.3\pm  3.2$&$  22.4\pm  2.3$&  0.58 &  0.41 &  0.01 \\
 HIP 67422 &   7.04 & $74.58\pm0.78$ &$ -20.8\pm  0.6$&$ -20.8\pm  0.3$&$ -24.4\pm  0.4$&$ -14.2\pm  0.6$&  0.98 &  0.02 &  0.00 \\
 HIP 67927 &   2.68 & $87.75\pm1.24$ &$   0.6\pm  1.0$&$   9.4\pm  0.3$&$ -17.0\pm  0.2$&$  -1.8\pm  1.0$&  0.99 &  0.01 &  0.00 \\
 HIP 68030 &   6.17 & $40.22\pm0.37$ &$ -10.7\pm  0.5$&$ -28.9\pm  0.5$&$ -19.9\pm  0.4$&$  -1.6\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 68085 &   7.59 & $18.14\pm0.56$ &$ -27.9\pm  0.5$&$  49.8\pm  1.4$&$ -55.9\pm  1.4$&$  22.2\pm  1.5$&  0.71 &  0.29 &  0.00 \\
 HIP 68184 &   6.52 & $99.36\pm0.32$ &$ -25.3\pm  2.0$&$  -2.9\pm  0.4$&$  -9.4\pm  1.1$&$ -25.6\pm  1.6$&  0.99 &  0.01 &  0.00 \\
 HIP 68594 &   6.20 &  $4.22\pm0.35$ &$ -23.3\pm  1.0$&$-132.3\pm 23.6$&$-217.5\pm 41.9$&$  16.3\pm  7.3$&  0.00 &  0.00 &  1.00 \\
 HIP 69210 &   8.98 & $13.81\pm0.80$ &$ -16.8\pm  0.5$&$   6.6\pm  0.4$&$  -8.6\pm  0.4$&$ -14.0\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 69232 &  10.59 &  $5.95\pm1.76$ &$ 122.3\pm  1.4$&$  20.0\pm 16.0$&$-411.6\pm106.4$&$ -49.2\pm 39.1$&  0.00 &  0.00 &  1.00 \\
 HIP 69535 &   7.63 & $17.53\pm1.03$ &$ -10.0\pm  6.0$&$   4.1\pm  0.6$&$  -2.7\pm  3.1$&$  -9.7\pm  5.1$&  0.99 &  0.01 &  0.00 \\
 HIP 69673 &  -0.05 & $88.83\pm0.54$ &$  -4.9\pm  3.8$&$  25.2\pm  1.3$&$-119.0\pm  1.0$&$  -2.7\pm  3.5$&  0.00 &  0.94 &  0.06 \\
 HIP 69701 &   4.08 & $44.97\pm0.19$ &$  12.4\pm  0.5$&$  23.5\pm  0.4$&$ -35.6\pm  0.6$&$ -12.5\pm  0.6$&  0.97 &  0.03 &  0.00 \\
 HIP 69972 &   6.65 & $84.76\pm0.69$ &$ -18.9\pm  0.6$&$ -40.6\pm  0.5$&$ -14.2\pm  0.5$&$ -34.9\pm  0.3$&  0.96 &  0.04 &  0.00 \\
 HIP 70319 &   6.27 & $58.17\pm0.53$ &$ -19.6\pm  0.5$&$  21.7\pm  0.7$&$ -15.3\pm  0.3$&$ -40.2\pm  0.6$&  0.95 &  0.04 &  0.00 \\
 HIP 70324 &   9.32 & $13.69\pm1.20$ &$ -48.7\pm  0.5$&$ -83.8\pm  6.5$&$-104.7\pm  9.9$&$  -7.0\pm  3.8$&  0.00 &  0.94 &  0.06 \\
 HIP 70520 &   7.29 & $22.26\pm0.67$ &$ -49.0\pm  0.5$&$  86.4\pm  4.0$&$ -84.0\pm  3.0$&$ -73.8\pm  1.2$&  0.00 &  0.89 &  0.11 \\
 HIP 70681 &   9.30 & $21.04\pm1.12$ &$ -45.7\pm  0.5$&$ -21.7\pm  0.8$&$ -46.9\pm  4.9$&$ -75.6\pm  3.6$&  0.06 &  0.91 &  0.03 \\
 HIP 71019 &   8.84 & $12.63\pm0.95$ &$  70.1\pm  0.5$&$ 114.9\pm  7.4$&$-113.6\pm  9.6$&$-124.2\pm 18.6$&  0.00 &  0.08 &  0.92 \\
 HIP 71076 &   7.84 & $17.24\pm0.75$ &$ -14.4\pm  0.5$&$ -52.1\pm  2.9$&$ -43.1\pm  2.5$&$  13.0\pm  1.7$&  0.91 &  0.09 &  0.00 \\
 HIP 71193 &   7.63 & $27.18\pm1.05$ &$ -75.0\pm  0.5$&$ -47.0\pm  1.9$&$ -41.4\pm  0.9$&$ -56.2\pm  0.9$&  0.45 &  0.54 &  0.01 \\
 HIP 71284 &   4.47 & $63.16\pm0.25$ &$   0.6\pm  0.5$&$   2.2\pm  0.1$&$  16.1\pm  0.2$&$  -4.8\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 71572 &   8.27 & $21.17\pm1.07$ &$ -18.2\pm  0.5$&$  11.9\pm  1.3$&$ -30.1\pm  1.9$&$ -24.0\pm  0.7$&  0.97 &  0.03 &  0.00 \\
 HIP 71681 &   1.36 & $796.92\pm25.9 &$ -25.1\pm  0.5$&$ -30.8\pm  0.4$&$   4.1\pm  0.4$&$  15.2\pm  0.1$&  0.99 &  0.01 &  0.00 \\
 HIP 71683 &   0.00 & $754.81\pm4.11 &$ -25.1\pm  0.5$&$ -32.0\pm  0.4$&$   2.9\pm  0.3$&$  12.6\pm  0.0$&  0.99 &  0.01 &  0.00 \\
 HIP 71819 &   8.39 & $14.27\pm0.97$ &$ -19.0\pm  0.5$&$ -76.1\pm  5.8$&$-106.7\pm  9.0$&$  30.7\pm  4.1$&  0.00 &  0.93 &  0.07 \\
 HIP 72199 &   8.57 &  $8.49\pm0.86$ &$ -40.5\pm  0.5$&$  46.8\pm  7.2$&$ -23.9\pm  1.1$&$ -45.5\pm  1.3$&  0.87 &  0.12 &  0.00 \\
 HIP 72407 &   9.74 & $10.65\pm0.73$ &$   1.5\pm  1.0$&$ -98.6\pm  8.7$&$ -65.9\pm  5.9$&$  40.8\pm  3.6$&  0.05 &  0.91 &  0.03 \\
 HIP 72467 &   8.16 &  $8.57\pm0.49$ &$ -23.9\pm  0.5$&$  16.0\pm  1.2$&$ -35.7\pm  1.8$&$  -2.3\pm  1.4$&  0.97 &  0.03 &  0.00 \\
 HIP 72604 &   7.50 & $26.53\pm0.56$ &$ -27.4\pm  0.5$&$ -49.7\pm  1.3$&$ -64.8\pm  1.9$&$   8.3\pm  1.1$&  0.56 &  0.44 &  0.00 \\
 HIP 72659 &   4.72 & $148.98\pm0.48 &$   2.3\pm  1.0$&$   5.4\pm  0.4$&$   2.0\pm  0.2$&$  -0.5\pm  0.9$&  0.99 &  0.01 &  0.00 \\
 HIP 72803 &   8.41 &  $8.43\pm0.85$ &$ -95.8\pm  2.4$&$-108.2\pm  7.6$&$ -89.5\pm  3.2$&$ -49.9\pm  3.1$&  0.00 &  0.90 &  0.09 \\
 HIP 72835 &   7.78 & $17.47\pm0.61$ &$  -6.3\pm  0.5$&$  -2.7\pm  0.2$&$   0.9\pm  0.3$&$  -7.1\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 72848 &   6.01 & $86.88\pm0.46$ &$ -33.4\pm  1.0$&$ -37.2\pm  0.5$&$ -13.9\pm  0.2$&$ -16.1\pm  0.9$&  0.98 &  0.02 &  0.00 \\
 HIP 73005 &   7.77 & $42.76\pm0.45$ &$ -15.0\pm  0.5$&$-108.8\pm  1.6$&$ -55.4\pm  0.8$&$  19.3\pm  0.6$&  0.29 &  0.69 &  0.02 \\
 HIP 73078 &   7.91 & $16.22\pm0.69$ &$  10.6\pm  1.0$&$ -36.2\pm  2.2$&$   6.2\pm  0.5$&$  14.6\pm  0.9$&  0.99 &  0.01 &  0.00 \\
 HIP 73385 &   8.51 & $10.23\pm0.84$ &$ 176.4\pm  0.5$&$  41.7\pm 10.3$&$-366.0\pm 32.7$&$  55.0\pm  3.9$&  0.00 &  0.00 &  1.00 \\
 HIP 73440 &   6.66 & $29.34\pm0.55$ &$ -50.6\pm  2.4$&$ -34.6\pm  1.4$&$ -74.9\pm  2.0$&$ -10.4\pm  1.7$&  0.29 &  0.70 &  0.01 \\
 HIP 73695 &   5.03 & $79.95\pm1.56$ &$ -24.1\pm  7.0$&$ -18.1\pm  0.7$&$ -29.8\pm  3.8$&$  -7.7\pm  5.9$&  0.98 &  0.02 &  0.00 \\
 HIP 73768 &   8.18 & $11.23\pm0.98$ &$  21.3\pm  0.5$&$  13.6\pm  1.0$&$ -42.4\pm  6.3$&$  33.1\pm  2.1$&  0.89 &  0.11 &  0.00 \\
 HIP 73815 &   8.18 & $17.39\pm0.80$ &$   3.6\pm  0.5$&$  36.0\pm  2.0$&$ -46.0\pm  2.6$&$ -19.7\pm  1.4$&  0.90 &  0.10 &  0.00 \\
 HIP 74033 &   8.26 & $13.91\pm1.21$ &$ -60.5\pm  0.5$&$-114.5\pm  6.9$&$-125.4\pm 10.5$&$  25.5\pm  6.5$&  0.00 &  0.73 &  0.27 \\
 HIP 74067 &   8.00 & $26.62\pm0.86$ &$ -61.2\pm  0.5$&$ -31.0\pm  0.6$&$ -65.9\pm  2.7$&$ -68.9\pm  1.1$&  0.02 &  0.95 &  0.03 \\
 HIP 74079 &   7.69 & $17.27\pm0.81$ &$  18.8\pm  0.5$&$  14.4\pm  0.4$&$  -2.2\pm  0.4$&$  12.6\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 74326 &   9.09 & $14.05\pm0.75$ &$ -85.8\pm  1.0$&$ -36.6\pm  3.5$&$ -98.1\pm  2.3$&$ -38.2\pm  1.3$&  0.00 &  0.96 &  0.04 \\
 HIP 74341 &   8.86 & $14.83\pm1.22$ &$   4.9\pm  0.5$&$   6.6\pm  0.6$&$ -23.4\pm  2.1$&$  10.9\pm  0.7$&  0.99 &  0.01 &  0.00 \\
 HIP 74442 &   8.37 & $12.53\pm0.87$ &$ -60.7\pm  0.5$&$  10.3\pm  2.5$&$ -47.2\pm  1.8$&$ -56.2\pm  0.6$&  0.44 &  0.55 &  0.01 \\
 HIP 74443 &   9.29 & $22.96\pm1.19$ &$ -60.5\pm  1.0$&$ -39.0\pm  0.7$&$ -70.0\pm  4.3$&$ -47.7\pm  0.8$&  0.09 &  0.89 &  0.02 \\
 HIP 74933 &   8.56 & $12.72\pm1.19$ &$   9.3\pm  1.0$&$  -0.8\pm  0.7$&$ -50.1\pm  4.8$&$  31.9\pm  2.3$&  0.81 &  0.19 &  0.00 \\
 HIP 75206 &   5.00 & $27.89\pm0.33$ &$ -12.1\pm  0.5$&$ -26.2\pm  0.6$&$ -20.0\pm  0.7$&$  -6.9\pm  0.2$&  0.99 &  0.01 &  0.00 \\
 HIP 75281 &   7.91 & $22.18\pm1.01$ &$ -49.0\pm  0.5$&$ -55.2\pm  1.5$&$ -53.9\pm  2.5$&$  -7.7\pm  1.8$&  0.80 &  0.20 &  0.00 \\
 HIP 75370 &   8.72 & $20.43\pm0.73$ &$ -35.1\pm  0.5$&$ -17.6\pm  1.7$&$ -64.9\pm  2.9$&$  10.7\pm  2.6$&  0.65 &  0.34 &  0.00 \\
 HIP 76219 &   4.62 & $34.57\pm0.22$ &$  48.9\pm  0.8$&$  70.6\pm  0.9$&$   0.5\pm  0.1$&$ -14.0\pm  1.1$&  0.98 &  0.02 &  0.00 \\
 HIP 76543 &   7.10 & $22.26\pm0.69$ &$  38.1\pm  0.5$&$  87.3\pm  2.7$&$ -29.8\pm  1.6$&$ -16.3\pm  2.0$&  0.90 &  0.10 &  0.00 \\
 HIP 76556 &   8.13 & $12.83\pm0.60$ &$ -51.1\pm  0.5$&$ -28.8\pm  1.7$&$ -67.4\pm  1.7$&$  -9.0\pm  1.5$&  0.56 &  0.44 &  0.00 \\
 HIP 76899 &   8.27 & $14.18\pm1.05$ &$ -82.5\pm  0.5$&$ -72.0\pm  1.5$&$ -59.8\pm  3.3$&$ -30.8\pm  2.4$&  0.37 &  0.62 &  0.01 \\
 HIP 76911 &   8.54 & $19.09\pm0.94$ &$ -49.2\pm  1.3$&$   4.4\pm  1.5$&$ -57.9\pm  2.2$&$ -31.8\pm  1.1$&  0.66 &  0.33 &  0.00 \\
 HIP 76963 &   7.41 & $17.86\pm0.65$ &$  33.0\pm  0.5$&$  20.7\pm  0.4$&$  -4.7\pm  0.6$&$  27.6\pm  0.5$&  0.98 &  0.02 &  0.00 \\
 HIP 76976 &   7.21 & $17.16\pm0.68$ &$-169.3\pm  1.0$&$-248.6\pm  6.1$&$-252.4\pm 14.5$&$  43.0\pm  7.7$&  0.00 &  0.00 &  1.00 \\
 HIP 77083 &   8.20 & $21.61\pm1.40$ &$   0.6\pm  1.3$&$  14.1\pm  1.4$&$   2.8\pm  0.5$&$ -11.6\pm  1.4$&  0.99 &  0.01 &  0.00 \\
 HIP 77159 &   8.04 & $13.79\pm1.12$ &$   4.7\pm  0.5$&$  26.9\pm  1.9$&$ -35.1\pm  2.8$&$ -13.2\pm  1.4$&  0.97 &  0.03 &  0.00 \\
 HIP 77257 &   4.43 & $82.48\pm0.32$ &$ -66.8\pm  0.5$&$ -49.4\pm  0.3$&$ -24.0\pm  0.1$&$ -40.2\pm  0.4$&  0.91 &  0.09 &  0.00 \\
 HIP 77358 &   6.01 & $65.13\pm0.40$ &$  -6.9\pm  0.5$&$ -20.5\pm  0.5$&$ -27.3\pm  0.4$&$   5.4\pm  0.1$&  0.98 &  0.02 &  0.00 \\
 HIP 77466 &   9.20 & $14.20\pm0.71$ &$ -53.6\pm  0.5$&$ -82.3\pm  4.6$&$ -76.2\pm  2.8$&$  10.6\pm  3.3$&  0.10 &  0.88 &  0.02 \\
 HIP 77655 &   4.81 & $32.79\pm0.21$ &$ -24.9\pm  0.5$&$  34.1\pm  0.8$&$ -41.6\pm  0.6$&$ -18.8\pm  0.4$&  0.93 &  0.07 &  0.00 \\
 HIP 78028 &   8.64 & $18.30\pm0.81$ &$ -20.7\pm  0.5$&$ -26.6\pm  1.1$&$ -44.5\pm  1.8$&$  16.4\pm  1.7$&  0.93 &  0.07 &  0.00 \\
 HIP 78030 &   8.63 & $10.69\pm0.95$ &$ -48.4\pm  0.5$&$ -30.9\pm  1.2$&$ -70.2\pm  7.5$&$ -21.4\pm  1.1$&  0.38 &  0.62 &  0.01 \\
 HIP 78072 &   3.85 & $88.86\pm0.18$ &$   6.4\pm  0.5$&$  56.2\pm  0.5$&$ -33.5\pm  0.3$&$ -24.4\pm  0.4$&  0.93 &  0.07 &  0.00 \\
 HIP 78640 &   9.80 &  $8.41\pm1.02$ &$-158.2\pm  2.5$&$ 107.6\pm 20.8$&$-269.6\pm 24.2$&$ -28.4\pm 12.7$&  0.00 &  0.00 &  1.00 \\
 HIP 78680 &   8.22 & $21.61\pm0.75$ &$   0.1\pm  0.5$&$  -0.9\pm  0.2$&$  11.5\pm  0.6$&$  -7.7\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 78747 &   5.90 & $26.40\pm0.43$ &$  -6.2\pm  0.5$&$ -17.1\pm  0.6$&$ -28.6\pm  0.9$&$  -0.9\pm  0.2$&  0.98 &  0.02 &  0.00 \\
 HIP 78775 &   6.66 & $68.87\pm0.33$ &$ -59.9\pm  0.5$&$ -36.1\pm  0.2$&$ -58.8\pm  0.4$&$ -18.9\pm  0.4$&  0.71 &  0.28 &  0.00 \\
 HIP 79186 &   8.31 & $17.66\pm0.74$ &$ -42.8\pm  0.5$&$ -86.9\pm  3.4$&$ -19.3\pm  0.5$&$  -6.8\pm  1.2$&  0.95 &  0.05 &  0.00 \\
 HIP 79190 &   7.11 & $68.17\pm0.64$ &$  36.1\pm  0.5$&$  36.3\pm  0.4$&$ -12.6\pm  0.3$&$  20.8\pm  0.3$&  0.98 &  0.02 &  0.00 \\
 HIP 79276 &   8.13 & $23.96\pm0.49$ &$ -68.0\pm  0.5$&$  19.2\pm  0.5$&$ -59.6\pm  0.5$&$ -35.5\pm  0.5$&  0.55 &  0.45 &  0.00 \\
 HIP 79304 &   8.67 & $16.09\pm1.08$ &$ -12.1\pm  0.5$&$ -10.5\pm  0.5$&$ -21.5\pm  1.5$&$   0.8\pm  0.8$&  0.99 &  0.01 &  0.00 \\
 HIP 79448 &   8.56 & $14.88\pm0.84$ &$ -57.0\pm  5.0$&$-122.5\pm  6.0$&$ -46.8\pm  3.1$&$  13.8\pm  4.8$&  0.37 &  0.61 &  0.02 \\
 HIP 79545 &   8.25 & $15.05\pm0.91$ &$  49.7\pm  0.5$&$  55.4\pm  1.0$&$   3.3\pm  0.4$&$   3.7\pm  1.6$&  0.99 &  0.01 &  0.00 \\
 HIP 79672 &   5.51 & $71.94\pm0.37$ &$  11.6\pm  0.5$&$  27.2\pm  0.5$&$ -14.5\pm  0.2$&$ -22.6\pm  0.4$&  0.98 &  0.02 &  0.00 \\
 HIP 79837 &   6.86 & $35.06\pm0.57$ &$ -36.3\pm  0.5$&$ -44.5\pm  0.7$&$  16.2\pm  0.9$&$ -36.5\pm  0.4$&  0.96 &  0.04 &  0.00 \\
 HIP 80162 &   9.85 & $17.59\pm1.34$ &$  -9.0\pm  1.0$&$  -1.8\pm  1.0$&$ -88.7\pm  7.5$&$  30.6\pm  3.2$&  0.03 &  0.95 &  0.02 \\
 HIP 80264 &   7.42 & $19.79\pm0.42$ &$ -32.0\pm  0.5$&$   1.3\pm  0.2$&$ -14.6\pm  0.4$&$ -31.6\pm  0.5$&  0.98 &  0.02 &  0.00 \\
 HIP 80337 &   5.39 & $78.26\pm0.37$ &$  12.6\pm  0.5$&$  13.2\pm  0.5$&$  -1.0\pm  0.2$&$  -1.4\pm  0.1$&  0.99 &  0.01 &  0.00 \\
 HIP 80686 &   4.90 & $82.53\pm0.52$ &$   4.8\pm  2.1$&$  10.7\pm  1.5$&$   7.1\pm  1.3$&$  -5.4\pm  0.5$&  0.99 &  0.01 &  0.00 \\
 HIP 80736 &   7.54 & $14.26\pm1.06$ &$ -23.7\pm  0.5$&$ -23.5\pm  0.5$&$ -59.2\pm  4.3$&$ -27.8\pm  1.4$&  0.66 &  0.34 &  0.00 \\
 HIP 80742 &   8.34 & $18.17\pm0.54$ &$ -68.0\pm  0.9$&$ -17.8\pm  0.6$&$ -63.8\pm  0.8$&$ -30.6\pm  0.8$&  0.50 &  0.49 &  0.01 \\
 HIP 80818 &   7.00 & $18.96\pm0.39$ &$ -47.5\pm  0.5$&$  46.7\pm  1.6$&$ -69.8\pm  1.1$&$ -11.0\pm  0.7$&  0.40 &  0.59 &  0.01 \\
 HIP 80837 &   7.28 & $23.41\pm0.79$ &$ -47.8\pm  0.5$&$  85.7\pm  4.6$&$-263.6\pm  9.2$&$ -78.0\pm  1.9$&  0.00 &  0.00 &  1.00 \\
 HIP 81072 &   8.47 &  $8.44\pm0.61$ &$ -48.9\pm  0.5$&$ -58.0\pm  4.1$&$ -47.8\pm  1.2$&$  -3.8\pm  2.5$&  0.87 &  0.12 &  0.00 \\
 HIP 81300 &   5.76 & $102.55\pm0.40 &$ -13.3\pm  0.5$&$   0.5\pm  0.4$&$  -0.5\pm  0.1$&$ -28.7\pm  0.3$&  0.98 &  0.02 &  0.00 \\
 HIP 81312 &   7.11 & $25.64\pm0.54$ &$  -6.5\pm  1.2$&$  70.3\pm  2.1$&$ -49.1\pm  1.5$&$ -15.8\pm  0.9$&  0.78 &  0.22 &  0.00 \\
 HIP 81461 &   8.49 & $14.14\pm1.00$ &$ -35.4\pm 12.8$&$  -3.1\pm 11.2$&$-114.9\pm  9.2$&$ -17.8\pm  6.0$&  0.00 &  0.95 &  0.05 \\
 HIP 81512 &   9.22 & $13.30\pm0.67$ &$ -11.0\pm  0.5$&$  50.0\pm  3.2$&$ -38.1\pm  1.9$&$   5.8\pm  0.9$&  0.95 &  0.05 &  0.00 \\
 HIP 81608 &   6.73 & $15.16\pm0.55$ &$  -7.1\pm  0.5$&$   4.5\pm  0.9$&$ -33.1\pm  2.2$&$ -12.7\pm  0.8$&  0.97 &  0.03 &  0.00 \\
 HIP 81681 &   7.24 & $33.82\pm0.58$ &$ -40.5\pm  0.5$&$  -8.4\pm  0.9$&$ -58.1\pm  1.4$&$ -45.5\pm  0.8$&  0.41 &  0.58 &  0.01 \\
 HIP 81693 &   2.81 & $93.32\pm0.47$ &$ -70.2\pm  0.5$&$ -53.3\pm  0.3$&$ -48.2\pm  0.3$&$ -25.2\pm  0.3$&  0.81 &  0.19 &  0.00 \\
 HIP 81748 &   7.96 & $20.97\pm0.79$ &$ -76.0\pm  1.0$&$ -14.0\pm  2.1$&$ -71.1\pm  2.1$&$ -64.1\pm  1.2$&  0.02 &  0.95 &  0.03 \\
 HIP 82265 &   8.09 & $25.89\pm1.04$ &$ -75.6\pm  0.5$&$ -65.2\pm  0.6$&$ -63.3\pm  2.7$&$ -44.5\pm  1.1$&  0.15 &  0.83 &  0.02 \\
 HIP 82268 &   8.92 & $15.55\pm0.69$ &$ -26.2\pm  1.0$&$  73.9\pm  4.2$&$  -6.8\pm  1.1$&$ -43.4\pm  1.6$&  0.88 &  0.12 &  0.00 \\
 HIP 82621 &   5.87 & $37.12\pm0.72$ &$ -17.9\pm  1.0$&$ -18.3\pm  1.0$&$  -7.6\pm  0.2$&$  -0.6\pm  0.3$&  0.99 &  0.01 &  0.00 \\
 HIP 82629 &   7.84 & $14.79\pm0.77$ &$ -21.0\pm  0.5$&$ -17.4\pm  0.4$&$ -20.2\pm  1.1$&$  -1.2\pm  0.7$&  0.99 &  0.01 &  0.00 \\
 HIP 82708 &   7.23 & $14.91\pm0.61$ &$ -22.6\pm  0.5$&$ -25.8\pm  0.6$&$ -21.9\pm  1.8$&$   6.0\pm  0.9$&  0.99 &  0.01 &  0.00 \\
 HIP 82750 &   7.07 & $25.43\pm0.39$ &$ -90.1\pm  0.5$&$   0.7\pm  0.1$&$-110.4\pm  0.9$&$  -3.8\pm  1.1$&  0.00 &  0.96 &  0.04 \\
 HIP 82935 &   8.27 & $13.49\pm1.01$ &$  -8.0\pm  0.5$&$ -16.0\pm  0.9$&$   3.8\pm  0.6$&$  12.0\pm  1.3$&  0.99 &  0.01 &  0.00 \\
 HIP 83058 &   8.35 & $13.65\pm1.00$ &$ -22.9\pm  0.5$&$ -18.6\pm  0.5$&$ -20.2\pm  1.4$&$  -3.9\pm  0.6$&  0.99 &  0.01 &  0.00 \\
 HIP 83069 &   8.04 & $15.03\pm0.54$ &$   0.4\pm  0.5$&$ -26.9\pm  1.3$&$  -9.6\pm  0.6$&$  21.6\pm  1.1$&  0.99 &  0.01 &  0.00 \\
 HIP 83204 &   7.39 & $23.59\pm0.59$ &$  -1.6\pm  0.5$&$  15.0\pm  0.7$&$  -3.1\pm  0.3$&$ -23.4\pm  0.9$&  0.99 &  0.01 &  0.00 \\
 HIP 83489 &   9.13 & $13.43\pm1.41$ &$ -56.5\pm  2.3$&$  -4.7\pm  4.2$&$-120.6\pm 10.8$&$  17.7\pm  5.7$&  0.00 &  0.93 &  0.07 \\
 HIP 83601 &   6.01 & $48.39\pm0.40$ &$ -17.1\pm  1.6$&$   1.1\pm  1.4$&$ -30.5\pm  0.7$&$ -20.3\pm  0.7$&  0.97 &  0.03 &  0.00 \\
 HIP 84217 &   6.64 & $14.39\pm0.58$ &$  60.9\pm  0.5$&$  65.0\pm  0.9$&$   6.3\pm  1.0$&$   7.0\pm  1.1$&  0.98 &  0.02 &  0.00 \\
 HIP 84405 &   5.05 & $168.54\pm0.54 &$   0.4\pm  0.6$&$   0.3\pm  0.6$&$ -34.3\pm  0.2$&$  -7.5\pm  0.1$&  0.97 &  0.03 &  0.00 \\
 HIP 84478 &   6.33 & $167.49\pm0.60 &$  -0.5\pm  0.5$&$  -0.6\pm  0.5$&$ -33.8\pm  0.2$&$  -7.1\pm  0.1$&  0.98 &  0.02 &  0.00 \\
 HIP 84506 &   8.23 & $11.93\pm1.01$ &$ -62.6\pm  1.0$&$ -20.6\pm  3.8$&$ -50.9\pm  2.9$&$ -45.9\pm  2.7$&  0.57 &  0.42 &  0.01 \\
 HIP 84551 &   5.54 & $20.67\pm0.37$ &$ -39.7\pm  0.5$&$ -42.8\pm  0.5$&$ -19.8\pm  0.9$&$   9.6\pm  0.4$&  0.98 &  0.02 &  0.00 \\
 HIP 84696 &   6.67 & $24.79\pm1.55$ &$ -16.8\pm  1.5$&$ -10.4\pm  1.4$&$ -27.7\pm  2.4$&$   3.5\pm  1.2$&  0.98 &  0.02 &  0.00 \\
 HIP 84720 &   5.56 & $113.61\pm0.69 &$  25.3\pm  0.5$&$  29.7\pm  0.5$&$  20.2\pm  0.4$&$ -35.0\pm  0.4$&  0.96 &  0.04 &  0.00 \\
 HIP 84781 &   8.16 & $13.07\pm0.96$ &$ -84.5\pm  0.5$&$ -93.7\pm  1.9$&$ -61.9\pm  1.8$&$  46.0\pm  5.8$&  0.07 &  0.90 &  0.03 \\
 HIP 84803 &   7.95 & $13.12\pm1.71$ &$ -91.4\pm  1.2$&$ -58.3\pm  3.4$&$ -85.3\pm  7.5$&$ -58.9\pm  4.0$&  0.00 &  0.95 &  0.05 \\
 HIP 84824 &   7.98 & $20.20\pm0.73$ &$ -11.6\pm  0.5$&$  40.4\pm  2.8$&$ -63.9\pm  3.2$&$ -31.3\pm  1.5$&  0.42 &  0.57 &  0.01 \\
 HIP 84862 &   5.39 & $69.80\pm0.25$ &$ -79.2\pm  0.5$&$  25.5\pm  0.6$&$ -81.5\pm  0.4$&$ -64.1\pm  0.3$&  0.00 &  0.96 &  0.04 \\
 HIP 85007 &   6.87 & $34.12\pm0.57$ &$  35.4\pm  0.5$&$  39.8\pm  0.5$&$  15.7\pm  0.4$&$   4.2\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 85042 &   6.28 & $51.22\pm0.40$ &$ -36.5\pm  0.5$&$ -27.7\pm  0.5$&$ -16.9\pm  0.2$&$ -20.0\pm  0.2$&  0.98 &  0.02 &  0.00 \\
 HIP 85090 &   7.79 & $10.18\pm0.78$ &$ -25.5\pm  0.7$&$ -19.9\pm  0.7$&$ -22.1\pm  1.8$&$  -2.1\pm  1.1$&  0.99 &  0.01 &  0.00 \\
 HIP 85235 &   6.43 & $78.11\pm0.30$ &$ -39.1\pm  0.5$&$   1.6\pm  0.1$&$ -50.4\pm  0.4$&$   5.2\pm  0.3$&  0.91 &  0.09 &  0.00 \\
 HIP 85378 &   8.50 & $14.57\pm0.87$ &$ -73.7\pm  0.5$&$ -66.1\pm  1.9$&$-106.2\pm  3.5$&$  65.9\pm  6.6$&  0.00 &  0.86 &  0.14 \\
 HIP 85400 &   8.62 & $11.80\pm0.86$ &$  -1.8\pm  1.7$&$  32.5\pm  2.5$&$ -43.7\pm  3.4$&$  44.9\pm  3.5$&  0.71 &  0.28 &  0.00 \\
 HIP 85650 &   9.61 &  $9.75\pm1.02$ &$ -31.8\pm  1.0$&$ 136.5\pm 16.9$&$-137.8\pm 13.1$&$  68.8\pm 10.0$&  0.00 &  0.20 &  0.80 \\
 HIP 85653 &   7.22 & $44.91\pm0.50$ &$ -84.4\pm  0.5$&$ -26.6\pm  0.2$&$ -56.0\pm  0.4$&$ -60.7\pm  0.3$&  0.15 &  0.83 &  0.02 \\
 HIP 85757 &   8.06 & $12.66\pm0.96$ &$   4.0\pm  0.5$&$  15.2\pm  1.2$&$ -80.8\pm  7.8$&$  64.7\pm  6.0$&  0.00 &  0.96 &  0.04 \\
 HIP 85940 &   7.85 & $11.89\pm0.73$ &$ -29.2\pm  0.5$&$  -8.1\pm  1.4$&$ -36.1\pm  2.1$&$ -14.5\pm  0.5$&  0.97 &  0.03 &  0.00 \\
 HIP 85964 &   7.31 & $15.12\pm0.38$ &$ -22.2\pm  0.5$&$  40.6\pm  1.4$&$ -11.7\pm  0.5$&$ -24.0\pm  0.5$&  0.98 &  0.02 &  0.00 \\
 HIP 86013 &   8.39 & $19.38\pm1.14$ &$-137.3\pm  0.6$&$-165.5\pm  3.1$&$ -62.8\pm  0.3$&$  80.6\pm  7.2$&  0.00 &  0.58 &  0.42 \\
 HIP 86036 &   5.23 & $70.47\pm0.37$ &$ -14.6\pm  0.5$&$  36.0\pm  0.3$&$  -2.6\pm  0.4$&$ -22.0\pm  0.3$&  0.98 &  0.01 &  0.00 \\
 HIP 86225 &   8.45 &  $6.99\pm1.00$ &$   1.9\pm  0.8$&$  11.7\pm  1.7$&$ -13.4\pm  2.2$&$  -3.7\pm  0.9$&  0.99 &  0.01 &  0.00 \\
 HIP 86321 &   9.64 &  $8.38\pm1.29$ &$-239.5\pm  0.5$&$ -84.1\pm 12.9$&$-263.7\pm 19.4$&$ -51.3\pm  7.8$&  0.00 &  0.00 &  1.00 \\
 HIP 86382 &   7.48 & $10.54\pm0.61$ &$  13.0\pm  5.0$&$  56.5\pm  5.0$&$ -22.3\pm  4.4$&$  -6.8\pm  2.5$&  0.98 &  0.02 &  0.00 \\
 HIP 86400 &   6.53 & $90.91\pm0.67$ &$  20.4\pm  1.4$&$  19.7\pm  1.2$&$   0.6\pm  0.6$&$  11.7\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 86431 &   8.38 & $18.07\pm0.66$ &$  33.9\pm  0.5$&$ 204.7\pm  8.1$&$-117.4\pm  6.1$&$  83.9\pm  2.9$&  0.00 &  0.04 &  0.96 \\
 HIP 86568 &   9.72 & $17.13\pm1.01$ &$ -51.3\pm  1.0$&$ -14.9\pm  1.4$&$ -77.1\pm  2.2$&$  21.1\pm  2.9$&  0.21 &  0.78 &  0.01 \\
 HIP 86796 &   5.13 & $64.47\pm0.31$ &$  -9.8\pm  0.5$&$ -14.4\pm  0.5$&$  -8.1\pm  0.2$&$  -3.8\pm  0.1$&  0.99 &  0.01 &  0.00 \\
 HIP 86830 &   9.65 &  $7.45\pm0.80$ &$ -82.5\pm  0.5$&$ 154.6\pm 19.1$&$-105.5\pm  4.7$&$  45.6\pm 11.6$&  0.00 &  0.62 &  0.38 \\
 HIP 86974 &   3.42 & $120.33\pm0.16 &$ -20.5\pm 11.4$&$  13.7\pm  6.3$&$ -34.7\pm  8.1$&$  -7.5\pm  4.9$&  0.97 &  0.03 &  0.00 \\
 HIP 87055 &   8.56 & $18.74\pm0.62$ &$ -50.0\pm  1.6$&$ -29.3\pm  1.7$&$ -69.1\pm  1.6$&$  -4.7\pm  1.1$&  0.51 &  0.48 &  0.00 \\
 HIP 87089 &   8.91 & $26.29\pm1.03$ &$ -96.0\pm  0.5$&$ -57.1\pm  1.1$&$-125.0\pm  3.5$&$  40.6\pm  3.0$&  0.00 &  0.85 &  0.15 \\
 HIP 87533 &   7.62 & $17.11\pm0.95$ &$-115.5\pm  0.5$&$ -78.4\pm  3.4$&$-111.4\pm  8.3$&$ -40.2\pm  2.7$&  0.00 &  0.90 &  0.10 \\
 HIP 87732 &   7.91 & $10.70\pm0.79$ &$  39.5\pm  0.5$&$  62.8\pm  3.4$&$   2.4\pm  2.2$&$ -21.1\pm  3.4$&  0.98 &  0.02 &  0.00 \\
 HIP 88010 &   9.59 & $14.72\pm2.12$ &$ 186.1\pm  0.5$&$ 267.9\pm 16.6$&$-284.3\pm 61.8$&$  31.9\pm  2.5$&  0.00 &  0.00 &  1.00 \\
 HIP 88039 &   8.77 &  $9.87\pm1.27$ &$ -18.5\pm  1.0$&$  -5.5\pm  2.0$&$-113.1\pm 14.9$&$  76.7\pm 10.3$&  0.00 &  0.82 &  0.18 \\
 HIP 88166 &   9.22 & $20.54\pm1.33$ &$ -12.7\pm  1.0$&$  41.3\pm  3.6$&$-102.2\pm  6.7$&$  68.5\pm  5.1$&  0.00 &  0.90 &  0.10 \\
 HIP 88194 &   7.07 & $35.26\pm0.50$ &$   2.1\pm  1.3$&$ -18.1\pm  0.8$&$   2.4\pm  1.0$&$  24.6\pm  0.7$&  0.99 &  0.01 &  0.00 \\
 HIP 88427 &   9.30 & $12.08\pm1.05$ &$ -11.9\pm  0.5$&$  64.9\pm  6.5$&$ -40.9\pm  2.9$&$ -15.3\pm  1.1$&  0.89 &  0.10 &  0.00 \\
 HIP 88601 &   4.25 & $196.72\pm0.83 &$ -10.4\pm  0.5$&$   3.0\pm  0.4$&$ -20.5\pm  0.3$&$ -15.1\pm  0.1$&  0.99 &  0.01 &  0.00 \\
 HIP 88745 &   5.05 & $63.93\pm0.34$ &$   1.7\pm  0.5$&$  -5.7\pm  0.3$&$   1.1\pm  0.4$&$   9.7\pm  0.2$&  0.99 &  0.01 &  0.00 \\
 HIP 88766 &   8.69 & $15.57\pm1.03$ &$  18.9\pm  4.2$&$  52.3\pm  4.0$&$ -27.7\pm  3.9$&$   0.1\pm  1.3$&  0.97 &  0.03 &  0.00 \\
 HIP 88945 &   6.85 & $40.29\pm0.49$ &$ -14.7\pm  0.7$&$ -14.5\pm  0.4$&$  -4.3\pm  0.6$&$ -10.6\pm  0.3$&  0.99 &  0.01 &  0.00 \\
 HIP 88972 &   6.40 & $90.71\pm0.30$ &$ -20.0\pm  0.5$&$  16.6\pm  0.2$&$ -31.8\pm  0.4$&$   0.0\pm  0.2$&  0.98 &  0.02 &  0.00 \\
 HIP 89268 &   9.22 & $14.40\pm1.02$ &$ -12.2\pm  0.5$&$  -2.1\pm  0.6$&$   5.7\pm  1.6$&$ -42.1\pm  3.8$&  0.96 &  0.04 &  0.00 \\
 HIP 89408 &   6.55 & $23.64\pm0.37$ &$   1.8\pm  0.5$&$  41.1\pm  1.1$&$ -17.6\pm  0.6$&$ -17.1\pm  0.5$&  0.98 &  0.02 &  0.00 \\
 HIP 89443 &   8.83 & $15.30\pm0.72$ &$ -16.5\pm  0.9$&$   4.5\pm  0.4$&$ -33.2\pm  1.2$&$  27.5\pm  1.7$&  0.96 &  0.04 &  0.00 \\
 HIP 89474 &   6.30 & $43.82\pm0.29$ &$ -64.9\pm  0.5$&$  -4.7\pm  0.2$&$ -62.4\pm  0.4$&$ -22.8\pm  0.2$&  0.65 &  0.35 &  0.00 \\
 HIP 89583 &   8.91 & $17.29\pm1.04$ &$ -57.7\pm  0.5$&$ -39.7\pm  1.1$&$ -56.4\pm  2.5$&$ -47.3\pm  3.0$&  0.35 &  0.64 &  0.01 \\
 HIP 89937 &   3.57 & $124.11\pm0.87 &$  32.4\pm  0.6$&$   3.6\pm  0.1$&$  40.2\pm  0.5$&$  -3.0\pm  0.3$&  0.97 &  0.03 &  0.00 \\
 HIP 90144 &   7.79 & $17.28\pm0.84$ &$  -1.2\pm  0.5$&$   6.4\pm  0.7$&$   4.2\pm  0.5$&$ -38.8\pm  2.7$&  0.97 &  0.03 &  0.00 \\
 HIP 90539 &   8.31 & $26.19\pm0.76$ &$ -58.0\pm  0.5$&$ -21.9\pm  1.3$&$ -85.7\pm  2.5$&$   2.4\pm  0.3$&  0.09 &  0.89 &  0.01 \\
 HIP 90542 &   8.35 & $12.61\pm0.59$ &$ -76.0\pm  8.7$&$ -87.1\pm  4.7$&$ -73.6\pm  7.8$&$ -21.8\pm  3.9$&  0.09 &  0.89 &  0.02 \\
 HIP 90655 &   8.80 &  $8.27\pm1.30$ &$ -87.3\pm  0.5$&$ -91.2\pm  1.0$&$ -37.2\pm  4.5$&$ -57.1\pm 11.4$&  0.23 &  0.75 &  0.02 \\
 HIP 90745 &   8.35 & $15.09\pm0.67$ &$ -76.2\pm  0.5$&$ -69.5\pm  2.0$&$ -66.8\pm  0.5$&$  32.8\pm  3.2$&  0.19 &  0.79 &  0.01 \\
 HIP 90790 &   6.81 & $75.46\pm0.70$ &$ -39.5\pm  6.4$&$ -34.5\pm  6.2$&$ -23.8\pm  1.5$&$   5.1\pm  0.5$&  0.98 &  0.02 &  0.00 \\
 HIP 90833 &   8.27 & $21.39\pm0.58$ &$ -18.3\pm  0.8$&$ -16.6\pm  0.6$&$ -18.3\pm  0.7$&$  -5.0\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 91058 &   7.57 & $20.15\pm0.52$ &$ -37.0\pm  0.5$&$ -66.9\pm  1.8$&$   4.7\pm  1.4$&$ -38.7\pm  1.0$&  0.93 &  0.07 &  0.00 \\
 HIP 91120 &   7.16 & $20.23\pm0.37$ &$ -62.5\pm  0.9$&$ -38.0\pm  0.6$&$ -50.6\pm  0.8$&$ -16.6\pm  0.4$&  0.86 &  0.14 &  0.00 \\
 HIP 91395 &   7.74 & $18.58\pm0.54$ &$ -45.3\pm  1.6$&$ -32.5\pm  1.2$&$ -62.7\pm  1.6$&$  15.4\pm  1.3$&  0.65 &  0.34 &  0.00 \\
 HIP 91438 &   5.86 & $76.43\pm0.47$ &$  36.6\pm  0.5$&$  37.7\pm  0.5$&$  -2.2\pm  0.2$&$  -4.4\pm  0.1$&  0.99 &  0.01 &  0.00 \\
 HIP 92270 &   6.12 & $34.78\pm0.41$ &$   3.1\pm  0.5$&$   1.7\pm  0.3$&$   3.4\pm  0.4$&$  -2.8\pm  0.1$&  0.99 &  0.01 &  0.00 \\
 HIP 92720 &   7.90 & $18.68\pm0.67$ &$ -68.3\pm  0.5$&$  -3.0\pm  0.9$&$ -70.5\pm  0.6$&$ -16.2\pm  0.2$&  0.46 &  0.54 &  0.01 \\
 HIP 93062 &   8.21 &  $8.84\pm0.55$ &$  -0.4\pm  0.5$&$  53.2\pm  4.1$&$   5.4\pm  0.7$&$  -2.2\pm  0.4$&  0.99 &  0.01 &  0.00 \\
 HIP 93269 &   9.17 & $13.93\pm0.76$ &$-142.1\pm  1.0$&$  60.2\pm  2.8$&$-144.9\pm  1.2$&$ -13.0\pm  2.5$&  0.00 &  0.71 &  0.29 \\
 HIP 93377 &   7.86 & $25.97\pm1.02$ &$  12.4\pm  4.0$&$  26.4\pm  2.8$&$ -13.4\pm  3.1$&$  54.0\pm  2.1$&  0.86 &  0.13 &  0.00 \\
 HIP 93827 &   7.25 & $26.28\pm0.65$ &$  -0.7\pm  0.5$&$  33.0\pm  1.2$&$ -77.0\pm  2.5$&$  -2.6\pm  0.2$&  0.26 &  0.74 &  0.01 \\
 HIP 94129 &   8.21 & $17.60\pm0.76$ &$ -45.3\pm  1.0$&$  -4.6\pm  2.3$&$-127.3\pm  6.3$&$  34.3\pm  1.4$&  0.00 &  0.89 &  0.11 \\
 HIP 94449 &   9.08 &  $8.15\pm1.43$ &$ -65.4\pm  1.0$&$ 145.5\pm 36.1$&$-314.9\pm 50.3$&$  53.3\pm  8.7$&  0.00 &  0.00 &  1.00 \\
 HIP 94615 &   9.65 & $11.18\pm1.50$ &$ -81.4\pm  1.0$&$ -59.2\pm  1.7$&$ -60.1\pm  1.1$&$  30.8\pm  5.6$&  0.44 &  0.55 &  0.01 \\
 HIP 94842 &   8.34 & $21.36\pm0.86$ &$ -89.2\pm  0.8$&$-102.5\pm  2.8$&$ -40.2\pm  1.9$&$ -17.5\pm  0.5$&  0.70 &  0.29 &  0.01 \\
 HIP 95446 &   8.19 & $16.27\pm0.75$ &$   2.5\pm  0.5$&$  16.7\pm  0.9$&$   0.0\pm  0.5$&$ -34.8\pm  2.0$&  0.98 &  0.02 &  0.00 \\
 HIP 96049 &   8.29 & $11.95\pm0.51$ &$ -63.2\pm  0.5$&$  41.6\pm  2.1$&$ -59.8\pm  0.5$&$ -15.3\pm  0.4$&  0.70 &  0.30 &  0.00 \\
 HIP 96100 &   4.68 & $173.77\pm0.18 &$  26.3\pm  0.5$&$  31.6\pm  0.1$&$  43.0\pm  0.5$&$ -19.1\pm  0.2$&  0.94 &  0.06 &  0.00 \\
 HIP 96142 &   9.40 & $12.77\pm1.70$ &$ -14.8\pm  2.1$&$  54.0\pm  9.5$&$ -89.9\pm 11.6$&$ -91.8\pm 13.5$&  0.00 &  0.82 &  0.18 \\
 HIP 96185 &   6.63 & $31.33\pm0.39$ &$-166.7\pm  0.5$&$ -65.0\pm  0.2$&$-162.0\pm  0.5$&$  58.5\pm  1.5$&  0.00 &  0.22 &  0.78 \\
 HIP 96901 &   6.23 & $47.14\pm0.27$ &$ -28.1\pm  0.6$&$  17.6\pm  0.2$&$ -30.7\pm  0.6$&$  -1.8\pm  0.2$&  0.98 &  0.02 &  0.00 \\
 HIP 96902 &   8.50 & $10.94\pm1.07$ &$-104.7\pm  1.0$&$ -13.0\pm  4.9$&$-113.9\pm  3.0$&$ -61.8\pm  7.4$&  0.00 &  0.88 &  0.12 \\
 HIP 96895 &   5.96 & $47.44\pm0.27$ &$ -27.5\pm  0.5$&$  18.0\pm  0.2$&$ -30.5\pm  0.5$&$  -0.3\pm  0.1$&  0.98 &  0.02 &  0.00 \\
 HIP 97023 &   6.86 & $22.53\pm0.60$ &$  -8.1\pm  0.5$&$  32.0\pm  1.4$&$ -27.0\pm  0.9$&$ -45.2\pm  1.7$&  0.89 &  0.11 &  0.00 \\
 HIP 97420 &   6.88 & $38.11\pm0.47$ &$ -33.3\pm  0.5$&$ -35.5\pm  0.4$&$ -20.0\pm  0.5$&$  14.1\pm  0.3$&  0.98 &  0.02 &  0.00 \\
 HIP 97846 &   7.57 & $17.88\pm0.53$ &$ -73.6\pm  0.5$&$ -92.1\pm  3.0$&$ -55.5\pm  0.8$&$  48.5\pm  2.3$&  0.11 &  0.86 &  0.03 \\
 HIP 97918 &   7.98 & $13.52\pm0.69$ &$ -86.3\pm  0.5$&$ -54.3\pm  0.6$&$ -69.5\pm  0.5$&$ -17.7\pm  1.6$&  0.34 &  0.66 &  0.01 \\
 HIP 98020 &   8.83 & $26.71\pm1.08$ &$-192.2\pm  0.5$&$-152.1\pm  1.4$&$-113.4\pm  1.5$&$  62.6\pm  1.6$&  0.00 &  0.43 &  0.57 \\
 HIP 98036 &   3.71 & $73.00\pm0.20$ &$ -39.7\pm  0.5$&$ -10.8\pm  0.4$&$ -48.5\pm  0.4$&$ -10.0\pm  0.2$&  0.92 &  0.08 &  0.00 \\
 HIP 98416 &   5.88 & $45.04\pm0.99$ &$  29.9\pm  0.5$&$  53.9\pm  1.1$&$ -29.7\pm  1.5$&$  -4.1\pm  0.4$&  0.97 &  0.03 &  0.00 \\
 HIP 98532 &   7.73 & $15.39\pm0.81$ &$ -13.0\pm  0.5$&$  75.2\pm  6.4$&$-127.5\pm  9.0$&$  43.3\pm  3.0$&  0.00 &  0.78 &  0.22 \\
 HIP 98792 &   7.27 & $63.43\pm0.57$ &$  -2.9\pm  0.5$&$  84.6\pm  1.2$&$ -46.2\pm  0.7$&$  27.3\pm  0.4$&  0.65 &  0.34 &  0.01 \\
 HIP 98819 &   5.80 & $56.28\pm0.35$ &$   4.8\pm  0.5$&$  42.0\pm  0.6$&$ -20.4\pm  0.5$&$   9.7\pm  0.2$&  0.98 &  0.02 &  0.00 \\
 HIP 98921 &   6.17 & $53.22\pm0.36$ &$ -26.1\pm  1.1$&$ -26.8\pm  0.4$&$ -18.8\pm  1.1$&$ -16.2\pm  0.2$&  0.98 &  0.02 &  0.00 \\
 HIP 99025 &   8.01 & $11.91\pm0.92$ &$   5.4\pm  0.5$&$  28.4\pm  3.2$&$ -26.6\pm  3.8$&$  -3.4\pm  0.8$&  0.98 &  0.02 &  0.00 \\
 HIP 99224 &   8.12 & $16.97\pm0.78$ &$  -1.9\pm  0.8$&$   7.6\pm  1.0$&$ -93.6\pm  6.4$&$ -75.1\pm  5.1$&  0.00 &  0.92 &  0.08 \\
 HIP 99240 &   3.56 & $163.71\pm0.17 &$ -21.9\pm  0.5$&$ -48.8\pm  0.4$&$ -13.4\pm  0.2$&$ -14.9\pm  0.3$&  0.98 &  0.02 &  0.00 \\
 HIP 99241 &   7.40 & $22.09\pm0.43$ &$  -8.9\pm  0.5$&$ -21.5\pm  0.5$&$  -6.7\pm  0.5$&$  -4.0\pm  0.2$&  0.99 &  0.01 &  0.00 \\
 HIP 99386 &   8.01 & $14.14\pm0.76$ &$ -33.0\pm  0.5$&$ -27.2\pm  0.8$&$ -23.5\pm  0.6$&$  -4.6\pm  0.6$&  0.98 &  0.02 &  0.00 \\
 HIP 99461 &   5.32 & $166.25\pm0.27 &$-129.4\pm  0.5$&$-118.4\pm  0.4$&$ -52.2\pm  0.2$&$  47.0\pm  0.3$&  0.06 &  0.89 &  0.04 \\
 HIP 99607 &   7.75 & $13.40\pm0.74$ &$  -1.2\pm 19.0$&$   7.6\pm 10.3$&$  -4.7\pm 15.7$&$   8.5\pm  3.3$&  0.99 &  0.01 &  0.00 \\
 HIP 99825 &   5.73 & $112.22\pm0.30 &$ -54.8\pm  0.5$&$ -72.7\pm  0.5$&$ -11.7\pm  0.1$&$ -18.2\pm  0.4$&  0.97 &  0.03 &  0.00 \\
HIP 100017 &   5.92 & $56.92\pm0.24$ &$  -4.7\pm  0.5$&$ -40.6\pm  0.4$&$  -5.7\pm  0.5$&$ -21.8\pm  0.2$&  0.98 &  0.02 &  0.00 \\
HIP 100568 &   8.65 & $22.78\pm1.00$ &$-170.8\pm  0.5$&$-155.0\pm  1.0$&$-245.3\pm 10.2$&$ -72.9\pm  8.5$&  0.00 &  0.00 &  1.00 \\
HIP 100783 &   7.49 & $10.17\pm0.56$ &$ -51.4\pm  0.5$&$ -44.3\pm  0.9$&$ -29.4\pm  0.5$&$   7.0\pm  1.2$&  0.97 &  0.03 &  0.00 \\
HIP 100963 &   7.09 & $35.42\pm0.59$ &$  -1.5\pm  0.5$&$  23.9\pm  0.6$&$ -16.3\pm  0.6$&$ -15.5\pm  0.4$&  0.99 &  0.01 &  0.00 \\
HIP 100970 &   6.89 & $25.96\pm0.99$ &$ -91.7\pm  0.5$&$ -71.9\pm  1.0$&$ -75.9\pm  0.4$&$ -37.5\pm  1.9$&  0.05 &  0.93 &  0.02 \\
HIP 101136 &   7.64 & $18.11\pm0.68$ &$ -11.7\pm  0.5$&$  -1.5\pm  0.6$&$ -24.9\pm  1.0$&$ -10.1\pm  0.8$&  0.98 &  0.02 &  0.00 \\
HIP 102081 &   8.31 & $18.03\pm0.73$ &$ -57.7\pm  1.0$&$ -49.4\pm  1.7$&$ -52.0\pm  1.0$&$ -50.9\pm  3.0$&  0.34 &  0.65 &  0.01 \\
HIP 102152 &   9.18 & $12.84\pm0.97$ &$ -44.2\pm  0.5$&$ -74.1\pm  3.9$&$ -11.2\pm  0.4$&$ -28.5\pm  5.3$&  0.95 &  0.05 &  0.00 \\
HIP 102379 &   8.22 & $14.15\pm0.93$ &$ -17.0\pm  0.5$&$ -20.8\pm  1.0$&$ -47.4\pm  3.8$&$ -43.8\pm  5.1$&  0.69 &  0.30 &  0.00 \\
HIP 102422 &   3.42 & $70.10\pm0.11$ &$ -87.3\pm  1.0$&$ -35.0\pm  0.4$&$ -97.0\pm  1.0$&$  10.6\pm  0.3$&  0.01 &  0.96 &  0.02 \\
HIP 102610 &   7.44 & $24.90\pm0.70$ &$ -33.4\pm  0.5$&$ -23.4\pm  0.4$&$ -22.7\pm  0.4$&$  11.0\pm  0.2$&  0.98 &  0.02 &  0.00 \\
HIP 102611 &   7.59 & $18.01\pm0.63$ &$  22.9\pm  0.5$&$  -5.1\pm  0.8$&$  17.3\pm  0.4$&$ -36.8\pm  1.5$&  0.97 &  0.03 &  0.00 \\
HIP 102762 &   8.13 & $17.11\pm0.88$ &$ -83.2\pm  0.5$&$ -87.2\pm  1.6$&$ -76.9\pm  3.0$&$ -15.3\pm  3.9$&  0.07 &  0.91 &  0.02 \\
HIP 102805 &   6.01 & $32.66\pm0.41$ &$   4.4\pm  0.5$&$ -10.9\pm  0.4$&$  12.0\pm  0.5$&$   0.1\pm  0.2$&  0.99 &  0.01 &  0.00 \\
HIP 103237 &   7.76 & $14.35\pm0.84$ &$ -28.9\pm  0.6$&$ -18.6\pm  0.5$&$ -21.6\pm  0.5$&$   8.0\pm  0.5$&  0.99 &  0.01 &  0.00 \\
HIP 103987 &   7.32 & $19.27\pm0.99$ &$  -4.9\pm  3.2$&$  96.0\pm  7.5$&$ -74.8\pm  5.6$&$   9.2\pm  1.7$&  0.08 &  0.90 &  0.02 \\
HIP 104347 &   8.30 &  $8.25\pm0.89$ &$  -8.6\pm  0.8$&$ -37.9\pm  4.3$&$  -3.3\pm  1.0$&$   9.4\pm  1.0$&  0.99 &  0.01 &  0.00 \\
HIP 104421 &   8.00 & $13.74\pm0.81$ &$  -4.2\pm  0.5$&$ -32.5\pm  2.3$&$  -2.4\pm  0.5$&$ -27.4\pm  2.1$&  0.98 &  0.02 &  0.00 \\
HIP 104504 &   8.54 & $20.06\pm0.94$ &$ -16.9\pm  0.5$&$ -40.3\pm  1.8$&$ -13.0\pm  0.6$&$ -23.3\pm  2.2$&  0.98 &  0.02 &  0.00 \\
HIP 104514 &   8.15 & $15.49\pm0.85$ &$  31.5\pm  1.8$&$  17.0\pm  0.8$&$  37.9\pm  1.8$&$  25.3\pm  2.6$&  0.95 &  0.04 &  0.00 \\
HIP 104520 &   8.01 & $12.77\pm0.52$ &$  42.1\pm  0.5$&$ -37.7\pm  1.9$&$  41.1\pm  0.5$&$ -13.5\pm  0.8$&  0.95 &  0.05 &  0.00 \\
HIP 104659 &   7.37 & $29.10\pm0.64$ &$ -44.9\pm  0.5$&$  91.8\pm  3.9$&$-115.4\pm  2.8$&$ -58.5\pm  2.7$&  0.00 &  0.78 &  0.22 \\
HIP 104660 &   8.06 & $18.60\pm0.92$ &$-103.4\pm  0.5$&$-129.6\pm  7.9$&$ -82.5\pm  1.0$&$ -37.2\pm  5.3$&  0.00 &  0.91 &  0.09 \\
HIP 105202 &   7.27 & $23.92\pm0.76$ &$  -1.1\pm  0.5$&$ -15.5\pm  0.6$&$  -6.7\pm  0.5$&$ -24.1\pm  0.9$&  0.99 &  0.01 &  0.00 \\
HIP 105481 &   7.46 & $16.15\pm0.70$ &$ -26.1\pm  0.5$&$ -25.8\pm  0.7$&$ -60.7\pm  3.7$&$ -24.8\pm  3.0$&  0.64 &  0.35 &  0.00 \\
HIP 105766 &   7.28 & $37.87\pm0.42$ &$ -76.9\pm  0.5$&$  15.5\pm  0.2$&$ -73.2\pm  0.5$&$ -19.1\pm  0.1$&  0.34 &  0.66 &  0.01 \\
HIP 105857 &   8.31 & $11.83\pm0.72$ &$  24.6\pm  0.5$&$   4.9\pm  0.4$&$  22.7\pm  0.5$&$ -19.1\pm  1.4$&  0.98 &  0.02 &  0.00 \\
HIP 105858 &   4.23 & $107.97\pm0.19 &$ -29.9\pm  0.5$&$ -13.1\pm  0.3$&$  43.9\pm  0.3$&$   5.8\pm  0.3$&  0.96 &  0.04 &  0.00 \\
HIP 105969 &   8.27 & $13.84\pm1.43$ &$ -92.4\pm  0.9$&$ -10.4\pm  2.5$&$ -89.7\pm  0.9$&$ -66.1\pm  6.4$&  0.00 &  0.95 &  0.05 \\
HIP 106040 &   7.80 & $16.69\pm0.91$ &$ -28.6\pm  0.6$&$ -34.5\pm  1.6$&$ -19.2\pm  0.7$&$  10.2\pm  0.3$&  0.98 &  0.02 &  0.00 \\
HIP 106122 &   7.91 & $34.36\pm0.61$ &$ -87.8\pm  0.5$&$ -77.2\pm  1.8$&$ -88.5\pm  0.5$&$   0.6\pm  0.2$&  0.02 &  0.95 &  0.03 \\
HIP 106157 &   7.62 & $14.56\pm0.66$ &$ -26.8\pm  0.5$&$  36.4\pm  3.2$&$ -44.2\pm  1.6$&$  10.4\pm  0.4$&  0.93 &  0.07 &  0.00 \\
HIP 106678 &   8.64 & $12.94\pm0.87$ &$ -74.6\pm  0.5$&$ -97.4\pm  5.9$&$ -51.8\pm  1.1$&$   4.1\pm  2.1$&  0.57 &  0.42 &  0.01 \\
HIP 106947 &   9.50 & $17.28\pm1.32$ &$-107.0\pm  1.0$&$ -65.3\pm  3.3$&$ -73.8\pm  2.0$&$  69.6\pm  2.4$&  0.00 &  0.94 &  0.05 \\
HIP 107236 &  10.14 & $11.21\pm1.11$ &$ -41.2\pm  1.0$&$ -81.6\pm  9.9$&$ -85.9\pm  5.1$&$  27.0\pm  4.0$&  0.01 &  0.95 &  0.03 \\
HIP 107294 &  10.00 &  $9.03\pm1.68$ &$ -95.0\pm  1.0$&$ 128.9\pm 26.9$&$-106.5\pm  3.6$&$  55.0\pm  4.1$&  0.00 &  0.72 &  0.28 \\
HIP 107350 &   5.94 & $55.91\pm0.45$ &$ -17.2\pm  0.5$&$ -14.7\pm  0.2$&$ -21.6\pm  0.4$&$ -10.8\pm  0.4$&  0.99 &  0.01 &  0.00 \\
HIP 107975 &   5.53 & $36.43\pm0.32$ &$  19.0\pm  0.5$&$  13.6\pm  0.2$&$  15.8\pm  0.5$&$  -7.4\pm  0.2$&  0.99 &  0.01 &  0.00 \\
HIP 108056 &   9.09 & $11.42\pm1.11$ &$ -98.3\pm  1.0$&$  -5.3\pm  0.4$&$ -73.0\pm  2.9$&$ 110.4\pm 10.8$&  0.00 &  0.79 &  0.21 \\
HIP 108490 &   6.96 & $34.78\pm0.41$ &$   9.1\pm  0.5$&$  73.2\pm  1.5$&$  -2.1\pm  0.5$&$ -11.0\pm  0.2$&  0.98 &  0.02 &  0.00 \\
HIP 108514 &   8.47 &  $4.83\pm0.93$ &$ -15.5\pm  1.6$&$   2.0\pm  0.8$&$ -16.6\pm  1.6$&$  -2.6\pm  1.7$&  0.99 &  0.01 &  0.00 \\
HIP 108708 &   8.94 & $14.59\pm1.38$ &$ -21.6\pm  0.5$&$ -35.5\pm  2.0$&$ -17.0\pm  0.8$&$  -4.2\pm  1.7$&  0.99 &  0.01 &  0.00 \\
HIP 108767 &   8.33 & $14.18\pm0.87$ &$ -51.8\pm  0.5$&$ -17.7\pm  1.1$&$ -44.8\pm  0.5$&$  21.3\pm  0.4$&  0.92 &  0.08 &  0.00 \\
HIP 108870 &   4.69 & $276.06\pm0.28 &$ -40.7\pm  0.5$&$ -80.9\pm  0.3$&$ -40.6\pm  0.2$&$   2.9\pm  0.4$&  0.87 &  0.13 &  0.00 \\
HIP 108996 &   8.89 & $17.26\pm1.39$ &$   3.0\pm  3.7$&$  10.3\pm  2.1$&$   4.5\pm  1.1$&$   4.9\pm  3.0$&  0.99 &  0.01 &  0.00 \\
HIP 109067 &   9.55 & $19.74\pm1.75$ &$-198.4\pm  1.0$&$ -34.9\pm  1.3$&$-218.7\pm  4.6$&$  29.3\pm  6.0$&  0.00 &  0.00 &  1.00 \\
HIP 109090 &   7.82 & $18.00\pm0.76$ &$  -1.9\pm  0.5$&$  22.5\pm  1.2$&$ -21.4\pm  1.1$&$ -41.5\pm  2.2$&  0.94 &  0.06 &  0.00 \\
HIP 109176 &   3.77 & $85.28\pm0.63$ &$ -14.8\pm 18.2$&$ -15.9\pm  2.2$&$ -15.4\pm 16.4$&$  -2.5\pm  7.5$&  0.99 &  0.01 &  0.00 \\
HIP 109310 &   8.44 & $19.69\pm0.97$ &$ -18.2\pm  0.5$&$ -31.7\pm  1.9$&$ -20.0\pm  0.5$&$  -1.3\pm  0.4$&  0.99 &  0.01 &  0.00 \\
HIP 109324 &   7.76 & $11.82\pm0.42$ &$  -3.6\pm  0.5$&$ -17.6\pm  0.9$&$  -4.5\pm  0.5$&$ -26.6\pm  1.2$&  0.98 &  0.02 &  0.00 \\
HIP 109372 &   7.94 & $12.95\pm0.72$ &$ -14.8\pm  0.5$&$  -6.5\pm  0.6$&$ -16.5\pm  0.5$&$  -5.8\pm  0.6$&  0.99 &  0.01 &  0.00 \\
HIP 109384 &   9.61 & $17.84\pm0.85$ &$ -64.8\pm  1.0$&$ -15.1\pm  1.9$&$ -60.8\pm  0.9$&$ -67.1\pm  2.6$&  0.05 &  0.93 &  0.02 \\
HIP 109450 &   7.59 & $19.56\pm0.61$ &$ -73.5\pm  0.5$&$ -74.4\pm  2.3$&$ -79.5\pm  0.8$&$ -14.8\pm  2.0$&  0.07 &  0.91 &  0.02 \\
HIP 109498 &   8.08 &  $2.76\pm0.78$ &$ -42.0\pm  0.5$&$ -30.7\pm  2.5$&$ -62.2\pm 13.4$&$  11.2\pm  5.9$&  0.69 &  0.31 &  0.00 \\
HIP 109608 &   8.31 &  $7.49\pm1.32$ &$ -21.5\pm  3.0$&$ -24.9\pm  3.1$&$  -7.7\pm  2.6$&$  14.7\pm  1.9$&  0.99 &  0.01 &  0.00 \\
HIP 109677 &   7.40 & $14.75\pm0.55$ &$  -5.7\pm  0.5$&$ -15.0\pm  0.8$&$  -0.2\pm  0.5$&$  16.5\pm  0.8$&  0.99 &  0.01 &  0.00 \\
HIP 109771 &   8.08 & $13.75\pm0.90$ &$ -14.7\pm 29.5$&$  16.3\pm  8.7$&$ -25.9\pm 21.1$&$   1.5\pm 18.9$&  0.98 &  0.02 &  0.00 \\
HIP 109881 &   7.59 & $13.14\pm0.66$ &$ -46.5\pm  0.5$&$ -72.9\pm  4.5$&$ -56.9\pm  0.9$&$ -20.7\pm  2.0$&  0.56 &  0.44 &  0.01 \\
HIP 109931 &   8.94 & $13.98\pm0.82$ &$   4.2\pm  0.8$&$  68.7\pm  5.7$&$   4.6\pm  0.7$&$  15.4\pm  1.4$&  0.98 &  0.02 &  0.00 \\
HIP 109951 &   8.78 & $16.09\pm1.07$ &$ -21.0\pm  1.0$&$  21.1\pm  3.0$&$-105.4\pm  9.5$&$ -37.5\pm  5.4$&  0.00 &  0.95 &  0.04 \\
HIP 110016 &   8.84 &  $8.45\pm0.71$ &$ -55.9\pm  0.8$&$  -2.1\pm  2.3$&$ -65.9\pm  1.7$&$   8.8\pm  2.2$&  0.64 &  0.35 &  0.00 \\
HIP 110035 &   7.04 & $32.22\pm0.52$ &$ -25.7\pm  0.8$&$-114.6\pm  3.2$&$ -35.2\pm  0.8$&$ -45.9\pm  1.8$&  0.27 &  0.70 &  0.03 \\
HIP 110109 &   5.36 & $72.54\pm0.36$ &$ -13.0\pm  0.5$&$ -29.6\pm  0.4$&$ -41.5\pm  0.4$&$   6.4\pm  0.4$&  0.95 &  0.05 &  0.00 \\
HIP 110187 &   8.90 & $11.71\pm1.19$ &$ -83.8\pm  1.0$&$ -83.1\pm  5.9$&$-109.1\pm  7.8$&$  -8.5\pm  8.5$&  0.00 &  0.93 &  0.07 \\
HIP 110291 &   8.52 & $17.08\pm0.86$ &$-106.6\pm  1.2$&$  66.2\pm  3.9$&$ -95.2\pm  1.4$&$  30.3\pm  1.1$&  0.00 &  0.96 &  0.04 \\
HIP 110785 &   5.75 & $26.21\pm0.93$ &$ -14.1\pm  0.5$&$ -52.8\pm  3.3$&$ -14.2\pm  0.5$&$ -13.5\pm  1.6$&  0.98 &  0.02 &  0.00 \\
HIP 110788 &   8.10 & $18.04\pm0.69$ &$  37.4\pm  0.5$&$ -66.9\pm  3.4$&$  29.3\pm  0.6$&$ -19.8\pm  0.6$&  0.95 &  0.05 &  0.00 \\
HIP 111050 &   9.16 & $13.69\pm1.08$ &$ -38.5\pm  0.5$&$ -60.6\pm  5.8$&$ -48.3\pm  1.3$&$ -12.7\pm  2.6$&  0.84 &  0.15 &  0.00 \\
HIP 111352 &   7.97 &  $7.69\pm0.73$ &$ -16.8\pm  0.5$&$  13.8\pm  2.0$&$ -31.0\pm  2.3$&$ -30.9\pm  5.3$&  0.95 &  0.05 &  0.00 \\
HIP 111431 &   8.02 &  $6.85\pm0.59$ &$   9.4\pm  1.2$&$ -62.8\pm  7.0$&$ -10.6\pm  2.5$&$  -4.8\pm  1.0$&  0.98 &  0.02 &  0.00 \\
HIP 111517 &   8.26 & $11.51\pm1.14$ &$ -12.2\pm  0.5$&$ -98.5\pm 10.2$&$-101.1\pm 10.1$&$-113.8\pm 13.3$&  0.00 &  0.30 &  0.70 \\
HIP 111549 &   9.39 &  $9.11\pm1.01$ &$-296.0\pm  1.0$&$ 179.6\pm  6.8$&$-266.0\pm  1.3$&$  34.3\pm 13.1$&  0.00 &  0.00 &  1.00 \\
HIP 111723 &   7.88 & $21.70\pm0.67$ &$ -13.6\pm  0.6$&$  10.6\pm  0.7$&$ -33.1\pm  1.2$&$ -18.9\pm  1.4$&  0.97 &  0.03 &  0.00 \\
HIP 111748 &   7.00 & $19.68\pm0.59$ &$ -37.7\pm  2.0$&$  48.5\pm  1.6$&$ -33.7\pm  1.9$&$ -16.6\pm  1.0$&  0.95 &  0.05 &  0.00 \\
HIP 111796 &   8.10 & $10.51\pm0.91$ &$  23.6\pm  0.5$&$  17.7\pm  2.3$&$  22.2\pm  0.5$&$ -11.0\pm  0.7$&  0.99 &  0.01 &  0.00 \\
HIP 111977 &   7.43 & $34.10\pm0.47$ &$ -47.5\pm  0.5$&$ -31.5\pm  0.9$&$ -66.2\pm  0.6$&$  26.8\pm  0.6$&  0.44 &  0.55 &  0.01 \\
HIP 112263 &   7.50 & $13.75\pm0.61$ &$  -7.4\pm  0.5$&$ -53.8\pm  3.4$&$ -20.4\pm  0.9$&$   2.8\pm  0.2$&  0.98 &  0.02 &  0.00 \\
HIP 112595 &   8.05 & $22.13\pm0.81$ &$ -70.9\pm  0.5$&$  55.6\pm  2.0$&$ -62.7\pm  0.5$&$   9.3\pm  0.5$&  0.59 &  0.41 &  0.00 \\
HIP 112666 &  10.10 & $11.33\pm1.11$ &$ -97.4\pm  1.0$&$ -41.1\pm  8.2$&$-108.2\pm  2.6$&$ -77.9\pm  5.0$&  0.00 &  0.82 &  0.18 \\
HIP 112697 &   6.75 & $15.93\pm0.41$ &$ -44.3\pm  0.5$&$  37.3\pm  1.1$&$ -41.0\pm  0.5$&$ -32.1\pm  1.6$&  0.88 &  0.12 &  0.00 \\
HIP 112811 &   9.34 & $16.56\pm1.22$ &$  -4.0\pm  1.0$&$  28.8\pm  2.7$&$ -90.1\pm  7.6$&$ -62.4\pm  5.7$&  0.00 &  0.95 &  0.05 \\
HIP 112935 &   5.16 & $36.66\pm0.29$ &$  11.4\pm  0.5$&$ -58.1\pm  1.2$&$  -7.0\pm  0.5$&$ -33.9\pm  0.6$&  0.96 &  0.04 &  0.00 \\
HIP 113044 &   6.03 & $30.66\pm0.39$ &$  -1.1\pm  0.5$&$ -27.5\pm  0.7$&$ -21.7\pm  0.6$&$ -10.4\pm  0.5$&  0.98 &  0.02 &  0.00 \\
HIP 113076 &   7.61 & $23.45\pm0.61$ &$ -35.6\pm  0.5$&$  40.9\pm  1.4$&$ -41.7\pm  0.6$&$ -18.5\pm  1.2$&  0.92 &  0.08 &  0.00 \\
HIP 113357 &   5.47 & $64.07\pm0.38$ &$ -33.7\pm  0.5$&$ -15.2\pm  0.2$&$ -30.0\pm  0.4$&$  15.9\pm  0.3$&  0.98 &  0.02 &  0.00 \\
HIP 113514 &   8.38 & $20.17\pm1.09$ &$-119.8\pm  1.0$&$ -56.2\pm  2.7$&$-132.9\pm  2.7$&$  26.6\pm  3.2$&  0.00 &  0.82 &  0.18 \\
HIP 113896 &   6.68 & $34.03\pm0.77$ &$ -12.9\pm  0.5$&$ -45.2\pm  1.2$&$ -16.9\pm  0.4$&$  -5.9\pm  0.6$&  0.98 &  0.02 &  0.00 \\
HIP 113980 &   7.07 & $22.39\pm0.45$ &$  -5.3\pm  0.5$&$ -12.0\pm  0.5$&$ -38.4\pm  1.5$&$ -27.2\pm  1.4$&  0.94 &  0.06 &  0.00 \\
HIP 114034 &   7.27 & $13.44\pm0.67$ &$   6.3\pm  0.5$&$  -5.9\pm  0.5$&$   7.8\pm  0.5$&$   0.2\pm  0.4$&  0.99 &  0.01 &  0.00 \\
HIP 114210 &   5.68 & $29.12\pm0.33$ &$  -2.5\pm  0.5$&$ -29.6\pm  0.7$&$  -9.3\pm  0.5$&$  10.2\pm  0.2$&  0.99 &  0.01 &  0.00 \\
HIP 114354 &   8.16 & $12.27\pm0.98$ &$ -43.4\pm  0.5$&$ -40.6\pm  3.9$&$ -58.0\pm  3.9$&$   4.4\pm  3.6$&  0.78 &  0.22 &  0.00 \\
HIP 114622 &   5.57 & $152.76\pm0.29 &$ -19.1\pm  0.5$&$ -52.4\pm  0.3$&$ -40.2\pm  0.5$&$ -14.2\pm  0.1$&  0.93 &  0.07 &  0.00 \\
HIP 114729 &   7.50 & $15.76\pm0.65$ &$  13.1\pm  0.5$&$  -4.0\pm  0.2$&$   3.9\pm  0.7$&$ -31.2\pm  1.6$&  0.98 &  0.02 &  0.00 \\
HIP 114838 &   7.61 & $11.94\pm0.69$ &$   8.2\pm  0.5$&$ -64.2\pm  5.2$&$  -8.9\pm  1.4$&$ -13.0\pm  0.9$&  0.98 &  0.02 &  0.00 \\
HIP 114856 &   7.99 & $10.50\pm0.87$ &$  42.5\pm 14.1$&$  -1.7\pm  2.7$&$  39.1\pm 12.6$&$ -17.8\pm  5.8$&  0.97 &  0.03 &  0.00 \\
HIP 114893 &   8.43 & $12.00\pm1.01$ &$  38.6\pm  3.0$&$  14.5\pm  1.5$&$   3.0\pm  3.4$&$ -58.1\pm  3.7$&  0.85 &  0.15 &  0.00 \\
HIP 114962 &   8.17 & $15.08\pm1.80$ &$  13.3\pm  0.5$&$ 382.6\pm 76.0$&$-330.4\pm 67.2$&$ -57.5\pm  9.2$&  0.00 &  0.00 &  1.00 \\
HIP 115012 &   7.88 & $15.87\pm1.17$ &$ -52.1\pm  1.4$&$ -53.9\pm  4.6$&$ -70.4\pm  4.3$&$   8.6\pm  3.6$&  0.36 &  0.63 &  0.01 \\
HIP 115066 &   8.39 & $19.25\pm0.92$ &$ -21.0\pm  0.5$&$  37.3\pm  2.0$&$ -40.9\pm  1.4$&$ -11.5\pm  1.5$&  0.94 &  0.06 &  0.00 \\
HIP 115220 &   6.65 & $20.52\pm0.43$ &$ -10.1\pm  0.5$&$ -46.0\pm  1.8$&$ -47.6\pm  1.7$&$ -23.7\pm  1.4$&  0.85 &  0.15 &  0.00 \\
HIP 115359 &   8.96 & $15.91\pm1.39$ &$ -38.9\pm  1.0$&$-102.1\pm  8.6$&$ -83.7\pm  4.6$&$ -28.4\pm  4.5$&  0.01 &  0.95 &  0.05 \\
HIP 115370 &   7.77 & $20.05\pm0.68$ &$ -45.3\pm  0.5$&$  18.8\pm  0.7$&$ -65.6\pm  1.5$&$ -11.4\pm  1.9$&  0.63 &  0.37 &  0.00 \\
HIP 115604 &   9.24 & $10.73\pm0.84$ &$ -14.6\pm  2.1$&$ -61.2\pm  5.6$&$ -39.1\pm  2.9$&$ -40.7\pm  3.2$&  0.74 &  0.25 &  0.00 \\
HIP 115704 &  10.32 &  $9.59\pm1.51$ &$-104.4\pm  6.3$&$-179.2\pm 35.5$&$-188.7\pm 16.0$&$ -57.0\pm  9.3$&  0.00 &  0.00 &  1.00 \\
HIP 115714 &   7.99 & $16.03\pm0.73$ &$ -21.6\pm  0.5$&$  17.1\pm  0.6$&$ -12.9\pm  0.6$&$  47.3\pm  2.4$&  0.93 &  0.07 &  0.00 \\
HIP 115721 &   9.01 &  $9.16\pm0.83$ &$ -55.2\pm  1.0$&$ -14.3\pm  3.5$&$ -68.2\pm  1.9$&$ -62.6\pm  6.4$&  0.04 &  0.94 &  0.02 \\
HIP 115761 &   7.59 & $10.52\pm0.83$ &$ -13.1\pm  1.1$&$ -26.4\pm  2.1$&$ -24.3\pm  1.3$&$  -0.7\pm  0.4$&  0.98 &  0.02 &  0.00 \\
HIP 116106 &   6.50 & $38.29\pm0.54$ &$ -12.9\pm  0.5$&$  -9.1\pm  0.2$&$ -33.6\pm  0.7$&$  -5.1\pm  0.6$&  0.98 &  0.02 &  0.00 \\
HIP 116421 &   6.85 & $30.34\pm0.50$ &$-112.3\pm  0.5$&$ -65.0\pm  2.1$&$-113.2\pm  0.6$&$  62.7\pm  0.3$&  0.00 &  0.84 &  0.16 \\
HIP 116478 &   7.64 & $27.32\pm1.59$ &$ -25.2\pm  1.1$&$-115.7\pm  3.7$&$ -44.2\pm  1.1$&$   9.0\pm  0.8$&  0.54 &  0.45 &  0.01 \\
HIP 116616 &   7.11 & $20.38\pm0.62$ &$ -44.2\pm  0.5$&$ -16.0\pm  1.3$&$ -61.4\pm  1.0$&$ -30.5\pm  1.7$&  0.57 &  0.42 &  0.00 \\
HIP 116727 &   3.21 & $70.91\pm0.40$ &$ -42.2\pm  0.5$&$  21.5\pm  0.2$&$ -37.3\pm  0.4$&$  -2.6\pm  0.1$&  0.97 &  0.03 &  0.00 \\
HIP 116771 &   4.12 & $72.92\pm0.15$ &$   5.4\pm  0.5$&$  -7.8\pm  0.1$&$ -26.3\pm  0.5$&$ -26.4\pm  0.5$&  0.97 &  0.03 &  0.00 \\
HIP 117029 &   7.14 & $21.80\pm0.48$ &$ -70.7\pm  0.5$&$ -72.0\pm  3.0$&$-104.0\pm  1.3$&$  82.5\pm  2.3$&  0.00 &  0.76 &  0.24 \\
HIP 117484 &   8.15 &  $9.65\pm0.88$ &$  -2.5\pm  0.5$&$  54.6\pm  5.7$&$  -2.5\pm  0.4$&$ -18.1\pm  2.1$&  0.98 &  0.02 &  0.00 \\
HIP 117582 &   8.28 & $14.11\pm0.91$ &$ -20.8\pm  0.5$&$ -55.7\pm  4.4$&$ -39.7\pm  1.6$&$  14.0\pm  0.5$&  0.92 &  0.08 &  0.00 \\
HIP 117762 &   6.53 & $19.44\pm0.38$ &$  -0.1\pm  3.7$&$  33.6\pm  1.7$&$   6.3\pm  3.2$&$ -12.2\pm  1.6$&  0.99 &  0.01 &  0.00 \\
HIP 117776 &   8.02 & $11.98\pm0.81$ &$  19.3\pm  0.5$&$ -25.9\pm  2.6$&$  19.2\pm  1.1$&$  -9.2\pm  0.9$&  0.99 &  0.01 &  0.00 \\
HIP 118010 &   7.67 & $19.69\pm0.60$ &$   3.6\pm  0.5$&$ -56.0\pm  2.0$&$ -20.8\pm  1.0$&$  55.3\pm  2.0$&  0.73 &  0.27 &  0.00 \\
HIP 118115 &   7.85 & $20.84\pm0.87$ &$ -31.4\pm  0.5$&$ -75.0\pm  4.3$&$ -83.8\pm  4.3$&$  -2.2\pm  1.9$&  0.05 &  0.93 &  0.02 \\
HIP 118159 &   9.02 & $14.13\pm1.25$ &$   4.3\pm  0.5$&$  15.3\pm  1.5$&$   3.9\pm  0.4$&$  -3.5\pm  0.4$&  0.99 &  0.01 &  0.00 \\
HIP 118162 &   6.64 & $40.77\pm0.49$ &$   8.2\pm  3.3$&$  -6.4\pm  1.3$&$  12.2\pm  2.9$&$  26.4\pm  0.8$&  0.98 &  0.02 &  0.00 \\
HIP 118225 &   7.82 & $16.74\pm0.51$ &$ -38.4\pm  0.9$&$ -41.3\pm  2.6$&$ -78.4\pm  2.4$&$ -29.2\pm  2.4$&  0.10 &  0.88 &  0.02 \\


==> t3_complete.tex <==
4630.12 & \fei\  & 2.280 & $-2.52$ & 72.4 \\
4635.85 & \fei\  & 2.850 & $-2.34$ & 54.1 \\
4683.56 & \fei\  & 2.830 & $-2.41$ & 55.9 \\
4690.14 & \fei\  & 3.690 & $-1.61$ & 55.5 \\
4745.80 & \fei\  & 3.650 & $-1.27$ & 78.3 \\
4749.95 & \fei\  & 4.560 & $-1.24$ & 34.4 \\
4779.44 & \fei\  & 3.420 & $-2.16$ & 41.7 \\
4788.76 & \fei\  & 3.240 & $-1.73$ & 67.6 \\
4799.41 & \fei\  & 3.640 & $-2.13$ & 36.0 \\
4808.15 & \fei\  & 3.250 & $-2.69$ & 30.6 \\
4962.57 & \fei\  & 4.180 & $-1.18$ & 53.9 \\
5044.21 & \fei\  & 2.851 & $-2.05$ & 75.6 \\
5054.64 & \fei\  & 3.640 & $-1.98$ & 40.8 \\
5145.09 & \fei\  & 2.200 & $-3.08$ & 55.6 \\
5217.92 & \fei\  & 3.640 & $-1.72$ & 50.4 \\
5225.52 & \fei\  & 0.110 & $-4.78$ & 73.4 \\
5228.38 & \fei\  & 4.220 & $-1.19$ & 63.1 \\
5247.05 & \fei\  & 0.087 & $-4.96$ & 67.1 \\
5250.20 & \fei\  & 0.121 & $-4.93$ & 69.7 \\
5253.46 & \fei\  & 3.280 & $-1.57$ & 81.4 \\
5285.13 & \fei\  & 4.430 & $-1.54$ & 32.6 \\
5288.52 & \fei\  & 3.690 & $-1.51$ & 60.5 \\
5293.96 & \fei\  & 4.140 & $-1.77$ & 32.0 \\
5295.31 & \fei\  & 4.420 & $-1.59$ & 29.1 \\
5322.04 & \fei\  & 2.280 & $-2.89$ & 61.2 \\
5373.71 & \fei\  & 4.470 & $-0.74$ & 65.2 \\
5379.57 & \fei\  & 3.690 & $-1.51$ & 61.8 \\
5386.33 & \fei\  & 4.150 & $-1.67$ & 32.5 \\
5441.34 & \fei\  & 4.310 & $-1.63$ & 35.6 \\
5464.28 & \fei\  & 4.140 & $-1.58$ & 38.6 \\
5472.71 & \fei\  & 4.210 & $-1.52$ & 46.0 \\
5473.90 & \fei\  & 4.150 & $-0.72$ & 85.3 \\
5483.10 & \fei\  & 4.150 & $-1.45$ & 46.9 \\
5487.15 & \fei\  & 4.420 & $-1.43$ & 39.9 \\
5491.83 & \fei\  & 4.186 & $-2.18$ & 12.2 \\
5522.45 & \fei\  & 4.210 & $-1.45$ & 45.1 \\
5525.54 & \fei\  & 4.230 & $-1.12$ & 58.2 \\
5543.94 & \fei\  & 4.220 & $-1.04$ & 64.2 \\
5546.51 & \fei\  & 4.370 & $-1.21$ & 53.0 \\
5560.21 & \fei\  & 4.430 & $-1.09$ & 52.5 \\
5584.76 & \fei\  & 3.570 & $-2.22$ & 39.0 \\
5618.63 & \fei\  & 4.210 & $-1.27$ & 53.2 \\
5633.95 & \fei\  & 4.990 & $-0.23$ & 71.0 \\
5638.26 & \fei\  & 4.220 & $-0.77$ & 78.9 \\
5651.46 & \fei\  & 4.473 & $-1.75$ & 19.3 \\
5661.34 & \fei\  & 4.284 & $-1.75$ & 22.8 \\
5679.02 & \fei\  & 4.652 & $-0.75$ & 59.7 \\
5696.09 & \fei\  & 4.548 & $-1.72$ & 18.4 \\
5701.54 & \fei\  & 2.559 & $-2.16$ & 87.9 \\
5705.46 & \fei\  & 4.301 & $-1.35$ & 40.5 \\
5717.83 & \fei\  & 4.280 & $-1.03$ & 67.5 \\
5731.76 & \fei\  & 4.260 & $-1.20$ & 58.9 \\
5778.45 & \fei\  & 2.588 & $-3.44$ & 21.5 \\
5793.91 & \fei\  & 4.220 & $-1.61$ & 40.3 \\
5806.73 & \fei\  & 4.610 & $-0.95$ & 57.2 \\
5809.21 & \fei\  & 3.883 & $-1.71$ & 52.3 \\
5852.22 & \fei\  & 4.550 & $-1.23$ & 40.6 \\
5855.07 & \fei\  & 4.608 & $-1.47$ & 22.2 \\
5856.09 & \fei\  & 4.290 & $-1.46$ & 33.5 \\
5905.67 & \fei\  & 4.650 & $-0.69$ & 60.6 \\
5909.97 & \fei\  & 3.210 & $-2.60$ & 36.6 \\
5916.25 & \fei\  & 2.450 & $-2.99$ & 57.5 \\
5927.79 & \fei\  & 4.650 & $-0.99$ & 42.6 \\
5929.68 & \fei\  & 4.550 & $-1.31$ & 41.4 \\
5934.65 & \fei\  & 3.930 & $-1.07$ & 79.5 \\
5952.72 & \fei\  & 3.980 & $-1.34$ & 66.9 \\
5956.69 & \fei\  & 0.859 & $-4.55$ & 55.2 \\
6003.01 & \fei\  & 3.880 & $-1.06$ & 88.9 \\
6027.05 & \fei\  & 4.076 & $-1.09$ & 66.8 \\
6056.00 & \fei\  & 4.730 & $-0.40$ & 76.0 \\
6065.48 & \fei\  & 2.609 & $-1.53$ & 122.1 \\
6079.01 & \fei\  & 4.650 & $-1.02$ & 47.7 \\
6082.71 & \fei\  & 2.220 & $-3.57$ & 35.2 \\
6093.64 & \fei\  & 4.607 & $-1.30$ & 34.6 \\
6096.66 & \fei\  & 3.984 & $-1.81$ & 41.0 \\
6127.91 & \fei\  & 4.140 & $-1.40$ & 50.4 \\
6151.61 & \fei\  & 2.176 & $-3.28$ & 50.5 \\
6165.36 & \fei\  & 4.143 & $-1.46$ & 45.9 \\
6170.51 & \fei\  & 4.800 & $-0.38$ & 85.5 \\
6173.33 & \fei\  & 2.223 & $-2.88$ & 71.3 \\
6180.20 & \fei\  & 2.730 & $-2.63$ & 59.6 \\
6187.99 & \fei\  & 3.940 & $-1.62$ & 50.1 \\
6200.31 & \fei\  & 2.609 & $-2.41$ & 76.6 \\
6213.43 & \fei\  & 2.223 & $-2.52$ & 84.1 \\
6229.23 & \fei\  & 2.850 & $-2.83$ & 39.5 \\
6232.64 & \fei\  & 3.650 & $-1.22$ & 87.2 \\
6240.64 & \fei\  & 2.223 & $-3.28$ & 49.3 \\
6265.13 & \fei\  & 2.176 & $-2.54$ & 89.5 \\
6270.22 & \fei\  & 2.858 & $-2.54$ & 54.4 \\
6297.79 & \fei\  & 2.223 & $-2.71$ & 80.5 \\
6311.50 & \fei\  & 2.831 & $-3.14$ & 32.6 \\
6380.74 & \fei\  & 4.190 & $-1.32$ & 52.9 \\
6419.95 & \fei\  & 4.730 & $-0.24$ & 87.6 \\
6430.84 & \fei\  & 2.176 & $-2.00$ & 119.5 \\
6481.87 & \fei\  & 2.280 & $-2.98$ & 67.8 \\
6498.93 & \fei\  & 0.958 & $-4.69$ & 47.9 \\
6518.36 & \fei\  & 2.831 & $-2.44$ & 62.5 \\
6593.87 & \fei\  & 2.433 & $-2.39$ & 86.4 \\
6597.56 & \fei\  & 4.800 & $-0.97$ & 43.6 \\
6609.11 & \fei\  & 2.559 & $-2.68$ & 67.8 \\
6699.14 & \fei\  & 4.593 & $-2.10$ & 9.2 \\
6703.56 & \fei\  & 2.759 & $-3.02$ & 38.8 \\
6705.10 & \fei\  & 4.607 & $-0.98$ & 48.1 \\
6713.74 & \fei\  & 4.795 & $-1.40$ & 21.1 \\
6726.66 & \fei\  & 4.607 & $-1.03$ & 48.6 \\
6739.52 & \fei\  & 1.557 & $-4.79$ & 13.0 \\
6750.15 & \fei\  & 2.424 & $-2.62$ & 77.8 \\
6752.71 & \fei\  & 4.640 & $-1.22$ & 38.0 \\
6793.25 & \fei\  & 4.076 & $-2.32$ & 15.4 \\
6810.26 & \fei\  & 4.607 & $-0.98$ & 47.8 \\
6828.59 & \fei\  & 4.640 & $-0.82$ & 55.7 \\
6837.00 & \fei\  & 4.593 & $-1.68$ & 16.0 \\
6841.34 & \fei\  & 4.610 & $-0.71$ & 71.5 \\
6842.69 & \fei\  & 4.640 & $-1.22$ & 40.0 \\
6843.66 & \fei\  & 4.550 & $-0.83$ & 60.7 \\
6854.82 & \fei\  & 4.593 & $-1.92$ & 12.9 \\
6855.16 & \fei\  & 4.560 & $-0.74$ & 75.6 \\
6858.15 & \fei\  & 4.610 & $-0.94$ & 52.1 \\
6945.20 & \fei\  & 2.424 & $-2.45$ & 84.1 \\
6978.85 & \fei\  & 2.484 & $-2.47$ & 83.0 \\
6999.88 & \fei\  & 4.100 & $-1.46$ & 58.7 \\
7022.95 & \fei\  & 4.190 & $-1.15$ & 73.4 \\
7038.22 & \fei\  & 4.220 & $-1.20$ & 67.1 \\
7090.38 & \fei\  & 4.230 & $-1.11$ & 68.6 \\
7132.99 & \fei\  & 4.080 & $-1.65$ & 42.5 \\
7401.68 & \fei\  & 4.186 & $-1.50$ & 43.2 \\
7583.79 & \fei\  & 3.020 & $-1.88$ & 86.0 \\
7710.36 & \fei\  & 4.220 & $-1.11$ & 73.4 \\
4576.33 & \feii\ & 2.844 & $-2.95$ & 64.4 \\
4620.51 & \feii\ & 2.828 & $-3.21$ & 52.4 \\
4629.34 & \feii\ & 2.810 & $-2.28$ & 97.2 \\
5197.57 & \feii\ & 3.231 & $-2.22$ & 81.7 \\
5234.62 & \feii\ & 3.221 & $-2.18$ & 83.9 \\
5264.80 & \feii\ & 3.230 & $-3.13$ & 50.8 \\
5414.07 & \feii\ & 3.221 & $-3.58$ & 30.0 \\
5425.25 & \feii\ & 3.200 & $-3.22$ & 44.6 \\
5525.12 & \feii\ & 3.270 & $-3.94$ & 16.9 \\
6369.46 & \feii\ & 2.891 & $-4.11$ & 19.2 \\
6432.67 & \feii\ & 2.891 & $-3.57$ & 44.9 \\
6516.07 & \feii\ & 2.891 & $-3.31$ & 59.7 \\
7222.39 & \feii\ & 3.889 & $-3.26$ & 18.2 \\
7224.47 & \feii\ & 3.889 & $-3.20$ & 19.7 \\
7515.83 & \feii\ & 3.903 & $-3.39$ & 12.1 \\
7711.72 & \feii\ & 3.903 & $-2.50$ & 54.5 \\


==> t4_complete.tex <==
HD 32071 & $5894\pm38$ & $4.23\pm0.12$ & $-0.34\pm0.04$ & 1.35 &  & $-0.34\pm0.04$ & $-0.33\pm0.07$ & noplx \\
HD 59490 & $5627\pm27$ & $4.49\pm0.11$ & $-0.17\pm0.04$ & 0.93 &  & $-0.17\pm0.03$ & $-0.17\pm0.08$ & noplx \\
HD 67163 & $5831\pm29$ & $4.26\pm0.09$ & $0.03\pm0.03$ & 1.26 &  & $0.03\pm0.03$ & $0.03\pm0.04$ & noplx \\
HD 82960 & $6450\pm129$ & $3.95\pm0.20$ & $0.04\pm0.04$ & 1.85 &  & $0.04\pm0.04$ & $0.02\pm0.07$ & manual \\
HD 130047 & $5590\pm33$ & $4.31\pm0.12$ & $-0.02\pm0.04$ & 0.91 &  & $-0.02\pm0.04$ & $-0.02\pm0.09$ & noplx \\
HD 144070 & $6532\pm87$ & $4.16\pm0.08$ & $0.02\pm0.10$ & 1.81 & + & $0.01\pm0.09$ & $0.07\pm0.13$ & main \\
HD 170058 & $5896\pm46$ & $4.21\pm0.14$ & $0.13\pm0.05$ & 1.29 &  & $0.13\pm0.04$ & $0.13\pm0.10$ & noplx \\
HD 171029 & $5562\pm54$ & $3.85\pm0.21$ & $-0.36\pm0.07$ & 0.97 &  & $-0.36\pm0.07$ & $-0.36\pm0.08$ & noplx \\
HD 183490 & $5759\pm43$ & $3.81\pm0.14$ & $0.06\pm0.05$ & 1.25 &  & $0.06\pm0.05$ & $0.07\pm0.05$ & noplx \\
HD 213746 & $5813\pm49$ & $4.12\pm0.18$ & $0.05\pm0.06$ & 1.34 &  & $0.05\pm0.05$ & $0.05\pm0.11$ & noplx \\
HD 223723 & $5946\pm41$ & $4.28\pm0.10$ & $0.01\pm0.03$ & 1.28 &  & $0.01\pm0.04$ & $-0.01\pm0.02$ & noplx \\
HIP 171 & $5510\pm66$ & $4.46\pm0.01$ & $-0.76\pm0.06$ & 0.96 &  & $-0.76\pm0.05$ & $-0.80\pm0.11$ & main \\
HIP 348 & $5746\pm55$ & $4.38\pm0.06$ & $-0.19\pm0.04$ & 1.13 &  & $-0.20\pm0.03$ & $-0.18\pm0.07$ & main \\
HIP 394 & $5635\pm37$ & $3.78\pm0.07$ & $-0.48\pm0.04$ & 1.24 &  & $-0.48\pm0.03$ & $-0.47\pm0.06$ & main \\
HIP 475 & $5836\pm72$ & $4.35\pm0.05$ & $-0.34\pm0.06$ & 1.18 &  & $-0.33\pm0.05$ & $-0.41\pm0.10$ & main \\
HIP 493 & $5960\pm44$ & $4.41\pm0.03$ & $-0.20\pm0.04$ & 1.16 &  & $-0.20\pm0.03$ & $-0.20\pm0.07$ & main \\
HIP 522 & $6251\pm44$ & $4.21\pm0.02$ & $0.05\pm0.05$ & 1.56 & + & $0.04\pm0.05$ & $0.07\pm0.06$ & main \\
HIP 530 & $5866\pm40$ & $3.90\pm0.05$ & $-0.01\pm0.05$ & 1.36 &  & $-0.02\pm0.03$ & $0.03\pm0.09$ & main \\
HIP 544 & $5458\pm40$ & $4.52\pm0.02$ & $0.14\pm0.06$ & 0.78 & + & $0.13\pm0.04$ & $0.17\pm0.13$ & main \\
HIP 656 & $5805\pm39$ & $3.82\pm0.06$ & $-0.24\pm0.06$ & 1.32 &  & $-0.25\pm0.05$ & $-0.15\pm0.07$ & main \\
HIP 768 & $5681\pm31$ & $3.99\pm0.04$ & $-0.01\pm0.06$ & 1.47 &  & $0.01\pm0.03$ & $-0.11\pm0.09$ & main \\
HIP 950 & $6495\pm85$ & $4.30\pm0.03$ & $-0.11\pm0.04$ & 1.63 &  & $-0.12\pm0.04$ & $-0.08\pm0.07$ & main \\
HIP 996 & $5817\pm26$ & $4.32\pm0.04$ & $-0.06\pm0.04$ & 1.21 &  & $-0.06\pm0.02$ & $-0.02\pm0.07$ & main \\
HIP 1105 & $6093\pm52$ & $3.92\pm0.04$ & $-0.24\pm0.04$ & 1.73 &  & $-0.25\pm0.03$ & $-0.19\pm0.05$ & main \\
HIP 1128 & $5658\pm38$ & $4.44\pm0.04$ & $-0.63\pm0.07$ & 1.02 & + & $-0.62\pm0.06$ & $-0.65\pm0.14$ & main \\
HIP 1297 & $5648\pm42$ & $4.35\pm0.06$ & $-0.01\pm0.04$ & 1.02 &  & $-0.01\pm0.04$ & $0.01\pm0.06$ & main \\
HIP 1411 & $5788\pm81$ & $4.45\pm0.05$ & $-0.03\pm0.06$ & 1.03 &  & $-0.01\pm0.04$ & $-0.16\pm0.07$ & main \\
HIP 1499 & $5759\pm79$ & $4.37\pm0.04$ & $0.18\pm0.03$ & 1.07 &  & $0.18\pm0.03$ & $0.16\pm0.05$ & main \\
HIP 1599 & $5947\pm52$ & $4.39\pm0.03$ & $-0.22\pm0.06$ & 1.20 &  & $-0.21\pm0.05$ & $-0.25\pm0.09$ & main \\
HIP 1813 & $5756\pm31$ & $4.30\pm0.02$ & $-0.03\pm0.05$ & 1.13 &  & $-0.03\pm0.04$ & $-0.03\pm0.10$ & main \\
HIP 2021 & $5819\pm54$ & $3.95\pm0.02$ & $-0.13\pm0.05$ & 1.34 &  & $-0.13\pm0.04$ & $-0.14\pm0.07$ & main \\
HIP 2131 & $5712\pm33$ & $4.29\pm0.07$ & $-0.22\pm0.03$ & 1.06 &  & $-0.22\pm0.03$ & $-0.26\pm0.01$ & main \\
HIP 2453 & $6110\pm42$ & $4.34\pm0.03$ & $-0.39\pm0.04$ & 1.42 &  & $-0.39\pm0.04$ & $-0.41\pm0.09$ & main \\
HIP 2711 & $6405\pm75$ & $4.22\pm0.03$ & $-0.14\pm0.09$ & 1.69 & + & $-0.14\pm0.08$ & $-0.13\pm0.12$ & main \\
HIP 2712 & $6063\pm33$ & $4.27\pm0.03$ & $-0.14\pm0.04$ & 1.40 &  & $-0.14\pm0.04$ & $-0.13\pm0.08$ & main \\
HIP 2760 & $5886\pm31$ & $4.19\pm0.05$ & $-0.08\pm0.04$ & 1.29 &  & $-0.08\pm0.04$ & $-0.06\pm0.05$ & main \\
HIP 2894 & $5775\pm30$ & $4.44\pm0.05$ & $-0.07\pm0.02$ & 1.10 &  & $-0.07\pm0.02$ & $-0.11\pm0.02$ & main \\
HIP 2909 & $5740\pm34$ & $4.18\pm0.04$ & $-0.22\pm0.05$ & 1.15 &  & $-0.22\pm0.03$ & $-0.22\pm0.12$ & main \\
HIP 2981 & $6185\pm29$ & $4.32\pm0.03$ & $-0.58\pm0.06$ & 1.47 &  & $-0.58\pm0.05$ & $-0.58\pm0.12$ & main \\
HIP 3014 & $6217\pm55$ & $4.11\pm0.06$ & $-0.31\pm0.08$ & 1.26 &  & $-0.33\pm0.04$ & $-0.16\pm0.14$ & main \\
HIP 3026 & $6319\pm62$ & $4.29\pm0.10$ & $-0.94\pm0.08$ & 1.53 &  & $-0.93\pm0.08$ & $-0.96\pm0.09$ & main \\
HIP 3086 & $5804\pm36$ & $4.07\pm0.03$ & $-0.15\pm0.04$ & 1.26 &  & $-0.15\pm0.03$ & $-0.16\pm0.12$ & main \\
HIP 3093 & $5303\pm63$ & $4.56\pm0.03$ & $0.18\pm0.07$ & 0.56 &  & $0.17\pm0.06$ & $0.16\pm0.13$ & main \\
HIP 3132 & $5929\pm65$ & $4.09\pm0.03$ & $-0.33\pm0.05$ & 1.35 &  & $-0.33\pm0.04$ & $-0.32\pm0.09$ & main \\
HIP 3185 & $5385\pm44$ & $3.84\pm0.11$ & $-0.61\pm0.04$ & 1.13 &  & $-0.61\pm0.03$ & $-0.60\pm0.10$ & giant \\
HIP 3206 & $5005\pm28$ & $4.57\pm0.02$ & $0.23\pm0.10$ & 0.19 &  & $0.21\pm0.05$ & $0.43\pm0.17$ & main \\
HIP 3272 & $6148\pm87$ & $4.23\pm0.05$ & $-0.42\pm0.07$ & 1.52 &  & $-0.41\pm0.06$ & $-0.45\pm0.10$ & main \\
HIP 3441 & $5797\pm41$ & $4.12\pm0.11$ & $-0.48\pm0.06$ & 1.05 &  & $-0.47\pm0.06$ & $-0.49\pm0.05$ & main \\
HIP 3765 & $5015\pm58$ & $4.60\pm0.02$ & $-0.31\pm0.05$ & 0.47 &  & $-0.31\pm0.04$ & $-0.32\pm0.09$ & main \\
HIP 3821 & $5952\pm65$ & $4.35\pm0.03$ & $-0.27\pm0.05$ & 1.27 &  & $-0.26\pm0.03$ & $-0.34\pm0.08$ & main \\
HIP 4039 & $6123\pm42$ & $4.03\pm0.13$ & $-1.10\pm0.07$ & 1.61 & + & $-1.09\pm0.07$ & $-1.16\pm0.05$ & main \\
HIP 4127 & $5918\pm44$ & $4.06\pm0.03$ & $-0.11\pm0.05$ & 1.31 &  & $-0.11\pm0.03$ & $-0.13\pm0.13$ & main \\
HIP 4148 & $4955\pm51$ & $4.62\pm0.02$ & $-0.11\pm0.05$ & 0.36 & + & $-0.12\pm0.04$ & $-0.11\pm0.13$ & main \\
HIP 4151 & $6149\pm64$ & $4.08\pm0.03$ & $0.06\pm0.04$ & 1.54 &  & $0.06\pm0.03$ & $0.03\pm0.09$ & main \\
HIP 4195 & $5750\pm47$ & $4.43\pm0.05$ & $-0.26\pm0.04$ & 1.07 &  & $-0.25\pm0.04$ & $-0.29\pm0.04$ & main \\
HIP 4457 & $5997\pm44$ & $4.03\pm0.05$ & $-0.23\pm0.08$ & 1.53 &  & $-0.24\pm0.07$ & $-0.10\pm0.11$ & main \\
HIP 4544 & $6080\pm45$ & $4.37\pm0.09$ & $-0.74\pm0.09$ & 1.32 &  & $-0.72\pm0.07$ & $-0.88\pm0.10$ & main \\
HIP 4909 & $5726\pm38$ & $4.37\pm0.06$ & $-0.06\pm0.03$ & 1.26 &  & $-0.07\pm0.03$ & $-0.03\pm0.04$ & main \\
HIP 5016 & $6143\pm27$ & $3.88\pm0.02$ & $-0.21\pm0.05$ & 1.65 &  & $-0.20\pm0.04$ & $-0.26\pm0.12$ & main \\
HIP 5106 & $5941\pm33$ & $4.42\pm0.04$ & $-0.24\pm0.05$ & 1.24 &  & $-0.24\pm0.03$ & $-0.24\pm0.13$ & main \\
HIP 5122 & $5278\pm51$ & $3.77\pm0.12$ & $-0.51\pm0.05$ & 1.03 &  & $-0.52\pm0.03$ & $-0.44\pm0.09$ & giant \\
HIP 5134 & $5712\pm79$ & $4.35\pm0.09$ & $-0.25\pm0.03$ & 1.03 &  & $-0.25\pm0.03$ & $-0.25\pm0.06$ & noplx \\
HIP 5163 & $5786\pm42$ & $4.31\pm0.11$ & $-0.56\pm0.07$ & 1.31 &  & $-0.55\pm0.05$ & $-0.70\pm0.10$ & main \\
HIP 5315 & $4962\pm52$ & $3.31\pm0.12$ & $-0.52\pm0.04$ & 1.04 &  & $-0.53\pm0.03$ & $-0.48\pm0.10$ & giant \\
HIP 5336 & $5412\pm79$ & $4.56\pm0.02$ & $-0.80\pm0.05$ & 0.92 &  & $-0.80\pm0.04$ & $-0.79\pm0.10$ & main \\
HIP 5441 & $6470\pm91$ & $4.26\pm0.06$ & $-0.59\pm0.07$ & 1.62 &  & $-0.59\pm0.06$ & $-0.53\pm0.09$ & main \\
HIP 5531 & $5956\pm35$ & $3.81\pm0.02$ & $-0.38\pm0.05$ & 1.53 &  & $-0.38\pm0.04$ & $-0.42\pm0.07$ & main \\
HIP 5682 & $6136\pm51$ & $4.14\pm0.03$ & $-0.12\pm0.05$ & 1.53 &  & $-0.13\pm0.04$ & $-0.07\pm0.10$ & main \\
HIP 5775 & $5799\pm37$ & $4.12\pm0.23$ & $-0.42\pm0.04$ & 1.20 &  & $-0.41\pm0.03$ & $-0.51\pm0.03$ & main \\
HIP 5862 & $6057\pm45$ & $4.29\pm0.02$ & $0.11\pm0.04$ & 1.36 &  & $0.10\pm0.03$ & $0.12\pm0.08$ & main \\
HIP 6159 & $5800\pm29$ & $4.35\pm0.07$ & $-0.58\pm0.08$ & 1.12 &  & $-0.58\pm0.03$ & $-0.54\pm0.21$ & main \\
HIP 6407 & $5860\pm41$ & $4.42\pm0.04$ & $-0.06\pm0.04$ & 1.20 &  & $-0.05\pm0.02$ & $-0.17\pm0.03$ & main \\
HIP 6607 & $5579\pm34$ & $4.47\pm0.04$ & $-0.32\pm0.06$ & 0.79 &  & $-0.30\pm0.03$ & $-0.45\pm0.09$ & main \\
HIP 6711 & $6242\pm41$ & $3.91\pm0.03$ & $-0.19\pm0.05$ & 1.73 &  & $-0.20\pm0.03$ & $-0.17\pm0.10$ & main \\
HIP 6762 & $5456\pm27$ & $4.56\pm0.03$ & $-0.12\pm0.04$ & 0.90 &  & $-0.13\pm0.02$ & $-0.07\pm0.09$ & main \\
HIP 6975 & $5938\pm28$ & $4.24\pm0.03$ & $-0.31\pm0.04$ & 1.24 &  & $-0.31\pm0.03$ & $-0.32\pm0.11$ & main \\
HIP 6978 & $5654\pm43$ & $4.47\pm0.03$ & $0.36\pm0.05$ & 0.82 &  & $0.35\pm0.03$ & $0.43\pm0.09$ & main \\
HIP 7221 & $5636\pm50$ & $4.44\pm0.04$ & $0.27\pm0.04$ & 0.86 &  & $0.27\pm0.04$ & $0.30\pm0.05$ & main \\
HIP 7245 & $5800\pm55$ & $4.43\pm0.05$ & $0.09\pm0.02$ & 1.14 &  & $0.09\pm0.02$ & $0.06\pm0.03$ & main \\
HIP 7312 & $5930\pm60$ & $4.06\pm0.11$ & $0.17\pm0.05$ & 1.32 &  & $0.17\pm0.05$ & $0.19\pm0.04$ & main \\
HIP 7357 & $6073\pm45$ & $4.23\pm0.03$ & $-0.27\pm0.04$ & 1.37 &  & $-0.27\pm0.04$ & $-0.27\pm0.07$ & main \\
HIP 7513 & $6155\pm67$ & $4.09\pm0.02$ & $0.02\pm0.06$ & 1.82 &  & $0.03\pm0.05$ & $-0.03\pm0.09$ & main \\
HIP 7612 & $5850\pm43$ & $4.10\pm0.05$ & $-0.02\pm0.03$ & 1.33 &  & $-0.02\pm0.03$ & $-0.01\pm0.04$ & main \\
HIP 7751B & $5117\pm84$ & $4.64\pm0.02$ & $-0.19\pm0.05$ & 0.61 &  & $-0.19\pm0.04$ & $-0.26\pm0.12$ & main \\
HIP 7751A & $5077\pm49$ & $4.62\pm0.02$ & $-0.24\pm0.03$ & 0.53 &  & $-0.24\pm0.02$ & $-0.30\pm0.07$ & main \\
HIP 7885 & $5778\pm28$ & $4.32\pm0.05$ & $0.05\pm0.03$ & 1.12 &  & $0.06\pm0.02$ & $0.04\pm0.03$ & main \\
HIP 7902 & $5635\pm33$ & $4.37\pm0.03$ & $-0.02\pm0.02$ & 1.01 &  & $-0.02\pm0.02$ & $0.00\pm0.03$ & main \\
HIP 7918 & $5880\pm63$ & $4.33\pm0.03$ & $0.01\pm0.03$ & 1.19 &  & $0.01\pm0.02$ & $0.00\pm0.07$ & main \\
HIP 7961 & $5679\pm35$ & $4.03\pm0.03$ & $-0.57\pm0.06$ & 1.13 &  & $-0.57\pm0.05$ & $-0.58\pm0.13$ & main \\
HIP 7978 & $6140\pm61$ & $4.41\pm0.02$ & $-0.06\pm0.04$ & 1.28 &  & $-0.06\pm0.03$ & $-0.08\pm0.08$ & main \\
HIP 7981 & $5251\pm62$ & $4.56\pm0.03$ & $0.01\pm0.07$ & 0.39 &  & $0.01\pm0.04$ & $0.07\pm0.17$ & main \\
HIP 8102 & $5390\pm69$ & $4.52\pm0.03$ & $-0.50\pm0.05$ & 0.78 &  & $-0.50\pm0.03$ & $-0.53\pm0.13$ & main \\
HIP 8121 & $5845\pm40$ & $4.29\pm0.04$ & $0.03\pm0.03$ & 1.16 &  & $0.03\pm0.02$ & $0.03\pm0.04$ & main \\
HIP 8362 & $5354\pm67$ & $4.53\pm0.04$ & $0.03\pm0.05$ & 0.69 &  & $0.03\pm0.04$ & $0.07\pm0.11$ & main \\
HIP 8433 & $5953\pm40$ & $4.03\pm0.02$ & $-0.23\pm0.04$ & 1.31 &  & $-0.23\pm0.03$ & $-0.24\pm0.10$ & main \\
HIP 8476 & $5780\pm49$ & $4.22\pm0.05$ & $-0.37\pm0.04$ & 1.11 &  & $-0.37\pm0.03$ & $-0.34\pm0.10$ & main \\
HIP 8507 & $5655\pm30$ & $4.49\pm0.05$ & $-0.10\pm0.03$ & 0.84 &  & $-0.10\pm0.02$ & $-0.04\pm0.05$ & main \\
HIP 8674 & $5588\pm44$ & $4.50\pm0.06$ & $-0.52\pm0.06$ & 0.89 &  & $-0.52\pm0.03$ & $-0.49\pm0.17$ & main \\
HIP 8720 & $5258\pm51$ & $4.62\pm0.04$ & $-0.57\pm0.06$ & 0.69 &  & $-0.57\pm0.05$ & $-0.53\pm0.14$ & main \\
HIP 8841 & $5700\pm45$ & $4.33\pm0.07$ & $-0.16\pm0.04$ & 1.16 &  & $-0.15\pm0.03$ & $-0.23\pm0.02$ & main \\
HIP 8859 & $6306\pm57$ & $4.20\pm0.03$ & $-0.36\pm0.07$ & 1.63 &  & $-0.37\pm0.05$ & $-0.34\pm0.17$ & main \\
HIP 9080 & $5380\pm107$ & $4.45\pm0.22$ & $-0.23\pm0.05$ & 0.80 &  & $-0.23\pm0.04$ & $-0.23\pm0.10$ & manual \\
HIP 9349 & $5781\pm28$ & $4.43\pm0.03$ & $-0.06\pm0.03$ & 1.21 &  & $-0.05\pm0.03$ & $-0.08\pm0.06$ & main \\
HIP 9519 & $5846\pm42$ & $4.41\pm0.04$ & $0.11\pm0.10$ & 1.14 & + & $0.10\pm0.09$ & $0.18\pm0.12$ & main \\
HIP 9643 & $5737\pm56$ & $4.48\pm0.04$ & $0.17\pm0.05$ & 0.92 &  & $0.16\pm0.04$ & $0.21\pm0.08$ & main \\
HIP 9884 & $4553\pm87$ & $2.20\pm0.19$ & $-0.27\pm0.07$ & 1.51 &  & $-0.27\pm0.06$ & $-0.27\pm0.12$ & giant \\
HIP 10138 & $5217\pm37$ & $4.56\pm0.02$ & $-0.23\pm0.05$ & 0.61 &  & $-0.22\pm0.04$ & $-0.29\pm0.07$ & main \\
HIP 10212 & $6103\pm27$ & $3.84\pm0.02$ & $0.11\pm0.07$ & 1.95 &  & $0.11\pm0.06$ & $0.09\pm0.13$ & main \\
HIP 10303 & $5735\pm25$ & $4.41\pm0.18$ & $0.10\pm0.04$ & 1.10 &  & $0.11\pm0.03$ & $0.04\pm0.05$ & main \\
HIP 10322 & $5636\pm36$ & $4.00\pm0.02$ & $-0.35\pm0.06$ & 1.08 &  & $-0.34\pm0.03$ & $-0.42\pm0.11$ & main \\
HIP 10449 & $5792\pm26$ & $4.43\pm0.06$ & $-0.83\pm0.07$ & 1.22 &  & $-0.82\pm0.07$ & $-0.88\pm0.10$ & main \\
HIP 10644 & $5786\pm75$ & $4.29\pm0.03$ & $-0.53\pm0.10$ & 1.18 & + & $-0.53\pm0.09$ & $-0.57\pm0.10$ & main \\
HIP 10652 & $5745\pm34$ & $4.43\pm0.06$ & $-0.60\pm0.06$ & 1.29 &  & $-0.59\pm0.04$ & $-0.64\pm0.14$ & main \\
HIP 10710 & $5711\pm29$ & $4.43\pm0.06$ & $-0.20\pm0.05$ & 1.03 &  & $-0.21\pm0.03$ & $-0.11\pm0.04$ & main \\
HIP 10711 & $5730\pm64$ & $4.08\pm0.08$ & $-0.73\pm0.04$ & 1.21 &  & $-0.72\pm0.04$ & $-0.77\pm0.05$ & main \\
HIP 10798 & $5476\pm66$ & $4.61\pm0.03$ & $-0.45\pm0.05$ & 0.94 &  & $-0.45\pm0.03$ & $-0.44\pm0.14$ & main \\
HIP 11072 & $5830\pm69$ & $3.97\pm0.03$ & $-0.09\pm0.05$ & 1.30 &  & $-0.10\pm0.04$ & $-0.01\pm0.03$ & main \\
HIP 11237 & $6114\pm62$ & $4.20\pm0.08$ & $-0.38\pm0.05$ & 1.36 &  & $-0.37\pm0.04$ & $-0.39\pm0.11$ & main \\
HIP 11309 & $6175\pm32$ & $3.96\pm0.03$ & $-0.37\pm0.07$ & 1.65 &  & $-0.36\pm0.05$ & $-0.43\pm0.12$ & main \\
HIP 11505 & $5707\pm31$ & $4.12\pm0.04$ & $0.02\pm0.06$ & 1.15 &  & $0.01\pm0.05$ & $0.08\pm0.08$ & main \\
HIP 11584 & $6095\pm48$ & $3.99\pm0.06$ & $-0.08\pm0.08$ & 1.68 &  & $-0.09\pm0.06$ & $0.05\pm0.12$ & main \\
HIP 11728 & $5733\pm42$ & $4.51\pm0.03$ & $0.06\pm0.04$ & 0.87 &  & $0.05\pm0.02$ & $0.12\pm0.10$ & main \\
HIP 11915 & $5780\pm36$ & $4.44\pm0.05$ & $-0.09\pm0.03$ & 1.12 &  & $-0.09\pm0.03$ & $-0.10\pm0.05$ & main \\
HIP 11923 & $5753\pm43$ & $4.16\pm0.04$ & $-0.40\pm0.07$ & 1.20 &  & $-0.39\pm0.06$ & $-0.41\pm0.14$ & main \\
HIP 12262 & $6074\pm42$ & $3.90\pm0.04$ & $-0.04\pm0.05$ & 1.64 &  & $-0.03\pm0.04$ & $-0.06\pm0.08$ & main \\
HIP 12294 & $6151\pm55$ & $4.45\pm0.20$ & $-0.87\pm0.17$ & 1.41 & + & $-0.88\pm0.17$ & $-0.77\pm0.22$ & main \\
HIP 12306 & $5805\pm40$ & $4.31\pm0.03$ & $-0.54\pm0.05$ & 1.28 &  & $-0.54\pm0.04$ & $-0.58\pm0.08$ & main \\
HIP 12381 & $6194\pm40$ & $4.18\pm0.05$ & $-0.19\pm0.05$ & 1.47 &  & $-0.19\pm0.05$ & $-0.20\pm0.03$ & main \\
HIP 12444 & $6241\pm47$ & $4.36\pm0.02$ & $-0.03\pm0.05$ & 1.36 &  & $-0.02\pm0.04$ & $-0.04\pm0.08$ & main \\
HIP 12579 & $5929\pm48$ & $4.40\pm0.08$ & $-0.84\pm0.05$ & 1.35 &  & $-0.84\pm0.04$ & $-0.81\pm0.10$ & main \\
HIP 12777 & $6312\pm62$ & $4.33\pm0.04$ & $-0.02\pm0.06$ & 1.72 &  & $-0.01\pm0.05$ & $-0.04\pm0.13$ & main \\
HIP 13336 & $5455\pm26$ & $4.39\pm0.01$ & $-0.40\pm0.05$ & 1.09 &  & $-0.41\pm0.04$ & $-0.34\pm0.09$ & main \\
HIP 13366 & $5890\pm42$ & $4.26\pm0.06$ & $-0.62\pm0.06$ & 1.21 &  & $-0.62\pm0.04$ & $-0.62\pm0.15$ & main \\
HIP 13402 & $5167\pm44$ & $4.58\pm0.02$ & $0.18\pm0.08$ & 0.53 & + & $0.18\pm0.07$ & $0.18\pm0.13$ & main \\
HIP 14023 & $5296\pm29$ & $4.55\pm0.03$ & $0.25\pm0.07$ & 0.51 &  & $0.23\pm0.05$ & $0.36\pm0.12$ & main \\
HIP 14086 & $5065\pm40$ & $3.50\pm0.09$ & $-0.62\pm0.03$ & 1.01 &  & $-0.62\pm0.03$ & $-0.64\pm0.07$ & giant \\
HIP 14241 & $5567\pm25$ & $4.46\pm0.04$ & $-0.42\pm0.05$ & 0.86 &  & $-0.42\pm0.03$ & $-0.41\pm0.18$ & main \\
HIP 14286 & $5691\pm35$ & $4.30\pm0.02$ & $-0.28\pm0.03$ & 1.00 &  & $-0.28\pm0.02$ & $-0.31\pm0.05$ & main \\
HIP 14594 & $6055\pm54$ & $4.43\pm0.03$ & $-1.83\pm0.06$ & 1.39 & + & $-1.80\pm0.06$ & $-1.87\pm0.01$ & main \\
HIP 14614 & $5822\pm25$ & $4.36\pm0.03$ & $-0.09\pm0.05$ & 1.07 &  & $-0.09\pm0.04$ & $-0.16\pm0.07$ & main \\
HIP 14632 & $5968\pm63$ & $4.19\pm0.03$ & $0.08\pm0.04$ & 1.36 &  & $0.08\pm0.03$ & $0.06\pm0.08$ & main \\
HIP 14668 & $4849\pm71$ & $2.88\pm0.14$ & $0.06\pm0.06$ & 1.37 &  & $0.05\pm0.04$ & $0.17\pm0.07$ & giant \\
HIP 14721 & $5694\pm49$ & $4.45\pm0.05$ & $0.17\pm0.05$ & 0.93 &  & $0.16\pm0.04$ & $0.23\pm0.07$ & main \\
HIP 14879 & $6073\pm78$ & $3.91\pm0.03$ & $-0.30\pm0.05$ & 1.52 &  & $-0.30\pm0.04$ & $-0.24\pm0.06$ & main \\
HIP 15126 & $5518\pm54$ & $4.58\pm0.05$ & $-0.78\pm0.06$ & 1.14 &  & $-0.78\pm0.06$ & $-0.79\pm0.06$ & main \\
HIP 15206 & $5803\pm48$ & $3.85\pm0.04$ & $0.00\pm0.04$ & 1.44 &  & $-0.01\pm0.04$ & $0.02\pm0.06$ & main \\
HIP 15249 & $5640\pm34$ & $4.28\pm0.05$ & $-0.05\pm0.04$ & 0.89 &  & $-0.05\pm0.03$ & $-0.08\pm0.08$ & main \\
HIP 15330 & $5712\pm48$ & $4.48\pm0.03$ & $-0.24\pm0.05$ & 1.11 &  & $-0.24\pm0.03$ & $-0.21\pm0.12$ & main \\
HIP 15371 & $5852\pm49$ & $4.43\pm0.02$ & $-0.25\pm0.05$ & 1.13 &  & $-0.25\pm0.04$ & $-0.25\pm0.12$ & main \\
HIP 15383 & $4684\pm71$ & $2.64\pm0.14$ & $-0.15\pm0.05$ & 1.38 &  & $-0.16\pm0.05$ & $-0.11\pm0.06$ & giant \\
HIP 15394 & $5303\pm43$ & $3.64\pm0.07$ & $-0.16\pm0.03$ & 1.24 &  & $-0.16\pm0.03$ & $-0.17\pm0.03$ & giant \\
HIP 15405 & $5200\pm104$ & $3.60\pm0.18$ & $-0.73\pm0.07$ & 1.00 &  & $-0.74\pm0.06$ & $-0.68\pm0.11$ & manual \\
HIP 15457 & $5663\pm47$ & $4.47\pm0.03$ & $0.00\pm0.04$ & 1.16 &  & $0.00\pm0.03$ & $0.04\pm0.09$ & main \\
HIP 15510 & $5446\pm44$ & $4.43\pm0.01$ & $-0.38\pm0.06$ & 0.93 &  & $-0.38\pm0.04$ & $-0.38\pm0.15$ & main \\
HIP 15565 & $6271\pm40$ & $4.03\pm0.04$ & $-0.41\pm0.07$ & 1.66 &  & $-0.42\pm0.03$ & $-0.36\pm0.16$ & main \\
HIP 15940 & $5621\pm40$ & $3.97\pm0.03$ & $-0.46\pm0.07$ & 1.48 &  & $-0.45\pm0.04$ & $-0.51\pm0.16$ & main \\
HIP 16072 & $5925\pm50$ & $4.60\pm0.09$ & $-1.21\pm0.12$ & 1.18 & + & $-1.23\pm0.10$ & $-1.04\pm0.13$ & main \\
HIP 16169 & $5733\pm44$ & $4.35\pm0.04$ & $-0.51\pm0.06$ & 1.11 & + & $-0.50\pm0.04$ & $-0.54\pm0.11$ & main \\
HIP 16467 & $5689\pm39$ & $4.33\pm0.08$ & $0.02\pm0.05$ & 0.97 &  & $0.04\pm0.01$ & $-0.05\pm0.09$ & main \\
HIP 16537 & $5079\pm64$ & $4.59\pm0.03$ & $-0.06\pm0.07$ & 0.59 &  & $-0.08\pm0.05$ & $0.03\pm0.17$ & main \\
HIP 16723 & $6229\pm72$ & $4.14\pm0.05$ & $-0.31\pm0.07$ & 1.60 &  & $-0.33\pm0.04$ & $-0.20\pm0.14$ & main \\
HIP 16738 & $6194\pm38$ & $4.01\pm0.08$ & $0.33\pm0.08$ & 1.65 &  & $0.34\pm0.07$ & $0.22\pm0.10$ & main \\
HIP 16818 & $6096\pm39$ & $4.32\pm0.04$ & $-0.43\pm0.05$ & 1.49 &  & $-0.43\pm0.04$ & $-0.45\pm0.11$ & main \\
HIP 16852 & $5971\pm50$ & $4.06\pm0.02$ & $-0.09\pm0.03$ & 1.32 &  & $-0.09\pm0.03$ & $-0.07\pm0.05$ & main \\
HIP 17022 & $5879\pm57$ & $4.03\pm0.04$ & $-0.21\pm0.05$ & 1.40 &  & $-0.21\pm0.04$ & $-0.14\pm0.07$ & main \\
HIP 17147 & $5910\pm62$ & $4.30\pm0.03$ & $-0.83\pm0.06$ & 1.30 &  & $-0.82\pm0.05$ & $-0.87\pm0.11$ & main \\
HIP 17231 & $5839\pm41$ & $3.97\pm0.06$ & $-0.10\pm0.04$ & 1.34 &  & $-0.10\pm0.03$ & $-0.10\pm0.06$ & main \\
HIP 17378 & $5012\pm77$ & $3.74\pm0.15$ & $0.09\pm0.05$ & 0.89 &  & $0.09\pm0.05$ & $0.12\pm0.10$ & giant \\
HIP 17409 & $5872\pm30$ & $4.22\pm0.03$ & $-0.41\pm0.03$ & 1.51 &  & $-0.40\pm0.02$ & $-0.43\pm0.06$ & main \\
HIP 17420 & $4960\pm48$ & $4.60\pm0.02$ & $-0.09\pm0.06$ & 0.13 &  & $-0.09\pm0.04$ & $-0.05\pm0.14$ & main \\
HIP 17655 & $5950\pm50$ & $4.29\pm0.05$ & $-0.26\pm0.04$ & 1.16 &  & $-0.26\pm0.03$ & $-0.29\pm0.09$ & main \\
HIP 17666 & $5148\pm30$ & $4.68\pm0.02$ & $-0.95\pm0.05$ & 0.37 &  & $-0.97\pm0.04$ & $-0.83\pm0.12$ & main \\
HIP 18235 & $5010\pm51$ & $3.21\pm0.12$ & $-0.73\pm0.04$ & 1.21 &  & $-0.73\pm0.04$ & $-0.76\pm0.06$ & giant \\
HIP 18261 & $5883\pm59$ & $4.41\pm0.04$ & $-0.04\pm0.03$ & 1.23 &  & $-0.04\pm0.02$ & $-0.07\pm0.06$ & main \\
HIP 18347 & $5934\pm40$ & $4.46\pm0.06$ & $-0.61\pm0.05$ & 1.35 &  & $-0.61\pm0.05$ & $-0.62\pm0.06$ & main \\
HIP 18366 & $6146\pm30$ & $4.19\pm0.02$ & $-0.34\pm0.05$ & 1.53 &  & $-0.34\pm0.04$ & $-0.37\pm0.08$ & main \\
HIP 18413 & $5533\pm36$ & $4.29\pm0.02$ & $-0.15\pm0.07$ & 0.77 &  & $-0.17\pm0.04$ & $-0.03\pm0.08$ & main \\
HIP 18606 & $4801\pm65$ & $3.13\pm0.13$ & $0.02\pm0.05$ & 1.10 &  & $0.02\pm0.04$ & $0.05\pm0.08$ & giant \\
HIP 19631 & $5888\pm55$ & $4.05\pm0.05$ & $-0.34\pm0.04$ & 1.38 &  & $-0.33\pm0.03$ & $-0.39\pm0.06$ & main \\
HIP 19696 & $5715\pm42$ & $4.16\pm0.12$ & $-0.10\pm0.07$ & 1.02 &  & $-0.09\pm0.03$ & $-0.18\pm0.19$ & main \\
HIP 19786 & $5807\pm37$ & $4.48\pm0.03$ & $0.15\pm0.05$ & 1.23 &  & $0.14\pm0.03$ & $0.20\pm0.11$ & main \\
HIP 19849 & $5202\pm49$ & $4.55\pm0.03$ & $-0.28\pm0.06$ & 0.47 &  & $-0.28\pm0.03$ & $-0.31\pm0.17$ & main \\
HIP 19911 & $5637\pm33$ & $4.48\pm0.07$ & $-0.14\pm0.05$ & 1.05 &  & $-0.16\pm0.03$ & $-0.06\pm0.05$ & main \\
HIP 20094 & $5563\pm27$ & $4.43\pm0.05$ & $-0.33\pm0.04$ & 0.87 &  & $-0.33\pm0.02$ & $-0.31\pm0.10$ & main \\
HIP 20298 & $5921\pm39$ & $4.20\pm0.15$ & $-0.67\pm0.07$ & 1.41 &  & $-0.65\pm0.04$ & $-0.87\pm0.04$ & main \\
HIP 20366 & $5751\pm44$ & $4.34\pm0.08$ & $-0.11\pm0.05$ & 1.47 &  & $-0.10\pm0.04$ & $-0.16\pm0.07$ & main \\
HIP 20753 & $5847\pm44$ & $3.95\pm0.04$ & $0.12\pm0.03$ & 1.40 &  & $0.12\pm0.03$ & $0.13\pm0.05$ & main \\
HIP 20754 & $6062\pm48$ & $3.97\pm0.06$ & $-0.48\pm0.04$ & 1.24 &  & $-0.48\pm0.04$ & $-0.48\pm0.06$ & main \\
HIP 20984 & $5764\pm46$ & $4.22\pm0.10$ & $-0.30\pm0.07$ & 1.44 &  & $-0.29\pm0.05$ & $-0.36\pm0.14$ & main \\
HIP 21227 & $6125\pm70$ & $4.27\pm0.16$ & $-0.27\pm0.09$ & 1.51 &  & $-0.25\pm0.04$ & $-0.48\pm0.08$ & main \\
HIP 21306 & $5825\pm48$ & $4.47\pm0.10$ & $-0.55\pm0.04$ & 1.17 &  & $-0.55\pm0.04$ & $-0.56\pm0.04$ & main \\
HIP 21703 & $5475\pm60$ & $4.41\pm0.06$ & $0.16\pm0.06$ & 0.84 &  & $0.16\pm0.04$ & $0.18\pm0.14$ & main \\
HIP 21847 & $5968\pm58$ & $4.03\pm0.04$ & $0.02\pm0.06$ & 1.72 &  & $0.02\pm0.04$ & $-0.01\pm0.14$ & main \\
HIP 21921 & $5343\pm43$ & $4.47\pm0.02$ & $-0.33\pm0.05$ & 0.61 &  & $-0.34\pm0.03$ & $-0.24\pm0.14$ & main \\
HIP 22020 & $5816\pm57$ & $4.22\pm0.12$ & $-0.22\pm0.04$ & 1.13 &  & $-0.21\pm0.03$ & $-0.28\pm0.08$ & main \\
HIP 22060 & $6010\pm66$ & $4.44\pm0.11$ & $-0.42\pm0.08$ & 1.28 & + & $-0.42\pm0.07$ & $-0.53\pm0.08$ & main \\
HIP 22263 & $5813\pm44$ & $4.48\pm0.02$ & $0.00\pm0.03$ & 1.18 &  & $0.00\pm0.03$ & $0.00\pm0.04$ & main \\
HIP 22336 & $5878\pm47$ & $4.11\pm0.02$ & $0.20\pm0.05$ & 1.29 &  & $0.19\pm0.03$ & $0.21\pm0.09$ & main \\
HIP 22349 & $5747\pm32$ & $4.26\pm0.02$ & $-0.36\pm0.04$ & 1.24 &  & $-0.36\pm0.04$ & $-0.39\pm0.03$ & main \\
HIP 22449 & $6477\pm56$ & $4.29\pm0.02$ & $0.00\pm0.08$ & 1.70 & + & $0.01\pm0.07$ & $-0.03\pm0.12$ & main \\
HIP 22489 & $4580\pm91$ & $2.30\pm0.12$ & $-0.04\pm0.11$ & 1.60 &  & $-0.04\pm0.10$ & $-0.06\pm0.20$ & manual \\
HIP 22528 & $5675\pm44$ & $4.34\pm0.07$ & $-0.38\pm0.04$ & 0.99 &  & $-0.38\pm0.03$ & $-0.35\pm0.06$ & main \\
HIP 22596 & $5808\pm30$ & $4.28\pm0.03$ & $-0.51\pm0.04$ & 1.25 &  & $-0.51\pm0.03$ & $-0.51\pm0.09$ & main \\
HIP 23080 & $5327\pm39$ & $4.47\pm0.02$ & $-0.33\pm0.05$ & 0.68 &  & $-0.34\pm0.02$ & $-0.21\pm0.10$ & main \\
HIP 23311 & $4745\pm42$ & $4.57\pm0.02$ & $0.19\pm0.08$ & 0.20 & + & $0.18\pm0.06$ & $0.29\pm0.16$ & main \\
HIP 23693 & $6147\pm53$ & $4.44\pm0.03$ & $-0.17\pm0.08$ & 1.38 & + & $-0.17\pm0.08$ & $-0.13\pm0.08$ & main \\
HIP 23835 & $5717\pm61$ & $4.06\pm0.03$ & $-0.22\pm0.04$ & 1.30 &  & $-0.21\pm0.03$ & $-0.25\pm0.07$ & main \\
HIP 23884 & $5727\pm32$ & $4.41\pm0.03$ & $0.11\pm0.05$ & 0.78 &  & $0.11\pm0.02$ & $0.14\pm0.11$ & main \\
HIP 23922 & $5852\pm60$ & $4.33\pm0.09$ & $-0.64\pm0.08$ & 1.42 &  & $-0.63\pm0.03$ & $-0.68\pm0.22$ & main \\
HIP 23941 & $6421\pm66$ & $4.05\pm0.02$ & $-0.33\pm0.06$ & 1.79 & + & $-0.33\pm0.05$ & $-0.34\pm0.09$ & main \\
HIP 24030 & $6059\pm44$ & $4.32\pm0.15$ & $-0.97\pm0.07$ & 1.41 & + & $-0.96\pm0.06$ & $-1.04\pm0.06$ & main \\
HIP 24037 & $5573\pm31$ & $4.41\pm0.04$ & $-0.44\pm0.04$ & 0.91 &  & $-0.44\pm0.03$ & $-0.49\pm0.10$ & main \\
HIP 24660 & $5819\pm33$ & $4.47\pm0.02$ & $0.24\pm0.04$ & 1.00 &  & $0.23\pm0.03$ & $0.26\pm0.09$ & main \\
HIP 24813 & $5872\pm66$ & $4.26\pm0.03$ & $0.05\pm0.04$ & 1.24 &  & $0.05\pm0.03$ & $0.04\pm0.07$ & main \\
HIP 25052 & $5749\pm53$ & $4.25\pm0.04$ & $0.09\pm0.03$ & 1.21 &  & $0.09\pm0.02$ & $0.11\pm0.05$ & main \\
HIP 25361 & $5701\pm35$ & $4.42\pm0.13$ & $-0.57\pm0.07$ & 1.13 &  & $-0.58\pm0.04$ & $-0.54\pm0.18$ & main \\
HIP 25528 & $6198\pm45$ & $3.70\pm0.05$ & $-0.47\pm0.05$ & 1.86 &  & $-0.47\pm0.05$ & $-0.46\pm0.07$ & main \\
HIP 25586 & $5633\pm38$ & $4.36\pm0.05$ & $-0.11\pm0.03$ & 1.03 &  & $-0.11\pm0.03$ & $-0.11\pm0.04$ & main \\
HIP 25670 & $5771\pm42$ & $4.44\pm0.04$ & $0.08\pm0.03$ & 0.95 &  & $0.07\pm0.02$ & $0.09\pm0.05$ & main \\
HIP 25840 & $6090\pm67$ & $4.14\pm0.06$ & $-0.17\pm0.06$ & 1.58 &  & $-0.16\pm0.04$ & $-0.28\pm0.07$ & main \\
HIP 25860 & $5618\pm39$ & $4.43\pm0.06$ & $-0.25\pm0.04$ & 0.71 &  & $-0.25\pm0.04$ & $-0.25\pm0.04$ & main \\
HIP 25973 & $5908\pm38$ & $3.95\pm0.02$ & $-0.02\pm0.04$ & 1.50 &  & $-0.02\pm0.04$ & $0.00\pm0.07$ & main \\
HIP 26100 & $5883\pm32$ & $3.91\pm0.03$ & $-0.42\pm0.05$ & 1.44 &  & $-0.41\pm0.04$ & $-0.43\pm0.10$ & main \\
HIP 26129 & $5904\pm41$ & $4.49\pm0.04$ & $0.00\pm0.04$ & 1.12 &  & $0.00\pm0.03$ & $0.01\pm0.08$ & main \\
HIP 26326 & $6034\pm44$ & $4.27\pm0.04$ & $-0.12\pm0.04$ & 1.24 &  & $-0.13\pm0.03$ & $-0.10\pm0.10$ & main \\
HIP 26437 & $5957\pm39$ & $4.32\pm0.03$ & $0.13\pm0.04$ & 1.19 &  & $0.12\pm0.03$ & $0.15\pm0.08$ & main \\
HIP 26452 & $5985\pm47$ & $4.51\pm0.08$ & $-0.71\pm0.08$ & 0.95 &  & $-0.71\pm0.07$ & $-0.66\pm0.16$ & main \\
HIP 26534 & $5913\pm40$ & $4.10\pm0.04$ & $-0.07\pm0.03$ & 1.37 &  & $-0.07\pm0.03$ & $-0.10\pm0.04$ & main \\
HIP 26617 & $5682\pm46$ & $4.51\pm0.13$ & $-0.64\pm0.06$ & 1.21 &  & $-0.63\pm0.04$ & $-0.75\pm0.05$ & main \\
HIP 26779 & $5257\pm29$ & $4.55\pm0.02$ & $0.08\pm0.07$ & 0.89 &  & $0.07\pm0.05$ & $0.15\pm0.13$ & main \\
HIP 26807 & $5654\pm60$ & $4.41\pm0.05$ & $0.07\pm0.05$ & 0.86 &  & $0.06\pm0.03$ & $0.10\pm0.10$ & main \\
HIP 26828 & $6435\pm36$ & $4.14\pm0.05$ & $-0.38\pm0.07$ & 1.91 &  & $-0.37\pm0.06$ & $-0.47\pm0.13$ & main \\
HIP 27072 & $6305\pm61$ & $4.29\pm0.02$ & $-0.09\pm0.07$ & 1.55 &  & $-0.08\pm0.06$ & $-0.10\pm0.12$ & main \\
HIP 27128 & $5905\pm58$ & $4.13\pm0.05$ & $-0.84\pm0.07$ & 1.37 & + & $-0.83\pm0.07$ & $-0.88\pm0.06$ & main \\
HIP 27207 & $5207\pm25$ & $4.46\pm0.02$ & $-0.04\pm0.07$ & 0.70 &  & $-0.06\pm0.03$ & $0.08\pm0.13$ & main \\
HIP 27878 & $5864\pm43$ & $4.20\pm0.04$ & $-0.07\pm0.03$ & 1.28 &  & $-0.07\pm0.03$ & $-0.04\pm0.02$ & main \\
HIP 27913 & $5949\pm64$ & $4.48\pm0.03$ & $-0.04\pm0.04$ & 1.34 &  & $-0.03\pm0.03$ & $-0.05\pm0.09$ & main \\
HIP 28066 & $5732\pm48$ & $4.24\pm0.03$ & $-0.16\pm0.04$ & 1.10 &  & $-0.16\pm0.03$ & $-0.21\pm0.07$ & main \\
HIP 28103 & $6989\pm100$ & $4.18\pm0.03$ & $-0.10\pm0.10$ & 2.16 & + & $-0.12\pm0.09$ & $-0.01\pm0.05$ & main \\
HIP 28145 & $5743\pm42$ & $4.36\pm0.06$ & $-0.27\pm0.07$ & 0.85 &  & $-0.29\pm0.05$ & $-0.10\pm0.04$ & main \\
HIP 28159 & $5667\pm43$ & $4.06\pm0.04$ & $-0.43\pm0.07$ & 1.55 &  & $-0.43\pm0.05$ & $-0.43\pm0.16$ & main \\
HIP 28336 & $5719\pm41$ & $4.49\pm0.06$ & $-0.20\pm0.03$ & 0.98 &  & $-0.19\pm0.02$ & $-0.24\pm0.03$ & main \\
HIP 28671 & $5577\pm40$ & $4.57\pm0.04$ & $-0.96\pm0.07$ & 0.82 &  & $-0.97\pm0.06$ & $-0.89\pm0.07$ & main \\
HIP 29001 & $6119\pm43$ & $4.43\pm0.04$ & $-0.55\pm0.04$ & 1.36 &  & $-0.55\pm0.04$ & $-0.54\pm0.09$ & main \\
HIP 29074 & $5874\pm43$ & $4.48\pm0.03$ & $0.04\pm0.04$ & 1.00 &  & $0.03\pm0.03$ & $0.07\pm0.05$ & main \\
HIP 29248 & $5671\pm39$ & $4.49\pm0.05$ & $-0.18\pm0.05$ & 0.90 &  & $-0.20\pm0.03$ & $-0.09\pm0.05$ & main \\
HIP 29269 & $5658\pm32$ & $4.03\pm0.06$ & $-0.62\pm0.07$ & 1.22 &  & $-0.60\pm0.06$ & $-0.75\pm0.07$ & main \\
HIP 29271 & $5569\pm40$ & $4.43\pm0.03$ & $0.11\pm0.05$ & 0.90 &  & $0.10\pm0.04$ & $0.14\pm0.09$ & main \\
HIP 29432 & $5764\pm38$ & $4.51\pm0.02$ & $-0.08\pm0.04$ & 0.89 &  & $-0.08\pm0.02$ & $-0.06\pm0.09$ & main \\
HIP 29650 & $6539\pm65$ & $4.29\pm0.02$ & $0.03\pm0.04$ & 1.65 &  & $0.03\pm0.04$ & $0.03\pm0.05$ & main \\
HIP 29716 & $6253\pm88$ & $3.94\pm0.04$ & $-0.19\pm0.05$ & 1.73 &  & $-0.19\pm0.04$ & $-0.17\pm0.10$ & main \\
HIP 30545 & $6040\pm38$ & $3.97\pm0.02$ & $-0.09\pm0.04$ & 1.47 &  & $-0.09\pm0.04$ & $-0.12\pm0.08$ & main \\
HIP 30990 & $5960\pm46$ & $4.14\pm0.07$ & $-0.80\pm0.07$ & 1.41 &  & $-0.80\pm0.07$ & $-0.82\pm0.10$ & main \\
HIP 31083 & $5538\pm51$ & $4.33\pm0.03$ & $-0.15\pm0.10$ & 0.95 & + & $-0.19\pm0.06$ & $0.02\pm0.12$ & main \\
HIP 31188 & $5911\pm55$ & $4.38\pm0.06$ & $-0.62\pm0.05$ & 1.30 &  & $-0.61\pm0.05$ & $-0.65\pm0.08$ & main \\
HIP 31419 & $5682\pm35$ & $4.32\pm0.05$ & $0.06\pm0.05$ & 1.13 &  & $0.05\pm0.04$ & $0.11\pm0.09$ & main \\
HIP 32650 & $5791\pm59$ & $4.15\pm0.05$ & $-0.42\pm0.06$ & 1.33 &  & $-0.41\pm0.04$ & $-0.47\pm0.12$ & main \\
HIP 32673 & $5730\pm35$ & $4.45\pm0.05$ & $0.08\pm0.03$ & 0.86 &  & $0.09\pm0.02$ & $0.08\pm0.08$ & main \\
HIP 32851 & $6620\pm78$ & $4.19\pm0.04$ & $-0.40\pm0.08$ & 1.88 & + & $-0.40\pm0.08$ & $-0.43\pm0.08$ & main \\
HIP 33287 & $5398\pm22$ & $4.45\pm0.01$ & $-0.42\pm0.04$ & 0.96 &  & $-0.42\pm0.02$ & $-0.39\pm0.11$ & main \\
HIP 33382 & $5609\pm32$ & $4.39\pm0.03$ & $0.00\pm0.04$ & 0.92 &  & $0.00\pm0.02$ & $0.05\pm0.11$ & main \\
HIP 33608 & $5971\pm41$ & $4.45\pm0.04$ & $0.07\pm0.05$ & 1.27 &  & $0.08\pm0.04$ & $0.07\pm0.09$ & main \\
HIP 34017 & $5916\pm60$ & $4.38\pm0.03$ & $-0.10\pm0.06$ & 1.11 &  & $-0.11\pm0.02$ & $-0.07\pm0.17$ & main \\
HIP 34164 & $5713\pm54$ & $3.92\pm0.11$ & $-0.58\pm0.06$ & 1.46 &  & $-0.56\pm0.03$ & $-0.64\pm0.14$ & main \\
HIP 34511 & $5785\pm38$ & $4.36\pm0.04$ & $-0.11\pm0.04$ & 1.06 &  & $-0.11\pm0.04$ & $-0.12\pm0.04$ & main \\
HIP 34521 & $5856\pm36$ & $3.84\pm0.05$ & $-0.15\pm0.07$ & 1.47 &  & $-0.16\pm0.03$ & $-0.04\pm0.16$ & main \\
HIP 34608 & $4970\pm57$ & $3.42\pm0.14$ & $-0.43\pm0.05$ & 1.09 &  & $-0.43\pm0.04$ & $-0.44\pm0.10$ & giant \\
HIP 34642 & $5783\pm55$ & $4.06\pm0.08$ & $-0.54\pm0.04$ & 1.41 &  & $-0.53\pm0.04$ & $-0.57\pm0.05$ & main \\
HIP 34653 & $5554\pm42$ & $4.26\pm0.08$ & $-0.18\pm0.03$ & 0.98 &  & $-0.17\pm0.03$ & $-0.21\pm0.05$ & main \\
HIP 34710 & $5778\pm39$ & $3.87\pm0.03$ & $0.02\pm0.04$ & 1.52 &  & $0.02\pm0.04$ & $0.01\pm0.04$ & main \\
HIP 35148 & $5821\pm43$ & $4.12\pm0.04$ & $-0.22\pm0.05$ & 1.10 &  & $-0.23\pm0.03$ & $-0.15\pm0.08$ & main \\
HIP 35185 & $5821\pm52$ & $4.42\pm0.04$ & $-0.04\pm0.06$ & 1.19 &  & $-0.04\pm0.05$ & $-0.03\pm0.09$ & main \\
HIP 35214 & $5741\pm31$ & $4.36\pm0.08$ & $-0.23\pm0.10$ & 0.96 &  & $-0.25\pm0.08$ & $-0.06\pm0.06$ & main \\
HIP 35599 & $5820\pm29$ & $4.18\pm0.09$ & $-0.10\pm0.04$ & 1.34 &  & $-0.10\pm0.03$ & $-0.10\pm0.10$ & main \\
HIP 35989 & $5208\pm99$ & $4.55\pm0.04$ & $-0.35\pm0.07$ & 0.59 & + & $-0.36\pm0.04$ & $-0.15\pm0.15$ & main \\
HIP 36210 & $5615\pm54$ & $4.40\pm0.03$ & $0.03\pm0.03$ & 0.89 &  & $0.03\pm0.03$ & $0.05\pm0.07$ & main \\
HIP 36439 & $6369\pm31$ & $4.30\pm0.01$ & $-0.28\pm0.06$ & 1.74 &  & $-0.28\pm0.05$ & $-0.30\pm0.09$ & main \\
HIP 36481 & $5819\pm35$ & $4.11\pm0.03$ & $-0.15\pm0.04$ & 1.27 &  & $-0.16\pm0.03$ & $-0.14\pm0.11$ & main \\
HIP 36515 & $5830\pm76$ & $4.49\pm0.03$ & $-0.07\pm0.04$ & 1.18 &  & $-0.07\pm0.03$ & $-0.08\pm0.05$ & main \\
HIP 36849 & $6018\pm37$ & $4.27\pm0.09$ & $-0.78\pm0.07$ & 1.29 &  & $-0.78\pm0.06$ & $-0.77\pm0.13$ & main \\
HIP 36874 & $5787\pm37$ & $4.25\pm0.03$ & $-0.08\pm0.04$ & 1.19 &  & $-0.08\pm0.03$ & $-0.08\pm0.08$ & main \\
HIP 37171 & $5605\pm31$ & $4.40\pm0.05$ & $0.17\pm0.05$ & 1.03 &  & $0.17\pm0.04$ & $0.22\pm0.09$ & main \\
HIP 37233 & $5722\pm44$ & $4.01\pm0.03$ & $-0.46\pm0.04$ & 1.15 &  & $-0.46\pm0.04$ & $-0.50\pm0.03$ & main \\
HIP 37279 & $6648\pm71$ & $4.01\pm0.03$ & $-0.02\pm0.06$ & 2.00 &  & $-0.02\pm0.05$ & $-0.01\pm0.11$ & main \\
HIP 37316 & $6109\pm64$ & $4.20\pm0.09$ & $-0.09\pm0.05$ & 1.53 &  & $-0.09\pm0.05$ & $-0.05\pm0.07$ & main \\
HIP 37349 & $4937\pm37$ & $4.60\pm0.02$ & $0.00\pm0.05$ & 0.32 &  & $-0.01\pm0.04$ & $0.01\pm0.09$ & main \\
HIP 37419 & $5762\pm60$ & $4.49\pm0.05$ & $-0.33\pm0.04$ & 1.12 &  & $-0.33\pm0.03$ & $-0.28\pm0.08$ & main \\
HIP 37789 & $5929\pm24$ & $4.13\pm0.02$ & $-0.66\pm0.05$ & 1.45 &  & $-0.66\pm0.05$ & $-0.66\pm0.06$ & main \\
HIP 37826 & $4832\pm76$ & $2.89\pm0.17$ & $0.05\pm0.07$ & 1.37 &  & $0.04\pm0.05$ & $0.14\pm0.11$ & giant \\
HIP 37853 & $5760\pm69$ & $4.20\pm0.01$ & $-0.86\pm0.06$ & 1.13 &  & $-0.87\pm0.05$ & $-0.82\pm0.09$ & main \\
HIP 37971 & $5720\pm32$ & $4.43\pm0.05$ & $0.20\pm0.08$ & 1.03 & + & $0.21\pm0.07$ & $0.16\pm0.14$ & main \\
HIP 38072 & $5768\pm30$ & $4.44\pm0.06$ & $0.01\pm0.03$ & 1.19 &  & $0.01\pm0.03$ & $0.03\pm0.05$ & main \\
HIP 38172 & $6164\pm41$ & $4.22\pm0.03$ & $-0.37\pm0.05$ & 1.41 &  & $-0.37\pm0.04$ & $-0.39\pm0.10$ & main \\
HIP 38228 & $5657\pm28$ & $4.52\pm0.02$ & $-0.01\pm0.05$ & 1.25 &  & $-0.02\pm0.03$ & $0.03\pm0.08$ & main \\
HIP 38325 & $6383\pm37$ & $4.27\pm0.02$ & $0.04\pm0.05$ & 1.74 &  & $0.04\pm0.04$ & $0.04\pm0.12$ & main \\
HIP 38613 & $5909\pm52$ & $4.28\pm0.08$ & $-0.54\pm0.07$ & 1.22 &  & $-0.53\pm0.06$ & $-0.63\pm0.06$ & main \\
HIP 38625 & $5224\pm52$ & $4.59\pm0.01$ & $-0.86\pm0.07$ & 0.61 & + & $-0.87\pm0.05$ & $-0.72\pm0.12$ & main \\
HIP 38769 & $5944\pm60$ & $4.12\pm0.07$ & $-0.71\pm0.09$ & 1.49 &  & $-0.71\pm0.07$ & $-0.79\pm0.17$ & main \\
HIP 39072 & $5744\pm31$ & $4.32\pm0.06$ & $-0.22\pm0.10$ & 0.94 &  & $-0.24\pm0.07$ & $-0.06\pm0.12$ & main \\
HIP 39157 & $5329\pm42$ & $4.56\pm0.01$ & $-0.67\pm0.04$ & 0.58 &  & $-0.67\pm0.04$ & $-0.66\pm0.08$ & main \\
HIP 39417 & $5667\pm58$ & $4.29\pm0.06$ & $0.26\pm0.04$ & 1.15 &  & $0.26\pm0.04$ & $0.30\pm0.07$ & main \\
HIP 39506 & $5715\pm47$ & $4.36\pm0.02$ & $-0.59\pm0.04$ & 1.04 &  & $-0.59\pm0.04$ & $-0.60\pm0.05$ & main \\
HIP 39616 & $6103\pm43$ & $4.38\pm0.04$ & $-0.37\pm0.04$ & 1.44 &  & $-0.37\pm0.03$ & $-0.40\pm0.11$ & main \\
HIP 39780 & $5809\pm59$ & $3.97\pm0.02$ & $0.11\pm0.04$ & 1.34 &  & $0.11\pm0.04$ & $0.13\pm0.07$ & main \\
HIP 39822 & $5740\pm37$ & $4.38\pm0.04$ & $-0.29\pm0.03$ & 1.06 &  & $-0.30\pm0.02$ & $-0.25\pm0.03$ & main \\
HIP 39893 & $5332\pm46$ & $3.79\pm0.07$ & $-0.84\pm0.10$ & 1.25 &  & $-0.82\pm0.08$ & $-1.01\pm0.12$ & main \\
HIP 40001 & $6075\pm27$ & $3.96\pm0.02$ & $-0.30\pm0.07$ & 1.76 &  & $-0.29\pm0.04$ & $-0.40\pm0.10$ & main \\
HIP 40023 & $5236\pm54$ & $3.53\pm0.12$ & $-0.09\pm0.04$ & 1.15 &  & $-0.09\pm0.03$ & $-0.16\pm0.11$ & giant \\
HIP 40118 & $5521\pm48$ & $4.40\pm0.02$ & $-0.46\pm0.04$ & 0.86 &  & $-0.46\pm0.03$ & $-0.40\pm0.03$ & main \\
HIP 40613 & $5868\pm42$ & $4.20\pm0.04$ & $-0.56\pm0.05$ & 1.41 &  & $-0.55\pm0.04$ & $-0.62\pm0.04$ & main \\
HIP 40674 & $5664\pm29$ & $4.43\pm0.07$ & $-0.29\pm0.05$ & 1.12 &  & $-0.28\pm0.02$ & $-0.34\pm0.10$ & main \\
HIP 40693 & $5442\pm30$ & $4.53\pm0.02$ & $-0.02\pm0.04$ & 0.72 &  & $-0.03\pm0.03$ & $0.01\pm0.11$ & main \\
HIP 40765 & $5978\pm82$ & $4.45\pm0.04$ & $-0.13\pm0.02$ & 1.11 &  & $-0.13\pm0.02$ & $-0.13\pm0.05$ & main \\
HIP 40843 & $6347\pm63$ & $4.30\pm0.03$ & $-0.26\pm0.05$ & 1.61 &  & $-0.26\pm0.03$ & $-0.29\pm0.12$ & main \\
HIP 40848 & $5191\pm23$ & $4.56\pm0.03$ & $-0.01\pm0.06$ & 0.70 &  & $-0.02\pm0.03$ & $0.11\pm0.11$ & main \\
HIP 41484 & $5801\pm41$ & $4.35\pm0.02$ & $0.02\pm0.03$ & 1.02 &  & $0.02\pm0.02$ & $0.04\pm0.08$ & main \\
HIP 41832 & $5799\pm36$ & $4.45\pm0.04$ & $-0.05\pm0.04$ & 1.04 &  & $-0.05\pm0.03$ & $-0.05\pm0.07$ & main \\
HIP 41926 & $5290\pm40$ & $4.56\pm0.03$ & $-0.36\pm0.06$ & 0.64 &  & $-0.36\pm0.03$ & $-0.36\pm0.18$ & main \\
HIP 42343 & $6249\pm50$ & $4.21\pm0.03$ & $-0.23\pm0.05$ & 1.64 &  & $-0.23\pm0.04$ & $-0.24\pm0.10$ & main \\
HIP 42438 & $5901\pm50$ & $4.49\pm0.01$ & $-0.02\pm0.09$ & 1.32 & + & $-0.01\pm0.08$ & $-0.03\pm0.15$ & main \\
HIP 42575 & $5695\pm44$ & $4.47\pm0.04$ & $0.04\pm0.04$ & 0.97 &  & $0.04\pm0.03$ & $0.07\pm0.07$ & main \\
HIP 42612 & $5794\pm31$ & $4.06\pm0.07$ & $-0.01\pm0.03$ & 1.27 &  & $-0.01\pm0.03$ & $-0.05\pm0.05$ & main \\
HIP 42734 & $5693\pm43$ & $4.03\pm0.03$ & $-0.65\pm0.05$ & 1.21 &  & $-0.66\pm0.04$ & $-0.59\pm0.09$ & main \\
HIP 42808 & $5005\pm29$ & $4.61\pm0.02$ & $-0.01\pm0.07$ & 0.67 &  & $0.00\pm0.06$ & $-0.07\pm0.17$ & main \\
HIP 43393 & $5406\pm32$ & $4.48\pm0.03$ & $-0.45\pm0.05$ & 0.77 &  & $-0.45\pm0.03$ & $-0.39\pm0.14$ & main \\
HIP 43587 & $5249\pm77$ & $4.42\pm0.04$ & $0.39\pm0.06$ & 0.50 &  & $0.39\pm0.05$ & $0.40\pm0.06$ & main \\
HIP 43595 & $5764\pm31$ & $4.47\pm0.12$ & $-0.72\pm0.07$ & 1.36 &  & $-0.71\pm0.06$ & $-0.84\pm0.10$ & main \\
HIP 43618 & $5629\pm38$ & $4.36\pm0.05$ & $0.19\pm0.05$ & 0.98 &  & $0.18\pm0.04$ & $0.27\pm0.03$ & main \\
HIP 43727 & $5886\pm38$ & $4.16\pm0.06$ & $0.09\pm0.04$ & 1.39 &  & $0.09\pm0.04$ & $0.12\pm0.03$ & main \\
HIP 43861 & $5381\pm50$ & $4.33\pm0.03$ & $-0.18\pm0.07$ & 0.81 &  & $-0.20\pm0.04$ & $-0.02\pm0.03$ & main \\
HIP 43904 & $6092\pm37$ & $4.23\pm0.03$ & $-0.41\pm0.05$ & 1.23 &  & $-0.42\pm0.04$ & $-0.39\pm0.10$ & main \\
HIP 43981 & $6100\pm50$ & $4.18\pm0.04$ & $-0.39\pm0.04$ & 1.41 &  & $-0.38\pm0.04$ & $-0.39\pm0.08$ & main \\
HIP 44075 & $5959\pm41$ & $4.16\pm0.02$ & $-0.83\pm0.07$ & 1.23 &  & $-0.84\pm0.06$ & $-0.84\pm0.17$ & main \\
HIP 44212 & $6044\pm36$ & $4.38\pm0.04$ & $-0.28\pm0.05$ & 1.24 &  & $-0.29\pm0.04$ & $-0.28\pm0.10$ & main \\
HIP 44324 & $5716\pm38$ & $4.34\pm0.04$ & $-0.15\pm0.06$ & 1.22 &  & $-0.17\pm0.04$ & $-0.04\pm0.09$ & main \\
HIP 44347 & $5951\pm48$ & $4.37\pm0.10$ & $-0.78\pm0.06$ & 1.20 &  & $-0.78\pm0.06$ & $-0.73\pm0.06$ & main \\
HIP 44441 & $6205\pm45$ & $4.10\pm0.04$ & $-0.32\pm0.06$ & 1.69 &  & $-0.31\pm0.04$ & $-0.37\pm0.13$ & main \\
HIP 44858 & $5973\pm37$ & $4.49\pm0.04$ & $-0.30\pm0.04$ & 0.90 &  & $-0.30\pm0.03$ & $-0.30\pm0.09$ & main \\
HIP 44860 & $5763\pm50$ & $4.19\pm0.03$ & $-0.43\pm0.04$ & 1.21 &  & $-0.43\pm0.03$ & $-0.48\pm0.04$ & main \\
HIP 44927 & $5932\pm42$ & $3.86\pm0.04$ & $-0.25\pm0.03$ & 1.58 &  & $-0.25\pm0.03$ & $-0.28\pm0.04$ & main \\
HIP 44997 & $5713\pm48$ & $4.37\pm0.04$ & $-0.03\pm0.03$ & 1.00 &  & $-0.03\pm0.01$ & $-0.04\pm0.05$ & main \\
HIP 45333 & $5973\pm72$ & $4.13\pm0.03$ & $0.05\pm0.04$ & 1.20 &  & $0.05\pm0.03$ & $0.06\pm0.10$ & main \\
HIP 45699 & $6100\pm76$ & $4.07\pm0.04$ & $-0.31\pm0.05$ & 1.43 &  & $-0.31\pm0.04$ & $-0.29\pm0.10$ & main \\
HIP 45718 & $5933\pm31$ & $4.45\pm0.04$ & $0.05\pm0.05$ & 1.34 &  & $0.05\pm0.05$ & $0.04\pm0.04$ & main \\
HIP 45947 & $4956\pm51$ & $3.30\pm0.11$ & $-0.47\pm0.04$ & 1.06 &  & $-0.47\pm0.04$ & $-0.48\pm0.06$ & giant \\
HIP 46066 & $5695\pm34$ & $4.47\pm0.06$ & $-0.10\pm0.03$ & 1.10 &  & $-0.10\pm0.02$ & $-0.13\pm0.06$ & main \\
HIP 46453 & $5921\pm59$ & $3.99\pm0.05$ & $0.19\pm0.03$ & 1.51 &  & $0.18\pm0.03$ & $0.21\pm0.04$ & main \\
HIP 46853 & $6364\pm63$ & $3.88\pm0.01$ & $-0.19\pm0.04$ & 1.90 &  & $-0.19\pm0.03$ & $-0.21\pm0.08$ & main \\
HIP 47080 & $5511\pm45$ & $4.46\pm0.03$ & $0.28\pm0.06$ & 1.02 &  & $0.27\pm0.04$ & $0.32\pm0.14$ & main \\
HIP 47173 & $5780\pm115$ & $4.50\pm0.23$ & $-0.33\pm0.07$ & 0.95 &  & $-0.33\pm0.06$ & $-0.34\pm0.17$ & manual \\
HIP 47292 & $5927\pm75$ & $4.17\pm0.05$ & $-0.34\pm0.04$ & 1.32 &  & $-0.35\pm0.03$ & $-0.28\pm0.07$ & main \\
HIP 47588 & $5566\pm43$ & $4.07\pm0.04$ & $-0.49\pm0.08$ & 0.88 &  & $-0.51\pm0.05$ & $-0.34\pm0.13$ & main \\
HIP 48113 & $5872\pm38$ & $4.10\pm0.02$ & $0.09\pm0.04$ & 1.25 &  & $0.08\pm0.03$ & $0.11\pm0.06$ & main \\
HIP 48152 & $6377\pm36$ & $4.15\pm0.06$ & $-2.02\pm0.08$ & 1.79 & + & $-2.03\pm0.07$ & $-2.01\pm0.10$ & main \\
HIP 48209 & $5588\pm40$ & $4.47\pm0.06$ & $-0.53\pm0.05$ & 1.01 &  & $-0.53\pm0.03$ & $-0.52\pm0.16$ & main \\
HIP 48468 & $5855\pm63$ & $3.74\pm0.03$ & $0.00\pm0.06$ & 1.81 &  & $0.00\pm0.05$ & $-0.02\pm0.10$ & main \\
HIP 48701 & $5750\pm41$ & $4.39\pm0.08$ & $-0.54\pm0.05$ & 1.07 &  & $-0.55\pm0.04$ & $-0.45\pm0.05$ & main \\
HIP 48833 & $6391\pm63$ & $3.98\pm0.03$ & $-0.32\pm0.09$ & 1.79 & + & $-0.32\pm0.08$ & $-0.33\pm0.13$ & main \\
HIP 49070 & $5936\pm53$ & $4.16\pm0.03$ & $-0.39\pm0.05$ & 1.36 &  & $-0.39\pm0.04$ & $-0.41\pm0.08$ & main \\
HIP 49130 & $5380\pm49$ & $4.39\pm0.02$ & $-0.15\pm0.06$ & 0.76 &  & $-0.16\pm0.04$ & $-0.03\pm0.10$ & main \\
HIP 49246 & $5988\pm37$ & $3.87\pm0.04$ & $-0.25\pm0.07$ & 1.58 &  & $-0.24\pm0.04$ & $-0.34\pm0.14$ & main \\
HIP 49572 & $5732\pm55$ & $4.36\pm0.08$ & $-0.05\pm0.03$ & 0.99 &  & $-0.06\pm0.02$ & $-0.01\pm0.02$ & main \\
HIP 49615 & $6097\pm55$ & $4.34\pm0.04$ & $-0.44\pm0.04$ & 1.31 &  & $-0.45\pm0.03$ & $-0.38\pm0.06$ & main \\
HIP 49621 & $5864\pm31$ & $4.51\pm0.04$ & $-0.15\pm0.04$ & 1.27 &  & $-0.16\pm0.04$ & $-0.13\pm0.06$ & main \\
HIP 49668 & $5808\pm27$ & $4.24\pm0.03$ & $-0.22\pm0.04$ & 1.18 &  & $-0.23\pm0.03$ & $-0.20\pm0.09$ & main \\
HIP 49756 & $5774\pm30$ & $4.44\pm0.03$ & $0.00\pm0.03$ & 1.20 &  & $0.00\pm0.02$ & $-0.02\pm0.06$ & main \\
HIP 49988 & $5958\pm36$ & $4.03\pm0.05$ & $-0.63\pm0.18$ & 1.46 & + & $-0.65\pm0.17$ & $-0.53\pm0.26$ & main \\
HIP 50005 & $5535\pm42$ & $4.55\pm0.07$ & $-0.32\pm0.07$ & 0.81 &  & $-0.33\pm0.06$ & $-0.30\pm0.13$ & main \\
HIP 50319 & $5678\pm41$ & $3.92\pm0.02$ & $-0.01\pm0.07$ & 1.27 &  & $-0.01\pm0.04$ & $-0.03\pm0.18$ & main \\
HIP 50355 & $5841\pm39$ & $4.37\pm0.04$ & $-0.14\pm0.03$ & 1.14 &  & $-0.14\pm0.03$ & $-0.15\pm0.03$ & main \\
HIP 50671 & $5984\pm43$ & $4.37\pm0.03$ & $-0.45\pm0.04$ & 1.21 &  & $-0.45\pm0.04$ & $-0.43\pm0.07$ & main \\
HIP 50965 & $5893\pm66$ & $4.39\pm0.12$ & $-0.45\pm0.06$ & 0.88 &  & $-0.45\pm0.05$ & $-0.46\pm0.12$ & main \\
HIP 51128 & $5800\pm36$ & $4.49\pm0.03$ & $0.03\pm0.03$ & 1.17 &  & $0.03\pm0.03$ & $0.02\pm0.06$ & main \\
HIP 51248 & $5734\pm68$ & $4.30\pm0.03$ & $-0.37\pm0.07$ & 1.29 &  & $-0.38\pm0.05$ & $-0.31\pm0.15$ & main \\
HIP 51406 & $6330\pm57$ & $3.87\pm0.05$ & $-0.29\pm0.05$ & 1.97 &  & $-0.30\pm0.03$ & $-0.26\pm0.09$ & main \\
HIP 51459 & $6186\pm63$ & $4.43\pm0.03$ & $-0.08\pm0.04$ & 1.28 &  & $-0.08\pm0.03$ & $-0.09\pm0.08$ & main \\
HIP 51477 & $5926\pm45$ & $4.04\pm0.06$ & $-0.91\pm0.07$ & 1.53 &  & $-0.89\pm0.06$ & $-1.02\pm0.05$ & main \\
HIP 51784 & $6212\pm51$ & $4.27\pm0.03$ & $-0.29\pm0.05$ & 1.52 &  & $-0.29\pm0.04$ & $-0.33\pm0.11$ & main \\
HIP 51933 & $6109\pm36$ & $4.11\pm0.02$ & $-0.29\pm0.06$ & 1.73 &  & $-0.28\pm0.04$ & $-0.37\pm0.08$ & main \\
HIP 51993 & $5639\pm34$ & $3.86\pm0.06$ & $-0.02\pm0.05$ & 1.32 &  & $-0.03\pm0.04$ & $0.04\pm0.01$ & main \\
HIP 52015 & $5726\pm32$ & $3.97\pm0.05$ & $0.10\pm0.04$ & 1.21 &  & $0.10\pm0.03$ & $0.12\pm0.09$ & main \\
HIP 52040 & $5787\pm33$ & $4.52\pm0.04$ & $-0.10\pm0.03$ & 1.02 &  & $-0.10\pm0.03$ & $-0.10\pm0.04$ & main \\
HIP 52137 & $5781\pm37$ & $4.49\pm0.03$ & $0.04\pm0.03$ & 1.11 &  & $0.04\pm0.03$ & $0.05\pm0.03$ & main \\
HIP 52153 & $5791\pm30$ & $4.16\pm0.05$ & $-0.17\pm0.04$ & 1.22 &  & $-0.18\pm0.04$ & $-0.11\pm0.04$ & main \\
HIP 52325 & $5477\pm36$ & $4.37\pm0.06$ & $-0.10\pm0.08$ & 1.01 &  & $-0.12\pm0.05$ & $0.10\pm0.10$ & main \\
HIP 52673 & $5714\pm44$ & $4.47\pm0.07$ & $-0.61\pm0.06$ & 1.40 &  & $-0.60\pm0.04$ & $-0.71\pm0.10$ & main \\
HIP 52761 & $5785\pm64$ & $4.44\pm0.07$ & $-0.13\pm0.06$ & 1.25 &  & $-0.12\pm0.04$ & $-0.13\pm0.12$ & main \\
HIP 52771 & $5937\pm29$ & $4.54\pm0.06$ & $-1.85\pm0.12$ & 1.25 & + & $-1.80\pm0.10$ & $-1.93\pm0.10$ & main \\
HIP 52990 & $5919\pm42$ & $4.19\pm0.03$ & $0.04\pm0.03$ & 1.32 &  & $0.04\pm0.03$ & $0.02\pm0.05$ & main \\
HIP 53049 & $6166\pm80$ & $4.39\pm0.05$ & $-0.46\pm0.05$ & 1.43 &  & $-0.46\pm0.04$ & $-0.41\pm0.09$ & main \\
HIP 53229 & $4733\pm76$ & $2.73\pm0.16$ & $-0.11\pm0.06$ & 1.32 &  & $-0.11\pm0.05$ & $-0.12\pm0.09$ & giant \\
HIP 53535 & $5791\pm39$ & $4.10\pm0.05$ & $0.32\pm0.05$ & 1.20 &  & $0.32\pm0.04$ & $0.36\pm0.10$ & main \\
HIP 53537 & $5828\pm46$ & $4.32\pm0.04$ & $0.10\pm0.04$ & 1.05 &  & $0.09\pm0.02$ & $0.18\pm0.08$ & main \\
HIP 53721 & $5894\pm59$ & $4.30\pm0.03$ & $0.02\pm0.03$ & 1.13 &  & $0.02\pm0.02$ & $0.03\pm0.07$ & main \\
HIP 53725 & $5756\pm31$ & $4.32\pm0.05$ & $-0.38\pm0.04$ & 1.26 &  & $-0.38\pm0.03$ & $-0.39\pm0.08$ & main \\
HIP 53898 & $5639\pm30$ & $4.43\pm0.04$ & $-0.04\pm0.04$ & 0.91 &  & $-0.05\pm0.03$ & $0.03\pm0.05$ & main \\
HIP 54196 & $5877\pm53$ & $4.09\pm0.03$ & $-0.35\pm0.06$ & 1.24 &  & $-0.36\pm0.05$ & $-0.31\pm0.15$ & main \\
HIP 54239 & $5856\pm34$ & $4.43\pm0.08$ & $-0.45\pm0.06$ & 1.06 &  & $-0.45\pm0.06$ & $-0.39\pm0.06$ & main \\
HIP 54582 & $5807\pm38$ & $4.22\pm0.02$ & $-0.13\pm0.05$ & 1.15 &  & $-0.13\pm0.03$ & $-0.12\pm0.12$ & main \\
HIP 54728 & $5785\pm30$ & $4.39\pm0.04$ & $0.03\pm0.04$ & 1.01 &  & $0.03\pm0.04$ & $0.07\pm0.07$ & main \\
HIP 55288A & $6244\pm101$ & $4.24\pm0.08$ & $0.02\pm0.05$ & 1.79 &  & $0.03\pm0.04$ & $-0.02\pm0.10$ & main \\
HIP 55288B & $5702\pm67$ & $4.30\pm0.07$ & $0.05\pm0.04$ & 1.03 &  & $0.05\pm0.03$ & $0.07\pm0.07$ & main \\
HIP 55459 & $5711\pm37$ & $4.32\pm0.03$ & $-0.01\pm0.03$ & 1.02 &  & $-0.02\pm0.03$ & $0.04\pm0.02$ & main \\
HIP 55592 & $6068\pm40$ & $4.36\pm0.13$ & $-0.85\pm0.08$ & 1.38 & + & $-0.86\pm0.07$ & $-0.81\pm0.11$ & main \\
HIP 55666 & $6117\pm47$ & $4.07\pm0.03$ & $-0.19\pm0.05$ & 1.57 &  & $-0.18\pm0.04$ & $-0.23\pm0.10$ & main \\
HIP 55761 & $5912\pm50$ & $4.35\pm0.04$ & $-0.57\pm0.04$ & 1.33 &  & $-0.56\pm0.04$ & $-0.62\pm0.03$ & main \\
HIP 56148 & $6074\pm54$ & $3.68\pm0.02$ & $-0.37\pm0.06$ & 1.68 &  & $-0.38\pm0.04$ & $-0.36\pm0.13$ & main \\
HIP 56186 & $6182\pm53$ & $4.32\pm0.03$ & $-0.37\pm0.06$ & 1.23 &  & $-0.38\pm0.03$ & $-0.30\pm0.12$ & main \\
HIP 56290 & $6155\pm37$ & $3.99\pm0.02$ & $-0.33\pm0.06$ & 1.49 &  & $-0.32\pm0.04$ & $-0.39\pm0.10$ & main \\
HIP 56423 & $6053\pm65$ & $4.19\pm0.04$ & $-0.46\pm0.05$ & 1.40 &  & $-0.46\pm0.04$ & $-0.48\pm0.09$ & main \\
HIP 56452 & $5241\pm50$ & $4.59\pm0.03$ & $-0.37\pm0.05$ & 0.66 &  & $-0.37\pm0.03$ & $-0.36\pm0.16$ & main \\
HIP 56948 & $5789\pm49$ & $4.39\pm0.05$ & $-0.01\pm0.03$ & 1.20 &  & $-0.01\pm0.02$ & $0.01\pm0.08$ & main \\
HIP 56960 & $6157\pm79$ & $4.44\pm0.03$ & $-0.10\pm0.04$ & 1.28 &  & $-0.11\pm0.03$ & $-0.01\pm0.05$ & main \\
HIP 56997 & $5528\pm37$ & $4.53\pm0.02$ & $-0.05\pm0.05$ & 0.96 &  & $-0.05\pm0.03$ & $-0.03\pm0.08$ & main \\
HIP 57080 & $6174\pm35$ & $4.14\pm0.03$ & $-0.45\pm0.06$ & 1.59 &  & $-0.45\pm0.05$ & $-0.44\pm0.10$ & main \\
HIP 57117 & $5964\pm52$ & $3.74\pm0.07$ & $-0.13\pm0.05$ & 1.63 &  & $-0.13\pm0.04$ & $-0.11\pm0.10$ & main \\
HIP 57300 & $6054\pm41$ & $4.23\pm0.08$ & $-0.36\pm0.04$ & 1.30 &  & $-0.36\pm0.04$ & $-0.37\pm0.10$ & main \\
HIP 57349 & $5791\pm30$ & $4.29\pm0.03$ & $-0.42\pm0.05$ & 1.18 &  & $-0.42\pm0.05$ & $-0.44\pm0.07$ & main \\
HIP 57443 & $5655\pm56$ & $4.44\pm0.03$ & $-0.29\pm0.04$ & 0.93 &  & $-0.30\pm0.03$ & $-0.29\pm0.07$ & main \\
HIP 57450 & $5725\pm33$ & $4.56\pm0.05$ & $-1.19\pm0.07$ & 1.24 &  & $-1.19\pm0.07$ & $-1.22\pm0.06$ & main \\
HIP 57532 & $5488\pm45$ & $4.38\pm0.05$ & $0.22\pm0.08$ & 0.94 &  & $0.20\pm0.03$ & $0.35\pm0.14$ & main \\
HIP 57617 & $6023\pm49$ & $4.12\pm0.05$ & $-0.29\pm0.05$ & 1.36 &  & $-0.29\pm0.04$ & $-0.32\pm0.11$ & main \\
HIP 57757 & $6103\pm51$ & $4.08\pm0.03$ & $0.11\pm0.04$ & 1.44 &  & $0.11\pm0.03$ & $0.12\pm0.09$ & main \\
HIP 57939 & $5149\pm31$ & $4.71\pm0.01$ & $-1.27\pm0.07$ & 0.52 & + & $-1.27\pm0.07$ & $-1.17\pm0.08$ & main \\
HIP 58171 & $5683\pm26$ & $4.45\pm0.06$ & $0.08\pm0.04$ & 0.87 &  & $0.08\pm0.03$ & $0.10\pm0.07$ & main \\
HIP 58201 & $5992\pm31$ & $4.44\pm0.04$ & $0.09\pm0.04$ & 1.09 &  & $0.09\pm0.03$ & $0.08\pm0.09$ & main \\
HIP 58229 & $6157\pm56$ & $4.23\pm0.19$ & $-0.65\pm0.10$ & 1.66 &  & $-0.63\pm0.08$ & $-0.74\pm0.16$ & main \\
HIP 58331 & $6018\pm63$ & $3.82\pm0.03$ & $-0.25\pm0.05$ & 1.62 &  & $-0.24\pm0.03$ & $-0.31\pm0.11$ & main \\
HIP 58576 & $5484\pm37$ & $4.39\pm0.03$ & $0.26\pm0.07$ & 0.79 &  & $0.25\pm0.04$ & $0.37\pm0.15$ & main \\
HIP 58843 & $5822\pm58$ & $4.42\pm0.08$ & $-0.75\pm0.04$ & 1.27 &  & $-0.74\pm0.04$ & $-0.79\pm0.02$ & main \\
HIP 59021 & $5799\pm65$ & $3.81\pm0.03$ & $-0.22\pm0.05$ & 1.33 &  & $-0.23\pm0.04$ & $-0.18\pm0.09$ & main \\
HIP 59233 & $5496\pm51$ & $4.54\pm0.04$ & $-0.73\pm0.05$ & 0.94 &  & $-0.74\pm0.03$ & $-0.65\pm0.08$ & main \\
HIP 59253 & $5694\pm42$ & $4.42\pm0.05$ & $0.11\pm0.04$ & 1.29 &  & $0.10\pm0.04$ & $0.16\pm0.05$ & main \\
HIP 59532 & $5666\pm34$ & $4.36\pm0.02$ & $0.16\pm0.04$ & 0.92 &  & $0.15\pm0.02$ & $0.18\pm0.08$ & main \\
HIP 59589 & $5664\pm31$ & $4.37\pm0.03$ & $-0.13\pm0.04$ & 0.94 &  & $-0.14\pm0.02$ & $-0.11\pm0.09$ & main \\
HIP 59735 & $5895\pm62$ & $4.36\pm0.06$ & $-0.44\pm0.04$ & 1.13 &  & $-0.45\pm0.03$ & $-0.36\pm0.02$ & main \\
HIP 59750 & $6258\pm39$ & $4.36\pm0.03$ & $-0.73\pm0.05$ & 1.46 &  & $-0.72\pm0.04$ & $-0.76\pm0.13$ & main \\
HIP 60019 & $5925\pm43$ & $3.94\pm0.03$ & $-0.39\pm0.05$ & 1.39 &  & $-0.40\pm0.04$ & $-0.38\pm0.10$ & main \\
HIP 60268 & $5669\pm34$ & $4.44\pm0.02$ & $-0.64\pm0.05$ & 1.03 &  & $-0.64\pm0.04$ & $-0.66\pm0.13$ & main \\
HIP 60314 & $5784\pm54$ & $4.41\pm0.05$ & $0.07\pm0.03$ & 1.13 &  & $0.07\pm0.03$ & $0.07\pm0.05$ & main \\
HIP 60331 & $5600\pm112$ & $4.60\pm0.23$ & $-0.60\pm0.09$ & 0.90 &  & $-0.59\pm0.09$ & $-0.66\pm0.12$ & manual \\
HIP 60366 & $5946\pm31$ & $4.49\pm0.02$ & $0.01\pm0.05$ & 1.18 &  & $0.00\pm0.05$ & $0.03\pm0.08$ & main \\
HIP 60588 & $5893\pm30$ & $4.21\pm0.03$ & $-0.33\pm0.05$ & 1.21 &  & $-0.32\pm0.04$ & $-0.35\pm0.10$ & main \\
HIP 60719 & $5250\pm105$ & $2.70\pm0.14$ & $-2.42\pm0.11$ & 1.50 &  & $-2.42\pm0.11$ & $-2.44\pm0.13$ & manual \\
HIP 60956 & $5425\pm27$ & $4.51\pm0.03$ & $-0.55\pm0.06$ & 0.64 &  & $-0.55\pm0.04$ & $-0.52\pm0.16$ & main \\
HIP 61044 & $5822\pm54$ & $4.37\pm0.04$ & $0.26\pm0.05$ & 1.19 &  & $0.26\pm0.03$ & $0.33\pm0.08$ & main \\
HIP 61157 & $6012\pm34$ & $3.80\pm0.03$ & $-0.39\pm0.06$ & 1.44 &  & $-0.41\pm0.04$ & $-0.27\pm0.07$ & main \\
HIP 61264 & $6040\pm52$ & $3.96\pm0.05$ & $-0.60\pm0.06$ & 1.51 &  & $-0.59\pm0.04$ & $-0.63\pm0.12$ & main \\
HIP 61272 & $5513\pm59$ & $4.04\pm0.21$ & $-0.10\pm0.07$ & 1.32 &  & $-0.10\pm0.07$ & $-0.10\pm0.08$ & noplx \\
HIP 61293 & $6143\pm24$ & $4.29\pm0.02$ & $-0.01\pm0.04$ & 1.53 &  & $-0.01\pm0.04$ & $-0.01\pm0.06$ & main \\
HIP 61317 & $5899\pm60$ & $4.38\pm0.03$ & $-0.22\pm0.04$ & 1.16 &  & $-0.22\pm0.03$ & $-0.24\pm0.09$ & main \\
HIP 62039 & $5658\pm48$ & $4.33\pm0.04$ & $0.11\pm0.05$ & 0.96 &  & $0.10\pm0.04$ & $0.20\pm0.05$ & main \\
HIP 62077 & $5810\pm45$ & $4.23\pm0.11$ & $-0.45\pm0.04$ & 1.00 &  & $-0.45\pm0.03$ & $-0.41\pm0.05$ & main \\
HIP 62162 & $6035\pm78$ & $4.01\pm0.05$ & $-0.71\pm0.06$ & 1.52 &  & $-0.72\pm0.04$ & $-0.59\pm0.05$ & main \\
HIP 62175 & $5776\pm34$ & $4.40\pm0.03$ & $0.10\pm0.03$ & 1.15 &  & $0.10\pm0.03$ & $0.10\pm0.04$ & main \\
HIP 62198 & $5712\pm49$ & $4.32\pm0.08$ & $0.07\pm0.04$ & 1.08 &  & $0.07\pm0.03$ & $0.10\pm0.06$ & main \\
HIP 62240 & $5869\pm68$ & $4.21\pm0.11$ & $-0.34\pm0.06$ & 1.37 &  & $-0.32\pm0.04$ & $-0.45\pm0.09$ & main \\
HIP 62307 & $6051\pm57$ & $3.92\pm0.07$ & $-0.51\pm0.04$ & 1.55 &  & $-0.50\pm0.03$ & $-0.57\pm0.07$ & main \\
HIP 62507 & $5804\pm40$ & $4.16\pm0.07$ & $-0.17\pm0.05$ & 1.14 &  & $-0.18\pm0.04$ & $-0.14\pm0.11$ & main \\
HIP 62527 & $5811\pm40$ & $4.31\pm0.03$ & $0.11\pm0.04$ & 1.18 &  & $0.10\pm0.04$ & $0.17\pm0.05$ & main \\
HIP 62607 & $5471\pm32$ & $4.51\pm0.02$ & $-0.56\pm0.05$ & 0.78 &  & $-0.56\pm0.04$ & $-0.64\pm0.12$ & main \\
HIP 62661 & $5945\pm59$ & $4.20\pm0.04$ & $0.02\pm0.04$ & 1.38 &  & $0.02\pm0.04$ & $0.01\pm0.06$ & main \\
HIP 62816 & $5805\pm42$ & $4.49\pm0.04$ & $0.01\pm0.04$ & 1.03 &  & $0.01\pm0.03$ & $0.04\pm0.08$ & main \\
HIP 62882 & $5819\pm56$ & $3.85\pm0.08$ & $-1.07\pm0.07$ & 1.45 & + & $-1.07\pm0.05$ & $-1.07\pm0.12$ & main \\
HIP 63330 & $6031\pm54$ & $4.07\pm0.03$ & $0.10\pm0.04$ & 1.53 &  & $0.10\pm0.03$ & $0.16\pm0.08$ & main \\
HIP 63354 & $6062\pm46$ & $4.40\pm0.04$ & $-0.35\pm0.05$ & 1.29 &  & $-0.35\pm0.04$ & $-0.34\pm0.11$ & main \\
HIP 63405 & $6374\pm56$ & $3.90\pm0.04$ & $-0.38\pm0.05$ & 2.01 &  & $-0.40\pm0.04$ & $-0.31\pm0.06$ & main \\
HIP 63881 & $5670\pm32$ & $4.30\pm0.06$ & $0.12\pm0.04$ & 1.11 &  & $0.11\pm0.03$ & $0.16\pm0.07$ & main \\
HIP 64103 & $5613\pm45$ & $4.50\pm0.06$ & $-0.14\pm0.06$ & 0.77 &  & $-0.14\pm0.03$ & $-0.12\pm0.15$ & main \\
HIP 64150 & $5723\pm39$ & $4.37\pm0.02$ & $0.05\pm0.04$ & 1.05 &  & $0.05\pm0.03$ & $0.10\pm0.07$ & main \\
HIP 64241 & $6406\pm72$ & $4.03\pm0.03$ & $-0.23\pm0.10$ & 1.79 & + & $-0.21\pm0.08$ & $-0.36\pm0.09$ & main \\
HIP 64254 & $5795\pm28$ & $4.45\pm0.07$ & $-0.30\pm0.04$ & 1.05 &  & $-0.30\pm0.04$ & $-0.29\pm0.07$ & main \\
HIP 64344 & $5726\pm28$ & $4.39\pm0.06$ & $0.04\pm0.07$ & 1.06 & + & $0.04\pm0.07$ & $0.06\pm0.09$ & main \\
HIP 64394 & $6034\pm61$ & $4.44\pm0.03$ & $0.06\pm0.03$ & 1.18 &  & $0.05\pm0.02$ & $0.09\pm0.05$ & main \\
HIP 64407 & $6375\pm67$ & $3.83\pm0.02$ & $-0.21\pm0.07$ & 1.86 & + & $-0.22\pm0.07$ & $-0.17\pm0.08$ & main \\
HIP 64426 & $5895\pm45$ & $4.21\pm0.03$ & $-0.71\pm0.06$ & 1.16 &  & $-0.71\pm0.05$ & $-0.65\pm0.14$ & main \\
HIP 64497 & $5827\pm42$ & $4.44\pm0.05$ & $0.12\pm0.04$ & 1.39 &  & $0.12\pm0.04$ & $0.11\pm0.04$ & main \\
HIP 64583 & $6303\pm51$ & $4.17\pm0.02$ & $-0.29\pm0.08$ & 1.64 & + & $-0.28\pm0.09$ & $-0.29\pm0.06$ & main \\
HIP 64698 & $5650\pm32$ & $4.34\pm0.06$ & $-0.11\pm0.03$ & 0.87 &  & $-0.10\pm0.02$ & $-0.11\pm0.06$ & main \\
HIP 64792 & $5995\pm41$ & $4.24\pm0.02$ & $0.11\pm0.05$ & 1.34 &  & $0.11\pm0.04$ & $0.14\pm0.10$ & main \\
HIP 64794 & $5788\pm30$ & $4.40\pm0.05$ & $-0.07\pm0.03$ & 1.07 &  & $-0.07\pm0.02$ & $-0.08\pm0.05$ & main \\
HIP 64797 & $5081\pm65$ & $4.62\pm0.03$ & $-0.16\pm0.06$ & 0.77 &  & $-0.16\pm0.05$ & $-0.16\pm0.13$ & main \\
HIP 64924 & $5571\pm44$ & $4.42\pm0.03$ & $-0.02\pm0.04$ & 0.90 &  & $-0.02\pm0.03$ & $0.01\pm0.09$ & main \\
HIP 65049 & $5539\pm42$ & $4.25\pm0.04$ & $0.20\pm0.06$ & 0.92 &  & $0.18\pm0.04$ & $0.29\pm0.08$ & main \\
HIP 65449 & $5584\pm30$ & $4.00\pm0.07$ & $-0.29\pm0.06$ & 1.11 &  & $-0.28\pm0.02$ & $-0.32\pm0.14$ & main \\
HIP 65641 & $5706\pm39$ & $4.43\pm0.05$ & $0.02\pm0.04$ & 0.97 &  & $0.02\pm0.04$ & $0.06\pm0.05$ & main \\
HIP 65708 & $5735\pm43$ & $4.18\pm0.03$ & $-0.07\pm0.03$ & 1.20 &  & $-0.07\pm0.02$ & $-0.06\pm0.04$ & main \\
HIP 65971 & $5841\pm51$ & $4.41\pm0.04$ & $-0.28\pm0.07$ & 1.07 &  & $-0.29\pm0.06$ & $-0.20\pm0.11$ & main \\
HIP 65982 & $5360\pm107$ & $4.45\pm0.22$ & $-0.37\pm0.06$ & 1.05 &  & $-0.38\pm0.03$ & $-0.36\pm0.15$ & manual \\
HIP 66051 & $5824\pm44$ & $4.07\pm0.04$ & $-0.57\pm0.04$ & 1.38 &  & $-0.57\pm0.03$ & $-0.57\pm0.09$ & main \\
HIP 66464 & $6126\pm44$ & $4.33\pm0.05$ & $-0.42\pm0.04$ & 1.36 &  & $-0.43\pm0.04$ & $-0.37\pm0.05$ & main \\
HIP 66514 & $5628\pm30$ & $4.21\pm0.04$ & $0.00\pm0.05$ & 1.32 &  & $0.00\pm0.05$ & $0.02\pm0.03$ & main \\
HIP 66860 & $6647\pm79$ & $4.24\pm0.03$ & $-0.20\pm0.06$ & 2.08 &  & $-0.20\pm0.04$ & $-0.24\pm0.13$ & main \\
HIP 66974 & $5706\pm37$ & $3.87\pm0.03$ & $-0.07\pm0.04$ & 1.36 &  & $-0.08\pm0.03$ & $-0.02\pm0.04$ & main \\
HIP 67422 & $4600\pm92$ & $4.60\pm0.23$ & $-0.07\pm0.07$ & 0.00 &  & $-0.07\pm0.06$ & $0.11\pm0.04$ & manual \\
HIP 67927 & $6047\pm62$ & $3.78\pm0.03$ & $0.26\pm0.10$ & 1.61 & + & $0.26\pm0.09$ & $0.24\pm0.15$ & main \\
HIP 68030 & $6139\pm37$ & $4.29\pm0.02$ & $-0.39\pm0.05$ & 1.36 &  & $-0.39\pm0.04$ & $-0.42\pm0.10$ & main \\
HIP 68085 & $5612\pm51$ & $3.99\pm0.03$ & $-0.20\pm0.05$ & 1.24 &  & $-0.20\pm0.04$ & $-0.21\pm0.09$ & main \\
HIP 68184 & $4851\pm78$ & $4.58\pm0.02$ & $0.11\pm0.06$ & 0.28 & + & $0.11\pm0.05$ & $0.09\pm0.16$ & main \\
HIP 68594 & $4590\pm91$ & $1.20\pm0.06$ & $-2.71\pm0.11$ & 2.50 &  & $-2.77\pm0.03$ & $-2.56\pm0.06$ & manual \\
HIP 69210 & $5963\pm38$ & $4.46\pm0.04$ & $-0.02\pm0.03$ & 1.02 &  & $-0.02\pm0.03$ & $-0.02\pm0.06$ & main \\
HIP 69232 & $5702\pm64$ & $4.43\pm0.26$ & $-0.59\pm0.10$ & 1.05 & + & $-0.60\pm0.10$ & $-0.50\pm0.09$ & main \\
HIP 69535 & $6174\pm41$ & $4.21\pm0.04$ & $-0.27\pm0.04$ & 1.55 &  & $-0.27\pm0.03$ & $-0.23\pm0.07$ & main \\
HIP 69673 & $4215\pm90$ & $1.53\pm0.20$ & $-0.60\pm0.08$ & 1.65 &  & $-0.61\pm0.07$ & $-0.50\pm0.11$ & giant \\
HIP 69701 & $6193\pm50$ & $3.72\pm0.03$ & $-0.23\pm0.11$ & 1.77 & + & $-0.23\pm0.11$ & $-0.24\pm0.13$ & main \\
HIP 69972 & $4899\pm48$ & $4.55\pm0.03$ & $0.28\pm0.08$ & 0.32 & + & $0.29\pm0.08$ & $0.16\pm0.13$ & main \\
HIP 70319 & $5691\pm30$ & $4.44\pm0.02$ & $-0.36\pm0.04$ & 1.07 &  & $-0.36\pm0.03$ & $-0.38\pm0.09$ & main \\
HIP 70324 & $5696\pm49$ & $4.40\pm0.07$ & $-0.45\pm0.06$ & 1.17 &  & $-0.46\pm0.03$ & $-0.41\pm0.11$ & main \\
HIP 70520 & $5825\pm60$ & $4.08\pm0.03$ & $-0.60\pm0.05$ & 1.31 &  & $-0.59\pm0.04$ & $-0.66\pm0.08$ & main \\
HIP 70681 & $5648\pm29$ & $4.66\pm0.04$ & $-1.09\pm0.04$ & 1.12 &  & $-1.09\pm0.04$ & $-1.08\pm0.08$ & main \\
HIP 71019 & $5338\pm65$ & $3.95\pm0.19$ & $-0.35\pm0.07$ & 1.06 &  & $-0.36\pm0.03$ & $-0.28\pm0.18$ & giant \\
HIP 71076 & $6080\pm63$ & $4.20\pm0.05$ & $-0.41\pm0.04$ & 1.17 &  & $-0.41\pm0.03$ & $-0.36\pm0.05$ & main \\
HIP 71193 & $5504\pm44$ & $4.28\pm0.04$ & $-0.08\pm0.04$ & 1.04 &  & $-0.09\pm0.02$ & $-0.04\pm0.07$ & main \\
HIP 71284 & $6745\pm73$ & $4.26\pm0.03$ & $-0.41\pm0.07$ & 2.08 &  & $-0.41\pm0.06$ & $-0.45\pm0.08$ & main \\
HIP 71572 & $5522\pm25$ & $4.34\pm0.04$ & $-0.17\pm0.11$ & 0.95 & + & $-0.17\pm0.12$ & $-0.17\pm0.07$ & main \\
HIP 71681 & $5230\pm79$ & $4.57\pm0.03$ & $0.27\pm0.06$ & 0.45 &  & $0.27\pm0.06$ & $0.24\pm0.11$ & main \\
HIP 71683 & $5809\pm80$ & $4.32\pm0.04$ & $0.23\pm0.05$ & 1.11 &  & $0.23\pm0.04$ & $0.24\pm0.10$ & main \\
HIP 71819 & $5812\pm68$ & $4.18\pm0.06$ & $-0.15\pm0.03$ & 1.16 &  & $-0.15\pm0.03$ & $-0.12\pm0.04$ & main \\
HIP 72199 & $5880\pm53$ & $3.89\pm0.07$ & $-0.11\pm0.05$ & 1.39 &  & $-0.11\pm0.04$ & $-0.13\pm0.10$ & main \\
HIP 72407 & $5694\pm44$ & $4.35\pm0.06$ & $-0.43\pm0.05$ & 0.93 &  & $-0.43\pm0.03$ & $-0.42\pm0.14$ & main \\
HIP 72467 & $6324\pm38$ & $3.96\pm0.04$ & $-0.17\pm0.10$ & 1.75 & + & $-0.18\pm0.09$ & $-0.11\pm0.15$ & main \\
HIP 72604 & $5679\pm58$ & $4.28\pm0.03$ & $-0.18\pm0.03$ & 1.08 &  & $-0.18\pm0.03$ & $-0.14\pm0.04$ & main \\
HIP 72659 & $5458\pm73$ & $4.54\pm0.03$ & $-0.15\pm0.05$ & 0.98 &  & $-0.16\pm0.03$ & $-0.11\pm0.09$ & main \\
HIP 72803 & $5262\pm48$ & $3.55\pm0.10$ & $-0.65\pm0.03$ & 1.11 &  & $-0.65\pm0.03$ & $-0.65\pm0.05$ & giant \\
HIP 72835 & $6260\pm47$ & $4.28\pm0.04$ & $-0.38\pm0.05$ & 1.26 &  & $-0.39\pm0.04$ & $-0.30\pm0.06$ & main \\
HIP 72848 & $5256\pm41$ & $4.51\pm0.03$ & $0.04\pm0.06$ & 0.95 &  & $0.04\pm0.05$ & $0.00\pm0.15$ & main \\
HIP 73005 & $5239\pm28$ & $4.54\pm0.02$ & $-0.40\pm0.05$ & 0.65 &  & $-0.40\pm0.04$ & $-0.41\pm0.11$ & main \\
HIP 73078 & $5378\pm63$ & $3.94\pm0.13$ & $0.05\pm0.04$ & 1.12 &  & $0.05\pm0.04$ & $0.07\pm0.09$ & giant \\
HIP 73385 & $5765\pm36$ & $3.81\pm0.05$ & $-1.44\pm0.09$ & 1.45 & + & $-1.43\pm0.08$ & $-1.50\pm0.11$ & main \\
HIP 73440 & $5744\pm26$ & $4.05\pm0.02$ & $-0.47\pm0.05$ & 1.34 &  & $-0.46\pm0.04$ & $-0.54\pm0.08$ & main \\
HIP 73695 & $5877\pm81$ & $4.33\pm0.05$ & $-0.24\pm0.04$ & 1.05 &  & $-0.23\pm0.03$ & $-0.27\pm0.08$ & main \\
HIP 73768 & $6007\pm83$ & $3.96\pm0.07$ & $-0.43\pm0.05$ & 1.39 &  & $-0.44\pm0.04$ & $-0.35\pm0.05$ & main \\
HIP 73815 & $5786\pm36$ & $4.27\pm0.04$ & $0.02\pm0.03$ & 1.13 &  & $0.02\pm0.02$ & $0.01\pm0.07$ & main \\
HIP 74033 & $5789\pm37$ & $4.02\pm0.06$ & $-0.75\pm0.06$ & 1.29 &  & $-0.74\pm0.05$ & $-0.85\pm0.07$ & main \\
HIP 74067 & $5777\pm34$ & $4.45\pm0.03$ & $-0.73\pm0.05$ & 1.28 &  & $-0.72\pm0.04$ & $-0.77\pm0.11$ & main \\
HIP 74079 & $5894\pm57$ & $4.05\pm0.04$ & $-0.79\pm0.06$ & 1.38 &  & $-0.79\pm0.05$ & $-0.79\pm0.10$ & main \\
HIP 74326 & $5704\pm34$ & $4.38\pm0.05$ & $-0.19\pm0.07$ & 1.17 &  & $-0.19\pm0.06$ & $-0.19\pm0.12$ & main \\
HIP 74341 & $5762\pm50$ & $4.42\pm0.07$ & $0.06\pm0.02$ & 0.95 &  & $0.06\pm0.02$ & $0.07\pm0.04$ & main \\
HIP 74442 & $5858\pm50$ & $4.11\pm0.06$ & $-0.08\pm0.06$ & 1.13 &  & $-0.08\pm0.03$ & $-0.08\pm0.15$ & main \\
HIP 74443 & $5248\pm22$ & $4.59\pm0.03$ & $-0.52\pm0.04$ & 0.73 &  & $-0.52\pm0.03$ & $-0.56\pm0.13$ & main \\
HIP 74933 & $5917\pm33$ & $4.16\pm0.08$ & $-0.32\pm0.06$ & 1.37 &  & $-0.32\pm0.04$ & $-0.36\pm0.14$ & main \\
HIP 75206 & $6284\pm71$ & $3.77\pm0.02$ & $-0.02\pm0.05$ & 2.00 &  & $-0.02\pm0.04$ & $-0.04\pm0.08$ & main \\
HIP 75281 & $5732\pm61$ & $4.32\pm0.05$ & $-0.29\pm0.04$ & 0.98 &  & $-0.29\pm0.03$ & $-0.27\pm0.07$ & main \\
HIP 75370 & $5543\pm28$ & $4.45\pm0.03$ & $-0.36\pm0.04$ & 0.95 &  & $-0.35\pm0.03$ & $-0.36\pm0.07$ & main \\
HIP 76219 & $4816\pm70$ & $3.05\pm0.19$ & $-0.05\pm0.06$ & 1.18 &  & $-0.05\pm0.04$ & $-0.03\pm0.15$ & giant \\
HIP 76543 & $6026\pm35$ & $4.11\pm0.03$ & $-0.49\pm0.05$ & 1.48 &  & $-0.49\pm0.04$ & $-0.44\pm0.09$ & main \\
HIP 76556 & $6085\pm51$ & $4.14\pm0.04$ & $-0.01\pm0.07$ & 1.46 &  & $-0.02\pm0.06$ & $0.06\pm0.09$ & main \\
HIP 76899 & $5775\pm40$ & $4.12\pm0.06$ & $-0.18\pm0.04$ & 1.37 &  & $-0.18\pm0.03$ & $-0.22\pm0.06$ & main \\
HIP 76911 & $5671\pm69$ & $4.39\pm0.06$ & $-0.21\pm0.03$ & 0.99 &  & $-0.22\pm0.02$ & $-0.19\pm0.06$ & main \\
HIP 76963 & $5913\pm41$ & $4.05\pm0.03$ & $-0.30\pm0.03$ & 1.27 &  & $-0.31\pm0.02$ & $-0.26\pm0.06$ & main \\
HIP 76976 & $5772\pm62$ & $3.68\pm0.04$ & $-2.30\pm0.12$ & 1.57 & + & $-2.32\pm0.10$ & $-2.28\pm0.12$ & main \\
HIP 77083 & $5747\pm44$ & $4.44\pm0.05$ & $0.02\pm0.05$ & 1.11 &  & $0.01\pm0.04$ & $0.09\pm0.07$ & main \\
HIP 77159 & $5721\pm33$ & $3.98\pm0.05$ & $-0.24\pm0.05$ & 1.15 &  & $-0.24\pm0.03$ & $-0.17\pm0.10$ & main \\
HIP 77257 & $5900\pm45$ & $4.17\pm0.03$ & $-0.01\pm0.04$ & 1.18 &  & $0.00\pm0.02$ & $-0.03\pm0.08$ & main \\
HIP 77358 & $5586\pm22$ & $4.45\pm0.02$ & $0.09\pm0.04$ & 0.84 &  & $0.09\pm0.03$ & $0.12\pm0.09$ & main \\
HIP 77466 & $5642\pm39$ & $4.37\pm0.05$ & $-0.28\pm0.07$ & 1.02 &  & $-0.29\pm0.06$ & $-0.24\pm0.09$ & main \\
HIP 77655 & $4848\pm85$ & $3.16\pm0.18$ & $0.10\pm0.06$ & 1.12 &  & $0.10\pm0.05$ & $0.09\pm0.11$ & giant \\
HIP 78028 & $5769\pm32$ & $4.46\pm0.04$ & $-0.09\pm0.05$ & 1.16 &  & $-0.10\pm0.04$ & $-0.03\pm0.07$ & main \\
HIP 78030 & $5636\pm36$ & $4.02\pm0.07$ & $0.28\pm0.05$ & 1.24 &  & $0.27\pm0.04$ & $0.34\pm0.08$ & main \\
HIP 78072 & $6313\pm67$ & $4.20\pm0.05$ & $-0.19\pm0.07$ & 1.79 &  & $-0.19\pm0.07$ & $-0.20\pm0.10$ & main \\
HIP 78640 & $6208\pm47$ & $4.32\pm0.10$ & $-1.26\pm0.10$ & 1.54 & + & $-1.24\pm0.09$ & $-1.32\pm0.12$ & main \\
HIP 78680 & $5823\pm61$ & $4.46\pm0.04$ & $-0.09\pm0.04$ & 1.27 &  & $-0.09\pm0.04$ & $-0.09\pm0.08$ & main \\
HIP 78747 & $6659\pm75$ & $4.08\pm0.04$ & $-0.39\pm0.17$ & 1.97 & + & $-0.41\pm0.16$ & $-0.29\pm0.20$ & main \\
HIP 78775 & $5321\pm44$ & $4.55\pm0.01$ & $-0.64\pm0.06$ & 0.73 &  & $-0.65\pm0.03$ & $-0.61\pm0.18$ & main \\
HIP 79186 & $5707\pm49$ & $4.29\pm0.04$ & $-0.10\pm0.03$ & 1.01 &  & $-0.10\pm0.02$ & $-0.09\pm0.08$ & main \\
HIP 79190 & $5090\pm32$ & $4.60\pm0.02$ & $-0.33\pm0.04$ & 0.30 &  & $-0.32\pm0.04$ & $-0.35\pm0.07$ & main \\
HIP 79276 & $5581\pm40$ & $4.39\pm0.03$ & $-0.15\pm0.04$ & 0.97 &  & $-0.16\pm0.03$ & $-0.12\pm0.08$ & main \\
HIP 79304 & $5827\pm39$ & $4.41\pm0.05$ & $0.09\pm0.02$ & 0.97 &  & $0.09\pm0.02$ & $0.10\pm0.05$ & main \\
HIP 79448 & $5535\pm27$ & $4.12\pm0.04$ & $-0.22\pm0.06$ & 1.18 &  & $-0.21\pm0.03$ & $-0.32\pm0.09$ & main \\
HIP 79545 & $5842\pm50$ & $4.11\pm0.05$ & $-0.63\pm0.05$ & 1.33 &  & $-0.64\pm0.04$ & $-0.56\pm0.07$ & main \\
HIP 79672 & $5789\pm46$ & $4.43\pm0.02$ & $0.02\pm0.04$ & 1.08 &  & $0.02\pm0.03$ & $0.02\pm0.06$ & main \\
HIP 79837 & $5684\pm60$ & $4.26\pm0.03$ & $-0.40\pm0.07$ & 1.15 &  & $-0.41\pm0.05$ & $-0.30\pm0.14$ & main \\
HIP 80162 & $5170\pm39$ & $4.61\pm0.03$ & $-0.56\pm0.05$ & 0.50 &  & $-0.57\pm0.04$ & $-0.42\pm0.09$ & main \\
HIP 80264 & $6071\pm41$ & $4.16\pm0.03$ & $-0.33\pm0.05$ & 1.37 &  & $-0.33\pm0.04$ & $-0.35\pm0.10$ & main \\
HIP 80337 & $5855\pm50$ & $4.50\pm0.02$ & $0.03\pm0.04$ & 1.14 &  & $0.03\pm0.04$ & $0.03\pm0.07$ & main \\
HIP 80686 & $6030\pm77$ & $4.43\pm0.03$ & $-0.08\pm0.04$ & 1.11 &  & $-0.08\pm0.04$ & $-0.05\pm0.08$ & main \\
HIP 80736 & $5656\pm37$ & $3.89\pm0.05$ & $0.22\pm0.06$ & 1.30 &  & $0.22\pm0.06$ & $0.20\pm0.09$ & main \\
HIP 80742 & $5783\pm40$ & $4.34\pm0.03$ & $-0.29\pm0.05$ & 1.19 &  & $-0.28\pm0.04$ & $-0.32\pm0.08$ & main \\
HIP 80818 & $5879\pm42$ & $3.96\pm0.02$ & $-0.20\pm0.05$ & 1.47 &  & $-0.20\pm0.04$ & $-0.20\pm0.11$ & main \\
HIP 80837 & $5925\pm33$ & $4.12\pm0.03$ & $-0.72\pm0.06$ & 1.35 &  & $-0.71\pm0.04$ & $-0.75\pm0.12$ & main \\
HIP 81072 & $6463\pm81$ & $4.07\pm0.06$ & $-0.23\pm0.09$ & 2.13 &  & $-0.22\pm0.07$ & $-0.31\pm0.16$ & main \\
HIP 81300 & $5248\pm38$ & $4.55\pm0.02$ & $0.01\pm0.07$ & 0.75 &  & $0.00\pm0.05$ & $0.06\pm0.15$ & main \\
HIP 81312 & $6060\pm45$ & $4.27\pm0.03$ & $-0.26\pm0.06$ & 1.43 &  & $-0.26\pm0.05$ & $-0.28\pm0.08$ & main \\
HIP 81461 & $5778\pm42$ & $4.16\pm0.06$ & $-0.43\pm0.07$ & 1.28 &  & $-0.41\pm0.06$ & $-0.54\pm0.10$ & main \\
HIP 81512 & $5755\pm32$ & $4.43\pm0.04$ & $-0.05\pm0.03$ & 1.08 &  & $-0.06\pm0.03$ & $-0.04\pm0.04$ & main \\
HIP 81608 & $6133\pm56$ & $3.86\pm0.04$ & $0.01\pm0.06$ & 1.74 &  & $0.00\pm0.05$ & $0.04\pm0.13$ & main \\
HIP 81681 & $5693\pm37$ & $4.36\pm0.03$ & $-0.36\pm0.04$ & 0.99 &  & $-0.36\pm0.04$ & $-0.37\pm0.09$ & main \\
HIP 81693 & $5766\pm60$ & $3.71\pm0.02$ & $0.02\pm0.04$ & 1.52 &  & $0.02\pm0.04$ & $-0.02\pm0.07$ & main \\
HIP 81748 & $5646\pm34$ & $4.28\pm0.04$ & $0.11\pm0.05$ & 1.00 &  & $0.11\pm0.03$ & $0.09\pm0.13$ & main \\
HIP 82265 & $5457\pm34$ & $4.41\pm0.04$ & $0.11\pm0.07$ & 0.73 &  & $0.11\pm0.05$ & $0.16\pm0.19$ & main \\
HIP 82268 & $5674\pm29$ & $4.41\pm0.04$ & $0.12\pm0.04$ & 0.92 &  & $0.12\pm0.03$ & $0.14\pm0.08$ & main \\
HIP 82621 & $5619\pm53$ & $3.98\pm0.03$ & $0.11\pm0.04$ & 1.13 &  & $0.10\pm0.03$ & $0.17\pm0.07$ & main \\
HIP 82629 & $6154\pm38$ & $4.15\pm0.05$ & $-0.03\pm0.04$ & 1.48 &  & $-0.04\pm0.03$ & $-0.01\pm0.07$ & main \\
HIP 82708 & $6166\pm48$ & $4.02\pm0.05$ & $0.18\pm0.05$ & 1.63 &  & $0.18\pm0.04$ & $0.17\pm0.09$ & main \\
HIP 82750 & $5696\pm27$ & $4.14\pm0.02$ & $0.04\pm0.03$ & 1.15 &  & $0.04\pm0.03$ & $0.04\pm0.03$ & main \\
HIP 82935 & $6113\pm44$ & $4.23\pm0.05$ & $-0.17\pm0.04$ & 1.42 &  & $-0.17\pm0.04$ & $-0.11\pm0.07$ & main \\
HIP 83058 & $6145\pm68$ & $4.32\pm0.07$ & $-0.09\pm0.07$ & 1.43 & + & $-0.10\pm0.07$ & $-0.01\pm0.08$ & main \\
HIP 83069 & $6110\pm51$ & $4.22\pm0.03$ & $-0.20\pm0.05$ & 1.45 &  & $-0.20\pm0.04$ & $-0.13\pm0.10$ & main \\
HIP 83204 & $5967\pm28$ & $4.27\pm0.02$ & $-0.31\pm0.03$ & 1.29 &  & $-0.31\pm0.03$ & $-0.28\pm0.06$ & main \\
HIP 83489 & $5731\pm35$ & $4.35\pm0.09$ & $-0.30\pm0.06$ & 1.28 &  & $-0.31\pm0.05$ & $-0.26\pm0.12$ & main \\
HIP 83601 & $6018\pm30$ & $4.38\pm0.02$ & $-0.03\pm0.04$ & 1.49 &  & $-0.03\pm0.04$ & $-0.01\pm0.07$ & main \\
HIP 84217 & $6208\pm41$ & $3.80\pm0.04$ & $-0.12\pm0.07$ & 1.79 &  & $-0.13\pm0.04$ & $0.04\pm0.08$ & main \\
HIP 84405 & $5087\pm44$ & $4.58\pm0.02$ & $-0.25\pm0.04$ & 0.66 &  & $-0.25\pm0.04$ & $-0.24\pm0.05$ & main \\
HIP 84478 & $4600\pm92$ & $4.70\pm0.23$ & $-0.34\pm0.07$ & 0.00 &  & $-0.34\pm0.07$ & $-0.34\pm0.04$ & manual \\
HIP 84506 & $5757\pm31$ & $4.01\pm0.06$ & $0.21\pm0.04$ & 1.32 &  & $0.21\pm0.04$ & $0.23\pm0.07$ & main \\
HIP 84551 & $6334\pm46$ & $3.75\pm0.02$ & $0.06\pm0.06$ & 1.97 &  & $0.06\pm0.05$ & $0.09\pm0.11$ & main \\
HIP 84696 & $6194\pm72$ & $4.15\pm0.05$ & $-0.10\pm0.06$ & 1.46 &  & $-0.09\pm0.04$ & $-0.14\pm0.14$ & main \\
HIP 84720 & $5273\pm60$ & $4.53\pm0.03$ & $-0.32\pm0.05$ & 0.66 &  & $-0.32\pm0.04$ & $-0.32\pm0.10$ & main \\
HIP 84781 & $5202\pm49$ & $3.79\pm0.10$ & $-0.27\pm0.05$ & 0.74 &  & $-0.28\pm0.04$ & $-0.13\pm0.05$ & giant \\
HIP 84803 & $5585\pm33$ & $3.86\pm0.08$ & $-0.47\pm0.07$ & 1.21 &  & $-0.47\pm0.04$ & $-0.46\pm0.16$ & main \\
HIP 84824 & $5901\pm33$ & $4.35\pm0.04$ & $-0.14\pm0.05$ & 1.25 &  & $-0.14\pm0.04$ & $-0.10\pm0.09$ & main \\
HIP 84862 & $5750\pm60$ & $4.26\pm0.03$ & $-0.39\pm0.04$ & 1.14 &  & $-0.38\pm0.04$ & $-0.45\pm0.09$ & main \\
HIP 85007 & $6020\pm51$ & $4.37\pm0.03$ & $-0.41\pm0.04$ & 1.23 &  & $-0.41\pm0.03$ & $-0.39\pm0.10$ & main \\
HIP 85042 & $5714\pm73$ & $4.41\pm0.04$ & $0.06\pm0.04$ & 0.94 &  & $0.06\pm0.03$ & $0.04\pm0.07$ & main \\
HIP 85090 & $5961\pm40$ & $3.87\pm0.06$ & $0.03\pm0.06$ & 1.78 &  & $0.03\pm0.05$ & $0.10\pm0.09$ & main \\
HIP 85235 & $5327\pm35$ & $4.56\pm0.02$ & $-0.42\pm0.06$ & 0.87 &  & $-0.43\pm0.03$ & $-0.40\pm0.17$ & main \\
HIP 85378 & $5782\pm32$ & $4.17\pm0.05$ & $-0.52\pm0.05$ & 1.27 &  & $-0.52\pm0.04$ & $-0.49\pm0.13$ & main \\
HIP 85400 & $5816\pm52$ & $4.09\pm0.06$ & $-0.36\pm0.05$ & 1.39 &  & $-0.36\pm0.04$ & $-0.38\pm0.11$ & main \\
HIP 85650 & $5763\pm32$ & $4.29\pm0.09$ & $-0.18\pm0.05$ & 1.13 &  & $-0.18\pm0.04$ & $-0.18\pm0.10$ & main \\
HIP 85653 & $5409\pm41$ & $4.45\pm0.02$ & $-0.38\pm0.05$ & 0.76 &  & $-0.37\pm0.03$ & $-0.42\pm0.13$ & main \\
HIP 85757 & $5681\pm32$ & $3.90\pm0.05$ & $-0.54\pm0.06$ & 1.28 &  & $-0.54\pm0.04$ & $-0.62\pm0.15$ & main \\
HIP 85940 & $5899\pm46$ & $3.89\pm0.04$ & $-0.18\pm0.08$ & 1.29 &  & $-0.20\pm0.05$ & $-0.06\pm0.14$ & main \\
HIP 85964 & $6127\pm78$ & $4.03\pm0.04$ & $-0.11\pm0.06$ & 1.58 &  & $-0.11\pm0.05$ & $-0.06\pm0.10$ & main \\
HIP 86013 & $5782\pm59$ & $4.37\pm0.05$ & $-0.74\pm0.05$ & 1.03 &  & $-0.74\pm0.04$ & $-0.71\pm0.11$ & main \\
HIP 86036 & $5885\pm63$ & $4.34\pm0.03$ & $-0.01\pm0.05$ & 1.14 &  & $-0.02\pm0.04$ & $0.01\pm0.09$ & main \\
HIP 86225 & $6180\pm36$ & $3.91\pm0.10$ & $-0.16\pm0.08$ & 1.71 &  & $-0.16\pm0.07$ & $-0.08\pm0.10$ & main \\
HIP 86321 & $6265\pm33$ & $4.34\pm0.11$ & $-0.77\pm0.09$ & 1.54 & + & $-0.77\pm0.08$ & $-0.74\pm0.21$ & main \\
HIP 86382 & $6242\pm75$ & $3.82\pm0.04$ & $-0.35\pm0.05$ & 1.75 &  & $-0.34\pm0.03$ & $-0.36\pm0.12$ & main \\
HIP 86400 & $4808\pm49$ & $4.56\pm0.01$ & $-0.08\pm0.08$ & 0.26 & + & $-0.09\pm0.07$ & $0.06\pm0.16$ & main \\
HIP 86431 & $5887\pm29$ & $4.36\pm0.04$ & $-0.48\pm0.05$ & 1.25 &  & $-0.48\pm0.03$ & $-0.51\pm0.13$ & main \\
HIP 86568 & $5335\pm33$ & $4.59\pm0.04$ & $-0.30\pm0.04$ & 0.31 &  & $-0.30\pm0.04$ & $-0.32\pm0.05$ & main \\
HIP 86796 & $5683\pm39$ & $4.20\pm0.02$ & $0.27\pm0.05$ & 1.01 &  & $0.26\pm0.03$ & $0.32\pm0.07$ & main \\
HIP 86830 & $5473\pm40$ & $3.97\pm0.06$ & $-0.44\pm0.04$ & 1.10 &  & $-0.44\pm0.04$ & $-0.50\pm0.10$ & main \\
HIP 86974 & $5485\pm68$ & $3.97\pm0.03$ & $0.22\pm0.07$ & 1.15 &  & $0.21\pm0.05$ & $0.31\pm0.12$ & main \\
HIP 87055 & $5688\pm26$ & $4.40\pm0.04$ & $-0.12\pm0.03$ & 1.04 &  & $-0.12\pm0.03$ & $-0.11\pm0.02$ & main \\
HIP 87089 & $5126\pm33$ & $4.56\pm0.02$ & $-0.35\pm0.06$ & 0.52 & + & $-0.36\pm0.04$ & $-0.24\pm0.14$ & main \\
HIP 87533 & $5817\pm35$ & $4.07\pm0.04$ & $-0.18\pm0.05$ & 1.23 &  & $-0.18\pm0.04$ & $-0.22\pm0.11$ & main \\
HIP 87732 & $5970\pm65$ & $3.89\pm0.05$ & $-0.04\pm0.08$ & 1.48 &  & $-0.04\pm0.05$ & $-0.04\pm0.18$ & main \\
HIP 88010 & $5562\pm60$ & $4.60\pm0.04$ & $-1.12\pm0.07$ & 0.77 &  & $-1.12\pm0.07$ & $-1.15\pm0.11$ & main \\
HIP 88039 & $5927\pm31$ & $3.99\pm0.09$ & $-0.70\pm0.07$ & 1.11 &  & $-0.70\pm0.05$ & $-0.70\pm0.18$ & main \\
HIP 88166 & $5474\pm35$ & $4.56\pm0.04$ & $-0.68\pm0.06$ & 0.85 &  & $-0.68\pm0.04$ & $-0.64\pm0.18$ & main \\
HIP 88194 & $5715\pm34$ & $4.38\pm0.02$ & $-0.11\pm0.03$ & 1.13 &  & $-0.11\pm0.03$ & $-0.11\pm0.07$ & main \\
HIP 88427 & $5803\pm38$ & $4.37\pm0.07$ & $-0.19\pm0.03$ & 1.15 &  & $-0.18\pm0.03$ & $-0.21\pm0.06$ & main \\
HIP 88601 & $5394\pm79$ & $4.56\pm0.03$ & $0.07\pm0.06$ & 0.91 &  & $0.06\pm0.04$ & $0.11\pm0.13$ & main \\
HIP 88745 & $6049\pm61$ & $4.18\pm0.03$ & $-0.58\pm0.05$ & 1.46 &  & $-0.58\pm0.04$ & $-0.59\pm0.08$ & main \\
HIP 88766 & $4860\pm97$ & $2.90\pm0.15$ & $-0.06\pm0.08$ & 1.70 &  & $-0.05\pm0.08$ & $-0.15\pm0.07$ & manual \\
HIP 88945 & $5795\pm33$ & $4.45\pm0.03$ & $0.02\pm0.12$ & 1.09 & + & $0.02\pm0.11$ & $0.00\pm0.16$ & main \\
HIP 88972 & $5048\pm34$ & $4.55\pm0.02$ & $-0.20\pm0.04$ & 0.33 &  & $-0.20\pm0.02$ & $-0.21\pm0.10$ & main \\
HIP 89268 & $5580\pm111$ & $4.50\pm0.23$ & $-0.24\pm0.04$ & 1.15 &  & $-0.24\pm0.04$ & $-0.24\pm0.07$ & manual \\
HIP 89408 & $5845\pm57$ & $3.92\pm0.02$ & $-0.39\pm0.06$ & 1.39 &  & $-0.40\pm0.04$ & $-0.33\pm0.13$ & main \\
HIP 89443 & $5691\pm36$ & $4.36\pm0.05$ & $-0.09\pm0.03$ & 1.06 &  & $-0.09\pm0.02$ & $-0.07\pm0.05$ & main \\
HIP 89474 & $5783\pm25$ & $4.31\pm0.01$ & $0.00\pm0.04$ & 1.16 &  & $-0.01\pm0.03$ & $0.04\pm0.08$ & main \\
HIP 89583 & $5513\pm31$ & $4.39\pm0.05$ & $-0.21\pm0.05$ & 0.76 &  & $-0.22\pm0.02$ & $-0.10\pm0.12$ & main \\
HIP 89937 & $6173\pm64$ & $4.22\pm0.03$ & $-0.58\pm0.08$ & 1.88 &  & $-0.56\pm0.06$ & $-0.72\pm0.11$ & main \\
HIP 90144 & $5916\pm41$ & $4.15\pm0.04$ & $-0.24\pm0.04$ & 1.24 &  & $-0.25\pm0.03$ & $-0.15\pm0.04$ & main \\
HIP 90539 & $5430\pm44$ & $4.46\pm0.04$ & $-0.17\pm0.06$ & 0.83 &  & $-0.18\pm0.01$ & $-0.11\pm0.14$ & main \\
HIP 90542 & $5554\pm47$ & $4.00\pm0.04$ & $-0.02\pm0.05$ & 1.05 &  & $-0.03\pm0.03$ & $0.04\pm0.10$ & main \\
HIP 90655 & $5832\pm34$ & $4.02\pm0.12$ & $0.14\pm0.06$ & 1.40 &  & $0.15\pm0.04$ & $0.09\pm0.09$ & main \\
HIP 90745 & $5840\pm39$ & $4.18\pm0.04$ & $-0.40\pm0.05$ & 1.19 &  & $-0.40\pm0.04$ & $-0.41\pm0.10$ & main \\
HIP 90790 & $5108\pm43$ & $4.61\pm0.02$ & $-0.16\pm0.05$ & 0.29 &  & $-0.15\pm0.04$ & $-0.19\pm0.14$ & main \\
HIP 90833 & $5746\pm31$ & $4.43\pm0.03$ & $-0.16\pm0.04$ & 0.93 &  & $-0.16\pm0.03$ & $-0.19\pm0.06$ & main \\
HIP 91058 & $6110\pm66$ & $4.26\pm0.04$ & $-0.46\pm0.06$ & 1.47 &  & $-0.46\pm0.05$ & $-0.44\pm0.12$ & main \\
HIP 91120 & $6356\pm50$ & $4.21\pm0.03$ & $-0.35\pm0.06$ & 1.66 & + & $-0.35\pm0.06$ & $-0.32\pm0.07$ & main \\
HIP 91395 & $5690\pm41$ & $4.09\pm0.03$ & $-0.31\pm0.05$ & 1.20 &  & $-0.31\pm0.04$ & $-0.37\pm0.09$ & main \\
HIP 91438 & $5651\pm35$ & $4.52\pm0.02$ & $-0.24\pm0.04$ & 1.06 &  & $-0.24\pm0.03$ & $-0.25\pm0.05$ & main \\
HIP 92270 & $6417\pm82$ & $4.36\pm0.03$ & $-0.01\pm0.05$ & 1.50 &  & $-0.01\pm0.03$ & $-0.06\pm0.10$ & main \\
HIP 92720 & $5772\pm56$ & $4.21\pm0.04$ & $0.09\pm0.03$ & 1.21 &  & $0.09\pm0.03$ & $0.11\pm0.05$ & main \\
HIP 93062 & $6156\pm37$ & $3.90\pm0.04$ & $-0.38\pm0.05$ & 1.72 &  & $-0.38\pm0.04$ & $-0.39\pm0.09$ & main \\
HIP 93269 & $5584\pm35$ & $4.32\pm0.05$ & $-0.23\pm0.05$ & 1.10 &  & $-0.23\pm0.03$ & $-0.26\pm0.11$ & main \\
HIP 93377 & $5551\pm51$ & $4.36\pm0.04$ & $-0.04\pm0.04$ & 0.93 &  & $-0.04\pm0.03$ & $-0.01\pm0.08$ & main \\
HIP 93827 & $5808\pm55$ & $4.16\pm0.03$ & $-0.67\pm0.06$ & 1.59 &  & $-0.67\pm0.05$ & $-0.67\pm0.10$ & main \\
HIP 94129 & $5695\pm33$ & $4.23\pm0.04$ & $-0.24\pm0.07$ & 0.88 &  & $-0.24\pm0.02$ & $-0.24\pm0.17$ & main \\
HIP 94449 & $6050\pm43$ & $4.02\pm0.14$ & $-0.92\pm0.08$ & 1.54 & + & $-0.91\pm0.07$ & $-1.04\pm0.12$ & main \\
HIP 94615 & $5533\pm67$ & $4.37\pm0.10$ & $0.09\pm0.06$ & 0.83 &  & $0.09\pm0.04$ & $0.11\pm0.14$ & main \\
HIP 94842 & $5533\pm54$ & $4.36\pm0.05$ & $-0.03\pm0.08$ & 1.03 &  & $-0.04\pm0.07$ & $0.01\pm0.10$ & main \\
HIP 95446 & $6039\pm67$ & $4.26\pm0.05$ & $-0.50\pm0.06$ & 1.47 &  & $-0.49\pm0.05$ & $-0.52\pm0.10$ & main \\
HIP 96049 & $5946\pm59$ & $3.99\pm0.04$ & $-0.80\pm0.06$ & 1.42 &  & $-0.80\pm0.06$ & $-0.79\pm0.06$ & main \\
HIP 96100 & $5331\pm66$ & $4.59\pm0.03$ & $-0.18\pm0.06$ & 0.60 &  & $-0.18\pm0.03$ & $-0.17\pm0.17$ & main \\
HIP 96142 & $5588\pm29$ & $4.36\pm0.10$ & $-0.27\pm0.06$ & 1.03 &  & $-0.27\pm0.03$ & $-0.29\pm0.14$ & main \\
HIP 96185 & $5804\pm28$ & $4.11\pm0.01$ & $-0.51\pm0.06$ & 1.20 &  & $-0.51\pm0.06$ & $-0.51\pm0.11$ & main \\
HIP 96901 & $5713\pm37$ & $4.31\pm0.02$ & $0.04\pm0.02$ & 1.06 &  & $0.04\pm0.02$ & $0.06\pm0.03$ & main \\
HIP 96902 & $5788\pm62$ & $3.99\pm0.07$ & $-0.27\pm0.06$ & 1.23 &  & $-0.25\pm0.02$ & $-0.40\pm0.07$ & main \\
HIP 96895 & $5787\pm32$ & $4.26\pm0.02$ & $0.05\pm0.04$ & 1.21 &  & $0.05\pm0.03$ & $0.05\pm0.08$ & main \\
HIP 97023 & $5899\pm41$ & $4.02\pm0.03$ & $-0.37\pm0.04$ & 1.40 &  & $-0.37\pm0.04$ & $-0.37\pm0.10$ & main \\
HIP 97420 & $5766\pm34$ & $4.43\pm0.02$ & $0.03\pm0.04$ & 0.97 &  & $0.03\pm0.03$ & $0.01\pm0.07$ & main \\
HIP 97846 & $5210\pm46$ & $3.83\pm0.09$ & $-0.18\pm0.04$ & 0.88 &  & $-0.19\pm0.03$ & $-0.08\pm0.04$ & giant \\
HIP 97918 & $5959\pm70$ & $4.11\pm0.04$ & $0.12\pm0.04$ & 1.39 &  & $0.12\pm0.03$ & $0.15\pm0.06$ & main \\
HIP 98020 & $5608\pm32$ & $4.62\pm0.03$ & $-1.41\pm0.05$ & 0.93 & + & $-1.40\pm0.05$ & $-1.47\pm0.03$ & main \\
HIP 98036 & $5062\pm57$ & $3.54\pm0.14$ & $-0.19\pm0.05$ & 0.97 &  & $-0.19\pm0.04$ & $-0.15\pm0.10$ & giant \\
HIP 98416 & $5931\pm57$ & $4.23\pm0.03$ & $-0.13\pm0.06$ & 1.35 &  & $-0.12\pm0.03$ & $-0.21\pm0.10$ & main \\
HIP 98532 & $5788\pm31$ & $3.88\pm0.04$ & $-1.08\pm0.06$ & 1.77 &  & $-1.07\pm0.04$ & $-1.16\pm0.11$ & main \\
HIP 98792 & $5038\pm43$ & $4.60\pm0.00$ & $-0.60\pm0.03$ & 0.38 &  & $-0.60\pm0.03$ & $-0.60\pm0.08$ & main \\
HIP 98819 & $5961\pm40$ & $4.42\pm0.02$ & $0.05\pm0.05$ & 1.06 &  & $0.05\pm0.02$ & $0.04\pm0.13$ & main \\
HIP 98921 & $5772\pm66$ & $4.44\pm0.03$ & $0.09\pm0.04$ & 1.30 &  & $0.09\pm0.03$ & $0.12\pm0.03$ & main \\
HIP 99025 & $6248\pm43$ & $4.08\pm0.07$ & $-0.03\pm0.04$ & 1.70 &  & $-0.03\pm0.04$ & $0.03\pm0.04$ & main \\
HIP 99224 & $5683\pm26$ & $4.17\pm0.04$ & $-0.09\pm0.06$ & 1.20 &  & $-0.09\pm0.03$ & $-0.05\pm0.17$ & main \\
HIP 99240 & $5517\pm60$ & $4.28\pm0.03$ & $0.33\pm0.07$ & 0.88 &  & $0.32\pm0.05$ & $0.40\pm0.10$ & main \\
HIP 99241 & $6081\pm64$ & $4.26\pm0.03$ & $-0.20\pm0.06$ & 1.46 &  & $-0.20\pm0.04$ & $-0.25\pm0.12$ & main \\
HIP 99386 & $6054\pm45$ & $4.12\pm0.04$ & $-0.45\pm0.05$ & 1.45 &  & $-0.45\pm0.04$ & $-0.49\pm0.09$ & main \\
HIP 99461 & $4969\pm66$ & $4.62\pm0.02$ & $-0.52\pm0.05$ & 0.38 & + & $-0.52\pm0.05$ & $-0.52\pm0.08$ & main \\
HIP 99607 & $6021\pm48$ & $4.00\pm0.05$ & $-0.31\pm0.06$ & 1.36 &  & $-0.33\pm0.04$ & $-0.19\pm0.06$ & main \\
HIP 99825 & $5104\pm43$ & $4.54\pm0.03$ & $0.06\pm0.06$ & 0.15 &  & $0.06\pm0.04$ & $0.05\pm0.15$ & main \\
HIP 100017 & $5915\pm61$ & $4.43\pm0.03$ & $-0.13\pm0.04$ & 1.16 &  & $-0.12\pm0.02$ & $-0.15\pm0.10$ & main \\
HIP 100568 & $5859\pm54$ & $4.60\pm0.04$ & $-0.94\pm0.09$ & 1.11 & + & $-0.95\pm0.07$ & $-0.88\pm0.19$ & main \\
HIP 100783 & $6198\pm45$ & $3.78\pm0.04$ & $-0.43\pm0.06$ & 1.89 &  & $-0.43\pm0.05$ & $-0.39\pm0.10$ & main \\
HIP 100963 & $5804\pm43$ & $4.44\pm0.03$ & $-0.04\pm0.03$ & 1.17 &  & $-0.03\pm0.02$ & $-0.06\pm0.07$ & main \\
HIP 100970 & $5642\pm53$ & $4.05\pm0.04$ & $-0.03\pm0.05$ & 1.22 &  & $-0.04\pm0.03$ & $0.04\pm0.07$ & main \\
HIP 101136 & $6127\pm53$ & $4.23\pm0.03$ & $-0.17\pm0.04$ & 1.39 &  & $-0.17\pm0.04$ & $-0.16\pm0.06$ & main \\
HIP 102081 & $5579\pm63$ & $4.25\pm0.05$ & $0.09\pm0.07$ & 0.89 &  & $0.07\pm0.04$ & $0.29\pm0.06$ & main \\
HIP 102152 & $5719\pm25$ & $4.36\pm0.07$ & $-0.02\pm0.02$ & 1.09 &  & $-0.02\pm0.02$ & $-0.03\pm0.05$ & main \\
HIP 102379 & $5990\pm35$ & $4.11\pm0.05$ & $-0.50\pm0.04$ & 1.56 &  & $-0.50\pm0.04$ & $-0.47\pm0.06$ & main \\
HIP 102422 & $4933\pm53$ & $3.28\pm0.13$ & $-0.16\pm0.05$ & 1.02 &  & $-0.16\pm0.04$ & $-0.10\pm0.08$ & giant \\
HIP 102610 & $5807\pm31$ & $4.25\pm0.03$ & $-0.28\pm0.04$ & 1.21 &  & $-0.29\pm0.03$ & $-0.23\pm0.04$ & main \\
HIP 102611 & $6196\pm38$ & $4.18\pm0.04$ & $-0.48\pm0.05$ & 1.46 &  & $-0.48\pm0.04$ & $-0.48\pm0.10$ & main \\
HIP 102762 & $5934\pm32$ & $4.29\pm0.05$ & $-0.11\pm0.06$ & 1.49 &  & $-0.10\pm0.04$ & $-0.15\pm0.13$ & main \\
HIP 102805 & $6431\pm50$ & $4.20\pm0.03$ & $-0.32\pm0.05$ & 1.80 &  & $-0.33\pm0.05$ & $-0.30\pm0.08$ & main \\
HIP 103237 & $6331\pm47$ & $4.18\pm0.05$ & $-0.23\pm0.08$ & 1.99 &  & $-0.23\pm0.07$ & $-0.24\pm0.15$ & main \\
HIP 103987 & $5827\pm60$ & $3.98\pm0.04$ & $-0.63\pm0.05$ & 1.28 &  & $-0.63\pm0.05$ & $-0.71\pm0.06$ & main \\
HIP 104347 & $6003\pm58$ & $3.79\pm0.07$ & $-0.59\pm0.07$ & 1.27 &  & $-0.61\pm0.04$ & $-0.46\pm0.10$ & main \\
HIP 104421 & $6070\pm74$ & $4.10\pm0.06$ & $-0.25\pm0.06$ & 1.60 &  & $-0.25\pm0.04$ & $-0.27\pm0.15$ & main \\
HIP 104504 & $5822\pm27$ & $4.52\pm0.03$ & $-0.17\pm0.03$ & 1.16 &  & $-0.17\pm0.03$ & $-0.17\pm0.05$ & main \\
HIP 104514 & $6132\pm48$ & $4.25\pm0.05$ & $-0.50\pm0.06$ & 1.23 &  & $-0.51\pm0.04$ & $-0.40\pm0.06$ & main \\
HIP 104520 & $6249\pm50$ & $4.14\pm0.04$ & $-0.40\pm0.05$ & 1.67 &  & $-0.40\pm0.05$ & $-0.36\pm0.08$ & main \\
HIP 104659 & $5985\pm37$ & $4.32\pm0.03$ & $-1.01\pm0.08$ & 1.47 & + & $-1.00\pm0.08$ & $-1.08\pm0.05$ & main \\
HIP 104660 & $5696\pm46$ & $4.08\pm0.05$ & $-0.79\pm0.05$ & 1.05 &  & $-0.78\pm0.04$ & $-0.80\pm0.09$ & main \\
HIP 105202 & $6285\pm45$ & $4.39\pm0.03$ & $-0.24\pm0.06$ & 1.62 &  & $-0.23\pm0.03$ & $-0.27\pm0.14$ & main \\
HIP 105481 & $5861\pm32$ & $4.00\pm0.03$ & $0.05\pm0.03$ & 1.48 &  & $0.05\pm0.03$ & $0.07\pm0.05$ & main \\
HIP 105766 & $5699\pm32$ & $4.42\pm0.01$ & $-0.75\pm0.05$ & 1.18 &  & $-0.75\pm0.04$ & $-0.80\pm0.06$ & main \\
HIP 105857 & $6026\pm32$ & $4.06\pm0.05$ & $-0.59\pm0.05$ & 1.23 &  & $-0.60\pm0.04$ & $-0.51\pm0.06$ & main \\
HIP 105858 & $6150\pm55$ & $4.35\pm0.03$ & $-0.66\pm0.05$ & 1.47 &  & $-0.66\pm0.05$ & $-0.69\pm0.04$ & main \\
HIP 105969 & $5833\pm67$ & $4.14\pm0.08$ & $-0.32\pm0.06$ & 1.29 & + & $-0.33\pm0.05$ & $-0.28\pm0.09$ & main \\
HIP 106040 & $6117\pm27$ & $4.18\pm0.05$ & $-0.36\pm0.06$ & 1.51 &  & $-0.35\pm0.04$ & $-0.41\pm0.11$ & main \\
HIP 106122 & $5426\pm23$ & $4.53\pm0.02$ & $-0.17\pm0.03$ & 0.71 &  & $-0.17\pm0.02$ & $-0.18\pm0.07$ & main \\
HIP 106157 & $6004\pm42$ & $3.99\pm0.04$ & $-0.45\pm0.04$ & 1.47 &  & $-0.45\pm0.04$ & $-0.42\pm0.05$ & main \\
HIP 106678 & $5644\pm43$ & $4.14\pm0.06$ & $0.01\pm0.04$ & 1.26 &  & $0.01\pm0.02$ & $0.02\pm0.07$ & main \\
HIP 106947 & $5334\pm39$ & $4.54\pm0.04$ & $-0.39\pm0.04$ & 0.71 &  & $-0.39\pm0.04$ & $-0.36\pm0.10$ & main \\
HIP 107236 & $5430\pm108$ & $4.30\pm0.22$ & $-0.42\pm0.06$ & 0.90 &  & $-0.42\pm0.04$ & $-0.41\pm0.16$ & manual \\
HIP 107294 & $6147\pm40$ & $4.46\pm0.12$ & $-1.15\pm0.06$ & 1.41 & + & $-1.14\pm0.06$ & $-1.18\pm0.10$ & main \\
HIP 107350 & $5961\pm85$ & $4.45\pm0.03$ & $-0.06\pm0.07$ & 1.35 & + & $-0.06\pm0.05$ & $-0.06\pm0.13$ & main \\
HIP 107975 & $6407\pm47$ & $4.10\pm0.02$ & $-0.56\pm0.05$ & 1.77 & + & $-0.56\pm0.04$ & $-0.54\pm0.07$ & main \\
HIP 108056 & $6102\pm42$ & $4.41\pm0.04$ & $0.18\pm0.06$ & 1.26 &  & $0.18\pm0.04$ & $0.19\pm0.14$ & main \\
HIP 108490 & $6049\pm41$ & $4.39\pm0.03$ & $-0.71\pm0.04$ & 1.39 &  & $-0.71\pm0.04$ & $-0.73\pm0.06$ & main \\
HIP 108514 & $6132\pm44$ & $3.59\pm0.13$ & $-0.18\pm0.11$ & 1.83 &  & $-0.20\pm0.07$ & $-0.10\pm0.23$ & main \\
HIP 108708 & $5819\pm35$ & $4.42\pm0.06$ & $0.09\pm0.04$ & 1.35 &  & $0.10\pm0.03$ & $0.05\pm0.05$ & main \\
HIP 108767 & $6080\pm50$ & $4.26\pm0.06$ & $-0.12\pm0.05$ & 1.42 &  & $-0.13\pm0.03$ & $-0.04\pm0.07$ & main \\
HIP 108870 & $4649\pm36$ & $4.63\pm0.01$ & $-0.19\pm0.07$ & 0.11 & + & $-0.20\pm0.06$ & $-0.12\pm0.11$ & main \\
HIP 108996 & $5778\pm35$ & $4.50\pm0.04$ & $0.02\pm0.03$ & 1.18 &  & $0.02\pm0.03$ & $0.03\pm0.03$ & main \\
HIP 109067 & $5486\pm38$ & $4.63\pm0.04$ & $-0.79\pm0.04$ & 0.58 &  & $-0.79\pm0.02$ & $-0.75\pm0.11$ & main \\
HIP 109090 & $5994\pm60$ & $4.22\pm0.05$ & $-0.23\pm0.04$ & 1.24 &  & $-0.24\pm0.03$ & $-0.17\pm0.04$ & main \\
HIP 109176 & $6495\pm67$ & $4.20\pm0.02$ & $-0.16\pm0.08$ & 1.45 &  & $-0.18\pm0.07$ & $-0.02\pm0.06$ & main \\
HIP 109310 & $5865\pm41$ & $4.50\pm0.04$ & $-0.09\pm0.04$ & 0.94 &  & $-0.09\pm0.03$ & $-0.05\pm0.06$ & main \\
HIP 109324 & $6352\pm48$ & $4.03\pm0.04$ & $-0.37\pm0.06$ & 1.65 &  & $-0.37\pm0.06$ & $-0.35\pm0.11$ & main \\
HIP 109372 & $6246\pm28$ & $4.14\pm0.04$ & $-0.26\pm0.04$ & 1.69 &  & $-0.27\pm0.04$ & $-0.22\pm0.06$ & main \\
HIP 109384 & $5274\pm31$ & $4.56\pm0.04$ & $-0.23\pm0.05$ & 0.42 &  & $-0.24\pm0.04$ & $-0.20\pm0.13$ & main \\
HIP 109450 & $5834\pm56$ & $4.17\pm0.04$ & $-0.12\pm0.04$ & 1.24 &  & $-0.12\pm0.03$ & $-0.08\pm0.06$ & main \\
HIP 109498 & $5840\pm116$ & $4.20\pm0.21$ & $-0.11\pm0.04$ & 1.15 &  & $-0.11\pm0.03$ & $-0.15\pm0.07$ & manual \\
HIP 109608 & $6137\pm41$ & $3.87\pm0.11$ & $-0.28\pm0.06$ & 1.45 &  & $-0.28\pm0.05$ & $-0.33\pm0.06$ & main \\
HIP 109677 & $6041\pm38$ & $3.95\pm0.03$ & $-0.20\pm0.05$ & 1.50 &  & $-0.21\pm0.04$ & $-0.13\pm0.06$ & main \\
HIP 109771 & $6077\pm53$ & $4.09\pm0.06$ & $-0.62\pm0.07$ & 1.52 &  & $-0.62\pm0.06$ & $-0.60\pm0.10$ & main \\
HIP 109881 & $6004\pm45$ & $4.00\pm0.04$ & $0.12\pm0.05$ & 1.47 &  & $0.12\pm0.04$ & $0.17\pm0.07$ & main \\
HIP 109931 & $5740\pm29$ & $4.37\pm0.05$ & $0.06\pm0.02$ & 1.01 &  & $0.06\pm0.02$ & $0.07\pm0.05$ & main \\
HIP 109951 & $5630\pm112$ & $4.40\pm0.22$ & $-0.33\pm0.07$ & 0.90 &  & $-0.33\pm0.06$ & $-0.33\pm0.12$ & manual \\
HIP 110016 & $6023\pm68$ & $4.03\pm0.07$ & $-0.29\pm0.05$ & 1.17 &  & $-0.30\pm0.05$ & $-0.28\pm0.08$ & main \\
HIP 110035 & $5830\pm36$ & $4.33\pm0.03$ & $-0.19\pm0.07$ & 1.37 &  & $-0.19\pm0.06$ & $-0.22\pm0.12$ & main \\
HIP 110109 & $5783\pm72$ & $4.34\pm0.04$ & $-0.25\pm0.05$ & 1.03 &  & $-0.26\pm0.05$ & $-0.22\pm0.08$ & main \\
HIP 110187 & $6007\pm48$ & $4.36\pm0.08$ & $0.10\pm0.04$ & 1.26 &  & $0.11\pm0.04$ & $0.06\pm0.06$ & main \\
HIP 110291 & $5944\pm60$ & $4.32\pm0.05$ & $-0.94\pm0.06$ & 1.31 & + & $-0.95\pm0.06$ & $-0.89\pm0.10$ & main \\
HIP 110785 & $6224\pm32$ & $3.94\pm0.03$ & $-0.01\pm0.06$ & 1.72 &  & $-0.01\pm0.04$ & $-0.04\pm0.12$ & main \\
HIP 110788 & $5989\pm58$ & $4.28\pm0.04$ & $-0.37\pm0.05$ & 1.26 &  & $-0.36\pm0.04$ & $-0.40\pm0.10$ & main \\
HIP 111050 & $5569\pm33$ & $4.36\pm0.06$ & $-0.26\pm0.06$ & 0.79 &  & $-0.27\pm0.04$ & $-0.19\pm0.10$ & main \\
HIP 111352 & $5750\pm50$ & $3.59\pm0.07$ & $-0.16\pm0.06$ & 1.49 &  & $-0.15\pm0.04$ & $-0.20\pm0.13$ & main \\
HIP 111431 & $6148\pm74$ & $3.69\pm0.08$ & $-0.05\pm0.06$ & 1.64 &  & $-0.05\pm0.05$ & $-0.10\pm0.10$ & main \\
HIP 111517 & $5584\pm45$ & $3.86\pm0.06$ & $-0.35\pm0.04$ & 1.30 &  & $-0.35\pm0.03$ & $-0.36\pm0.11$ & main \\
HIP 111549 & $5770\pm115$ & $4.50\pm0.23$ & $-0.99\pm0.08$ & 0.90 &  & $-0.99\pm0.08$ & $-1.00\pm0.12$ & manual \\
HIP 111723 & $6006\pm68$ & $4.41\pm0.04$ & $-0.25\pm0.04$ & 1.16 &  & $-0.26\pm0.04$ & $-0.20\pm0.06$ & main \\
HIP 111748 & $6087\pm34$ & $4.09\pm0.03$ & $0.07\pm0.07$ & 1.33 &  & $0.08\pm0.04$ & $0.02\pm0.17$ & main \\
HIP 111796 & $6441\pm40$ & $4.06\pm0.07$ & $-0.52\pm0.07$ & 1.72 &  & $-0.53\pm0.05$ & $-0.49\pm0.17$ & main \\
HIP 111977 & $5734\pm33$ & $4.45\pm0.03$ & $-0.47\pm0.06$ & 1.43 &  & $-0.47\pm0.02$ & $-0.54\pm0.13$ & main \\
HIP 112263 & $6009\pm45$ & $3.93\pm0.04$ & $-0.15\pm0.06$ & 1.54 &  & $-0.15\pm0.05$ & $-0.11\pm0.13$ & main \\
HIP 112595 & $5662\pm39$ & $4.34\pm0.04$ & $-0.17\pm0.04$ & 0.99 &  & $-0.18\pm0.03$ & $-0.10\pm0.06$ & main \\
HIP 112666 & $5270\pm43$ & $4.52\pm0.04$ & $-0.36\pm0.07$ & 0.66 & + & $-0.37\pm0.04$ & $-0.26\pm0.14$ & main \\
HIP 112697 & $5968\pm32$ & $3.77\pm0.02$ & $-0.33\pm0.06$ & 1.72 &  & $-0.33\pm0.05$ & $-0.33\pm0.14$ & main \\
HIP 112811 & $5481\pm33$ & $4.53\pm0.03$ & $-0.68\pm0.05$ & 0.86 &  & $-0.68\pm0.03$ & $-0.75\pm0.13$ & main \\
HIP 112935 & $6292\pm50$ & $3.99\pm0.03$ & $-0.22\pm0.06$ & 1.59 &  & $-0.22\pm0.04$ & $-0.22\pm0.12$ & main \\
HIP 113044 & $5962\pm89$ & $4.06\pm0.03$ & $0.19\pm0.04$ & 1.39 &  & $0.19\pm0.03$ & $0.17\pm0.08$ & main \\
HIP 113076 & $6117\pm67$ & $4.41\pm0.04$ & $-0.42\pm0.06$ & 1.40 &  & $-0.42\pm0.04$ & $-0.44\pm0.12$ & main \\
HIP 113357 & $5752\pm31$ & $4.32\pm0.02$ & $0.19\pm0.04$ & 1.04 &  & $0.19\pm0.03$ & $0.24\pm0.05$ & main \\
HIP 113514 & $5780\pm32$ & $4.39\pm0.05$ & $-0.59\pm0.05$ & 1.04 &  & $-0.59\pm0.05$ & $-0.58\pm0.09$ & main \\
HIP 113896 & $6021\pm57$ & $4.35\pm0.03$ & $-0.10\pm0.05$ & 1.26 &  & $-0.10\pm0.03$ & $-0.17\pm0.10$ & main \\
HIP 113980 & $6356\pm64$ & $4.29\pm0.04$ & $-0.30\pm0.06$ & 1.49 &  & $-0.30\pm0.04$ & $-0.30\pm0.13$ & main \\
HIP 114034 & $5965\pm46$ & $3.85\pm0.03$ & $-0.21\pm0.05$ & 1.58 &  & $-0.22\pm0.04$ & $-0.14\pm0.07$ & main \\
HIP 114210 & $6605\pm61$ & $4.12\pm0.02$ & $-0.09\pm0.05$ & 1.93 &  & $-0.09\pm0.04$ & $-0.07\pm0.11$ & main \\
HIP 114354 & $6053\pm44$ & $4.06\pm0.06$ & $-0.27\pm0.04$ & 1.45 &  & $-0.26\pm0.04$ & $-0.30\pm0.06$ & main \\
HIP 114622 & $4833\pm60$ & $4.59\pm0.02$ & $0.00\pm0.06$ & 0.26 & + & $0.00\pm0.06$ & $-0.01\pm0.11$ & main \\
HIP 114729 & $6099\pm49$ & $4.06\pm0.04$ & $-0.27\pm0.04$ & 1.48 &  & $-0.27\pm0.04$ & $-0.23\pm0.06$ & main \\
HIP 114838 & $5920\pm64$ & $3.81\pm0.04$ & $-0.59\pm0.05$ & 1.54 &  & $-0.60\pm0.03$ & $-0.49\pm0.08$ & main \\
HIP 114856 & $5912\pm53$ & $3.82\pm0.05$ & $-0.50\pm0.08$ & 1.51 & + & $-0.51\pm0.06$ & $-0.36\pm0.07$ & main \\
HIP 114893 & $5974\pm48$ & $4.12\pm0.07$ & $-0.38\pm0.08$ & 1.24 &  & $-0.39\pm0.07$ & $-0.26\pm0.07$ & main \\
HIP 114962 & $6087\pm47$ & $4.10\pm0.10$ & $-1.29\pm0.12$ & 1.55 & + & $-1.30\pm0.09$ & $-1.24\pm0.23$ & main \\
HIP 115012 & $5649\pm26$ & $4.02\pm0.05$ & $-0.02\pm0.05$ & 1.20 &  & $-0.02\pm0.05$ & $-0.07\pm0.06$ & main \\
HIP 115066 & $5636\pm32$ & $4.38\pm0.05$ & $0.11\pm0.05$ & 1.04 &  & $0.10\pm0.04$ & $0.14\pm0.09$ & main \\
HIP 115220 & $6172\pm54$ & $3.98\pm0.03$ & $-0.20\pm0.07$ & 1.61 &  & $-0.19\pm0.05$ & $-0.25\pm0.14$ & main \\
HIP 115359 & $5664\pm60$ & $4.41\pm0.07$ & $-0.56\pm0.06$ & 1.15 &  & $-0.56\pm0.04$ & $-0.54\pm0.13$ & main \\
HIP 115370 & $5896\pm52$ & $4.29\pm0.04$ & $-0.02\pm0.04$ & 1.23 &  & $-0.03\pm0.03$ & $0.05\pm0.07$ & main \\
HIP 115604 & $5760\pm49$ & $4.30\pm0.06$ & $0.12\pm0.02$ & 1.10 &  & $0.12\pm0.01$ & $0.11\pm0.04$ & main \\
HIP 115704 & $5780\pm115$ & $4.30\pm0.22$ & $-1.86\pm0.23$ & 1.00 &  & $-1.99\pm0.06$ & $-1.78\pm0.27$ & manual \\
HIP 115714 & $5941\pm49$ & $4.19\pm0.04$ & $-0.20\pm0.05$ & 1.34 &  & $-0.20\pm0.04$ & $-0.21\pm0.10$ & main \\
HIP 115721 & $5761\pm45$ & $4.04\pm0.06$ & $-0.37\pm0.05$ & 1.13 &  & $-0.37\pm0.04$ & $-0.41\pm0.13$ & main \\
HIP 115761 & $6103\pm48$ & $3.82\pm0.06$ & $-0.14\pm0.06$ & 1.70 &  & $-0.13\pm0.04$ & $-0.21\pm0.10$ & main \\
HIP 116106 & $6120\pm55$ & $4.39\pm0.03$ & $-0.25\pm0.06$ & 1.34 &  & $-0.23\pm0.03$ & $-0.33\pm0.11$ & main \\
HIP 116421 & $5776\pm59$ & $4.15\pm0.03$ & $-0.41\pm0.06$ & 1.18 &  & $-0.41\pm0.03$ & $-0.44\pm0.15$ & main \\
HIP 116478 & $5586\pm40$ & $4.32\pm0.06$ & $-0.02\pm0.04$ & 0.92 &  & $-0.03\pm0.02$ & $0.00\pm0.09$ & main \\
HIP 116616 & $5699\pm25$ & $3.97\pm0.02$ & $-0.18\pm0.04$ & 1.24 &  & $-0.17\pm0.02$ & $-0.21\pm0.11$ & main \\
HIP 116727 & $4803\pm99$ & $3.08\pm0.20$ & $0.05\pm0.07$ & 1.24 &  & $0.05\pm0.07$ & $-0.01\pm0.10$ & giant \\
HIP 116771 & $6211\pm52$ & $4.11\pm0.02$ & $-0.12\pm0.04$ & 1.52 &  & $-0.12\pm0.04$ & $-0.13\pm0.06$ & main \\
HIP 117029 & $5594\pm43$ & $3.91\pm0.02$ & $-0.68\pm0.05$ & 1.20 &  & $-0.69\pm0.05$ & $-0.66\pm0.10$ & main \\
HIP 117484 & $6205\pm49$ & $3.99\pm0.06$ & $-0.03\pm0.06$ & 1.65 &  & $-0.02\pm0.06$ & $-0.08\pm0.09$ & main \\
HIP 117582 & $5969\pm78$ & $4.16\pm0.06$ & $-0.45\pm0.04$ & 1.29 &  & $-0.45\pm0.03$ & $-0.43\pm0.05$ & main \\
HIP 117762 & $6040\pm64$ & $3.87\pm0.03$ & $-0.24\pm0.06$ & 1.69 &  & $-0.23\pm0.05$ & $-0.28\pm0.10$ & main \\
HIP 117776 & $6095\pm39$ & $4.00\pm0.05$ & $-0.56\pm0.06$ & 1.57 &  & $-0.57\pm0.04$ & $-0.51\pm0.14$ & main \\
HIP 118010 & $5757\pm36$ & $4.15\pm0.03$ & $-0.12\pm0.05$ & 1.18 &  & $-0.12\pm0.03$ & $-0.17\pm0.12$ & main \\
HIP 118115 & $5836\pm63$ & $4.31\pm0.05$ & $0.00\pm0.03$ & 1.15 &  & $0.00\pm0.03$ & $-0.01\pm0.04$ & main \\
HIP 118159 & $5838\pm41$ & $4.43\pm0.06$ & $-0.06\pm0.04$ & 1.11 &  & $-0.06\pm0.02$ & $-0.10\pm0.08$ & main \\
HIP 118162 & $5819\pm46$ & $4.41\pm0.03$ & $0.10\pm0.04$ & 1.05 &  & $0.11\pm0.03$ & $0.04\pm0.07$ & main \\
HIP 118225 & $5760\pm35$ & $4.12\pm0.03$ & $0.11\pm0.04$ & 1.19 &  & $0.10\pm0.03$ & $0.17\pm0.06$ & main \\


==> t5_complete.tex <==
  HD 32071& 9.09& 7.12& 9.68& 3.92&10.75  & 0.942& 0.929& 0.992& 0.906& 1.054\\
  HD 59490& 6.43& 3.44&10.64& 1.15&12.89  & 0.918& 0.895& 0.936& 0.877& 0.956\\
  HD 67163& 7.31& 5.64& 7.74& 3.31& 8.46  & 1.032& 1.016& 1.062& 1.000& 1.096\\
  HD 82960& 2.01& 1.71& 2.89& 1.06& 3.84  & 1.313& 1.313& 1.692& 1.215& 1.873\\
 HD 130047&11.65& 7.10&12.17& 2.88&13.39  & 0.936& 0.914& 0.957& 0.898& 0.993\\
 HD 144070& 2.14& 1.73& 2.55& 1.12& 3.00  & 1.384& 1.334& 1.453& 1.283& 1.520\\
 HD 170058& 5.22& 4.01& 6.29& 1.81& 7.20  & 1.102& 1.078& 1.195& 1.037& 1.281\\
 HD 171029& 6.89& 4.37&12.53& 2.24&14.36  & 0.940& 0.906& 1.242& 0.851& 1.535\\
 HD 183490& 3.90& 3.24& 6.60& 2.21& 8.36  & 1.242& 1.139& 1.446& 1.052& 1.637\\
 HD 213746& 7.16& 5.04& 8.03& 2.65& 9.20  & 1.058& 1.013& 1.158& 0.982& 1.323\\
 HD 223723& 5.70& 3.96& 6.22& 1.83& 7.04  & 1.078& 1.053& 1.119& 1.031& 1.169\\
   HIP 171&14.46&12.65&14.56&10.92&14.78  & 0.759& 0.751& 0.771& 0.744& 0.787\\
   HIP 348& 8.67& 5.28&10.20& 2.63&12.19  & 0.930& 0.913& 0.963& 0.891& 0.993\\
   HIP 394& 5.00& 3.93& 7.22& 3.01& 9.34  & 1.132& 1.053& 1.257& 0.977& 1.369\\
   HIP 475& 8.75& 7.09&11.47& 4.45&13.32  & 0.923& 0.891& 0.954& 0.863& 0.989\\
   HIP 493& 5.39& 3.21& 6.06& 1.78& 7.21  & 1.004& 0.986& 1.034& 0.966& 1.057\\
   HIP 522& 3.00& 2.70& 3.40& 2.37& 3.63  & 1.244& 1.232& 1.258& 1.222& 1.274\\
   HIP 530& 4.90& 4.40& 5.60& 3.85& 6.16  & 1.222& 1.184& 1.284& 1.142& 1.333\\
   HIP 544& 3.51& 1.59& 6.23& 0.46& 8.80  & 0.950& 0.919& 0.976& 0.892& 0.995\\
   HIP 656& 4.19& 3.51& 5.39& 2.90& 6.51  & 1.254& 1.178& 1.346& 1.109& 1.429\\
   HIP 768& 7.89& 7.23& 8.81& 6.51& 9.60  & 1.077& 1.047& 1.113& 1.018& 1.149\\
   HIP 950& 2.13& 1.44& 2.67& 0.69& 3.17  & 1.246& 1.232& 1.273& 1.216& 1.302\\
   HIP 996& 7.14& 6.21& 8.21& 4.57& 9.11  & 0.993& 0.983& 1.012& 0.968& 1.027\\
  HIP 1105& 4.55& 4.07& 4.97& 3.68& 5.39  & 1.229& 1.189& 1.268& 1.156& 1.314\\
  HIP 1128&13.15& 9.52&13.89& 6.32&14.53  & 0.778& 0.772& 0.816& 0.759& 0.845\\
  HIP 1297& 9.75& 6.91&10.75& 4.16&12.27  & 0.950& 0.932& 0.968& 0.914& 0.991\\
  HIP 1411& 4.84& 2.23& 7.51& 0.86&10.14  & 0.990& 0.955& 1.024& 0.925& 1.054\\
  HIP 1499& 4.66& 3.29& 7.37& 1.47& 9.38  & 1.059& 1.024& 1.083& 0.993& 1.114\\
  HIP 1599& 6.31& 4.07& 7.14& 2.64& 8.67  & 0.991& 0.971& 1.026& 0.946& 1.055\\
  HIP 1813& 8.25& 7.46& 9.33& 6.54&10.24  & 0.981& 0.967& 1.001& 0.950& 1.018\\
  HIP 2021& 6.09& 5.88& 6.32& 5.68& 6.50  & 1.141& 1.134& 1.159& 1.120& 1.170\\
  HIP 2131&11.22& 9.16&12.00& 6.82&12.99  & 0.917& 0.902& 0.932& 0.888& 0.948\\
  HIP 2453& 5.43& 4.20& 6.34& 3.14& 7.23  & 1.005& 0.984& 1.026& 0.966& 1.052\\
  HIP 2711& 2.99& 2.32& 3.41& 1.78& 4.51  & 1.245& 1.209& 1.263& 1.154& 1.290\\
  HIP 2712& 5.09& 4.29& 5.84& 3.75& 6.42  & 1.089& 1.066& 1.111& 1.048& 1.130\\
  HIP 2760& 7.42& 6.90& 7.98& 6.30& 8.55  & 1.048& 1.030& 1.070& 1.011& 1.092\\
  HIP 2894& 4.95& 2.78& 7.11& 1.02& 8.65  & 0.973& 0.967& 1.002& 0.954& 1.021\\
  HIP 2909&10.86&10.23&11.70& 9.41&12.46  & 0.944& 0.926& 0.964& 0.907& 0.984\\
  HIP 2981& 5.97& 5.26& 6.82& 4.36& 7.54  & 0.972& 0.952& 0.993& 0.934& 1.016\\
  HIP 3014& 5.30& 4.04& 5.46& 3.44& 6.04  & 1.130& 1.101& 1.187& 1.065& 1.247\\
  HIP 3026& 6.71& 4.45& 7.85& 2.15& 9.00  & 0.943& 0.909& 0.966& 0.882& 0.994\\
  HIP 3086& 8.35& 7.86& 8.81& 7.40& 9.31  & 1.038& 1.024& 1.059& 1.007& 1.078\\
  HIP 3093& 1.96& 2.05& 9.22& 0.82&12.84  & 0.913& 0.874& 0.940& 0.843& 0.959\\
  HIP 3132& 7.65& 7.22& 8.43& 6.62& 8.87  & 1.035& 1.012& 1.049& 0.996& 1.069\\
  HIP 3185&11.15&10.79&11.71&10.35&12.20  & 0.919& 0.903& 0.932& 0.890& 0.948\\
  HIP 3206& 3.45& 2.76&10.20& 1.03&13.53  & 0.846& 0.807& 0.870& 0.780& 0.889\\
  HIP 3272& 5.45& 4.78& 7.40& 3.49& 8.71  & 1.029& 0.992& 1.065& 0.960& 1.104\\
  HIP 3441&11.64& 9.98&12.76& 8.28&13.98  & 0.897& 0.864& 0.944& 0.834& 1.002\\
  HIP 3765&12.39& 4.37&12.75& 1.55&14.35  & 0.729& 0.722& 0.764& 0.709& 0.783\\
  HIP 3821& 7.42& 4.04& 7.69& 2.30& 9.58  & 0.982& 0.957& 1.017& 0.929& 1.049\\
  HIP 4039&10.72& 9.08&11.66& 7.36&12.80  & 0.859& 0.831& 0.911& 0.805& 0.976\\
  HIP 4127& 6.66& 6.19& 6.99& 5.85& 7.44  & 1.112& 1.088& 1.123& 1.070& 1.140\\
  HIP 4148& 7.23& 3.86&12.34& 1.14&14.28  & 0.755& 0.743& 0.787& 0.731& 0.802\\
  HIP 4151& 3.40& 3.33& 4.71& 3.04& 5.12  & 1.300& 1.214& 1.308& 1.197& 1.315\\
  HIP 4195& 6.35& 4.46& 9.44& 2.03&11.49  & 0.921& 0.899& 0.949& 0.876& 0.978\\
  HIP 4457& 6.12& 5.62& 6.63& 5.20& 7.25  & 1.109& 1.082& 1.149& 1.050& 1.184\\
  HIP 4544& 8.21& 4.41& 9.33& 1.67&10.92  & 0.893& 0.869& 0.924& 0.845& 0.954\\
  HIP 4909& 7.29& 4.81& 9.10& 2.25&10.57  & 0.960& 0.948& 0.984& 0.933& 1.006\\
  HIP 5016& 3.84& 3.59& 4.03& 3.39& 4.28  & 1.296& 1.273& 1.328& 1.249& 1.354\\
  HIP 5106& 4.18& 2.61& 6.07& 1.04& 7.42  & 0.986& 0.970& 1.018& 0.950& 1.042\\
  HIP 5122&10.34& 8.58&12.04& 7.17&13.75  & 0.952& 0.914& 1.009& 0.874& 1.065\\
  HIP 5134& 5.47& 3.83& 8.16& 2.67&10.62  & 1.123& 1.049& 1.308& 0.966& 1.468\\
  HIP 5163&13.14&10.20&13.77& 5.82&14.50  & 0.848& 0.821& 0.874& 0.799& 0.907\\
  HIP 5315&13.32& 9.90&13.96& 8.06&14.65  & 0.894& 0.884& 0.975& 0.870& 1.038\\
  HIP 5336&-1.00& 7.99&13.78& 3.98&14.51  & 0.718& 0.712& 0.756& 0.706& 0.785\\
  HIP 5441& 4.53& 3.33& 5.29& 2.17& 6.15  & 1.064& 1.043& 1.118& 1.014& 1.159\\
  HIP 5531& 4.15& 3.82& 4.39& 3.63& 4.67  & 1.243& 1.225& 1.278& 1.199& 1.308\\
  HIP 5682& 5.10& 3.91& 5.26& 3.47& 5.69  & 1.162& 1.141& 1.220& 1.117& 1.256\\
  HIP 5775&11.65& 6.24&11.70& 2.81&13.03  & 0.914& 0.875& 1.031& 0.856& 1.233\\
  HIP 5862& 3.92& 3.04& 4.13& 2.37& 4.67  & 1.170& 1.147& 1.178& 1.133& 1.195\\
  HIP 6159&13.14& 9.16&13.44& 5.67&14.42  & 0.834& 0.812& 0.865& 0.792& 0.897\\
  HIP 6407& 4.18& 2.16& 5.98& 0.81& 7.46  & 1.019& 0.992& 1.038& 0.971& 1.057\\
  HIP 6607& 8.67& 5.76&11.72& 2.69&13.84  & 0.858& 0.832& 0.886& 0.810& 0.916\\
  HIP 6711& 3.43& 3.05& 3.87& 2.83& 4.04  & 1.300& 1.288& 1.387& 1.264& 1.416\\
  HIP 6762& 2.85& 1.54& 6.05& 0.64& 8.53  & 0.903& 0.876& 0.911& 0.857& 0.925\\
  HIP 6975& 8.52& 7.75& 8.95& 7.13& 9.49  & 0.981& 0.966& 1.000& 0.951& 1.016\\
  HIP 6978& 2.10& 1.28& 4.13& 0.56& 5.59  & 1.063& 1.045& 1.082& 1.027& 1.099\\
  HIP 7221& 4.34& 2.31& 6.21& 0.86& 8.30  & 1.038& 1.016& 1.061& 0.990& 1.083\\
  HIP 7245& 4.35& 2.09& 6.09& 0.74& 7.82  & 1.035& 1.010& 1.058& 0.988& 1.080\\
  HIP 7312& 4.55& 3.75& 5.35& 3.21& 6.21  & 1.268& 1.193& 1.361& 1.129& 1.461\\
  HIP 7357& 6.09& 5.06& 6.81& 4.27& 7.58  & 1.042& 1.028& 1.072& 1.009& 1.098\\
  HIP 7513& 4.50& 3.47& 4.78& 3.16& 5.12  & 1.228& 1.204& 1.288& 1.182& 1.306\\
  HIP 7612& 7.30& 6.65& 7.80& 6.17& 8.37  & 1.079& 1.061& 1.109& 1.040& 1.137\\
 HIP 7751B& 3.45& 2.37&10.59& 0.91&13.85  & 0.768& 0.734& 0.774& 0.717& 0.789\\
 HIP 7751A& 4.94& 2.63&10.83& 0.91&13.88  & 0.772& 0.744& 0.786& 0.728& 0.798\\
  HIP 7885& 7.47& 6.23& 8.27& 4.65& 9.04  & 1.012& 1.001& 1.031& 0.988& 1.048\\
  HIP 7902& 8.98& 8.09&10.60& 6.64&11.76  & 0.941& 0.929& 0.953& 0.917& 0.966\\
  HIP 7918& 6.20& 4.50& 7.31& 3.17& 8.64  & 1.041& 1.019& 1.066& 0.997& 1.090\\
  HIP 7961&12.27&11.73&13.36&11.02&14.20  & 0.887& 0.864& 0.908& 0.844& 0.930\\
  HIP 7978& 1.50& 0.82& 2.98& 0.32& 4.27  & 1.118& 1.098& 1.144& 1.073& 1.160\\
  HIP 7981& 4.27& 2.92&10.34& 1.21&13.56  & 0.862& 0.822& 0.878& 0.798& 0.899\\
  HIP 8102&13.16& 7.44&13.64& 3.35&14.49  & 0.764& 0.757& 0.803& 0.745& 0.838\\
  HIP 8121& 7.15& 5.85& 7.74& 4.79& 8.55  & 1.036& 1.024& 1.059& 1.007& 1.080\\
  HIP 8362& 6.43& 2.69&10.37& 0.86&13.56  & 0.897& 0.853& 0.917& 0.829& 0.937\\
  HIP 8433& 6.40& 6.15& 6.72& 5.83& 6.97  & 1.103& 1.091& 1.116& 1.079& 1.128\\
  HIP 8476&11.73&10.61&12.54& 9.48&13.53  & 0.907& 0.890& 0.929& 0.871& 0.948\\
  HIP 8507& 4.79& 2.66& 7.69& 0.99& 9.86  & 0.943& 0.924& 0.965& 0.909& 0.984\\
  HIP 8674&13.14& 6.21&13.29& 2.36&14.43  & 0.798& 0.782& 0.836& 0.763& 0.867\\
  HIP 8720&13.14& 3.90&12.75& 1.22&14.36  & 0.727& 0.709& 0.755& 0.690& 0.779\\
  HIP 8841&10.16& 7.18&11.51& 3.66&12.97  & 0.931& 0.910& 0.950& 0.891& 0.974\\
  HIP 8859& 4.08& 3.66& 5.04& 3.19& 5.70  & 1.129& 1.093& 1.161& 1.063& 1.190\\
  HIP 9080&13.14& 4.47&13.16& 1.37&14.42  & 0.841& 0.800& 0.880& 0.767& 0.945\\
  HIP 9349& 5.72& 3.36& 6.64& 1.57& 7.90  & 0.978& 0.969& 1.006& 0.955& 1.025\\
  HIP 9519& 3.54& 1.97& 5.70& 0.75& 7.39  & 1.051& 1.015& 1.091& 0.984& 1.126\\
  HIP 9643& 1.95& 1.38& 5.16& 0.57& 7.38  & 1.041& 1.009& 1.063& 0.980& 1.087\\
  HIP 9884& 4.00& 2.66& 7.29& 1.71&11.44  & 1.270& 1.110& 1.514& 0.980& 1.764\\
 HIP 10138& 7.44& 5.32&12.08& 2.49&14.19  & 0.797& 0.775& 0.823& 0.760& 0.846\\
 HIP 10212& 2.92& 2.59& 3.29& 2.41& 3.43  & 1.525& 1.436& 1.545& 1.412& 1.579\\
 HIP 10303& 8.24& 4.15& 8.39& 1.40& 9.24  & 1.011& 1.003& 1.103& 0.989& 1.288\\
 HIP 10322&10.80&10.00&11.07& 9.56&11.63  & 0.971& 0.947& 0.985& 0.928& 1.004\\
 HIP 10449&13.14& 8.73&13.78& 4.48&14.51  & 0.777& 0.770& 0.805& 0.756& 0.832\\
 HIP 10644&13.41& 9.91&13.77& 7.47&14.54  & 0.843& 0.826& 0.890& 0.808& 0.930\\
 HIP 10652&13.14& 7.87&13.46& 3.80&14.45  & 0.812& 0.796& 0.844& 0.779& 0.873\\
 HIP 10710& 8.32& 4.61&10.06& 1.82&11.83  & 0.920& 0.905& 0.948& 0.887& 0.974\\
 HIP 10711&14.60&12.78&14.57&11.48&14.83  & 0.833& 0.819& 0.860& 0.802& 0.891\\
 HIP 10798& 3.45& 2.40& 9.51& 0.93&13.26  & 0.811& 0.773& 0.827& 0.748& 0.843\\
 HIP 11072& 6.19& 5.89& 6.49& 5.61& 6.78  & 1.150& 1.128& 1.159& 1.112& 1.175\\
 HIP 11237& 6.26& 5.03& 7.15& 3.66& 8.09  & 1.026& 1.002& 1.066& 0.973& 1.099\\
 HIP 11309& 5.09& 4.73& 5.35& 4.47& 5.70  & 1.158& 1.130& 1.186& 1.101& 1.215\\
 HIP 11505& 9.01& 8.43& 9.64& 7.83&10.27  & 1.032& 1.013& 1.058& 0.992& 1.083\\
 HIP 11584& 4.55& 3.74& 4.93& 3.25& 5.37  & 1.242& 1.197& 1.307& 1.157& 1.375\\
 HIP 11728& 2.10& 1.33& 4.76& 0.59& 6.54  & 1.009& 0.983& 1.025& 0.962& 1.044\\
 HIP 11915& 6.54& 3.41& 7.69& 1.34& 9.22  & 0.976& 0.959& 0.999& 0.944& 1.021\\
 HIP 11923&12.24&11.07&12.76&10.25&13.70  & 0.910& 0.885& 0.933& 0.862& 0.956\\
 HIP 12262& 3.83& 3.55& 4.23& 3.08& 4.58  & 1.301& 1.276& 1.364& 1.245& 1.427\\
 HIP 12294& 8.67& 4.22& 9.68& 1.40&11.70  & 0.883& 0.851& 0.962& 0.805& 1.085\\
 HIP 12306&12.34&11.05&13.61& 9.74&14.53  & 0.845& 0.830& 0.868& 0.814& 0.889\\
 HIP 12381& 4.81& 3.72& 5.00& 3.27& 5.51  & 1.144& 1.120& 1.192& 1.091& 1.236\\
 HIP 12444& 1.90& 1.11& 2.67& 0.51& 3.34  & 1.168& 1.149& 1.193& 1.132& 1.215\\
 HIP 12579&11.65& 6.71&12.57& 2.92&14.15  & 0.823& 0.801& 0.849& 0.783& 0.876\\
 HIP 12777& 2.19& 1.27& 2.85& 0.53& 3.44  & 1.201& 1.183& 1.230& 1.168& 1.262\\
 HIP 13336&14.54&14.44&14.85&14.18&14.89  & 0.827& 0.820& 0.832& 0.818& 0.841\\
 HIP 13366&11.36&10.50&12.80& 9.19&13.91  & 0.857& 0.841& 0.884& 0.821& 0.907\\
 HIP 13402& 1.96& 1.62& 7.76& 0.74&11.60  & 0.889& 0.841& 0.895& 0.812& 0.909\\
 HIP 14023& 3.45& 1.83& 7.17& 0.78&10.32  & 0.943& 0.904& 0.954& 0.875& 0.971\\
 HIP 14086&11.94&10.29&13.57& 9.11&14.62  & 0.905& 0.874& 0.948& 0.855& 0.981\\
 HIP 14241&11.67& 7.43&12.71& 4.34&14.26  & 0.823& 0.803& 0.849& 0.784& 0.875\\
 HIP 14286&12.76&10.98&13.11& 9.82&14.12  & 0.888& 0.876& 0.904& 0.863& 0.919\\
 HIP 14594&13.22& 9.83&13.93& 7.51&14.63  & 0.727& 0.725& 0.760& 0.716& 0.781\\
 HIP 14614& 7.39& 5.79& 7.92& 4.27& 8.91  & 0.988& 0.970& 1.005& 0.954& 1.023\\
 HIP 14632& 5.58& 4.41& 6.26& 3.78& 7.05  & 1.173& 1.107& 1.181& 1.087& 1.189\\
 HIP 14668& 1.54& 1.03& 1.62& 0.94& 2.15  & 2.147& 1.860& 2.189& 1.680& 2.296\\
 HIP 14721& 4.49& 2.13& 6.38& 0.83& 8.55  & 1.030& 0.999& 1.052& 0.971& 1.078\\
 HIP 14879& 4.77& 4.60& 4.99& 4.37& 5.17  & 1.202& 1.185& 1.216& 1.171& 1.232\\
 HIP 15126&13.14& 4.19&12.94& 1.31&14.39  & 0.741& 0.723& 0.771& 0.705& 0.794\\
 HIP 15206& 4.60& 4.07& 5.27& 3.63& 5.82  & 1.261& 1.219& 1.322& 1.175& 1.380\\
 HIP 15249&11.32& 9.64&11.98& 8.05&12.91  & 0.940& 0.926& 0.957& 0.910& 0.973\\
 HIP 15330& 7.24& 2.81& 7.35& 1.14& 9.57  & 0.916& 0.899& 0.954& 0.874& 0.977\\
 HIP 15371& 6.17& 3.56& 6.97& 1.85& 8.93  & 0.955& 0.935& 0.988& 0.910& 1.015\\
 HIP 15383& 4.31& 3.23& 7.78& 2.19&11.51  & 1.264& 1.107& 1.445& 0.993& 1.636\\
 HIP 15394& 2.85& 2.58& 3.65& 2.21& 4.39  & 1.416& 1.353& 1.519& 1.275& 1.601\\
 HIP 15405&14.65& 5.52&12.99& 2.77&14.42  & 0.910& 0.884& 1.132& 0.851& 1.372\\
 HIP 15457& 5.11& 3.36& 7.33& 1.63& 9.20  & 0.958& 0.941& 0.990& 0.920& 1.014\\
 HIP 15510&14.26&11.51&14.24& 9.44&14.68  & 0.813& 0.801& 0.831& 0.788& 0.852\\
 HIP 15565& 4.71& 4.40& 5.04& 3.98& 5.44  & 1.164& 1.134& 1.198& 1.103& 1.242\\
 HIP 15940&10.02& 9.47&11.33& 8.63&12.33  & 0.957& 0.926& 0.986& 0.898& 1.017\\
 HIP 16072&10.16& 3.62&12.45& 1.16&14.30  & 0.766& 0.745& 0.801& 0.722& 0.832\\
 HIP 16169&12.90&10.52&13.91& 8.22&14.59  & 0.831& 0.816& 0.860& 0.799& 0.886\\
 HIP 16467& 9.01& 6.25&10.12& 3.18&11.37  & 0.969& 0.955& 0.997& 0.936& 1.023\\
 HIP 16537& 9.45& 3.38&11.64& 1.19&14.18  & 0.804& 0.771& 0.821& 0.754& 0.839\\
 HIP 16723& 5.03& 3.87& 5.51& 3.32& 6.18  & 1.112& 1.098& 1.177& 1.065& 1.223\\
 HIP 16738& 2.67& 2.32& 2.81& 2.05& 3.29  & 1.405& 1.372& 1.506& 1.318& 1.581\\
 HIP 16818& 6.71& 5.11& 7.18& 3.71& 8.05  & 0.990& 0.969& 1.013& 0.948& 1.036\\
 HIP 16852& 5.88& 5.55& 6.17& 5.24& 6.51  & 1.143& 1.128& 1.151& 1.117& 1.163\\
 HIP 17022& 6.90& 6.76& 7.99& 6.24& 8.59  & 1.069& 1.044& 1.095& 1.020& 1.120\\
 HIP 17147&13.02&10.81&13.96& 8.98&14.65  & 0.808& 0.799& 0.841& 0.788& 0.864\\
 HIP 17231& 5.69& 5.19& 6.82& 4.39& 7.72  & 1.144& 1.107& 1.212& 1.065& 1.280\\
 HIP 17378& 6.58& 6.50& 7.96& 6.30&10.44  & 1.179& 1.112& 1.180& 1.037& 1.201\\
 HIP 17409&10.39& 9.71&10.87& 9.09&11.44  & 0.929& 0.914& 0.941& 0.901& 0.954\\
 HIP 17420&11.67& 4.21&12.55& 1.46&14.32  & 0.761& 0.746& 0.790& 0.733& 0.808\\
 HIP 17655& 7.95& 5.80& 8.36& 4.05& 9.47  & 0.994& 0.970& 1.013& 0.949& 1.037\\
 HIP 17666&13.14& 4.75&13.15& 1.55&14.42  & 0.655& 0.645& 0.673& 0.635& 0.688\\
 HIP 18235&12.73& 9.62&13.82& 7.81&14.62  & 0.858& 0.841& 0.957& 0.825& 1.016\\
 HIP 18261& 4.90& 2.61& 6.31& 0.95& 7.92  & 1.023& 0.999& 1.052& 0.978& 1.079\\
 HIP 18347& 7.61& 3.87& 9.34& 1.40&11.20  & 0.878& 0.855& 0.906& 0.834& 0.933\\
 HIP 18366& 6.00& 5.08& 6.23& 4.38& 6.69  & 1.062& 1.045& 1.088& 1.025& 1.117\\
 HIP 18413&14.50&12.47&14.49&11.16&14.79  & 0.878& 0.870& 0.902& 0.859& 0.921\\
 HIP 18606& 6.29& 4.80&10.15& 3.35&13.34  & 1.139& 1.046& 1.296& 0.976& 1.437\\
 HIP 19631& 8.11& 7.34& 8.89& 6.68& 9.71  & 1.016& 0.993& 1.054& 0.966& 1.087\\
 HIP 19696&10.02& 8.16&10.94& 5.91&12.14  & 0.967& 0.945& 1.034& 0.913& 1.108\\
 HIP 19786& 1.95& 1.00& 3.95& 0.41& 5.54  & 1.058& 1.035& 1.080& 1.010& 1.100\\
 HIP 19849&11.67& 6.70&13.36& 2.96&14.45  & 0.773& 0.764& 0.811& 0.753& 0.837\\
 HIP 19911& 8.67& 4.04&10.43& 1.45&12.59  & 0.922& 0.899& 0.945& 0.879& 0.970\\
 HIP 20094&13.16& 8.57&13.53& 4.95&14.47  & 0.836& 0.827& 0.863& 0.813& 0.886\\
 HIP 20298&11.65& 7.25&12.11& 2.76&13.51  & 0.857& 0.835& 0.893& 0.812& 0.937\\
 HIP 20366& 9.28& 5.45&10.05& 2.30&11.41  & 0.957& 0.940& 0.985& 0.920& 1.010\\
 HIP 20753& 5.15& 4.88& 5.68& 4.50& 6.11  & 1.229& 1.195& 1.258& 1.165& 1.296\\
 HIP 20754& 6.14& 5.46& 6.70& 4.88& 7.21  & 1.088& 1.053& 1.129& 1.022& 1.171\\
 HIP 20984&10.99& 9.47&12.16& 7.33&13.36  & 0.923& 0.897& 0.961& 0.868& 1.002\\
 HIP 21227& 5.09& 3.01& 6.17& 1.00& 7.44  & 1.058& 1.017& 1.131& 0.971& 1.225\\
 HIP 21306&11.65& 3.92&11.78& 1.26&13.73  & 0.861& 0.837& 0.889& 0.814& 0.917\\
 HIP 21703& 8.67& 5.09&11.50& 2.08&13.75  & 0.939& 0.913& 0.979& 0.886& 1.010\\
 HIP 21847& 5.45& 4.36& 5.74& 3.79& 6.05  & 1.173& 1.164& 1.253& 1.143& 1.289\\
 HIP 21921&-1.00&11.07&14.26& 8.44&14.63  & 0.804& 0.790& 0.819& 0.777& 0.838\\
 HIP 22020& 9.28& 7.60&10.37& 4.77&11.62  & 0.973& 0.944& 1.016& 0.916& 1.074\\
 HIP 22060& 6.61& 2.60& 8.08& 0.91&10.01  & 0.956& 0.922& 0.996& 0.885& 1.036\\
 HIP 22263& 2.30& 1.49& 4.48& 0.43& 6.12  & 1.016& 0.995& 1.040& 0.972& 1.059\\
 HIP 22336& 5.65& 4.44& 5.83& 3.94& 6.35  & 1.187& 1.178& 1.256& 1.150& 1.282\\
 HIP 22349&12.15&11.22&13.08&10.17&13.95  & 0.891& 0.873& 0.903& 0.858& 0.919\\
 HIP 22449& 1.80& 1.06& 2.05& 0.45& 2.65  & 1.280& 1.243& 1.293& 1.223& 1.328\\
 HIP 22489& 1.22& 1.18& 9.76& 0.55&13.77  & 1.002& 1.127& 2.272& 0.957& 3.094\\
 HIP 22528&13.14& 9.15&13.74& 5.12&14.50  & 0.854& 0.841& 0.880& 0.824& 0.906\\
 HIP 22596&12.24&11.49&13.24&10.61&14.04  & 0.864& 0.847& 0.877& 0.833& 0.892\\
 HIP 23080&-1.00&11.65&14.36& 9.44&14.68  & 0.798& 0.788& 0.814& 0.777& 0.831\\
 HIP 23311&-1.00& 7.20&13.71& 3.16&14.50  & 0.780& 0.764& 0.801& 0.751& 0.824\\
 HIP 23693& 1.14& 1.27& 3.81& 0.79& 5.19  & 1.079& 1.051& 1.113& 1.018& 1.135\\
 HIP 23835&10.15& 9.33&10.36& 8.77&10.75  & 0.991& 0.981& 1.007& 0.971& 1.020\\
 HIP 23884& 4.99& 3.55& 6.71& 1.96& 8.02  & 1.018& 0.990& 1.041& 0.969& 1.065\\
 HIP 23922&11.65& 8.72&13.40& 4.61&14.42  & 0.837& 0.815& 0.872& 0.792& 0.907\\
 HIP 23941& 4.05& 3.07& 4.12& 2.70& 4.43  & 1.214& 1.208& 1.303& 1.185& 1.327\\
 HIP 24030&10.16& 6.94&11.83& 2.59&13.27  & 0.840& 0.821& 0.878& 0.797& 0.919\\
 HIP 24037&-1.00& 9.70&13.93& 6.41&14.54  & 0.814& 0.801& 0.835& 0.787& 0.857\\
 HIP 24660& 1.20& 0.63& 2.30& 0.29& 3.31  & 1.084& 1.071& 1.104& 1.054& 1.123\\
 HIP 24813& 6.48& 5.36& 7.75& 4.29& 8.81  & 1.065& 1.043& 1.098& 1.023& 1.124\\
 HIP 25052& 8.25& 6.92& 9.17& 5.62&10.10  & 1.028& 1.011& 1.055& 0.991& 1.082\\
 HIP 25361&-1.00& 7.83&14.02& 2.86&14.54  & 0.828& 0.798& 0.854& 0.777& 0.891\\
 HIP 25528& 2.88& 2.43& 3.08& 2.23& 3.52  & 1.414& 1.338& 1.461& 1.284& 1.522\\
 HIP 25586&10.61& 8.43&12.09& 5.85&13.45  & 0.918& 0.904& 0.935& 0.888& 0.951\\
 HIP 25670& 4.10& 1.96& 5.70& 0.70& 7.32  & 1.025& 1.000& 1.046& 0.979& 1.068\\
 HIP 25840& 5.52& 4.24& 6.04& 3.65& 6.64  & 1.121& 1.103& 1.182& 1.078& 1.220\\
 HIP 25860& 8.67& 5.31&11.54& 2.18&13.68  & 0.885& 0.863& 0.910& 0.843& 0.937\\
 HIP 25973& 5.28& 5.09& 5.53& 4.86& 5.69  & 1.201& 1.187& 1.216& 1.174& 1.230\\
 HIP 26100& 6.50& 5.88& 6.88& 5.32& 7.37  & 1.089& 1.067& 1.127& 1.041& 1.161\\
 HIP 26129& 1.90& 1.14& 4.53& 0.45& 6.06  & 1.049& 1.025& 1.065& 1.003& 1.087\\
 HIP 26326& 5.37& 4.27& 6.18& 3.44& 6.96  & 1.080& 1.057& 1.109& 1.035& 1.137\\
 HIP 26437& 3.94& 3.39& 4.93& 2.55& 5.98  & 1.129& 1.101& 1.144& 1.079& 1.162\\
 HIP 26452& 6.43& 2.79& 9.09& 1.00&11.55  & 0.873& 0.847& 0.903& 0.820& 0.932\\
 HIP 26534& 6.55& 6.25& 7.14& 5.88& 7.65  & 1.093& 1.080& 1.119& 1.062& 1.137\\
 HIP 26617&-1.00& 5.06&13.53& 1.55&14.48  & 0.808& 0.777& 0.847& 0.759& 0.923\\
 HIP 26779& 3.76& 2.40& 8.14& 1.25&10.97  & 0.871& 0.851& 0.903& 0.828& 0.922\\
 HIP 26807& 6.43& 4.43& 9.28& 2.08&11.45  & 0.973& 0.946& 1.006& 0.921& 1.038\\
 HIP 26828& 4.20& 3.18& 4.30& 2.76& 4.71  & 1.156& 1.135& 1.214& 1.102& 1.256\\
 HIP 27072& 3.03& 2.27& 3.30& 1.28& 3.79  & 1.180& 1.171& 1.207& 1.152& 1.238\\
 HIP 27128&13.24&11.72&13.83&10.65&14.63  & 0.840& 0.823& 0.865& 0.806& 0.887\\
 HIP 27207&-1.00&11.32&14.29& 8.97&14.64  & 0.821& 0.812& 0.841& 0.803& 0.863\\
 HIP 27878& 7.68& 6.99& 8.40& 6.14& 9.07  & 1.043& 1.021& 1.056& 1.004& 1.075\\
 HIP 27913& 2.47& 1.05& 4.39& 0.50& 6.14  & 1.042& 1.016& 1.073& 0.987& 1.088\\
 HIP 28066&11.11& 9.41&11.65& 8.20&12.68  & 0.945& 0.929& 0.964& 0.913& 0.984\\
 HIP 28103& 1.26& 0.98& 1.50& 0.68& 1.83  & 1.449& 1.429& 1.481& 1.401& 1.516\\
 HIP 28145&10.16& 7.05&11.61& 3.84&13.28  & 0.910& 0.885& 0.939& 0.859& 0.968\\
 HIP 28159&12.75&11.32&13.32&10.43&14.32  & 0.911& 0.880& 0.936& 0.855& 0.964\\
 HIP 28336& 6.75& 3.32& 9.10& 1.11&11.35  & 0.928& 0.911& 0.957& 0.892& 0.981\\
 HIP 28671&-1.00& 5.82&13.58& 1.95&14.48  & 0.728& 0.711& 0.753& 0.695& 0.778\\
 HIP 29001& 4.61& 3.02& 5.93& 1.49& 7.32  & 0.950& 0.935& 0.982& 0.914& 1.008\\
 HIP 29074& 1.34& 0.86& 3.44& 0.39& 5.07  & 1.048& 1.025& 1.063& 1.002& 1.079\\
 HIP 29248& 6.43& 3.51& 9.08& 1.31&11.43  & 0.921& 0.900& 0.950& 0.877& 0.975\\
 HIP 29269&12.69&11.12&14.21& 9.15&14.71  & 0.857& 0.843& 0.914& 0.827& 0.969\\
 HIP 29271& 6.28& 5.12& 9.07& 3.10&10.87  & 0.962& 0.935& 0.988& 0.912& 1.017\\
 HIP 29432& 2.58& 1.71& 4.96& 0.82& 6.53  & 0.986& 0.962& 1.005& 0.941& 1.023\\
 HIP 29650& 1.15& 0.85& 1.76& 0.13& 2.36  & 1.291& 1.273& 1.314& 1.257& 1.339\\
 HIP 29716& 3.26& 2.89& 3.68& 2.65& 3.86  & 1.321& 1.310& 1.404& 1.290& 1.432\\
 HIP 30545& 4.89& 4.69& 5.12& 4.47& 5.32  & 1.213& 1.197& 1.229& 1.185& 1.245\\
 HIP 30990&11.17&10.35&12.49& 9.42&13.64  & 0.863& 0.844& 0.897& 0.820& 0.927\\
 HIP 31083&14.13&10.73&14.04& 8.62&14.62  & 0.882& 0.864& 0.913& 0.846& 0.942\\
 HIP 31188& 9.45& 7.44&11.80& 4.76&13.54  & 0.859& 0.837& 0.887& 0.815& 0.917\\
 HIP 31419& 9.39& 6.88& 9.85& 4.98&11.03  & 0.974& 0.963& 1.006& 0.946& 1.035\\
 HIP 32650&11.56&10.50&12.70& 9.40&13.83  & 0.911& 0.883& 0.933& 0.859& 0.958\\
 HIP 32673& 5.56& 2.55& 6.89& 0.90& 8.51  & 1.002& 0.988& 1.028& 0.970& 1.048\\
 HIP 32851& 2.93& 2.20& 3.74& 1.61& 4.34  & 1.236& 1.167& 1.256& 1.125& 1.276\\
 HIP 33287&-1.00&13.88&14.82&12.96&14.93  & 0.790& 0.788& 0.802& 0.786& 0.810\\
 HIP 33382& 9.21& 7.53&10.37& 5.97&11.66  & 0.937& 0.922& 0.954& 0.907& 0.972\\
 HIP 33608& 2.24& 0.94& 3.45& 0.37& 4.84  & 1.077& 1.066& 1.109& 1.043& 1.130\\
 HIP 34017& 6.03& 3.85& 7.07& 2.33& 8.67  & 1.011& 0.994& 1.052& 0.968& 1.081\\
 HIP 34164& 8.59& 7.26&12.52& 4.93&14.27  & 0.907& 0.879& 1.040& 0.840& 1.164\\
 HIP 34511& 7.94& 6.12& 8.92& 4.16&10.14  & 0.966& 0.952& 0.988& 0.936& 1.009\\
 HIP 34521& 4.00& 3.47& 4.55& 3.02& 5.16  & 1.288& 1.252& 1.374& 1.199& 1.429\\
 HIP 34608&11.06& 8.57&13.39& 6.68&14.54  & 0.929& 0.905& 1.031& 0.883& 1.106\\
 HIP 34642&12.30&10.07&13.00& 8.54&14.26  & 0.889& 0.863& 0.942& 0.835& 0.994\\
 HIP 34653&13.98&12.52&14.44&10.63&14.75  & 0.888& 0.874& 0.909& 0.859& 0.933\\
 HIP 34710& 4.95& 4.54& 5.34& 4.17& 5.72  & 1.228& 1.214& 1.280& 1.188& 1.314\\
 HIP 35148& 9.22& 8.37& 9.74& 7.70&10.48  & 1.006& 0.979& 1.028& 0.957& 1.054\\
 HIP 35185& 5.07& 2.55& 6.70& 0.94& 8.52  & 1.006& 0.975& 1.033& 0.951& 1.059\\
 HIP 35214&10.16& 5.77&11.26& 2.41&13.02  & 0.927& 0.891& 0.957& 0.858& 0.990\\
 HIP 35599& 8.50& 7.50& 9.04& 6.53& 9.67  & 1.008& 0.989& 1.048& 0.967& 1.092\\
 HIP 35989&13.14& 5.03&13.25& 1.62&14.43  & 0.773& 0.757& 0.813& 0.734& 0.844\\
 HIP 36210& 8.28& 6.04&10.20& 3.84&12.15  & 0.948& 0.926& 0.972& 0.906& 1.001\\
 HIP 36439& 2.85& 2.69& 3.38& 2.17& 3.68  & 1.147& 1.137& 1.167& 1.120& 1.187\\
 HIP 36481& 8.60& 8.20& 9.20& 7.67& 9.65  & 1.023& 1.006& 1.037& 0.990& 1.052\\
 HIP 36515& 0.47& 1.44& 5.62& 0.40& 7.88  & 1.015& 0.963& 1.026& 0.936& 1.044\\
 HIP 36849&10.16& 8.65&11.40& 6.20&12.50  & 0.866& 0.847& 0.889& 0.827& 0.913\\
 HIP 36874& 8.54& 7.88& 9.71& 6.98&10.46  & 0.988& 0.972& 1.006& 0.957& 1.023\\
 HIP 37171& 7.40& 4.31& 8.47& 1.94&10.09  & 1.004& 0.971& 1.019& 0.949& 1.040\\
 HIP 37233&10.81& 9.80&11.07& 9.23&11.73  & 0.953& 0.929& 0.967& 0.910& 0.987\\
 HIP 37279& 1.97& 1.74& 2.16& 1.59& 2.35  & 1.492& 1.484& 1.514& 1.472& 1.542\\
 HIP 37316& 3.95& 3.13& 5.44& 1.39& 6.35  & 1.117& 1.090& 1.165& 1.057& 1.213\\
 HIP 37349& 7.23& 3.36&11.74& 1.07&14.11  & 0.777& 0.757& 0.799& 0.743& 0.814\\
 HIP 37419& 6.43& 3.00& 8.80& 1.12&11.58  & 0.908& 0.882& 0.942& 0.855& 0.970\\
 HIP 37789&10.90&10.14&11.16& 9.75&11.77  & 0.902& 0.885& 0.914& 0.872& 0.930\\
 HIP 37826& 1.60& 0.96& 1.68& 0.85& 2.34  & 1.997& 1.813& 2.194& 1.614& 2.340\\
 HIP 37853&-1.00&13.65&14.78&12.67&14.88  & 0.811& 0.802& 0.821& 0.797& 0.835\\
 HIP 37971& 4.65& 2.11& 5.90& 0.80& 7.92  & 1.058& 1.012& 1.074& 0.978& 1.097\\
 HIP 38072& 5.56& 2.78& 7.13& 0.99& 8.56  & 0.998& 0.982& 1.019& 0.968& 1.038\\
 HIP 38172& 5.90& 4.89& 6.31& 4.17& 6.91  & 1.068& 1.035& 1.081& 1.014& 1.111\\
 HIP 38228& 1.62& 1.42& 4.26& 0.41& 5.86  & 0.975& 0.954& 0.993& 0.933& 1.011\\
 HIP 38325& 2.10& 1.75& 2.57& 1.36& 2.84  & 1.259& 1.240& 1.274& 1.227& 1.295\\
 HIP 38613&10.96& 8.82&11.77& 6.67&13.13  & 0.886& 0.865& 0.922& 0.839& 0.951\\
 HIP 38625&-1.00&12.48&14.63&10.80&14.81  & 0.699& 0.693& 0.710& 0.690& 0.721\\
 HIP 38769&10.88& 9.82&12.43& 8.62&13.76  & 0.878& 0.850& 0.914& 0.822& 0.950\\
 HIP 39072&10.96& 8.29&11.79& 5.91&13.26  & 0.932& 0.896& 0.958& 0.864& 0.989\\
 HIP 39157&14.14&11.03&14.27& 8.55&14.65  & 0.720& 0.717& 0.739& 0.710& 0.756\\
 HIP 39417& 5.85& 4.94& 8.45& 3.01& 9.93  & 1.063& 1.029& 1.087& 1.002& 1.114\\
 HIP 39506&14.43&12.15&14.40&10.56&14.75  & 0.809& 0.800& 0.828& 0.791& 0.846\\
 HIP 39616& 4.72& 3.47& 6.09& 2.09& 7.19  & 1.005& 0.988& 1.033& 0.968& 1.057\\
 HIP 39780& 5.64& 5.50& 5.99& 5.15& 6.13  & 1.192& 1.176& 1.209& 1.166& 1.229\\
 HIP 39822& 9.91& 7.58&11.06& 5.45&12.55  & 0.903& 0.888& 0.922& 0.871& 0.941\\
 HIP 39893&-1.00&11.02&14.28& 8.89&14.71  & 0.833& 0.832& 0.905& 0.814& 0.966\\
 HIP 40001& 5.35& 5.06& 5.58& 4.82& 5.88  & 1.153& 1.135& 1.178& 1.110& 1.201\\
 HIP 40023& 2.50& 2.37& 2.64& 2.31& 2.69  & 1.553& 1.531& 1.579& 1.511& 1.594\\
 HIP 40118&14.60&12.78&14.59&11.44&14.83  & 0.814& 0.804& 0.825& 0.795& 0.839\\
 HIP 40613&11.33&10.70&12.30& 9.92&13.23  & 0.888& 0.867& 0.907& 0.849& 0.927\\
 HIP 40674& 8.67& 4.92&11.40& 1.86&13.50  & 0.884& 0.866& 0.914& 0.845& 0.940\\
 HIP 40693& 4.86& 2.62& 7.03& 1.23& 9.18  & 0.906& 0.887& 0.930& 0.869& 0.946\\
 HIP 40765& 2.28& 1.50& 5.50& 0.63& 7.46  & 1.035& 0.994& 1.059& 0.968& 1.079\\
 HIP 40843& 3.39& 2.57& 3.70& 1.86& 4.67  & 1.160& 1.138& 1.175& 1.107& 1.192\\
 HIP 40848& 8.67& 4.21&11.06& 1.49&13.67  & 0.841& 0.815& 0.860& 0.796& 0.882\\
 HIP 41484& 6.66& 5.27& 7.61& 4.02& 8.64  & 1.008& 0.993& 1.028& 0.978& 1.049\\
 HIP 41832& 4.95& 2.42& 6.39& 0.82& 7.94  & 1.003& 0.975& 1.020& 0.957& 1.042\\
 HIP 41926& 8.67& 4.17&11.81& 1.59&14.09  & 0.788& 0.760& 0.814& 0.741& 0.836\\
 HIP 42343& 4.41& 3.56& 4.80& 3.10& 5.39  & 1.156& 1.119& 1.176& 1.096& 1.197\\
 HIP 42438& 1.15& 1.02& 3.92& 0.55& 5.84  & 1.017& 0.996& 1.050& 0.962& 1.066\\
 HIP 42575& 3.74& 2.17& 6.34& 0.79& 8.22  & 0.980& 0.963& 1.011& 0.942& 1.031\\
 HIP 42612& 7.92& 6.88& 8.38& 6.05& 9.01  & 1.063& 1.039& 1.114& 1.012& 1.162\\
 HIP 42734&12.81&12.35&13.86&11.64&14.54  & 0.865& 0.848& 0.883& 0.833& 0.902\\
 HIP 42808& 2.96& 2.97& 9.66& 1.13&13.10  & 0.805& 0.771& 0.813& 0.751& 0.831\\
 HIP 43393&-1.00& 9.52&14.04& 5.50&14.55  & 0.785& 0.768& 0.803& 0.754& 0.826\\
 HIP 43587& 8.67& 4.38&11.71& 1.58&14.03  & 0.933& 0.899& 0.962& 0.879& 0.991\\
 HIP 43595&-1.00& 4.51&13.39& 1.38&14.46  & 0.797& 0.782& 0.840& 0.763& 0.880\\
 HIP 43618& 7.58& 5.22& 8.90& 2.85&10.40  & 1.014& 0.987& 1.039& 0.963& 1.063\\
 HIP 43727& 5.98& 5.22& 6.76& 4.55& 7.38  & 1.119& 1.095& 1.166& 1.068& 1.211\\
 HIP 43861&-1.00&13.57&14.73&12.55&14.87  & 0.866& 0.855& 0.880& 0.844& 0.894\\
 HIP 43904& 6.96& 6.07& 7.45& 5.31& 8.03  & 1.016& 0.990& 1.033& 0.970& 1.055\\
 HIP 43981& 6.53& 5.91& 7.21& 5.11& 7.77  & 1.038& 1.016& 1.058& 0.995& 1.079\\
 HIP 44075&11.86&11.14&12.83&10.29&13.81  & 0.853& 0.838& 0.871& 0.821& 0.888\\
 HIP 44212& 5.22& 3.17& 5.95& 1.68& 7.01  & 1.012& 0.994& 1.041& 0.973& 1.064\\
 HIP 44324& 9.59& 8.04&11.03& 6.49&12.46  & 0.937& 0.913& 0.955& 0.892& 0.976\\
 HIP 44347&10.16& 4.94&11.81& 1.68&13.65  & 0.846& 0.821& 0.871& 0.798& 0.898\\
 HIP 44441& 5.20& 4.62& 5.56& 3.68& 5.95  & 1.132& 1.104& 1.157& 1.081& 1.219\\
 HIP 44858& 2.41& 1.22& 4.80& 0.46& 6.51  & 0.991& 0.970& 1.014& 0.948& 1.030\\
 HIP 44860&12.85&11.58&13.51&10.48&14.33  & 0.884& 0.866& 0.900& 0.852& 0.918\\
 HIP 44927& 4.60& 4.43& 5.52& 3.96& 6.01  & 1.191& 1.166& 1.250& 1.130& 1.292\\
 HIP 44997& 8.49& 6.07& 9.57& 3.87&11.06  & 0.959& 0.947& 0.985& 0.930& 1.009\\
 HIP 45333& 5.41& 4.39& 6.17& 3.82& 6.76  & 1.213& 1.131& 1.214& 1.114& 1.231\\
 HIP 45699& 5.89& 5.28& 6.53& 4.43& 7.01  & 1.099& 1.075& 1.121& 1.054& 1.158\\
 HIP 45718& 2.44& 1.07& 4.09& 0.39& 5.41  & 1.069& 1.051& 1.093& 1.030& 1.114\\
 HIP 45947&12.37& 8.63&13.59& 6.32&14.54  & 0.895& 0.869& 1.024& 0.843& 1.119\\
 HIP 46066& 7.52& 3.33& 8.70& 1.12&10.59  & 0.945& 0.932& 0.972& 0.916& 0.994\\
 HIP 46453& 4.55& 3.72& 4.75& 3.30& 5.14  & 1.318& 1.274& 1.375& 1.235& 1.426\\
 HIP 46853& 2.72& 2.73& 3.04& 2.34& 3.09  & 1.401& 1.392& 1.436& 1.376& 1.502\\
 HIP 47080& 4.39& 3.23& 7.15& 1.22& 9.38  & 1.004& 0.970& 1.020& 0.943& 1.047\\
 HIP 47173& 8.67& 3.75&11.41& 1.20&13.80  & 0.902& 0.865& 0.961& 0.824& 1.023\\
 HIP 47292& 8.73& 7.61& 9.66& 6.44&10.63  & 0.985& 0.963& 1.013& 0.941& 1.039\\
 HIP 47588&14.19&13.11&14.61&12.06&14.85  & 0.869& 0.855& 0.895& 0.841& 0.922\\
 HIP 48113& 6.45& 5.63& 6.83& 4.67& 7.18  & 1.134& 1.113& 1.162& 1.101& 1.212\\
 HIP 48152&-1.00& 0.00&15.00& 0.00&15.00  & 0.000& 0.000& 0.000& 0.000& 0.000\\
 HIP 48209&13.14& 6.55&13.53& 2.44&14.47  & 0.798& 0.782& 0.829& 0.764& 0.858\\
 HIP 48468& 3.31& 3.09& 3.44& 3.01& 3.62  & 1.431& 1.405& 1.450& 1.384& 1.472\\
 HIP 48701&13.14& 9.21&13.76& 5.10&14.50  & 0.827& 0.815& 0.857& 0.797& 0.883\\
 HIP 48833& 3.75& 2.92& 3.90& 2.60& 4.20  & 1.274& 1.244& 1.356& 1.204& 1.394\\
 HIP 49070& 8.80& 8.05& 9.63& 7.29&10.36  & 0.973& 0.954& 0.995& 0.934& 1.017\\
 HIP 49130&-1.00&12.17&14.47&10.31&14.75  & 0.852& 0.840& 0.867& 0.829& 0.885\\
 HIP 49246& 4.50& 4.12& 5.11& 3.71& 5.60  & 1.225& 1.185& 1.271& 1.148& 1.317\\
 HIP 49572& 8.41& 4.84& 9.82& 1.92&11.38  & 0.968& 0.950& 0.995& 0.930& 1.020\\
 HIP 49615& 6.05& 4.56& 7.21& 3.02& 8.45  & 0.985& 0.960& 1.009& 0.938& 1.035\\
 HIP 49621& 2.80& 1.05& 4.58& 0.38& 6.30  & 1.010& 0.980& 1.021& 0.959& 1.037\\
 HIP 49668& 9.59& 9.03&10.45& 8.27&11.14  & 0.958& 0.942& 0.971& 0.928& 0.986\\
 HIP 49756& 4.38& 3.31& 6.20& 1.79& 7.39  & 0.998& 0.981& 1.018& 0.966& 1.035\\
 HIP 49988& 9.09& 7.87&10.25& 6.95&11.50  & 0.935& 0.907& 1.004& 0.866& 1.060\\
 HIP 50005& 6.43& 3.46&12.13& 1.11&14.23  & 0.852& 0.822& 0.880& 0.797& 0.907\\
 HIP 50319& 6.44& 6.03& 6.74& 5.75& 7.14  & 1.152& 1.131& 1.173& 1.108& 1.196\\
 HIP 50355& 7.02& 5.47& 8.11& 3.82& 9.28  & 0.979& 0.964& 0.998& 0.949& 1.021\\
 HIP 50671& 7.44& 5.51& 8.30& 4.04& 9.59  & 0.934& 0.918& 0.960& 0.897& 0.985\\
 HIP 50965&10.16& 5.14&10.87& 1.86&12.69  & 0.909& 0.881& 0.947& 0.851& 0.982\\
 HIP 51128& 2.57& 1.09& 4.22& 0.47& 5.84  & 1.025& 1.004& 1.043& 0.984& 1.061\\
 HIP 51248&12.03&10.18&13.70& 8.27&14.56  & 0.871& 0.857& 0.912& 0.838& 0.941\\
 HIP 51406& 3.03& 2.67& 3.43& 2.28& 3.78  & 1.351& 1.318& 1.443& 1.272& 1.500\\
 HIP 51459& 0.80& 0.67& 3.05& 0.42& 4.08  & 1.111& 1.100& 1.155& 1.080& 1.165\\
 HIP 51477&11.94&10.75&13.12& 9.65&14.27  & 0.861& 0.833& 0.891& 0.809& 0.923\\
 HIP 51784& 4.51& 3.70& 5.26& 3.09& 6.03  & 1.107& 1.069& 1.122& 1.046& 1.142\\
 HIP 51933& 5.60& 5.50& 6.36& 4.91& 6.64  & 1.094& 1.070& 1.111& 1.050& 1.139\\
 HIP 51993& 5.24& 4.47& 6.72& 3.76& 8.01  & 1.204& 1.137& 1.284& 1.079& 1.357\\
 HIP 52015& 7.01& 5.96& 7.39& 5.34& 8.07  & 1.147& 1.109& 1.186& 1.076& 1.233\\
 HIP 52040& 2.22& 1.43& 5.53& 0.65& 7.37  & 0.991& 0.966& 1.004& 0.948& 1.023\\
 HIP 52137& 1.95& 1.20& 4.53& 0.51& 6.33  & 1.022& 0.998& 1.036& 0.979& 1.056\\
 HIP 52153& 9.28& 8.78&10.01& 8.15&10.68  & 0.995& 0.971& 1.017& 0.951& 1.044\\
 HIP 52325&13.14& 9.02&13.88& 4.80&14.52  & 0.873& 0.857& 0.902& 0.837& 0.929\\
 HIP 52673&10.16& 4.48&12.43& 1.49&14.26  & 0.812& 0.789& 0.847& 0.769& 0.876\\
 HIP 52761& 6.35& 3.08& 8.84& 1.10&11.13  & 0.968& 0.937& 0.999& 0.909& 1.030\\
 HIP 52771&13.14& 5.45&13.33& 1.71&14.44  & 0.720& 0.710& 0.749& 0.699& 0.771\\
 HIP 52990& 6.21& 5.17& 6.83& 4.61& 7.43  & 1.089& 1.081& 1.135& 1.064& 1.161\\
 HIP 53049& 4.65& 2.72& 6.38& 1.08& 8.13  & 0.997& 0.967& 1.034& 0.936& 1.069\\
 HIP 53229& 3.62& 3.10& 7.59& 2.15&11.20  & 1.326& 1.119& 1.470& 1.002& 1.663\\
 HIP 53535& 6.10& 4.47& 6.17& 3.96& 6.77  & 1.221& 1.168& 1.273& 1.132& 1.326\\
 HIP 53537& 5.84& 4.36& 7.01& 3.09& 8.17  & 1.062& 1.028& 1.078& 1.007& 1.099\\
 HIP 53721& 6.33& 4.99& 7.27& 3.87& 8.44  & 1.056& 1.037& 1.078& 1.014& 1.100\\
 HIP 53725&11.78&10.21&12.73& 8.60&13.71  & 0.883& 0.865& 0.899& 0.850& 0.915\\
 HIP 53898& 7.58& 5.03& 8.75& 2.84&10.34  & 0.941& 0.927& 0.963& 0.911& 0.985\\
 HIP 54196& 8.72& 8.14& 9.40& 7.52&10.06  & 0.995& 0.975& 1.019& 0.953& 1.041\\
 HIP 54239& 8.55& 5.29&10.60& 2.19&12.16  & 0.896& 0.872& 0.925& 0.849& 0.954\\
 HIP 54582& 9.01& 8.28& 9.95& 7.46&10.57  & 0.990& 0.973& 1.009& 0.956& 1.028\\
 HIP 54728& 6.35& 4.10& 7.16& 2.28& 8.35  & 1.004& 0.991& 1.027& 0.976& 1.048\\
HIP 55288A& 2.86& 2.25& 4.18& 1.05& 5.37  & 1.235& 1.189& 1.263& 1.150& 1.302\\
HIP 55288B& 8.91& 6.94&10.45& 4.55&11.90  & 0.986& 0.967& 1.021& 0.944& 1.050\\
 HIP 55459& 8.50& 7.59& 9.78& 6.53&10.82  & 0.965& 0.957& 0.986& 0.943& 0.999\\
 HIP 55592&10.16& 4.78&10.44& 1.63&11.93  & 0.873& 0.849& 0.898& 0.824& 0.929\\
 HIP 55666& 5.15& 4.76& 5.53& 3.64& 5.87  & 1.162& 1.136& 1.183& 1.117& 1.254\\
 HIP 55761&10.03& 8.26&11.44& 6.46&12.88  & 0.876& 0.853& 0.897& 0.834& 0.920\\
 HIP 56148& 2.68& 2.53& 2.83& 2.47& 2.89  & 1.436& 1.411& 1.452& 1.390& 1.472\\
 HIP 56186& 4.66& 3.66& 5.90& 2.67& 6.90  & 1.042& 1.015& 1.072& 0.989& 1.100\\
 HIP 56290& 5.16& 4.83& 5.30& 4.70& 5.62  & 1.156& 1.140& 1.178& 1.122& 1.197\\
 HIP 56423& 7.64& 6.67& 8.76& 5.46& 9.75  & 0.977& 0.954& 1.004& 0.932& 1.032\\
 HIP 56452& 7.92& 3.64&11.76& 1.23&14.14  & 0.774& 0.748& 0.800& 0.731& 0.821\\
 HIP 56948& 7.16& 4.66& 8.09& 2.72& 9.45  & 0.995& 0.979& 1.021& 0.961& 1.044\\
 HIP 56960& 1.67& 0.98& 3.38& 0.42& 5.09  & 1.084& 1.068& 1.121& 1.036& 1.143\\
 HIP 56997& 2.15& 1.77& 5.76& 0.00& 7.96  & 0.930& 0.904& 0.951& 0.881& 0.967\\
 HIP 57080& 6.06& 5.63& 6.60& 5.11& 7.05  & 1.049& 1.031& 1.077& 1.009& 1.098\\
 HIP 57117& 2.75& 2.41& 3.32& 2.03& 3.84  & 1.422& 1.392& 1.554& 1.321& 1.643\\
 HIP 57300& 7.07& 6.01& 7.56& 4.78& 8.26  & 1.015& 0.993& 1.046& 0.969& 1.076\\
 HIP 57349&12.04&10.66&12.68& 9.49&13.56  & 0.882& 0.865& 0.902& 0.848& 0.920\\
 HIP 57443& 9.68& 7.15&12.02& 4.45&14.07  & 0.884& 0.856& 0.908& 0.835& 0.940\\
 HIP 57450&-1.00& 6.07&13.57& 2.04&14.48  & 0.721& 0.708& 0.748& 0.694& 0.774\\
 HIP 57532& 8.67& 6.13&11.18& 3.55&13.28  & 0.965& 0.934& 0.997& 0.903& 1.026\\
 HIP 57617& 6.47& 6.17& 7.35& 5.66& 8.02  & 1.061& 1.033& 1.084& 1.008& 1.109\\
 HIP 57757& 3.50& 3.38& 4.76& 3.13& 5.06  & 1.298& 1.228& 1.311& 1.208& 1.327\\
 HIP 57939&13.88& 6.44&13.48& 2.96&14.46  & 0.619& 0.614& 0.642& 0.608& 0.657\\
 HIP 58171& 5.56& 2.55& 7.68& 0.77& 9.39  & 0.993& 0.973& 1.016& 0.956& 1.034\\
 HIP 58201& 2.02& 1.05& 3.37& 0.39& 4.43  & 1.104& 1.087& 1.123& 1.070& 1.148\\
 HIP 58229& 7.17& 4.87& 8.14& 2.01& 9.38  & 0.953& 0.920& 1.024& 0.881& 1.127\\
 HIP 58331& 3.86& 3.55& 4.04& 3.46& 4.27  & 1.304& 1.274& 1.326& 1.251& 1.350\\
 HIP 58576& 7.93& 6.15& 9.95& 4.66&11.73  & 0.977& 0.949& 1.002& 0.923& 1.021\\
 HIP 58843&13.14& 7.20&13.42& 3.01&14.45  & 0.798& 0.788& 0.835& 0.772& 0.865\\
 HIP 59021& 4.05& 3.64& 4.35& 3.33& 4.77  & 1.278& 1.258& 1.336& 1.225& 1.374\\
 HIP 59233&-1.00& 9.44&14.11& 6.24&14.56  & 0.748& 0.732& 0.762& 0.720& 0.781\\
 HIP 59253& 6.19& 3.45& 7.54& 1.40& 9.27  & 1.001& 0.980& 1.029& 0.959& 1.053\\
 HIP 59532& 6.88& 5.69& 8.29& 4.69& 9.51  & 1.018& 0.991& 1.037& 0.972& 1.053\\
 HIP 59589& 9.23& 8.15&10.79& 6.70&12.06  & 0.925& 0.907& 0.938& 0.892& 0.953\\
 HIP 59735& 8.67& 6.58&10.80& 3.96&12.46  & 0.913& 0.885& 0.939& 0.862& 0.968\\
 HIP 59750& 5.57& 4.24& 6.15& 3.38& 7.04  & 0.958& 0.939& 0.973& 0.922& 0.993\\
 HIP 60019& 6.40& 5.84& 6.60& 5.42& 7.00  & 1.100& 1.079& 1.128& 1.055& 1.155\\
 HIP 60268&-1.00&11.25&14.24& 9.21&14.67  & 0.783& 0.773& 0.804& 0.764& 0.825\\
 HIP 60314& 5.77& 2.93& 7.10& 1.03& 8.78  & 1.012& 0.996& 1.047& 0.976& 1.071\\
 HIP 60331&13.14& 3.94&12.82& 1.23&14.37  & 0.791& 0.759& 0.838& 0.726& 0.882\\
 HIP 60366& 0.56& 0.62& 2.86& 0.31& 4.22  & 1.072& 1.047& 1.086& 1.029& 1.103\\
 HIP 60588& 9.49& 8.63& 9.92& 7.98&10.48  & 0.961& 0.945& 0.980& 0.927& 0.998\\
 HIP 60719&-1.00& 0.00&15.00& 0.00&15.00  & 0.000& 0.000& 0.000& 0.000& 0.000\\
 HIP 60956&-1.00& 9.19&13.96& 5.21&14.53  & 0.759& 0.748& 0.785& 0.734& 0.810\\
 HIP 61044& 4.01& 2.72& 4.90& 1.36& 6.24  & 1.116& 1.091& 1.132& 1.067& 1.155\\
 HIP 61157& 3.92& 3.57& 4.16& 3.34& 4.50  & 1.275& 1.237& 1.306& 1.207& 1.339\\
 HIP 61264& 6.61& 6.23& 7.48& 5.61& 8.24  & 1.035& 1.004& 1.072& 0.971& 1.111\\
 HIP 61272&14.21&11.30&14.23& 9.20&14.67  & 0.894& 0.877& 0.916& 0.861& 0.939\\
 HIP 61293& 3.42& 3.21& 3.78& 2.84& 4.00  & 1.162& 1.150& 1.174& 1.139& 1.185\\
 HIP 61317& 6.81& 4.29& 8.18& 2.74& 9.59  & 0.969& 0.954& 1.011& 0.931& 1.039\\
 HIP 62039& 8.45& 6.38& 9.82& 4.74&11.33  & 0.985& 0.966& 1.021& 0.945& 1.048\\
 HIP 62077&11.67& 9.55&12.50& 6.11&13.71  & 0.882& 0.866& 0.918& 0.845& 0.955\\
 HIP 62162& 8.20& 7.56& 9.00& 6.99& 9.80  & 0.971& 0.945& 0.993& 0.923& 1.017\\
 HIP 62175& 4.88& 3.92& 6.51& 2.50& 7.66  & 1.029& 1.009& 1.048& 0.992& 1.067\\
 HIP 62198& 8.60& 5.60& 9.46& 2.68&10.76  & 0.998& 0.977& 1.026& 0.956& 1.053\\
 HIP 62240& 9.41& 7.49&10.76& 4.38&12.26  & 0.949& 0.917& 0.986& 0.885& 1.026\\
 HIP 62307& 5.92& 5.01& 6.58& 4.23& 7.30  & 1.096& 1.058& 1.157& 1.018& 1.218\\
 HIP 62507& 9.55& 8.33& 9.91& 7.52&10.77  & 1.001& 0.970& 1.028& 0.946& 1.064\\
 HIP 62527& 6.01& 5.00& 7.30& 4.11& 8.29  & 1.049& 1.029& 1.079& 1.010& 1.098\\
 HIP 62607&-1.00& 9.84&14.02& 6.89&14.55  & 0.764& 0.753& 0.787& 0.742& 0.811\\
 HIP 62661& 6.32& 4.86& 6.76& 4.15& 7.62  & 1.092& 1.084& 1.150& 1.061& 1.181\\
 HIP 62816& 2.58& 1.41& 5.03& 0.50& 6.70  & 1.023& 0.993& 1.039& 0.971& 1.059\\
 HIP 62882& 9.78& 7.85&12.00& 6.06&13.93  & 0.897& 0.853& 0.971& 0.815& 1.046\\
 HIP 63330& 4.90& 3.80& 5.05& 3.43& 5.51  & 1.265& 1.204& 1.293& 1.179& 1.321\\
 HIP 63354& 5.24& 2.98& 6.21& 1.38& 7.49  & 0.991& 0.975& 1.028& 0.952& 1.052\\
 HIP 63405& 3.35& 3.23& 3.83& 2.62& 4.08  & 1.281& 1.247& 1.336& 1.215& 1.404\\
 HIP 63881& 8.66& 6.90& 9.64& 5.23&10.61  & 1.003& 0.984& 1.030& 0.965& 1.056\\
 HIP 64103& 4.94& 2.56& 9.32& 0.93&12.37  & 0.922& 0.891& 0.945& 0.865& 0.969\\
 HIP 64150& 7.14& 5.85& 8.46& 4.50& 9.70  & 0.984& 0.972& 1.011& 0.956& 1.035\\
 HIP 64241& 3.75& 2.89& 4.00& 2.57& 4.36  & 1.256& 1.230& 1.337& 1.193& 1.368\\
 HIP 64254& 7.58& 3.93& 9.29& 1.41&11.04  & 0.923& 0.908& 0.949& 0.889& 0.973\\
 HIP 64344& 7.66& 4.17& 8.53& 1.73& 9.95  & 0.990& 0.968& 1.020& 0.947& 1.052\\
 HIP 64394& 0.89& 0.89& 3.27& 0.56& 4.72  & 1.131& 1.087& 1.134& 1.060& 1.143\\
 HIP 64407& 2.56& 2.34& 2.80& 2.24& 2.89  & 1.484& 1.423& 1.523& 1.395& 1.556\\
 HIP 64426&12.15&11.45&13.56&10.46&14.45  & 0.844& 0.830& 0.866& 0.814& 0.885\\
 HIP 64497& 3.51& 1.62& 5.19& 0.57& 6.86  & 1.057& 1.033& 1.078& 1.008& 1.099\\
 HIP 64583& 4.65& 3.56& 4.76& 3.13& 5.34  & 1.160& 1.124& 1.193& 1.092& 1.220\\
 HIP 64698&10.51& 8.59&11.75& 6.19&12.91  & 0.924& 0.911& 0.939& 0.897& 0.953\\
 HIP 64792& 4.27& 3.93& 5.48& 3.42& 6.30  & 1.164& 1.127& 1.182& 1.097& 1.199\\
 HIP 64794& 6.95& 4.39& 8.02& 2.21& 9.21  & 0.982& 0.968& 1.000& 0.954& 1.020\\
 HIP 64797& 7.18& 2.91&11.20& 0.93&13.98  & 0.786& 0.752& 0.797& 0.735& 0.812\\
 HIP 64924& 9.18& 6.51&10.49& 4.41&12.51  & 0.917& 0.903& 0.945& 0.884& 0.971\\
 HIP 65049&10.62& 8.71&11.68& 7.02&12.89  & 0.992& 0.964& 1.018& 0.939& 1.054\\
 HIP 65449&11.32& 9.13&13.07& 7.26&14.32  & 0.949& 0.911& 1.017& 0.877& 1.087\\
 HIP 65641& 6.24& 3.64& 7.88& 1.55& 9.56  & 0.974& 0.960& 1.003& 0.942& 1.025\\
 HIP 65708&10.02& 9.04&10.38& 8.36&10.97  & 0.997& 0.981& 1.010& 0.967& 1.024\\
 HIP 65971& 5.54& 4.16& 8.55& 2.06&10.65  & 0.942& 0.914& 0.978& 0.884& 1.012\\
 HIP 65982&13.14& 4.46&13.14& 1.38&14.42  & 0.798& 0.764& 0.842& 0.730& 0.904\\
 HIP 66051&11.02&10.35&11.86& 9.68&12.71  & 0.902& 0.887& 0.928& 0.869& 0.948\\
 HIP 66464& 5.79& 4.22& 6.60& 2.69& 7.53  & 1.007& 0.982& 1.026& 0.962& 1.049\\
 HIP 66514&11.45&10.43&11.85& 9.55&12.63  & 0.962& 0.945& 0.977& 0.930& 0.995\\
 HIP 66860& 2.00& 1.64& 2.47& 1.02& 2.90  & 1.292& 1.266& 1.312& 1.246& 1.335\\
 HIP 66974& 5.55& 5.09& 5.94& 4.67& 6.41  & 1.209& 1.167& 1.226& 1.142& 1.260\\
 HIP 67422&13.14& 3.89&12.81& 1.20&14.37  & 0.688& 0.664& 0.715& 0.641& 0.741\\
 HIP 67927& 2.48& 2.18& 2.90& 1.97& 2.99  & 1.538& 1.528& 1.648& 1.495& 1.696\\
 HIP 68030& 6.09& 4.80& 6.38& 4.09& 7.16  & 1.015& 1.000& 1.041& 0.980& 1.064\\
 HIP 68085& 9.75& 9.07&10.29& 8.54&10.91  & 1.009& 0.990& 1.030& 0.971& 1.050\\
 HIP 68184&13.89& 4.24&12.73& 1.68&14.36  & 0.772& 0.757& 0.800& 0.745& 0.820\\
 HIP 68594&-1.00& 0.00&15.00& 0.00&15.00  & 0.000& 0.000& 0.000& 0.000& 0.000\\
 HIP 69210& 1.94& 1.05& 4.01& 0.45& 5.36  & 1.073& 1.045& 1.082& 1.025& 1.100\\
 HIP 69232&13.14& 6.97&13.71& 2.40&14.50  & 0.837& 0.799& 0.909& 0.765& 1.044\\
 HIP 69535& 5.10& 4.13& 5.52& 3.58& 6.03  & 1.097& 1.078& 1.131& 1.055& 1.163\\
 HIP 69673&12.69& 7.74&13.47& 5.04&14.51  & 0.901& 0.893& 1.054& 0.870& 1.194\\
 HIP 69701& 2.60& 2.54& 2.83& 2.32& 2.89  & 1.438& 1.413& 1.479& 1.386& 1.583\\
 HIP 69972& 8.67& 3.80&12.26& 1.24&14.24  & 0.828& 0.801& 0.851& 0.783& 0.870\\
 HIP 70319& 9.11& 7.40&10.68& 5.60&12.17  & 0.867& 0.855& 0.893& 0.837& 0.914\\
 HIP 70324&13.14& 7.02&13.33& 2.95&14.43  & 0.845& 0.824& 0.877& 0.802& 0.910\\
 HIP 70520&11.25&10.48&11.99& 9.75&12.81  & 0.903& 0.883& 0.921& 0.866& 0.940\\
 HIP 70681& 6.43& 2.94&11.09& 1.05&13.86  & 0.739& 0.711& 0.756& 0.694& 0.769\\
 HIP 71019&14.59&12.74&14.57&11.33&14.82  & 0.898& 0.884& 0.927& 0.870& 0.961\\
 HIP 71076& 7.17& 5.93& 7.89& 4.90& 8.80  & 1.006& 0.986& 1.035& 0.962& 1.061\\
 HIP 71193&14.16&12.42&14.45&11.00&14.78  & 0.894& 0.880& 0.907& 0.869& 0.923\\
 HIP 71284& 2.11& 1.23& 2.44& 0.79& 2.92  & 1.229& 1.208& 1.261& 1.180& 1.289\\
 HIP 71572&14.12&11.60&14.24& 9.54&14.64  & 0.873& 0.860& 0.905& 0.840& 0.931\\
 HIP 71681& 3.45& 2.12& 9.39& 0.86&13.17  & 0.905& 0.866& 0.923& 0.839& 0.941\\
 HIP 71683& 4.75& 3.57& 7.05& 2.22& 8.80  & 1.110& 1.066& 1.128& 1.030& 1.154\\
 HIP 71819& 9.17& 7.87&10.05& 6.75&11.10  & 0.994& 0.974& 1.026& 0.951& 1.052\\
 HIP 72199& 5.29& 4.34& 6.05& 3.68& 6.97  & 1.205& 1.144& 1.275& 1.093& 1.346\\
 HIP 72407&13.16& 9.52&13.76& 6.11&14.51  & 0.842& 0.830& 0.872& 0.812& 0.899\\
 HIP 72467& 3.40& 2.76& 3.64& 2.44& 3.97  & 1.354& 1.298& 1.414& 1.244& 1.469\\
 HIP 72604&12.21&10.02&12.96& 8.47&14.18  & 0.919& 0.901& 0.938& 0.884& 0.958\\
 HIP 72659& 7.23& 2.52& 9.56& 1.06&13.27  & 0.873& 0.841& 0.901& 0.813& 0.918\\
 HIP 72803& 6.19& 4.72& 7.53& 3.60& 9.18  & 1.083& 1.025& 1.173& 0.965& 1.269\\
 HIP 72835& 4.42& 3.53& 5.10& 2.70& 5.89  & 1.078& 1.052& 1.102& 1.028& 1.125\\
 HIP 72848&10.19& 5.29&11.81& 2.63&13.96  & 0.857& 0.833& 0.886& 0.815& 0.912\\
 HIP 73005&13.92& 9.75&13.97& 6.76&14.55  & 0.756& 0.747& 0.778& 0.737& 0.800\\
 HIP 73078& 9.69& 8.75&10.66& 7.86&11.54  & 1.034& 1.015& 1.075& 0.990& 1.109\\
 HIP 73385&13.24&11.30&14.06& 9.71&14.69  & 0.810& 0.794& 0.854& 0.784& 0.893\\
 HIP 73440&10.85&10.44&11.33&10.05&11.81  & 0.934& 0.917& 0.949& 0.900& 0.964\\
 HIP 73695& 8.21& 5.53& 9.84& 3.28&11.72  & 0.968& 0.937& 0.999& 0.911& 1.037\\
 HIP 73768& 6.55& 5.63& 7.28& 4.91& 8.20  & 1.078& 1.036& 1.125& 0.997& 1.177\\
 HIP 73815& 8.15& 7.07& 8.80& 6.12& 9.56  & 1.015& 1.000& 1.032& 0.984& 1.048\\
 HIP 74033&12.11&10.75&13.60& 9.30&14.54  & 0.865& 0.840& 0.907& 0.819& 0.947\\
 HIP 74067&11.51& 9.51&13.48& 7.20&14.48  & 0.792& 0.779& 0.815& 0.767& 0.837\\
 HIP 74079&10.85&10.07&11.87& 9.31&12.84  & 0.887& 0.871& 0.916& 0.851& 0.938\\
 HIP 74326&10.16& 7.15&11.24& 4.32&12.90  & 0.925& 0.896& 0.945& 0.873& 0.972\\
 HIP 74341& 6.54& 3.34& 7.80& 1.16& 9.32  & 1.009& 0.988& 1.032& 0.970& 1.056\\
 HIP 74442& 7.29& 6.71& 8.22& 6.09& 8.93  & 1.068& 1.039& 1.100& 1.010& 1.135\\
 HIP 74443&13.14& 4.85&13.01& 1.64&14.39  & 0.729& 0.720& 0.759& 0.707& 0.779\\
 HIP 74933& 8.19& 7.77& 9.29& 6.90&10.13  & 0.978& 0.956& 1.017& 0.930& 1.054\\
 HIP 75206& 2.35& 2.15& 2.62& 2.02& 2.69  & 1.511& 1.500& 1.618& 1.489& 1.648\\
 HIP 75281&11.84& 9.39&12.91& 7.49&14.19  & 0.898& 0.881& 0.926& 0.863& 0.949\\
 HIP 75370&12.59& 9.52&13.62& 6.78&14.50  & 0.821& 0.814& 0.848& 0.800& 0.869\\
 HIP 76219& 6.23& 4.29& 9.69& 2.97&13.08  & 1.135& 1.053& 1.329& 0.970& 1.484\\
 HIP 76543& 7.50& 7.39& 8.31& 6.96& 8.93  & 0.991& 0.973& 1.013& 0.954& 1.034\\
 HIP 76556& 5.10& 3.85& 5.33& 3.49& 5.91  & 1.166& 1.146& 1.230& 1.114& 1.265\\
 HIP 76899& 9.31& 8.61&10.11& 7.76&10.96  & 1.004& 0.974& 1.031& 0.950& 1.066\\
 HIP 76911&10.16& 6.02&11.95& 2.84&13.91  & 0.907& 0.881& 0.937& 0.858& 0.972\\
 HIP 76963& 7.50& 6.95& 7.80& 6.51& 8.23  & 1.057& 1.039& 1.076& 1.021& 1.095\\
 HIP 76976&-1.00& 0.00&15.00& 0.00&15.00  & 0.000& 0.000& 0.000& 0.000& 0.000\\
 HIP 77083& 5.11& 2.65& 7.25& 0.98& 9.05  & 0.998& 0.971& 1.020& 0.950& 1.045\\
 HIP 77159& 8.57& 7.36& 9.68& 6.30&10.75  & 1.041& 0.996& 1.083& 0.961& 1.133\\
 HIP 77257& 7.20& 5.77& 7.43& 4.89& 8.11  & 1.071& 1.060& 1.106& 1.044& 1.139\\
 HIP 77358& 6.04& 4.75& 7.35& 3.46& 8.56  & 0.954& 0.945& 0.983& 0.929& 1.002\\
 HIP 77466&11.65& 8.60&13.11& 5.59&14.35  & 0.873& 0.852& 0.903& 0.831& 0.931\\
 HIP 77655& 4.11& 3.14& 7.58& 2.48&11.41  & 1.346& 1.146& 1.498& 1.019& 1.654\\
 HIP 78028& 4.23& 2.32& 6.37& 0.95& 8.01  & 0.977& 0.956& 1.002& 0.936& 1.024\\
 HIP 78030& 7.10& 6.05& 7.89& 5.23& 8.75  & 1.138& 1.104& 1.198& 1.068& 1.253\\
 HIP 78072& 4.50& 3.10& 4.53& 2.72& 5.09  & 1.227& 1.154& 1.227& 1.125& 1.244\\
 HIP 78640&10.16& 6.60&11.41& 3.14&13.00  & 0.827& 0.807& 0.860& 0.784& 0.888\\
 HIP 78680& 3.24& 1.85& 6.23& 0.70& 8.20  & 0.996& 0.963& 1.022& 0.940& 1.044\\
 HIP 78747& 2.69& 2.37& 3.84& 1.90& 4.47  & 1.256& 1.192& 1.346& 1.134& 1.388\\
 HIP 78775&-1.00&10.75&14.22& 8.03&14.61  & 0.734& 0.725& 0.752& 0.717& 0.774\\
 HIP 79186&10.42& 8.88&11.41& 7.56&12.51  & 0.952& 0.935& 0.970& 0.918& 0.988\\
 HIP 79190& 8.67& 4.72&12.37& 1.87&14.26  & 0.745& 0.730& 0.772& 0.718& 0.790\\
 HIP 79276&10.65& 8.90&12.67& 7.12&14.10  & 0.889& 0.873& 0.911& 0.856& 0.930\\
 HIP 79304& 3.80& 2.10& 5.72& 0.71& 7.11  & 1.054& 1.027& 1.065& 1.008& 1.081\\
 HIP 79448&14.27&13.12&14.58&12.28&14.85  & 0.897& 0.886& 0.923& 0.875& 0.947\\
 HIP 79545&12.24&10.93&12.86&10.03&13.89  & 0.883& 0.857& 0.904& 0.836& 0.929\\
 HIP 79672& 4.47& 3.10& 6.32& 1.57& 7.67  & 1.003& 0.983& 1.033& 0.966& 1.059\\
 HIP 79837&14.44&12.24&14.39&10.66&14.75  & 0.865& 0.850& 0.889& 0.835& 0.915\\
 HIP 80162&13.14& 5.32&13.37& 1.75&14.45  & 0.714& 0.700& 0.738& 0.685& 0.760\\
 HIP 80264& 6.43& 6.02& 7.18& 5.31& 7.71  & 1.040& 1.025& 1.066& 1.006& 1.087\\
 HIP 80337& 0.67& 0.85& 3.71& 0.42& 5.40  & 1.050& 1.012& 1.055& 0.987& 1.068\\
 HIP 80686& 2.08& 1.66& 5.05& 0.69& 6.65  & 1.087& 1.035& 1.096& 1.009& 1.124\\
 HIP 80736& 5.41& 4.59& 5.91& 4.08& 6.71  & 1.255& 1.206& 1.316& 1.158& 1.371\\
 HIP 80742& 9.87& 8.74&11.44& 7.42&12.69  & 0.917& 0.897& 0.938& 0.878& 0.958\\
 HIP 80818& 6.03& 5.74& 6.34& 5.46& 6.60  & 1.137& 1.122& 1.158& 1.106& 1.175\\
 HIP 80837&11.38&10.79&12.22&10.09&12.94  & 0.875& 0.860& 0.893& 0.844& 0.912\\
 HIP 81072& 2.78& 2.70& 3.85& 2.34& 4.33  & 1.289& 1.229& 1.343& 1.180& 1.395\\
 HIP 81300& 6.66& 3.44& 9.64& 1.39&12.87  & 0.859& 0.830& 0.883& 0.806& 0.906\\
 HIP 81312& 6.07& 4.90& 6.86& 3.96& 7.72  & 1.040& 1.016& 1.069& 0.993& 1.097\\
 HIP 81461&11.48&10.65&12.66& 9.74&13.72  & 0.906& 0.879& 0.938& 0.852& 0.968\\
 HIP 81512& 5.66& 3.58& 7.50& 1.57& 8.90  & 0.975& 0.962& 0.999& 0.949& 1.019\\
 HIP 81608& 3.06& 2.68& 3.49& 2.46& 3.67  & 1.409& 1.390& 1.497& 1.360& 1.541\\
 HIP 81681&12.11&10.26&13.24& 8.71&14.34  & 0.865& 0.848& 0.884& 0.833& 0.903\\
 HIP 81693& 3.19& 3.08& 3.30& 3.04& 3.34  & 1.443& 1.424& 1.455& 1.412& 1.473\\
 HIP 81748& 9.79& 7.82&10.32& 6.30&11.37  & 0.988& 0.970& 1.019& 0.951& 1.051\\
 HIP 82265&10.16& 6.71&11.97& 3.86&13.80  & 0.916& 0.894& 0.953& 0.872& 0.983\\
 HIP 82268& 5.37& 3.54& 7.26& 1.54& 8.75  & 1.004& 0.980& 1.024& 0.961& 1.043\\
 HIP 82621& 7.54& 7.17& 7.87& 6.85& 8.22  & 1.114& 1.100& 1.134& 1.085& 1.151\\
 HIP 82629& 3.50& 3.49& 4.78& 3.30& 5.20  & 1.208& 1.171& 1.235& 1.142& 1.266\\
 HIP 82708& 3.00& 2.86& 4.11& 2.64& 4.41  & 1.397& 1.325& 1.432& 1.284& 1.464\\
 HIP 82750& 9.20& 8.87& 9.59& 8.42& 9.96  & 1.026& 1.017& 1.037& 1.007& 1.050\\
 HIP 82935& 5.35& 4.00& 5.62& 3.30& 6.29  & 1.107& 1.084& 1.144& 1.058& 1.181\\
 HIP 83058& 3.54& 2.57& 5.06& 1.14& 6.20  & 1.141& 1.096& 1.165& 1.059& 1.198\\
 HIP 83069& 5.43& 4.25& 5.95& 3.68& 6.71  & 1.091& 1.072& 1.133& 1.049& 1.162\\
 HIP 83204& 7.60& 7.27& 8.38& 6.64& 8.98  & 0.987& 0.974& 1.001& 0.961& 1.014\\
 HIP 83489&11.65& 6.81&12.18& 2.90&13.61  & 0.902& 0.878& 0.927& 0.855& 0.953\\
 HIP 83601& 3.15& 2.42& 3.97& 1.55& 5.02  & 1.084& 1.065& 1.096& 1.043& 1.115\\
 HIP 84217& 2.82& 2.52& 3.15& 2.26& 3.37  & 1.427& 1.412& 1.523& 1.377& 1.574\\
 HIP 84405&11.67& 5.52&13.05& 1.71&14.40  & 0.754& 0.746& 0.788& 0.735& 0.812\\
 HIP 84478&13.14& 3.79&12.75& 1.17&14.36  & 0.646& 0.626& 0.674& 0.605& 0.699\\
 HIP 84506& 6.42& 5.56& 6.93& 4.83& 7.58  & 1.160& 1.128& 1.213& 1.093& 1.263\\
 HIP 84551& 2.19& 1.96& 2.55& 1.75& 2.64  & 1.570& 1.559& 1.666& 1.533& 1.711\\
 HIP 84696& 3.62& 3.47& 4.98& 2.86& 5.65  & 1.190& 1.149& 1.231& 1.114& 1.272\\
 HIP 84720&13.15& 6.04&13.24& 2.25&14.43  & 0.772& 0.769& 0.820& 0.757& 0.851\\
 HIP 84781& 8.25& 7.03&10.32& 5.70&12.25  & 1.035& 0.992& 1.106& 0.943& 1.172\\
 HIP 84803& 7.44& 5.90&10.56& 4.17&13.06  & 0.995& 0.947& 1.122& 0.885& 1.239\\
 HIP 84824& 6.29& 5.06& 7.45& 3.62& 8.48  & 1.006& 0.985& 1.025& 0.967& 1.048\\
 HIP 84862&13.13&10.59&13.50& 9.05&14.64  & 0.869& 0.860& 0.903& 0.845& 0.926\\
 HIP 85007& 6.07& 4.61& 7.53& 3.05& 8.96  & 0.973& 0.942& 0.990& 0.919& 1.018\\
 HIP 85042& 5.88& 3.73& 8.40& 1.55&10.74  & 0.992& 0.961& 1.024& 0.936& 1.055\\
 HIP 85090& 3.75& 3.42& 4.30& 3.05& 4.76  & 1.335& 1.291& 1.406& 1.245& 1.461\\
 HIP 85235& 8.67& 5.16&12.33& 2.26&14.25  & 0.775& 0.753& 0.808& 0.737& 0.832\\
 HIP 85378&12.48&11.72&13.40&10.94&14.24  & 0.877& 0.854& 0.899& 0.835& 0.923\\
 HIP 85400& 9.25& 8.75&10.66& 7.91&11.66  & 0.967& 0.941& 1.003& 0.914& 1.037\\
 HIP 85650& 9.89& 6.51&10.47& 2.88&11.65  & 0.946& 0.928& 0.969& 0.909& 0.993\\
 HIP 85653&-1.00&11.12&14.26& 8.76&14.66  & 0.797& 0.788& 0.818& 0.779& 0.839\\
 HIP 85757& 8.49& 7.76&10.41& 6.63&11.81  & 0.969& 0.937& 1.026& 0.900& 1.077\\
 HIP 85940& 5.50& 4.76& 5.90& 4.19& 6.47  & 1.189& 1.146& 1.234& 1.107& 1.283\\
 HIP 85964& 4.65& 3.61& 4.86& 3.20& 5.21  & 1.222& 1.206& 1.303& 1.182& 1.342\\
 HIP 86013&-1.00&11.35&14.30& 8.99&14.68  & 0.797& 0.787& 0.821& 0.775& 0.842\\
 HIP 86036& 5.33& 4.08& 7.21& 2.61& 8.72  & 1.030& 1.011& 1.065& 0.985& 1.093\\
 HIP 86225& 3.40& 2.95& 4.21& 2.46& 4.77  & 1.332& 1.254& 1.446& 1.185& 1.546\\
 HIP 86321& 6.16& 2.74& 6.73& 0.92& 7.90  & 0.962& 0.932& 0.979& 0.909& 1.006\\
 HIP 86382& 3.36& 3.10& 3.65& 2.71& 4.02  & 1.314& 1.288& 1.370& 1.246& 1.422\\
 HIP 86400&14.08&11.27&14.30& 8.34&14.64  & 0.756& 0.754& 0.777& 0.750& 0.796\\
 HIP 86431&10.35& 8.16&10.70& 6.75&11.78  & 0.891& 0.875& 0.914& 0.856& 0.934\\
 HIP 86568& 6.43& 3.17&11.18& 1.10&13.91  & 0.811& 0.791& 0.836& 0.772& 0.856\\
 HIP 86796& 8.18& 5.85& 8.18& 5.22& 8.94  & 1.075& 1.073& 1.150& 1.053& 1.168\\
 HIP 86830&12.39& 9.88&13.83& 7.85&14.63  & 0.904& 0.883& 0.977& 0.866& 1.043\\
 HIP 86974& 7.88& 7.52& 8.28& 7.23& 8.54  & 1.135& 1.101& 1.140& 1.081& 1.157\\
 HIP 87055& 8.15& 6.02& 9.20& 4.04&10.46  & 0.931& 0.923& 0.951& 0.910& 0.970\\
 HIP 87089&-1.00& 8.37&13.88& 4.15&14.53  & 0.752& 0.740& 0.774& 0.726& 0.797\\
 HIP 87533& 7.90& 7.32& 8.66& 6.73& 9.34  & 1.044& 1.024& 1.080& 0.999& 1.110\\
 HIP 87732& 4.40& 3.93& 4.97& 3.42& 5.49  & 1.268& 1.219& 1.321& 1.176& 1.387\\
 HIP 88010&-1.00& 5.24&13.44& 1.66&14.46  & 0.702& 0.688& 0.733& 0.673& 0.759\\
 HIP 88039&10.05& 8.20&11.23& 6.69&12.53  & 0.921& 0.881& 0.980& 0.846& 1.045\\
 HIP 88166&13.14& 4.97&13.05& 1.65&14.40  & 0.740& 0.730& 0.776& 0.715& 0.800\\
 HIP 88194& 8.92& 7.28& 9.59& 6.01&10.73  & 0.951& 0.930& 0.958& 0.916& 0.974\\
 HIP 88427& 8.34& 4.58& 9.27& 1.84&10.64  & 0.956& 0.940& 0.977& 0.923& 0.999\\
 HIP 88601& 3.45& 2.06& 8.33& 0.98&12.11  & 0.897& 0.858& 0.909& 0.830& 0.926\\
 HIP 88745& 8.72& 7.62& 9.58& 6.73&10.37  & 0.942& 0.925& 0.966& 0.906& 0.988\\
 HIP 88766& 1.40& 1.72& 9.82& 0.81&13.74  & 1.096& 1.088& 1.941& 0.989& 2.510\\
 HIP 88945& 3.64& 1.73& 5.52& 0.68& 7.40  & 1.017& 0.972& 1.047& 0.937& 1.079\\
 HIP 88972&-1.00& 7.95&13.68& 3.82&14.51  & 0.750& 0.748& 0.782& 0.740& 0.807\\
 HIP 89268&11.65& 4.19&12.75& 1.29&14.33  & 0.870& 0.846& 0.925& 0.809& 0.980\\
 HIP 89408& 6.71& 6.41& 6.97& 6.15& 7.27  & 1.087& 1.066& 1.104& 1.047& 1.122\\
 HIP 89443& 9.76& 7.69&10.64& 5.59&11.83  & 0.941& 0.929& 0.958& 0.914& 0.974\\
 HIP 89474& 7.74& 7.03& 8.53& 6.36& 9.21  & 1.005& 0.988& 1.016& 0.976& 1.031\\
 HIP 89583&13.14& 9.83&13.92& 6.51&14.53  & 0.854& 0.843& 0.877& 0.828& 0.899\\
 HIP 89937& 6.93& 5.85& 7.94& 4.80& 9.02  & 0.970& 0.952& 1.011& 0.926& 1.046\\
 HIP 90144& 7.98& 7.41& 8.60& 6.83& 9.23  & 1.024& 1.002& 1.044& 0.983& 1.065\\
 HIP 90539&11.65& 7.38&13.08& 3.99&14.38  & 0.845& 0.830& 0.879& 0.812& 0.909\\
 HIP 90542& 9.11& 8.16& 9.84& 7.32&10.61  & 1.048& 1.025& 1.082& 0.999& 1.116\\
 HIP 90655& 5.39& 4.54& 6.51& 3.66& 7.39  & 1.164& 1.127& 1.290& 1.074& 1.398\\
 HIP 90745&10.75& 9.90&11.34& 9.15&12.14  & 0.926& 0.909& 0.949& 0.889& 0.970\\
 HIP 90790& 4.94& 2.66&10.52& 0.98&13.73  & 0.794& 0.767& 0.813& 0.748& 0.826\\
 HIP 90833& 6.91& 4.59& 7.98& 2.77& 9.39  & 0.944& 0.930& 0.969& 0.913& 0.991\\
 HIP 91058& 6.91& 5.70& 7.98& 4.60& 9.04  & 0.997& 0.968& 1.026& 0.943& 1.056\\
 HIP 91120& 3.51& 3.35& 4.57& 2.91& 5.02  & 1.145& 1.112& 1.169& 1.085& 1.189\\
 HIP 91395&10.91&10.60&11.73&10.00&12.38  & 0.947& 0.932& 0.967& 0.916& 0.984\\
 HIP 91438& 4.71& 2.27& 6.18& 1.26& 8.24  & 0.913& 0.894& 0.939& 0.873& 0.953\\
 HIP 92270& 0.95& 0.95& 2.34& 0.31& 3.02  & 1.246& 1.208& 1.251& 1.188& 1.276\\
 HIP 92720& 7.63& 6.61& 8.83& 5.35& 9.78  & 1.042& 1.022& 1.068& 1.002& 1.099\\
 HIP 93062& 4.45& 3.95& 4.80& 3.57& 5.22  & 1.221& 1.180& 1.256& 1.143& 1.303\\
 HIP 93269&13.56&11.03&14.09& 8.78&14.62  & 0.868& 0.856& 0.890& 0.841& 0.909\\
 HIP 93377&12.12& 9.11&13.14& 6.74&14.37  & 0.908& 0.889& 0.930& 0.873& 0.951\\
 HIP 93827&13.72&12.48&14.34&11.45&14.77  & 0.840& 0.826& 0.859& 0.815& 0.879\\
 HIP 94129&12.34&11.14&12.95&10.21&13.84  & 0.918& 0.897& 0.941& 0.876& 0.963\\
 HIP 94449& 9.63& 8.06&11.24& 6.12&12.62  & 0.876& 0.854& 0.966& 0.817& 1.054\\
 HIP 94615&11.65& 5.13&12.30& 1.70&14.06  & 0.940& 0.913& 0.977& 0.886& 1.012\\
 HIP 94842&11.65& 8.37&13.11& 5.42&14.37  & 0.900& 0.881& 0.936& 0.860& 0.971\\
 HIP 95446& 7.67& 6.67& 9.36& 5.13&10.64  & 0.949& 0.924& 0.981& 0.897& 1.011\\
 HIP 96049& 9.50& 8.71&10.14& 8.08&10.91  & 0.938& 0.911& 0.955& 0.890& 0.977\\
 HIP 96100& 6.43& 2.14& 9.64& 0.67&13.18  & 0.827& 0.805& 0.859& 0.780& 0.874\\
 HIP 96142&13.88& 7.15&13.82& 2.61&14.51  & 0.863& 0.849& 0.894& 0.828& 0.922\\
 HIP 96185&11.14&10.76&11.84&10.28&12.43  & 0.914& 0.892& 0.928& 0.875& 0.945\\
 HIP 96901& 8.91& 7.61& 9.60& 6.67&10.26  & 0.984& 0.972& 0.999& 0.962& 1.012\\
 HIP 96902& 8.23& 7.19& 9.68& 6.07&10.89  & 1.020& 0.985& 1.081& 0.947& 1.139\\
 HIP 96895& 7.84& 7.00& 8.60& 6.10& 9.36  & 1.032& 1.012& 1.047& 0.996& 1.071\\
 HIP 97023& 7.46& 7.08& 7.79& 6.73& 8.18  & 1.045& 1.032& 1.064& 1.015& 1.081\\
 HIP 97420& 5.39& 3.93& 6.61& 2.65& 7.71  & 0.997& 0.982& 1.023& 0.965& 1.044\\
 HIP 97846& 8.77& 8.06& 9.51& 7.37&10.25  & 1.048& 1.026& 1.077& 1.002& 1.104\\
 HIP 97918& 4.90& 4.20& 5.76& 3.66& 6.47  & 1.199& 1.160& 1.251& 1.128& 1.291\\
 HIP 98020&13.14& 6.67&13.51& 2.32&14.47  & 0.674& 0.666& 0.695& 0.657& 0.720\\
 HIP 98036& 4.08& 3.95& 6.04& 3.70& 7.75  & 1.307& 1.170& 1.324& 1.094& 1.366\\
 HIP 98416& 7.24& 5.84& 8.12& 4.68& 9.14  & 1.039& 1.013& 1.069& 0.990& 1.103\\
 HIP 98532&11.63&10.43&12.60& 9.44&13.73  & 0.861& 0.842& 0.894& 0.818& 0.923\\
 HIP 98792&-1.00&12.76&14.57&10.80&14.80  & 0.692& 0.689& 0.701& 0.687& 0.711\\
 HIP 98819& 2.24& 1.78& 3.92& 1.06& 5.16  & 1.074& 1.057& 1.102& 1.032& 1.120\\
 HIP 98921& 3.64& 2.52& 6.51& 1.06& 8.45  & 1.020& 0.990& 1.051& 0.965& 1.076\\
 HIP 99025& 3.20& 3.17& 4.23& 2.91& 4.60  & 1.252& 1.230& 1.313& 1.198& 1.361\\
 HIP 99224&10.62&10.03&11.33& 9.44&11.97  & 0.964& 0.953& 0.993& 0.933& 1.013\\
 HIP 99240&10.65& 7.20&10.92& 5.91&12.44  & 1.001& 0.993& 1.059& 0.967& 1.080\\
 HIP 99241& 5.51& 4.09& 6.44& 3.14& 7.57  & 1.062& 1.040& 1.102& 1.012& 1.126\\
 HIP 99386& 7.52& 6.65& 7.73& 6.11& 8.39  & 1.022& 0.998& 1.049& 0.973& 1.073\\
 HIP 99461&-1.00& 6.57&13.62& 2.54&14.49  & 0.694& 0.688& 0.722& 0.679& 0.745\\
 HIP 99607& 5.80& 5.42& 6.36& 5.00& 6.80  & 1.115& 1.092& 1.154& 1.064& 1.186\\
 HIP 99825& 9.41& 5.25&12.43& 2.39&14.26  & 0.816& 0.800& 0.852& 0.786& 0.875\\
HIP 100017& 3.91& 2.35& 5.86& 0.90& 7.68  & 1.011& 0.983& 1.044& 0.960& 1.071\\
HIP 100568& 4.94& 2.68& 9.47& 1.01&12.65  & 0.797& 0.771& 0.832& 0.744& 0.858\\
HIP 100783& 3.43& 3.01& 3.66& 2.85& 4.02  & 1.333& 1.283& 1.366& 1.240& 1.410\\
HIP 100963& 4.52& 2.66& 5.97& 1.05& 7.39  & 0.990& 0.977& 1.024& 0.959& 1.048\\
HIP 100970& 9.28& 8.79&10.09& 8.22&10.73  & 1.030& 1.009& 1.050& 0.989& 1.071\\
HIP 101136& 4.19& 3.99& 5.63& 3.42& 6.34  & 1.113& 1.087& 1.145& 1.064& 1.170\\
HIP 102081&10.61& 8.99&12.57& 6.75&13.94  & 0.955& 0.936& 0.998& 0.912& 1.039\\
HIP 102152& 8.86& 5.40& 9.21& 2.57&10.26  & 0.974& 0.961& 0.985& 0.950& 1.003\\
HIP 102379& 8.79& 7.97& 9.20& 7.50& 9.86  & 0.961& 0.943& 0.988& 0.922& 1.014\\
HIP 102422& 5.47& 4.19& 7.89& 3.37&10.50  & 1.170& 1.093& 1.319& 1.011& 1.430\\
HIP 102610&10.20& 9.53&11.07& 8.72&11.79  & 0.937& 0.922& 0.953& 0.908& 0.968\\
HIP 102611& 5.79& 5.45& 6.61& 4.81& 7.08  & 1.038& 1.012& 1.056& 0.992& 1.080\\
HIP 102762& 7.10& 5.37& 7.36& 4.12& 8.22  & 1.034& 1.013& 1.060& 0.990& 1.085\\
HIP 102805& 3.00& 2.89& 4.10& 2.65& 4.57  & 1.197& 1.148& 1.205& 1.124& 1.219\\
HIP 103237& 3.89& 3.15& 4.41& 2.77& 4.86  & 1.190& 1.153& 1.231& 1.119& 1.270\\
HIP 103987& 9.05& 8.78&10.51& 7.98&11.45  & 0.938& 0.918& 0.972& 0.893& 1.000\\
HIP 104347& 5.35& 3.72& 5.70& 2.95& 6.77  & 1.132& 1.098& 1.252& 1.039& 1.339\\
HIP 104421& 6.45& 5.10& 6.74& 3.98& 7.57  & 1.096& 1.064& 1.131& 1.034& 1.178\\
HIP 104504& 1.92& 1.26& 4.68& 0.53& 6.40  & 0.990& 0.966& 0.999& 0.947& 1.018\\
HIP 104514& 6.63& 5.78& 7.61& 4.66& 8.52  & 0.990& 0.963& 1.016& 0.939& 1.044\\
HIP 104520& 4.90& 4.74& 5.60& 3.68& 6.03  & 1.109& 1.086& 1.133& 1.062& 1.179\\
HIP 104659&12.69&10.76&13.67& 9.27&14.59  & 0.796& 0.783& 0.825& 0.770& 0.847\\
HIP 104660&14.35&14.24&14.86&13.76&14.94  & 0.821& 0.817& 0.833& 0.811& 0.844\\
HIP 105202& 2.40& 1.28& 3.04& 0.49& 3.84  & 1.110& 1.097& 1.142& 1.072& 1.173\\
HIP 105481& 5.96& 5.58& 6.30& 5.25& 6.68  & 1.156& 1.144& 1.191& 1.125& 1.215\\
HIP 105766&-1.00&12.62&14.52&11.16&14.79  & 0.773& 0.765& 0.785& 0.759& 0.801\\
HIP 105857& 7.59& 7.30& 8.54& 6.78& 9.17  & 0.976& 0.962& 1.016& 0.938& 1.045\\
HIP 105858& 6.86& 5.42& 8.05& 4.30& 9.27  & 0.932& 0.911& 0.957& 0.891& 0.981\\
HIP 105969& 9.08& 8.07&10.51& 7.01&11.76  & 0.972& 0.944& 1.027& 0.910& 1.075\\
HIP 106040& 6.02& 5.59& 6.73& 4.84& 7.24  & 1.048& 1.022& 1.072& 0.997& 1.098\\
HIP 106122& 5.19& 3.25& 7.83& 1.26&10.02  & 0.865& 0.854& 0.890& 0.838& 0.907\\
HIP 106157& 6.70& 6.18& 7.02& 5.77& 7.43  & 1.062& 1.047& 1.095& 1.027& 1.121\\
HIP 106678&10.30& 9.49&11.06& 8.76&11.86  & 0.996& 0.972& 1.023& 0.951& 1.051\\
HIP 106947&13.14& 5.88&13.43& 2.06&14.46  & 0.780& 0.766& 0.808& 0.751& 0.832\\
HIP 107236&14.63& 5.71&13.54& 1.85&14.48  & 0.816& 0.769& 0.893& 0.739& 1.045\\
HIP 107294&10.16& 3.98&10.70& 1.34&12.35  & 0.837& 0.818& 0.863& 0.797& 0.887\\
HIP 107350& 3.17& 1.41& 5.45& 0.70& 7.55  & 1.046& 0.999& 1.072& 0.968& 1.096\\
HIP 107975& 5.04& 4.66& 5.36& 4.36& 5.71  & 1.104& 1.085& 1.125& 1.067& 1.148\\
HIP 108056& 1.39& 0.74& 2.69& 0.32& 3.51  & 1.182& 1.147& 1.203& 1.123& 1.228\\
HIP 108490& 7.72& 6.45& 9.04& 5.15&10.27  & 0.884& 0.867& 0.904& 0.851& 0.925\\
HIP 108514& 1.89& 1.67& 2.92& 1.23& 3.77  & 1.550& 1.438& 1.758& 1.300& 1.955\\
HIP 108708& 4.52& 1.93& 5.99& 0.61& 7.47  & 1.043& 1.021& 1.066& 1.001& 1.086\\
HIP 108767& 4.35& 3.67& 5.73& 2.50& 6.62  & 1.102& 1.071& 1.130& 1.044& 1.160\\
HIP 108870&13.96& 9.04&13.93& 4.92&14.55  & 0.697& 0.689& 0.713& 0.679& 0.731\\
HIP 108996& 2.10& 1.43& 5.35& 0.62& 7.13  & 1.012& 0.991& 1.030& 0.973& 1.049\\
HIP 109067& 8.67& 3.46&12.26& 1.14&14.26  & 0.745& 0.718& 0.762& 0.702& 0.780\\
HIP 109090& 7.24& 5.77& 7.91& 4.57& 8.80  & 1.033& 1.009& 1.060& 0.987& 1.091\\
HIP 109176& 2.25& 2.19& 2.99& 1.76& 3.72  & 1.268& 1.244& 1.286& 1.207& 1.309\\
HIP 109310& 2.52& 1.22& 4.89& 0.50& 6.57  & 1.012& 0.989& 1.034& 0.966& 1.050\\
HIP 109324& 4.35& 3.43& 4.51& 3.02& 4.81  & 1.199& 1.176& 1.268& 1.149& 1.314\\
HIP 109372& 4.50& 3.66& 4.86& 3.44& 5.15  & 1.163& 1.141& 1.210& 1.118& 1.253\\
HIP 109384& 8.67& 4.13&12.11& 1.40&14.19  & 0.808& 0.789& 0.835& 0.772& 0.857\\
HIP 109450& 8.06& 7.70& 9.17& 6.88& 9.90  & 1.025& 1.008& 1.046& 0.990& 1.066\\
HIP 109498& 6.43& 4.63& 9.53& 1.87&11.96  & 0.981& 0.953& 1.097& 0.905& 1.257\\
HIP 109608& 3.61& 2.95& 4.79& 2.27& 5.56  & 1.232& 1.191& 1.408& 1.118& 1.553\\
HIP 109677& 5.12& 4.84& 5.39& 4.56& 5.68  & 1.180& 1.161& 1.208& 1.139& 1.234\\
HIP 109771& 8.05& 7.25& 8.70& 6.61& 9.56  & 0.973& 0.946& 1.004& 0.920& 1.036\\
HIP 109881& 4.55& 3.59& 4.67& 3.23& 5.04  & 1.290& 1.261& 1.369& 1.221& 1.414\\
HIP 109931& 7.19& 5.04& 8.11& 2.84& 9.16  & 0.999& 0.987& 1.015& 0.975& 1.032\\
HIP 109951&11.65& 4.99&13.05& 1.55&14.39  & 0.868& 0.833& 0.925& 0.790& 1.002\\
HIP 110016& 5.79& 5.45& 6.75& 4.84& 7.55  & 1.106& 1.071& 1.150& 1.036& 1.196\\
HIP 110035& 8.62& 6.99& 9.48& 5.76&10.70  & 0.963& 0.938& 0.986& 0.915& 1.009\\
HIP 110109& 8.49& 7.29&11.55& 5.17&13.28  & 0.928& 0.902& 0.959& 0.877& 0.991\\
HIP 110187& 4.24& 2.00& 4.62& 0.66& 5.87  & 1.116& 1.100& 1.157& 1.074& 1.197\\
HIP 110291&13.66&10.36&13.89& 8.29&14.60  & 0.802& 0.789& 0.831& 0.775& 0.856\\
HIP 110785& 3.28& 2.94& 3.66& 2.68& 3.87  & 1.357& 1.339& 1.434& 1.308& 1.473\\
HIP 110788& 7.03& 5.96& 8.79& 4.30&10.14  & 0.973& 0.944& 0.996& 0.920& 1.024\\
HIP 111050&13.97&11.22&14.24& 8.27&14.60  & 0.867& 0.848& 0.885& 0.831& 0.905\\
HIP 111352& 2.65& 2.24& 3.10& 1.89& 3.61  & 1.505& 1.421& 1.591& 1.350& 1.675\\
HIP 111431& 2.63& 2.28& 2.89& 1.97& 3.29  & 1.531& 1.468& 1.607& 1.410& 1.674\\
HIP 111517& 8.45& 6.16& 9.59& 4.76&11.48  & 1.030& 0.992& 1.127& 0.941& 1.212\\
HIP 111549&13.14& 4.54&13.18& 1.42&14.42  & 0.775& 0.736& 0.808& 0.704& 0.851\\
HIP 111723& 4.15& 2.75& 6.44& 1.12& 8.19  & 1.005& 0.980& 1.042& 0.954& 1.072\\
HIP 111748& 3.60& 3.59& 4.91& 3.28& 5.20  & 1.285& 1.200& 1.290& 1.173& 1.322\\
HIP 111796& 4.50& 3.90& 4.92& 3.21& 5.35  & 1.149& 1.107& 1.198& 1.072& 1.261\\
HIP 111977& 8.75& 7.15&11.33& 4.96&13.31  & 0.850& 0.828& 0.881& 0.803& 0.910\\
HIP 112263& 4.96& 4.59& 5.28& 4.26& 5.65  & 1.203& 1.179& 1.240& 1.152& 1.274\\
HIP 112595&11.10& 9.52&12.40& 7.93&13.64  & 0.913& 0.895& 0.929& 0.878& 0.945\\
HIP 112666&-1.00& 7.93&13.88& 3.32&14.52  & 0.786& 0.765& 0.808& 0.747& 0.834\\
HIP 112697& 3.78& 3.48& 3.92& 3.40& 4.16  & 1.308& 1.275& 1.329& 1.246& 1.354\\
HIP 112811&-1.00& 9.15&14.03& 5.15&14.55  & 0.747& 0.734& 0.765& 0.722& 0.786\\
HIP 112935& 3.60& 3.14& 4.05& 2.87& 4.34  & 1.275& 1.249& 1.349& 1.227& 1.372\\
HIP 113044& 5.10& 3.88& 5.22& 3.41& 5.68  & 1.237& 1.224& 1.312& 1.201& 1.334\\
HIP 113076& 4.23& 2.87& 6.36& 1.27& 7.97  & 0.993& 0.964& 1.032& 0.934& 1.067\\
HIP 113357& 5.05& 4.99& 6.94& 4.34& 8.01  & 1.076& 1.044& 1.086& 1.021& 1.099\\
HIP 113514&12.53&10.05&13.67& 7.53&14.50  & 0.820& 0.807& 0.845& 0.792& 0.867\\
HIP 113896& 4.47& 3.26& 5.79& 1.95& 7.04  & 1.073& 1.039& 1.091& 1.014& 1.116\\
HIP 113980& 3.55& 2.54& 4.02& 1.77& 4.92  & 1.150& 1.120& 1.170& 1.088& 1.190\\
HIP 114034& 4.05& 3.78& 4.58& 3.48& 5.00  & 1.275& 1.237& 1.313& 1.201& 1.354\\
HIP 114210& 2.28& 2.03& 2.40& 1.95& 2.62  & 1.386& 1.375& 1.396& 1.363& 1.410\\
HIP 114354& 6.11& 5.65& 6.63& 5.17& 7.21  & 1.092& 1.065& 1.127& 1.038& 1.162\\
HIP 114622&10.93& 5.39&13.07& 2.12&14.39  & 0.751& 0.743& 0.781& 0.732& 0.801\\
HIP 114729& 5.60& 5.27& 5.97& 4.88& 6.41  & 1.123& 1.105& 1.148& 1.084& 1.168\\
HIP 114838& 5.41& 4.40& 5.73& 3.88& 6.43  & 1.134& 1.101& 1.192& 1.065& 1.242\\
HIP 114856& 5.29& 4.44& 6.28& 3.67& 7.19  & 1.139& 1.082& 1.206& 1.033& 1.277\\
HIP 114893& 7.67& 6.94& 8.61& 6.25& 9.47  & 1.009& 0.978& 1.054& 0.944& 1.095\\
HIP 114962&12.47&11.37&13.91& 9.94&14.63  & 0.802& 0.782& 0.841& 0.764& 0.880\\
HIP 115012& 9.16& 7.75& 9.82& 6.83&10.72  & 1.039& 1.014& 1.090& 0.985& 1.134\\
HIP 115066& 8.29& 5.65& 9.26& 3.44&10.71  & 0.982& 0.960& 1.009& 0.940& 1.033\\
HIP 115220& 4.65& 3.82& 4.92& 3.28& 5.21  & 1.202& 1.184& 1.272& 1.160& 1.325\\
HIP 115359&-1.00& 9.17&13.98& 4.86&14.54  & 0.817& 0.794& 0.841& 0.775& 0.870\\
HIP 115370& 6.79& 5.30& 7.56& 4.20& 8.57  & 1.051& 1.027& 1.073& 1.008& 1.097\\
HIP 115604& 7.46& 5.53& 8.34& 3.73& 9.40  & 1.050& 1.021& 1.067& 1.000& 1.092\\
HIP 115704&14.63& 6.01&13.64& 1.85&14.49  & 0.704& 0.681& 0.754& 0.659& 0.828\\
HIP 115714& 7.36& 6.77& 8.25& 5.82& 8.98  & 1.032& 1.012& 1.059& 0.990& 1.084\\
HIP 115721& 9.68& 8.32&10.87& 7.15&12.04  & 0.972& 0.942& 1.025& 0.909& 1.073\\
HIP 115761& 3.60& 3.16& 3.98& 2.83& 4.51  & 1.363& 1.291& 1.407& 1.242& 1.463\\
HIP 116106& 3.24& 2.08& 4.82& 1.03& 6.17  & 1.063& 1.021& 1.080& 0.994& 1.110\\
HIP 116421&11.85&10.76&12.60& 9.76&13.46  & 0.914& 0.891& 0.931& 0.871& 0.953\\
HIP 116478&11.12& 8.82&12.44& 6.31&13.81  & 0.928& 0.909& 0.944& 0.892& 0.962\\
HIP 116616& 7.90& 7.33& 8.28& 6.90& 8.78  & 1.077& 1.054& 1.094& 1.035& 1.114\\
HIP 116727& 4.77& 4.33&11.17& 2.81&14.05  & 1.076& 1.026& 1.344& 0.967& 1.532\\
HIP 116771& 4.40& 3.53& 4.66& 3.21& 5.07  & 1.194& 1.187& 1.259& 1.168& 1.276\\
HIP 117029&11.71&10.80&11.99&10.26&12.61  & 0.905& 0.886& 0.919& 0.871& 0.937\\
HIP 117484& 3.95& 3.14& 4.16& 2.77& 4.57  & 1.281& 1.257& 1.386& 1.213& 1.453\\
HIP 117582& 8.81& 7.62& 9.76& 6.45&10.85  & 0.969& 0.941& 0.997& 0.916& 1.025\\
HIP 117762& 4.31& 4.08& 4.54& 3.87& 4.75  & 1.247& 1.228& 1.273& 1.207& 1.292\\
HIP 117776& 6.91& 5.92& 7.04& 5.41& 7.61  & 1.049& 1.021& 1.087& 0.991& 1.126\\
HIP 118010& 9.92& 9.00&10.21& 8.45&10.81  & 0.994& 0.980& 1.014& 0.962& 1.031\\
HIP 118115& 6.85& 5.20& 8.30& 3.48& 9.69  & 1.025& 1.000& 1.049& 0.978& 1.074\\
HIP 118159& 6.14& 2.42& 6.87& 0.78& 8.46  & 1.010& 0.985& 1.030& 0.965& 1.050\\
HIP 118162& 4.61& 2.60& 5.54& 1.22& 6.97  & 1.039& 1.019& 1.070& 0.996& 1.097\\
HIP 118225& 7.60& 7.19& 8.22& 6.70& 8.69  & 1.084& 1.066& 1.105& 1.048& 1.126\\


==> t6_complete.tex <==
  HD 32071&8.71&8.69&8.71&8.47&8.45&8.50& $-0.08\pm0.01$& $-0.18\pm0.02$\\
  HD 59490&8.67&8.66&8.71&8.54&8.55&8.59& $-0.10\pm0.03$& $-0.09\pm0.02$\\
  HD 67163&8.88&8.87&8.89&8.70&8.69&8.73& $ 0.10\pm0.02$& $ 0.05\pm0.02$\\
  HD 82960&9.12&9.09&9.09&8.75&8.73&8.76& $ 0.32\pm0.01$& $ 0.09\pm0.01$\\
 HD 130047&8.96&8.94&8.94&8.80&8.80&8.81& $ 0.16\pm0.01$& $ 0.15\pm0.01$\\
 HD 144070&9.31&9.19&9.12&8.94&8.85&8.81& $ 0.42\pm0.07$& $ 0.21\pm0.05$\\
 HD 170058&9.03&9.04&9.05&8.83&8.83&8.87& $ 0.26\pm0.02$& $ 0.19\pm0.02$\\
 HD 171029&8.90&8.90&8.96&8.63&8.62&8.70& $ 0.14\pm0.04$& $-0.00\pm0.04$\\
 HD 183490&9.10&9.09&9.03&8.81&8.81&8.80& $ 0.29\pm0.02$& $ 0.15\pm0.01$\\
 HD 213746&8.84&8.87&8.88&8.64&8.67&8.71& $ 0.08\pm0.03$& $ 0.02\pm0.03$\\
 HD 223723&8.94&8.90&8.94&8.72&8.70&8.75& $ 0.14\pm0.02$& $ 0.07\pm0.02$\\
   HIP 171&8.54&8.44&8.52&8.36&8.27&8.36& $-0.26\pm0.02$& $-0.30\pm0.02$\\
   HIP 348&8.73&8.72&8.68&8.57&8.56&8.54& $-0.07\pm0.01$& $-0.10\pm0.01$\\
   HIP 394&8.71&8.64&8.64&8.42&8.37&8.40& $-0.11\pm0.02$& $-0.25\pm0.01$\\
   HIP 475&8.55&8.53&8.53&8.36&8.36&8.38& $-0.25\pm0.01$& $-0.30\pm0.01$\\
   HIP 493&8.69&8.67&8.58&8.50&8.49&8.43& $-0.14\pm0.04$& $-0.18\pm0.03$\\
   HIP 522&9.11&9.02&8.99&8.81&8.75&8.76& $ 0.26\pm0.04$& $ 0.12\pm0.02$\\
   HIP 530&9.10&9.06&9.03&8.80&8.78&8.77& $ 0.28\pm0.02$& $ 0.13\pm0.01$\\
   HIP 544&8.98&8.93&8.89&8.88&8.83&8.80& $ 0.15\pm0.02$& $ 0.18\pm0.03$\\
   HIP 656&8.98&8.93&8.87&8.64&8.62&8.59& $ 0.14\pm0.03$& $-0.04\pm0.02$\\
   HIP 768&8.84&8.83&8.81&8.63&8.64&8.63& $ 0.04\pm0.01$& $-0.02\pm0.01$\\
   HIP 950&8.91&8.88&8.84&8.60&8.60&8.59& $ 0.09\pm0.02$& $-0.06\pm0.01$\\
   HIP 996&8.85&8.86&8.82&8.67&8.68&8.66& $ 0.06\pm0.01$& $ 0.02\pm0.01$\\
  HIP 1105&8.96&8.91&8.89&8.59&8.56&8.58& $ 0.14\pm0.02$& $-0.08\pm0.01$\\
  HIP 1128&8.62&8.57&8.61&8.42&8.38&8.44& $-0.18\pm0.02$& $-0.24\pm0.02$\\
  HIP 1297&8.94&8.93&8.90&8.78&8.78&8.76& $ 0.14\pm0.01$& $ 0.12\pm0.01$\\
  HIP 1411&8.62&8.66&8.68&8.50&8.54&8.56& $-0.10\pm0.02$& $-0.10\pm0.02$\\
  HIP 1499&8.90&8.90&8.92&8.78&8.77&8.80& $ 0.12\pm0.02$& $ 0.13\pm0.01$\\
  HIP 1599&8.69&8.66&8.72&8.49&8.48&8.54& $-0.11\pm0.02$& $-0.16\pm0.02$\\
  HIP 1813&8.75&8.72&8.76&8.60&8.58&8.61& $-0.04\pm0.02$& $-0.06\pm0.01$\\
  HIP 2021&8.86&8.82&8.86&8.59&8.58&8.63& $ 0.06\pm0.01$& $-0.07\pm0.01$\\
  HIP 2131&8.73&8.69&8.65&8.55&8.52&8.51& $-0.09\pm0.02$& $-0.13\pm0.01$\\
  HIP 2453&8.65&8.60&8.61&8.39&8.36&8.39& $-0.16\pm0.01$& $-0.27\pm0.01$\\
  HIP 2711&9.03&8.95&8.88&8.69&8.64&8.61& $ 0.17\pm0.05$& $-0.01\pm0.03$\\
  HIP 2712&8.85&8.79&8.82&8.61&8.57&8.61& $ 0.04\pm0.02$& $-0.06\pm0.02$\\
  HIP 2760&8.93&8.89&8.87&8.69&8.66&8.67& $ 0.11\pm0.01$& $ 0.02\pm0.01$\\
  HIP 2894&8.70&8.69&8.73&8.56&8.56&8.60& $-0.08\pm0.03$& $-0.08\pm0.02$\\
  HIP 2909&8.96&8.88&8.81&8.73&8.66&8.63& $ 0.10\pm0.05$& $ 0.02\pm0.04$\\
  HIP 2981&8.58&8.52&8.52&8.29&8.24&8.27& $-0.24\pm0.02$& $-0.39\pm0.02$\\
  HIP 3014&8.93&8.93&8.86&8.57&8.58&8.56& $ 0.12\pm0.02$& $-0.08\pm0.01$\\
  HIP 3026&8.04&7.98&8.05&7.78&7.74&7.80& $-0.76\pm0.03$& $-0.88\pm0.02$\\
  HIP 3086&8.84&8.78&8.71&8.60&8.56&8.52& $-0.01\pm0.04$& $-0.09\pm0.03$\\
  HIP 3093&8.84&8.78&8.83&8.78&8.72&8.77& $ 0.05\pm0.01$& $ 0.12\pm0.01$\\
  HIP 3132&8.79&8.75&8.72&8.50&8.49&8.48& $-0.03\pm0.02$& $-0.16\pm0.01$\\
  HIP 3185&8.62&8.64&8.66&8.39&8.41&8.45& $-0.14\pm0.03$& $-0.24\pm0.03$\\
  HIP 3206&8.86&9.02&8.96&8.82&8.97&8.90& $ 0.16\pm0.08$& $ 0.24\pm0.07$\\
  HIP 3272&8.71&8.63&8.55&8.41&8.36&8.32& $-0.15\pm0.05$& $-0.29\pm0.03$\\
  HIP 3441&8.84&8.77&8.73&8.55&8.50&8.50& $-0.00\pm0.03$& $-0.14\pm0.02$\\
  HIP 3765&8.62&8.59&8.61&8.57&8.52&8.55& $-0.18\pm0.01$& $-0.11\pm0.02$\\
  HIP 3821&8.68&8.66&8.62&8.48&8.46&8.45& $-0.13\pm0.01$& $-0.19\pm0.01$\\
  HIP 4039&8.11&8.05&8.00&7.78&7.74&7.71& $-0.73\pm0.03$& $-0.91\pm0.02$\\
  HIP 4127&8.93&8.87&8.84&8.65&8.62&8.62& $ 0.10\pm0.02$& $-0.02\pm0.01$\\
  HIP 4148&8.68&8.62&8.80&8.64&8.58&8.74& $-0.08\pm0.08$& $ 0.00\pm0.07$\\
  HIP 4151&8.91&8.85&8.86&8.66&8.60&8.64& $ 0.09\pm0.02$& $-0.02\pm0.02$\\
  HIP 4195&8.56&8.52&8.58&8.42&8.39&8.45& $-0.23\pm0.03$& $-0.23\pm0.02$\\
  HIP 4457&9.12&9.05&9.02&8.76&8.72&8.72& $ 0.28\pm0.03$& $ 0.08\pm0.01$\\
  HIP 4544&8.26&8.15&8.18&8.03&7.95&7.98& $-0.59\pm0.04$& $-0.67\pm0.03$\\
  HIP 4909&8.83&8.83&8.82&8.66&8.68&8.68& $ 0.04\pm0.01$& $ 0.02\pm0.01$\\
  HIP 5016&8.92&8.90&8.85&8.55&8.55&8.54& $ 0.11\pm0.02$& $-0.11\pm0.01$\\
  HIP 5106&8.62&8.62&8.64&8.44&8.45&8.48& $-0.16\pm0.02$& $-0.20\pm0.02$\\
  HIP 5122&8.73&8.66&8.58&8.51&8.45&8.38& $-0.13\pm0.05$& $-0.21\pm0.05$\\
  HIP 5134&8.76&8.67&8.69&8.58&8.51&8.54& $-0.08\pm0.03$& $-0.11\pm0.02$\\
  HIP 5163&8.43&0.00&8.40&8.23&0.00&8.23& $-0.37\pm0.01$& $-0.43\pm0.01$\\
  HIP 5315&8.85&8.92&8.93&8.57&8.64&8.68& $ 0.12\pm0.05$& $-0.02\pm0.05$\\
  HIP 5336&8.43&8.41&8.44&8.28&8.27&8.30& $-0.34\pm0.02$& $-0.36\pm0.01$\\
  HIP 5441&8.64&8.60&8.57&8.28&8.27&8.27& $-0.18\pm0.02$& $-0.38\pm0.01$\\
  HIP 5531&8.71&8.68&8.64&8.37&8.36&8.37& $-0.11\pm0.02$& $-0.29\pm0.01$\\
  HIP 5682&8.94&8.91&8.91&8.64&8.64&8.65& $ 0.14\pm0.01$& $-0.01\pm0.01$\\
  HIP 5775&8.71&8.69&8.68&8.45&8.44&8.47& $-0.09\pm0.01$& $-0.20\pm0.01$\\
  HIP 5862&9.02&8.98&8.96&8.81&8.78&8.78& $ 0.20\pm0.01$& $ 0.14\pm0.01$\\
  HIP 6159&8.59&8.57&8.64&8.35&8.35&8.44& $-0.18\pm0.04$& $-0.27\pm0.04$\\
  HIP 6407&8.66&8.65&8.64&8.52&8.51&8.52& $-0.13\pm0.01$& $-0.14\pm0.01$\\
  HIP 6607&8.68&8.66&8.67&8.54&8.52&8.54& $-0.11\pm0.01$& $-0.12\pm0.01$\\
  HIP 6711&8.91&8.85&8.80&8.54&8.50&8.50& $ 0.07\pm0.03$& $-0.14\pm0.01$\\
  HIP 6762&8.59&8.66&8.71&8.52&8.57&8.62& $-0.13\pm0.06$& $-0.08\pm0.04$\\
  HIP 6975&8.70&8.65&8.62&8.47&8.43&8.43& $-0.13\pm0.02$& $-0.21\pm0.01$\\
  HIP 6978&9.04&9.09&9.08&8.95&8.99&9.00& $ 0.29\pm0.03$& $ 0.33\pm0.03$\\
  HIP 7221&8.99&8.89&8.94&8.90&8.80&8.85& $ 0.16\pm0.03$& $ 0.20\pm0.04$\\
  HIP 7245&8.81&8.81&8.83&8.68&8.69&8.72& $ 0.03\pm0.02$& $ 0.04\pm0.02$\\
  HIP 7312&9.10&8.99&9.02&8.86&8.78&8.83& $ 0.25\pm0.04$& $ 0.17\pm0.03$\\
  HIP 7357&8.80&8.75&8.70&8.53&8.49&8.48& $-0.03\pm0.03$& $-0.15\pm0.02$\\
  HIP 7513&9.01&8.97&8.94&8.73&8.70&8.70& $ 0.20\pm0.01$& $ 0.06\pm0.01$\\
  HIP 7612&8.88&8.83&8.88&8.65&8.63&8.68& $ 0.08\pm0.02$& $ 0.00\pm0.02$\\
 HIP 7751B&8.64&8.56&8.68&8.59&8.50&8.62& $-0.16\pm0.05$& $-0.08\pm0.05$\\
 HIP 7751A&8.60&8.62&8.59&8.55&8.57&8.53& $-0.18\pm0.02$& $-0.10\pm0.02$\\
  HIP 7885&8.81&8.84&8.85&8.65&8.69&8.71& $ 0.05\pm0.03$& $ 0.03\pm0.03$\\
  HIP 7902&8.88&8.88&8.83&8.73&8.74&8.71& $ 0.08\pm0.02$& $ 0.07\pm0.01$\\
  HIP 7918&8.85&8.85&8.86&8.68&8.68&8.69& $ 0.07\pm0.02$& $ 0.03\pm0.01$\\
  HIP 7961&8.82&8.78&8.73&8.53&8.52&8.48& $-0.01\pm0.02$& $-0.14\pm0.02$\\
  HIP 7978&8.88&8.78&8.76&8.65&8.58&8.59& $ 0.02\pm0.04$& $-0.05\pm0.03$\\
  HIP 7981&8.70&8.71&8.73&8.63&8.64&8.67& $-0.07\pm0.02$& $-0.01\pm0.02$\\
  HIP 8102&8.58&8.59&8.57&8.47&8.48&8.45& $-0.20\pm0.01$& $-0.19\pm0.01$\\
  HIP 8121&8.82&8.82&8.75&8.66&8.65&8.62& $ 0.01\pm0.02$& $-0.01\pm0.01$\\
  HIP 8362&8.78&8.82&8.79&8.71&8.74&8.71& $ 0.01\pm0.02$& $ 0.07\pm0.02$\\
  HIP 8433&8.79&8.75&8.76&8.50&8.49&8.52& $-0.02\pm0.01$& $-0.15\pm0.01$\\
  HIP 8476&8.91&8.88&8.86&8.65&8.63&8.63& $ 0.10\pm0.01$& $-0.02\pm0.01$\\
  HIP 8507&8.81&8.76&8.81&8.67&8.64&8.69& $ 0.01\pm0.02$& $ 0.01\pm0.02$\\
  HIP 8674&8.62&8.66&8.58&8.47&8.50&8.44& $-0.16\pm0.03$& $-0.18\pm0.02$\\
  HIP 8720&8.72&8.70&8.62&8.61&8.59&8.51& $-0.10\pm0.03$& $-0.08\pm0.04$\\
  HIP 8841&8.57&8.62&8.62&8.44&8.48&8.49& $-0.18\pm0.04$& $-0.18\pm0.03$\\
  HIP 8859&8.77&8.73&8.70&8.43&8.43&8.43& $-0.05\pm0.02$& $-0.22\pm0.01$\\
  HIP 9080&0.00&8.58&8.48&0.00&8.49&8.40& $-0.25\pm0.05$& $-0.20\pm0.05$\\
  HIP 9349&8.81&8.79&8.81&8.66&8.65&8.67& $ 0.02\pm0.01$& $ 0.01\pm0.01$\\
  HIP 9519&8.95&8.83&8.85&8.80&8.68&8.74& $ 0.09\pm0.04$& $ 0.09\pm0.04$\\
  HIP 9643&8.84&8.85&8.93&8.73&8.74&8.83& $ 0.09\pm0.05$& $ 0.11\pm0.05$\\
  HIP 9884&8.66&9.03&9.00&8.42&8.71&8.71& $ 0.11\pm0.18$& $-0.04\pm0.14$\\
 HIP 10138&8.77&8.76&8.63&8.69&8.69&8.56& $-0.06\pm0.05$& $-0.01\pm0.06$\\
 HIP 10212&9.14&9.03&9.02&8.79&8.72&8.75& $ 0.28\pm0.04$& $ 0.10\pm0.02$\\
 HIP 10303&8.79&8.75&8.77&8.67&8.64&8.67& $-0.01\pm0.01$& $ 0.01\pm0.01$\\
 HIP 10322&8.84&8.79&8.78&8.59&8.55&8.56& $ 0.02\pm0.01$& $-0.09\pm0.01$\\
 HIP 10449&8.30&8.34&8.24&8.09&8.13&8.05& $-0.49\pm0.04$& $-0.56\pm0.03$\\
 HIP 10644&8.54&8.53&8.53&8.32&8.32&8.34& $-0.25\pm0.01$& $-0.33\pm0.01$\\
 HIP 10652&8.53&8.60&8.60&8.33&8.40&8.41& $-0.23\pm0.05$& $-0.29\pm0.04$\\
 HIP 10710&8.78&8.82&8.85&8.62&8.66&8.69& $ 0.03\pm0.04$& $ 0.00\pm0.03$\\
 HIP 10711&8.64&8.62&8.61&8.34&8.34&8.36& $-0.16\pm0.01$& $-0.31\pm0.01$\\
 HIP 10798&8.38&8.40&8.41&8.28&8.31&8.31& $-0.39\pm0.02$& $-0.35\pm0.02$\\
 HIP 11072&8.97&8.90&8.87&8.69&8.64&8.65& $ 0.13\pm0.03$& $ 0.01\pm0.02$\\
 HIP 11237&8.73&8.71&8.66&8.43&8.43&8.41& $-0.08\pm0.02$& $-0.23\pm0.01$\\
 HIP 11309&8.71&8.71&8.66&8.36&8.38&8.38& $-0.09\pm0.02$& $-0.28\pm0.01$\\
 HIP 11505&8.97&8.89&8.88&8.76&8.71&8.72& $ 0.13\pm0.03$& $ 0.08\pm0.02$\\
 HIP 11584&9.13&9.13&9.08&8.77&8.78&8.77& $ 0.33\pm0.02$& $ 0.12\pm0.01$\\
 HIP 11728&8.88&8.86&8.87&8.75&8.75&8.76& $ 0.09\pm0.01$& $ 0.10\pm0.01$\\
 HIP 11915&8.69&8.78&8.69&8.55&8.63&8.56& $-0.06\pm0.05$& $-0.07\pm0.04$\\
 HIP 11923&8.80&8.73&8.78&8.55&8.51&8.57& $-0.01\pm0.03$& $-0.11\pm0.02$\\
 HIP 12262&8.98&8.96&8.88&8.64&8.64&8.60& $ 0.16\pm0.03$& $-0.03\pm0.02$\\
 HIP 12294&7.99&7.97&0.00&7.78&7.77&0.00& $-0.81\pm0.01$& $-0.88\pm0.01$\\
 HIP 12306&8.68&8.76&8.67&8.44&8.51&8.46& $-0.08\pm0.04$& $-0.18\pm0.03$\\
 HIP 12381&8.94&8.88&8.89&8.63&8.60&8.62& $ 0.12\pm0.02$& $-0.04\pm0.01$\\
 HIP 12444&8.90&8.83&8.83&8.65&8.61&8.63& $ 0.07\pm0.02$& $-0.02\pm0.01$\\
 HIP 12579&8.56&8.52&8.55&8.28&8.25&8.30& $-0.24\pm0.02$& $-0.38\pm0.02$\\
 HIP 12777&8.95&8.90&8.91&8.69&8.66&8.69& $ 0.14\pm0.01$& $ 0.04\pm0.01$\\
 HIP 13336&8.66&8.70&8.76&8.51&8.56&8.62& $-0.08\pm0.05$& $-0.09\pm0.05$\\
 HIP 13366&8.67&8.64&8.54&8.40&8.38&8.32& $-0.17\pm0.04$& $-0.29\pm0.03$\\
 HIP 13402&8.89&8.91&8.94&8.85&8.86&8.88& $ 0.13\pm0.03$& $ 0.21\pm0.02$\\
 HIP 14023&8.93&9.00&9.01&8.88&8.93&8.94& $ 0.20\pm0.05$& $ 0.26\pm0.03$\\
 HIP 14086&8.69&8.63&8.52&8.44&8.41&8.34& $-0.17\pm0.06$& $-0.26\pm0.04$\\
 HIP 14241&8.76&8.69&8.77&8.60&8.54&8.62& $-0.04\pm0.04$& $-0.07\pm0.03$\\
 HIP 14286&8.84&8.83&8.76&8.64&8.63&8.60& $ 0.02\pm0.03$& $-0.03\pm0.01$\\
 HIP 14594&7.42&7.28&7.46&7.20&7.07&7.30& $-1.40\pm0.08$& $-1.46\pm0.09$\\
 HIP 14614&8.71&8.67&8.64&8.55&8.52&8.51& $-0.09\pm0.01$& $-0.11\pm0.01$\\
 HIP 14632&8.96&8.95&8.93&8.74&8.74&8.74& $ 0.16\pm0.01$& $ 0.08\pm0.01$\\
 HIP 14668&9.09&9.33&9.25&8.82&9.05&9.01& $ 0.44\pm0.11$& $ 0.31\pm0.10$\\
 HIP 14721&8.99&8.94&8.98&8.87&8.82&8.88& $ 0.19\pm0.02$& $ 0.20\pm0.02$\\
 HIP 14879&8.90&8.90&8.84&8.53&8.54&8.54& $ 0.09\pm0.02$& $-0.12\pm0.01$\\
 HIP 15126&8.23&8.16&8.21&8.09&8.03&8.07& $-0.58\pm0.03$& $-0.59\pm0.02$\\
 HIP 15206&9.06&9.02&8.98&8.76&8.75&8.74& $ 0.24\pm0.02$& $ 0.10\pm0.01$\\
 HIP 15249&8.88&8.88&8.90&8.71&8.73&8.75& $ 0.10\pm0.02$& $ 0.08\pm0.02$\\
 HIP 15330&8.71&8.69&8.75&8.56&8.54&8.61& $-0.07\pm0.03$& $-0.08\pm0.03$\\
 HIP 15371&8.74&8.69&8.72&8.55&8.51&8.56& $-0.06\pm0.01$& $-0.11\pm0.01$\\
 HIP 15383&8.84&9.08&9.10&8.59&8.80&8.84& $ 0.22\pm0.13$& $ 0.09\pm0.11$\\
 HIP 15394&8.64&8.73&8.56&8.46&8.54&8.39& $-0.14\pm0.07$& $-0.19\pm0.06$\\
 HIP 15405&8.35&8.45&8.42&8.15&8.24&8.22& $-0.38\pm0.05$& $-0.45\pm0.04$\\
 HIP 15457&8.93&8.89&8.85&8.79&8.76&8.74& $ 0.11\pm0.01$& $ 0.11\pm0.01$\\
 HIP 15510&8.81&8.78&8.82&8.66&8.63&8.68& $ 0.02\pm0.02$& $ 0.00\pm0.02$\\
 HIP 15565&8.79&8.76&8.67&8.41&8.42&8.37& $-0.04\pm0.04$& $-0.25\pm0.02$\\
 HIP 15940&8.71&8.71&8.65&8.45&8.48&8.45& $-0.09\pm0.02$& $-0.19\pm0.02$\\
 HIP 16072&8.39&8.24&8.29&8.11&7.98&8.02& $-0.48\pm0.05$& $-0.62\pm0.05$\\
 HIP 16169&8.69&8.68&8.68&8.47&8.48&8.49& $-0.10\pm0.01$& $-0.17\pm0.01$\\
 HIP 16467&8.72&8.66&8.65&8.59&8.54&8.55& $-0.11\pm0.02$& $-0.09\pm0.02$\\
 HIP 16537&8.77&8.82&8.79&8.71&8.75&8.72& $ 0.03\pm0.01$& $ 0.09\pm0.01$\\
 HIP 16723&8.78&8.78&8.79&8.46&8.47&8.51& $-0.00\pm0.02$& $-0.17\pm0.02$\\
 HIP 16738&9.12&9.04&9.10&8.88&8.81&8.89& $ 0.30\pm0.03$& $ 0.21\pm0.03$\\
 HIP 16818&8.70&8.62&8.64&8.41&8.37&8.41& $-0.13\pm0.02$& $-0.26\pm0.02$\\
 HIP 16852&8.88&8.87&8.85&8.61&8.61&8.61& $ 0.08\pm0.01$& $-0.04\pm0.01$\\
 HIP 17022&8.87&8.82&8.84&8.59&8.57&8.60& $ 0.06\pm0.01$& $-0.07\pm0.01$\\
 HIP 17147&8.53&8.51&8.48&8.24&8.23&8.23& $-0.28\pm0.01$& $-0.42\pm0.01$\\
 HIP 17231&8.90&8.87&8.85&8.63&8.61&8.63& $ 0.09\pm0.01$& $-0.03\pm0.01$\\
 HIP 17378&9.05&9.11&9.07&8.89&8.94&8.93& $ 0.26\pm0.03$& $ 0.24\pm0.02$\\
 HIP 17409&8.73&8.76&8.74&8.47&8.51&8.52& $-0.04\pm0.02$& $-0.15\pm0.03$\\
 HIP 17420&8.79&8.83&8.81&8.74&8.77&8.75& $ 0.03\pm0.03$& $ 0.10\pm0.02$\\
 HIP 17655&8.73&8.72&8.67&8.49&8.51&8.48& $-0.08\pm0.02$& $-0.16\pm0.01$\\
 HIP 17666&8.46&8.42&8.49&8.32&8.28&8.34& $-0.30\pm0.03$& $-0.32\pm0.02$\\
 HIP 18235&8.70&8.74&8.69&8.40&8.45&8.42& $-0.07\pm0.02$& $-0.23\pm0.02$\\
 HIP 18261&8.75&8.77&8.77&8.59&8.61&8.61& $-0.02\pm0.02$& $-0.05\pm0.01$\\
 HIP 18347&8.58&8.60&8.59&8.35&8.37&8.38& $-0.19\pm0.02$& $-0.29\pm0.02$\\
 HIP 18366&8.66&8.62&8.60&8.37&8.36&8.37& $-0.16\pm0.01$& $-0.29\pm0.01$\\
 HIP 18413&8.87&8.86&8.90&8.71&8.71&8.76& $ 0.09\pm0.03$& $ 0.07\pm0.03$\\
 HIP 18606&8.90&9.15&9.10&8.71&8.92&8.90& $ 0.27\pm0.12$& $ 0.19\pm0.10$\\
 HIP 19631&8.71&8.71&8.73&8.44&8.45&8.49& $-0.07\pm0.02$& $-0.19\pm0.02$\\
 HIP 19696&8.78&8.85&8.83&8.59&8.66&8.65& $ 0.04\pm0.04$& $-0.02\pm0.04$\\
 HIP 19786&9.05&8.98&8.95&8.92&8.83&8.84& $ 0.21\pm0.03$& $ 0.21\pm0.04$\\
 HIP 19849&8.74&8.71&8.70&8.66&8.63&8.61& $-0.07\pm0.01$& $-0.02\pm0.02$\\
 HIP 19911&8.99&8.86&8.89&8.83&8.72&8.75& $ 0.13\pm0.05$& $ 0.11\pm0.04$\\
 HIP 20094&8.82&8.77&8.79&8.66&8.61&8.64& $ 0.01\pm0.01$& $-0.02\pm0.02$\\
 HIP 20298&8.40&8.43&8.45&8.15&8.18&8.22& $-0.36\pm0.03$& $-0.47\pm0.03$\\
 HIP 20366&8.90&8.81&8.81&8.72&8.65&8.66& $ 0.06\pm0.03$& $ 0.02\pm0.03$\\
 HIP 20753&9.05&9.01&8.96&8.80&8.77&8.77& $ 0.22\pm0.02$& $ 0.13\pm0.01$\\
 HIP 20754&8.66&8.63&8.54&8.31&8.31&8.28& $-0.17\pm0.04$& $-0.35\pm0.01$\\
 HIP 20984&8.80&8.79&8.85&8.57&8.58&8.64& $ 0.03\pm0.04$& $-0.06\pm0.03$\\
 HIP 21227&8.53&8.55&8.59&8.30&8.34&8.38& $-0.23\pm0.04$& $-0.31\pm0.04$\\
 HIP 21306&8.68&8.64&8.67&8.46&8.44&8.48& $-0.12\pm0.02$& $-0.19\pm0.02$\\
 HIP 21703&8.93&8.88&8.88&8.82&8.79&8.78& $ 0.11\pm0.01$& $ 0.14\pm0.01$\\
 HIP 21847&9.02&9.01&8.97&8.75&8.75&8.73& $ 0.22\pm0.01$& $ 0.09\pm0.01$\\
 HIP 21921&8.88&8.81&8.84&8.75&8.69&8.72& $ 0.06\pm0.02$& $ 0.07\pm0.02$\\
 HIP 22020&8.77&8.82&0.00&8.56&8.62&0.00& $ 0.01\pm0.03$& $-0.06\pm0.03$\\
 HIP 22060&8.32&8.32&8.40&8.16&8.15&8.25& $-0.44\pm0.05$& $-0.47\pm0.05$\\
 HIP 22263&8.80&8.77&8.78&8.66&8.64&8.65& $ 0.00\pm0.01$& $-0.00\pm0.01$\\
 HIP 22336&9.00&8.98&8.94&8.81&8.79&8.79& $ 0.19\pm0.01$& $ 0.14\pm0.01$\\
 HIP 22349&8.86&8.85&8.84&8.63&8.62&8.63& $ 0.07\pm0.01$& $-0.03\pm0.01$\\
 HIP 22449&9.05&9.02&8.98&8.75&8.73&8.73& $ 0.23\pm0.02$& $ 0.08\pm0.01$\\
 HIP 22489&8.75&0.00&8.94&8.53&0.00&8.73& $ 0.06\pm0.11$& $-0.03\pm0.11$\\
 HIP 22528&8.77&8.74&8.69&8.58&8.54&8.52& $-0.05\pm0.02$& $-0.11\pm0.02$\\
 HIP 22596&8.76&8.72&8.74&8.50&8.49&8.51& $-0.04\pm0.01$& $-0.15\pm0.01$\\
 HIP 23080&8.76&8.76&8.86&8.65&8.64&8.74& $ 0.01\pm0.06$& $ 0.02\pm0.05$\\
 HIP 23311&9.06&9.39&9.28&9.02&9.32&9.21& $ 0.46\pm0.15$& $ 0.53\pm0.13$\\
 HIP 23693&8.92&8.79&8.80&8.67&8.59&8.60& $ 0.05\pm0.05$& $-0.03\pm0.03$\\
 HIP 23835&8.88&8.84&8.86&8.63&8.61&8.65& $ 0.08\pm0.01$& $-0.02\pm0.02$\\
 HIP 23884&8.93&8.84&8.87&8.79&8.72&8.76& $ 0.10\pm0.03$& $ 0.10\pm0.02$\\
 HIP 23922&8.60&8.55&8.48&8.34&8.31&8.27& $-0.24\pm0.04$& $-0.35\pm0.02$\\
 HIP 23941&8.85&8.88&8.72&8.46&8.50&8.42& $ 0.03\pm0.06$& $-0.19\pm0.03$\\
 HIP 24030&8.27&8.16&8.29&7.99&7.90&8.04& $-0.54\pm0.06$& $-0.68\pm0.06$\\
 HIP 24037&8.69&8.68&8.68&8.53&8.52&8.52& $-0.10\pm0.01$& $-0.13\pm0.01$\\
 HIP 24660&9.00&8.91&8.91&8.89&8.80&8.81& $ 0.16\pm0.03$& $ 0.18\pm0.04$\\
 HIP 24813&8.93&8.91&8.90&8.74&8.72&8.73& $ 0.13\pm0.01$& $ 0.08\pm0.01$\\
 HIP 25052&8.98&8.99&8.93&8.81&8.81&8.79& $ 0.18\pm0.02$& $ 0.15\pm0.01$\\
 HIP 25361&8.72&8.65&8.68&8.51&8.45&8.50& $-0.10\pm0.02$& $-0.17\pm0.02$\\
 HIP 25528&9.29&9.21&9.15&8.72&8.68&8.66& $ 0.43\pm0.04$& $ 0.03\pm0.02$\\
 HIP 25586&8.82&8.78&8.77&8.66&8.64&8.64& $ 0.01\pm0.01$& $-0.01\pm0.01$\\
 HIP 25670&8.85&8.82&8.83&8.71&8.69&8.72& $ 0.05\pm0.01$& $ 0.05\pm0.01$\\
 HIP 25840&8.73&8.71&8.69&8.48&8.48&8.47& $-0.08\pm0.01$& $-0.18\pm0.01$\\
 HIP 25860&8.83&8.88&8.93&8.66&8.71&8.76& $ 0.10\pm0.05$& $ 0.06\pm0.04$\\
 HIP 25973&9.00&8.94&8.91&8.71&8.67&8.68& $ 0.17\pm0.02$& $ 0.03\pm0.01$\\
 HIP 26100&8.75&8.69&8.60&8.43&8.39&8.37& $-0.10\pm0.05$& $-0.26\pm0.02$\\
 HIP 26129&8.85&8.71&8.72&8.69&8.57&8.59& $-0.02\pm0.05$& $-0.04\pm0.05$\\
 HIP 26326&8.87&8.84&8.81&8.62&8.61&8.60& $ 0.06\pm0.01$& $-0.04\pm0.01$\\
 HIP 26437&8.97&8.97&8.87&8.79&8.80&8.72& $ 0.15\pm0.04$& $ 0.12\pm0.03$\\
 HIP 26452&8.48&8.42&8.46&8.24&8.20&8.24& $-0.33\pm0.02$& $-0.43\pm0.02$\\
 HIP 26534&8.87&8.83&8.81&8.62&8.61&8.60& $ 0.05\pm0.01$& $-0.04\pm0.01$\\
 HIP 26617&8.56&8.50&8.56&8.36&8.33&8.39& $-0.24\pm0.03$& $-0.29\pm0.02$\\
 HIP 26779&8.85&8.91&8.86&8.78&8.83&8.79& $ 0.09\pm0.03$& $ 0.15\pm0.02$\\
 HIP 26807&8.95&8.89&8.91&8.81&8.77&8.80& $ 0.13\pm0.02$& $ 0.14\pm0.01$\\
 HIP 26828&8.94&8.93&8.91&8.53&8.55&8.57& $ 0.14\pm0.01$& $-0.10\pm0.02$\\
 HIP 27072&8.88&8.88&8.87&8.61&8.62&8.64& $ 0.09\pm0.01$& $-0.03\pm0.02$\\
 HIP 27128&8.56&8.54&8.54&8.23&8.23&8.26& $-0.24\pm0.01$& $-0.41\pm0.02$\\
 HIP 27207&8.83&8.94&8.91&8.76&8.84&8.82& $ 0.11\pm0.06$& $ 0.15\pm0.04$\\
 HIP 27878&8.93&8.86&8.85&8.70&8.65&8.67& $ 0.10\pm0.02$& $ 0.02\pm0.02$\\
 HIP 27913&8.82&8.78&8.75&8.65&8.63&8.61& $-0.00\pm0.02$& $-0.02\pm0.01$\\
 HIP 28066&8.92&8.90&8.84&8.71&8.70&8.67& $ 0.10\pm0.02$& $ 0.04\pm0.01$\\
 HIP 28103&9.51&9.39&9.31&9.08&8.96&8.91& $ 0.62\pm0.07$& $ 0.33\pm0.07$\\
 HIP 28145&8.90&8.98&8.86&8.70&8.76&8.68& $ 0.13\pm0.05$& $ 0.06\pm0.04$\\
 HIP 28159&8.90&8.84&8.80&8.63&8.59&8.58& $ 0.06\pm0.03$& $-0.05\pm0.02$\\
 HIP 28336&8.59&8.64&8.54&8.46&8.51&8.43& $-0.19\pm0.04$& $-0.19\pm0.03$\\
 HIP 28671&8.24&8.14&8.32&8.06&7.96&8.13& $-0.55\pm0.08$& $-0.60\pm0.07$\\
 HIP 29001&8.48&8.41&8.47&8.24&8.18&8.26& $-0.33\pm0.03$& $-0.43\pm0.03$\\
 HIP 29074&8.83&8.83&8.82&8.69&8.69&8.69& $ 0.04\pm0.01$& $ 0.04\pm0.01$\\
 HIP 29248&8.90&8.87&8.88&8.74&8.72&8.73& $ 0.10\pm0.01$& $ 0.08\pm0.01$\\
 HIP 29269&8.58&8.55&8.61&8.33&8.31&8.38& $-0.20\pm0.03$& $-0.31\pm0.03$\\
 HIP 29271&8.83&8.82&8.90&8.72&8.72&8.79& $ 0.07\pm0.04$& $ 0.09\pm0.04$\\
 HIP 29432&8.71&8.70&8.70&8.57&8.57&8.58& $-0.08\pm0.01$& $-0.08\pm0.01$\\
 HIP 29650&8.99&8.97&8.91&8.70&8.70&8.67& $ 0.17\pm0.02$& $ 0.04\pm0.01$\\
 HIP 29716&8.95&8.90&8.87&8.58&8.55&8.56& $ 0.12\pm0.02$& $-0.09\pm0.01$\\
 HIP 30545&8.84&8.81&8.77&8.54&8.53&8.52& $ 0.01\pm0.02$& $-0.13\pm0.01$\\
 HIP 30990&8.52&8.49&8.45&8.21&8.19&8.19& $-0.28\pm0.01$& $-0.45\pm0.01$\\
 HIP 31083&8.86&8.99&8.93&8.70&8.82&8.78& $ 0.14\pm0.06$& $ 0.11\pm0.05$\\
 HIP 31188&8.44&8.42&8.40&8.22&8.21&8.21& $-0.36\pm0.01$& $-0.44\pm0.01$\\
 HIP 31419&8.95&9.00&9.06&8.79&8.85&8.90& $ 0.22\pm0.06$& $ 0.19\pm0.05$\\
 HIP 32650&8.63&8.55&8.54&8.40&8.34&8.35& $-0.21\pm0.03$& $-0.29\pm0.02$\\
 HIP 32673&8.84&8.92&8.86&8.72&8.79&8.75& $ 0.09\pm0.04$& $ 0.10\pm0.03$\\
 HIP 32851&8.84&8.81&8.69&8.45&8.44&8.39& $-0.00\pm0.05$& $-0.23\pm0.02$\\
 HIP 33287&8.60&8.62&8.66&8.48&8.50&8.53& $-0.16\pm0.04$& $-0.15\pm0.02$\\
 HIP 33382&8.87&8.84&8.82&8.72&8.72&8.70& $ 0.05\pm0.01$& $ 0.06\pm0.01$\\
 HIP 33608&8.88&8.78&8.81&8.72&8.64&8.67& $ 0.04\pm0.03$& $ 0.02\pm0.03$\\
 HIP 34017&8.78&8.73&8.71&8.59&8.56&8.55& $-0.04\pm0.02$& $-0.09\pm0.01$\\
 HIP 34164&8.80&8.75&8.72&8.47&8.44&8.46& $-0.03\pm0.02$& $-0.20\pm0.01$\\
 HIP 34511&8.74&8.74&8.71&8.58&8.58&8.57& $-0.05\pm0.01$& $-0.08\pm0.01$\\
 HIP 34521&8.98&8.93&8.90&8.65&8.63&8.63& $ 0.15\pm0.02$& $-0.02\pm0.01$\\
 HIP 34608&8.84&8.81&8.78&8.60&8.59&8.57& $ 0.03\pm0.01$& $-0.07\pm0.01$\\
 HIP 34642&8.80&8.70&8.70&8.50&8.42&8.45& $-0.05\pm0.04$& $-0.20\pm0.03$\\
 HIP 34653&8.92&8.91&8.87&8.74&8.73&8.71& $ 0.12\pm0.01$& $ 0.07\pm0.01$\\
 HIP 34710&9.02&9.01&8.99&8.75&8.74&8.75& $ 0.22\pm0.01$& $ 0.09\pm0.01$\\
 HIP 35148&8.81&8.82&8.77&8.57&8.60&8.56& $ 0.02\pm0.02$& $-0.08\pm0.02$\\
 HIP 35185&8.90&8.78&8.78&8.72&8.62&8.64& $ 0.04\pm0.04$& $ 0.01\pm0.04$\\
 HIP 35214&8.92&8.89&8.93&8.72&8.69&8.74& $ 0.13\pm0.02$& $ 0.06\pm0.02$\\
 HIP 35599&8.91&8.92&8.84&8.68&8.71&8.65& $ 0.11\pm0.03$& $ 0.03\pm0.02$\\
 HIP 35989&8.79&8.78&8.75&8.69&8.69&8.65& $-0.01\pm0.01$& $ 0.02\pm0.02$\\
 HIP 36210&8.83&8.84&8.81&8.70&8.72&8.69& $ 0.04\pm0.01$& $ 0.05\pm0.01$\\
 HIP 36439&8.84&8.75&8.68&8.52&8.47&8.44& $-0.03\pm0.05$& $-0.18\pm0.03$\\
 HIP 36481&8.85&8.85&8.82&8.62&8.63&8.62& $ 0.06\pm0.01$& $-0.03\pm0.01$\\
 HIP 36515&8.77&8.74&8.73&8.63&8.60&8.61& $-0.04\pm0.01$& $-0.04\pm0.01$\\
 HIP 36849&8.46&8.44&8.36&8.17&8.17&8.11& $-0.36\pm0.03$& $-0.50\pm0.03$\\
 HIP 36874&8.89&8.84&8.83&8.69&8.65&8.66& $ 0.07\pm0.01$& $ 0.01\pm0.01$\\
 HIP 37171&9.01&8.99&8.87&8.88&8.88&8.77& $ 0.17\pm0.05$& $ 0.19\pm0.05$\\
 HIP 37233&8.69&8.74&8.61&8.43&8.48&8.39& $-0.10\pm0.05$& $-0.22\pm0.04$\\
 HIP 37279&9.18&9.06&9.00&8.76&8.70&8.68& $ 0.37\pm0.03$& $ 0.10\pm0.01$\\
 HIP 37316&8.97&8.96&8.92&8.68&8.69&8.68& $ 0.17\pm0.01$& $ 0.03\pm0.01$\\
 HIP 37349&8.77&8.83&8.84&8.73&8.78&8.78& $ 0.03\pm0.04$& $ 0.11\pm0.03$\\
 HIP 37419&8.64&8.62&8.53&8.48&8.46&8.40& $-0.19\pm0.04$& $-0.21\pm0.03$\\
 HIP 37789&8.58&8.58&8.57&8.28&8.29&8.31& $-0.21\pm0.01$& $-0.36\pm0.02$\\
 HIP 37826&8.98&9.17&9.10&8.74&8.92&8.88& $ 0.30\pm0.09$& $ 0.19\pm0.08$\\
 HIP 37853&8.66&8.64&8.63&8.35&8.35&8.36& $-0.14\pm0.01$& $-0.30\pm0.01$\\
 HIP 37971&9.06&8.90&9.01&8.94&8.79&8.89& $ 0.21\pm0.06$& $ 0.22\pm0.06$\\
 HIP 38072&8.92&8.82&8.87&8.76&8.69&8.73& $ 0.09\pm0.03$& $ 0.07\pm0.02$\\
 HIP 38172&8.71&8.71&8.66&8.42&8.43&8.42& $-0.09\pm0.02$& $-0.23\pm0.01$\\
 HIP 38228&8.81&8.87&8.77&8.69&8.75&8.67& $ 0.03\pm0.04$& $ 0.05\pm0.04$\\
 HIP 38325&8.97&8.91&8.89&8.70&8.66&8.67& $ 0.14\pm0.02$& $ 0.02\pm0.01$\\
 HIP 38613&8.58&8.54&8.46&8.33&8.30&8.26& $-0.26\pm0.04$& $-0.36\pm0.02$\\
 HIP 38625&8.58&8.50&8.59&8.44&8.36&8.44& $-0.23\pm0.04$& $-0.24\pm0.04$\\
 HIP 38769&8.54&8.58&8.64&8.23&8.27&8.35& $-0.20\pm0.05$& $-0.37\pm0.05$\\
 HIP 39072&8.89&8.81&8.85&8.68&8.62&8.68& $ 0.07\pm0.03$& $ 0.01\pm0.03$\\
 HIP 39157&8.67&8.59&8.52&8.54&8.46&8.39& $-0.19\pm0.05$& $-0.19\pm0.06$\\
 HIP 39417&9.04&9.06&9.05&8.91&8.93&8.93& $ 0.27\pm0.02$& $ 0.27\pm0.01$\\
 HIP 39506&8.68&8.61&8.65&8.45&8.41&8.46& $-0.14\pm0.02$& $-0.21\pm0.02$\\
 HIP 39616&8.63&8.57&8.54&8.39&8.35&8.36& $-0.20\pm0.02$& $-0.29\pm0.01$\\
 HIP 39780&8.93&9.01&8.95&8.70&8.78&8.77& $ 0.18\pm0.04$& $ 0.10\pm0.04$\\
 HIP 39822&8.69&8.72&8.69&8.52&8.54&8.54& $-0.08\pm0.02$& $-0.12\pm0.01$\\
 HIP 39893&8.46&8.41&8.28&8.21&8.18&8.08& $-0.40\pm0.06$& $-0.50\pm0.05$\\
 HIP 40001&8.72&8.68&8.65&8.39&8.38&8.40& $-0.10\pm0.02$& $-0.26\pm0.01$\\
 HIP 40023&8.80&8.84&8.78&8.58&8.63&8.60& $ 0.02\pm0.03$& $-0.05\pm0.02$\\
 HIP 40118&8.83&8.81&8.80&8.64&8.63&8.63& $ 0.03\pm0.01$& $-0.02\pm0.01$\\
 HIP 40613&8.75&8.67&8.76&8.46&8.41&8.50& $-0.06\pm0.04$& $-0.20\pm0.04$\\
 HIP 40674&8.59&8.48&8.55&8.45&8.36&8.43& $-0.24\pm0.04$& $-0.24\pm0.04$\\
 HIP 40693&8.67&8.72&8.69&8.60&8.63&8.61& $-0.09\pm0.03$& $-0.04\pm0.02$\\
 HIP 40765&8.69&8.65&8.65&8.51&8.49&8.51& $-0.12\pm0.01$& $-0.15\pm0.01$\\
 HIP 40843&8.76&8.68&8.68&8.47&8.42&8.46& $-0.09\pm0.01$& $-0.21\pm0.02$\\
 HIP 40848&8.61&8.73&8.76&8.57&8.67&8.70& $-0.08\pm0.08$& $-0.01\pm0.06$\\
 HIP 41484&8.87&8.86&8.82&8.70&8.71&8.68& $ 0.07\pm0.01$& $ 0.04\pm0.01$\\
 HIP 41832&8.75&8.75&8.73&8.61&8.62&8.62& $-0.04\pm0.01$& $-0.04\pm0.01$\\
 HIP 41926&8.44&8.54&8.51&8.37&8.46&8.42& $-0.29\pm0.05$& $-0.24\pm0.04$\\
 HIP 42343&8.81&8.80&8.76&8.51&8.51&8.50& $ 0.01\pm0.01$& $-0.15\pm0.01$\\
 HIP 42438&8.79&8.77&8.74&8.64&8.63&8.62& $-0.01\pm0.01$& $-0.02\pm0.01$\\
 HIP 42575&8.84&8.80&8.74&8.72&8.69&8.64& $ 0.01\pm0.03$& $ 0.03\pm0.03$\\
 HIP 42612&8.88&8.91&8.84&8.66&8.70&8.66& $ 0.09\pm0.03$& $ 0.02\pm0.02$\\
 HIP 42734&8.77&8.76&8.71&8.48&8.48&8.45& $-0.04\pm0.02$& $-0.18\pm0.01$\\
 HIP 42808&8.94&8.85&8.94&8.88&8.79&8.88& $ 0.13\pm0.04$& $ 0.20\pm0.04$\\
 HIP 43393&8.60&8.50&8.54&8.48&8.40&8.43& $-0.24\pm0.03$& $-0.22\pm0.03$\\
 HIP 43587&9.09&9.19&9.03&9.03&9.11&8.97& $ 0.32\pm0.06$& $ 0.38\pm0.06$\\
 HIP 43595&8.31&8.36&8.38&8.13&8.17&8.21& $-0.43\pm0.04$& $-0.48\pm0.04$\\
 HIP 43618&9.05&9.00&8.98&8.93&8.88&8.86& $ 0.23\pm0.02$& $ 0.24\pm0.02$\\
 HIP 43727&9.01&8.99&8.95&8.80&8.78&8.78& $ 0.20\pm0.01$& $ 0.13\pm0.01$\\
 HIP 43861&9.07&8.99&8.96&8.91&8.85&8.82& $ 0.22\pm0.03$& $ 0.21\pm0.03$\\
 HIP 43904&8.68&8.69&8.60&8.39&8.41&8.37& $-0.13\pm0.03$& $-0.26\pm0.02$\\
 HIP 43981&8.73&8.67&8.67&8.43&8.39&8.42& $-0.09\pm0.02$& $-0.24\pm0.01$\\
 HIP 44075&8.49&8.47&8.45&8.17&8.18&8.18& $-0.31\pm0.01$& $-0.48\pm0.01$\\
 HIP 44212&8.72&8.68&8.67&8.49&8.46&8.48& $-0.09\pm0.01$& $-0.18\pm0.01$\\
 HIP 44324&8.90&8.92&8.86&8.72&8.74&8.70& $ 0.11\pm0.02$& $ 0.07\pm0.02$\\
 HIP 44347&8.57&8.45&8.42&8.28&8.19&8.19& $-0.30\pm0.05$& $-0.43\pm0.04$\\
 HIP 44441&8.77&8.72&8.69&8.45&8.43&8.43& $-0.06\pm0.02$& $-0.22\pm0.01$\\
 HIP 44858&8.59&8.57&8.52&8.41&8.39&8.38& $-0.22\pm0.02$& $-0.26\pm0.01$\\
 HIP 44860&8.79&8.73&8.74&8.54&8.50&8.53& $-0.03\pm0.02$& $-0.13\pm0.01$\\
 HIP 44927&9.14&9.06&9.03&8.75&8.70&8.69& $ 0.29\pm0.03$& $ 0.06\pm0.02$\\
 HIP 44997&8.84&8.75&8.71&8.67&8.61&8.60& $-0.02\pm0.04$& $-0.03\pm0.03$\\
 HIP 45333&8.84&8.93&8.84&8.62&8.70&8.64& $ 0.09\pm0.05$& $ 0.00\pm0.04$\\
 HIP 45699&8.92&8.89&8.88&8.58&8.56&8.59& $ 0.11\pm0.01$& $-0.08\pm0.01$\\
 HIP 45718&8.90&8.78&8.77&8.73&8.64&8.64& $ 0.03\pm0.05$& $ 0.02\pm0.04$\\
 HIP 45947&8.90&8.86&8.81&8.62&8.59&8.58& $ 0.07\pm0.02$& $-0.06\pm0.01$\\
 HIP 46066&8.64&8.65&8.64&8.52&8.54&8.53& $-0.14\pm0.01$& $-0.12\pm0.01$\\
 HIP 46453&9.16&9.11&9.11&8.91&8.88&8.90& $ 0.34\pm0.01$& $ 0.24\pm0.01$\\
 HIP 46853&8.92&8.86&8.83&8.52&8.49&8.50& $ 0.09\pm0.02$& $-0.15\pm0.01$\\
 HIP 47080&8.98&8.99&8.96&8.89&8.89&8.88& $ 0.19\pm0.01$& $ 0.23\pm0.01$\\
 HIP 47173&8.76&8.68&8.63&8.59&8.52&8.49& $-0.09\pm0.04$& $-0.12\pm0.04$\\
 HIP 47292&8.83&8.78&8.76&8.55&8.51&8.53& $ 0.01\pm0.02$& $-0.12\pm0.01$\\
 HIP 47588&8.94&8.94&0.00&8.68&8.67&0.00& $ 0.15\pm0.01$& $ 0.02\pm0.01$\\
 HIP 48113&9.03&9.02&8.94&8.81&8.81&8.76& $ 0.21\pm0.03$& $ 0.14\pm0.02$\\
 HIP 48152&7.41&7.30&0.00&7.20&7.06&0.00& $-1.40\pm0.03$& $-1.47\pm0.04$\\
 HIP 48209&8.58&8.61&8.65&8.42&8.45&8.50& $-0.17\pm0.04$& $-0.20\pm0.04$\\
 HIP 48468&9.08&9.06&9.01&8.75&8.75&8.73& $ 0.27\pm0.02$& $ 0.09\pm0.01$\\
 HIP 48701&8.66&8.64&8.60&8.44&8.44&8.42& $-0.15\pm0.01$& $-0.22\pm0.01$\\
 HIP 48833&8.75&8.78&8.68&8.37&8.43&8.39& $-0.05\pm0.04$& $-0.26\pm0.03$\\
 HIP 49070&8.72&8.70&8.66&8.44&8.44&8.44& $-0.09\pm0.01$& $-0.21\pm0.01$\\
 HIP 49130&8.98&8.98&8.99&8.85&8.85&8.85& $ 0.20\pm0.02$& $ 0.20\pm0.01$\\
 HIP 49246&8.74&8.72&8.70&8.42&8.43&8.44& $-0.06\pm0.01$& $-0.22\pm0.01$\\
 HIP 49572&8.90&8.92&8.91&8.73&8.75&8.76& $ 0.13\pm0.02$& $ 0.09\pm0.02$\\
 HIP 49615&8.62&8.59&8.58&8.35&8.34&8.36& $-0.19\pm0.01$& $-0.30\pm0.01$\\
 HIP 49621&8.84&8.77&8.72&8.67&8.61&8.58& $-0.01\pm0.04$& $-0.03\pm0.03$\\
 HIP 49668&8.76&8.71&8.70&8.55&8.53&8.53& $-0.06\pm0.01$& $-0.12\pm0.01$\\
 HIP 49756&8.80&8.80&8.83&8.66&8.67&8.70& $ 0.03\pm0.02$& $ 0.02\pm0.02$\\
 HIP 49988&8.01&8.00&8.12&7.81&7.80&7.91& $-0.74\pm0.06$& $-0.81\pm0.05$\\
 HIP 50005&8.79&8.84&8.69&8.66&8.69&8.58& $-0.01\pm0.06$& $-0.01\pm0.05$\\
 HIP 50319&8.95&8.98&8.93&8.71&8.75&8.73& $ 0.17\pm0.02$& $ 0.08\pm0.02$\\
 HIP 50355&8.77&8.73&8.72&8.59&8.57&8.57& $-0.04\pm0.01$& $-0.08\pm0.01$\\
 HIP 50671&8.63&8.61&8.58&8.39&8.38&8.38& $-0.18\pm0.01$& $-0.27\pm0.01$\\
 HIP 50965&8.67&8.67&8.66&8.45&8.44&8.47& $-0.12\pm0.01$& $-0.20\pm0.01$\\
 HIP 51128&8.82&8.82&8.75&8.69&8.69&8.64& $ 0.01\pm0.02$& $ 0.02\pm0.02$\\
 HIP 51248&8.78&8.77&8.75&8.57&8.57&8.56& $-0.02\pm0.01$& $-0.09\pm0.01$\\
 HIP 51406&9.02&8.95&8.84&8.58&8.54&8.50& $ 0.15\pm0.06$& $-0.11\pm0.03$\\
 HIP 51459&8.78&8.74&8.74&8.55&8.55&8.57& $-0.03\pm0.01$& $-0.10\pm0.01$\\
 HIP 51477&8.36&8.35&8.34&8.05&8.06&8.05& $-0.43\pm0.01$& $-0.60\pm0.01$\\
 HIP 51784&8.70&8.70&8.66&8.43&8.44&8.43& $-0.10\pm0.01$& $-0.22\pm0.01$\\
 HIP 51933&8.75&8.71&8.64&8.45&8.43&8.40& $-0.08\pm0.03$& $-0.23\pm0.02$\\
 HIP 51993&8.95&8.82&8.82&8.70&8.62&8.64& $ 0.08\pm0.05$& $ 0.00\pm0.03$\\
 HIP 52015&8.97&8.95&8.91&8.75&8.75&8.74& $ 0.16\pm0.01$& $ 0.09\pm0.01$\\
 HIP 52040&8.74&8.74&8.70&8.60&8.61&8.58& $-0.06\pm0.01$& $-0.06\pm0.01$\\
 HIP 52137&8.81&8.82&8.80&8.68&8.69&8.69& $ 0.03\pm0.01$& $ 0.03\pm0.01$\\
 HIP 52153&8.88&8.90&8.79&8.65&8.68&8.60& $ 0.07\pm0.04$& $-0.01\pm0.03$\\
 HIP 52325&8.90&8.92&8.92&8.76&8.78&8.79& $ 0.13\pm0.02$& $ 0.12\pm0.02$\\
 HIP 52673&8.58&8.60&8.48&8.39&8.40&8.32& $-0.23\pm0.05$& $-0.28\pm0.03$\\
 HIP 52761&8.91&8.76&8.83&8.74&8.61&8.67& $ 0.05\pm0.05$& $ 0.02\pm0.05$\\
 HIP 52771&7.39&7.41&7.48&7.17&7.15&7.25& $-1.36\pm0.05$& $-1.46\pm0.04$\\
 HIP 52990&8.94&8.96&8.91&8.72&8.74&8.72& $ 0.15\pm0.02$& $ 0.07\pm0.01$\\
 HIP 53049&8.64&8.60&8.61&8.37&8.35&8.39& $-0.17\pm0.01$& $-0.28\pm0.02$\\
 HIP 53229&8.83&9.09&9.05&8.59&8.81&8.81& $ 0.21\pm0.13$& $ 0.08\pm0.11$\\
 HIP 53535&9.09&9.10&9.04&8.92&8.93&8.89& $ 0.29\pm0.02$& $ 0.26\pm0.02$\\
 HIP 53537&9.05&9.01&9.00&8.87&8.83&8.84& $ 0.24\pm0.01$& $ 0.19\pm0.01$\\
 HIP 53721&8.88&8.84&8.84&8.69&8.67&8.68& $ 0.07\pm0.01$& $ 0.03\pm0.01$\\
 HIP 53725&8.73&8.64&8.65&8.51&8.45&8.47& $-0.11\pm0.03$& $-0.18\pm0.02$\\
 HIP 53898&8.90&8.86&8.77&8.76&8.73&8.66& $ 0.06\pm0.04$& $ 0.06\pm0.04$\\
 HIP 54196&8.72&8.72&8.69&8.46&8.47&8.46& $-0.07\pm0.01$& $-0.19\pm0.01$\\
 HIP 54239&8.62&8.64&8.66&8.42&8.44&8.48& $-0.14\pm0.03$& $-0.21\pm0.03$\\
 HIP 54582&8.89&8.88&8.82&8.66&8.67&8.63& $ 0.08\pm0.02$& $ 0.00\pm0.02$\\
 HIP 54728&8.83&8.90&8.89&8.68&8.74&8.75& $ 0.09\pm0.04$& $ 0.07\pm0.04$\\
HIP 55288A&9.13&9.12&9.11&8.84&8.84&8.85& $ 0.34\pm0.01$& $ 0.19\pm0.01$\\
HIP 55288B&9.01&8.95&8.98&8.84&8.80&8.82& $ 0.20\pm0.02$& $ 0.17\pm0.01$\\
 HIP 55459&8.98&8.86&8.91&8.80&8.71&8.77& $ 0.13\pm0.04$& $ 0.11\pm0.03$\\
 HIP 55592&8.31&8.33&8.31&8.05&8.08&8.06& $-0.47\pm0.02$& $-0.59\pm0.02$\\
 HIP 55666&8.93&8.93&8.87&8.61&8.61&8.60& $ 0.13\pm0.02$& $-0.05\pm0.01$\\
 HIP 55761&8.45&8.46&8.44&8.23&8.25&8.25& $-0.33\pm0.01$& $-0.41\pm0.01$\\
 HIP 56148&8.92&8.90&8.78&8.48&8.49&8.43& $ 0.08\pm0.05$& $-0.19\pm0.02$\\
 HIP 56186&8.76&8.73&8.73&8.47&8.46&8.49& $-0.04\pm0.01$& $-0.18\pm0.01$\\
 HIP 56290&8.74&8.67&8.67&8.40&8.36&8.40& $-0.09\pm0.02$& $-0.27\pm0.02$\\
 HIP 56423&8.64&8.62&8.59&8.35&8.34&8.36& $-0.17\pm0.01$& $-0.30\pm0.01$\\
 HIP 56452&8.45&8.51&8.52&8.37&8.42&8.44& $-0.29\pm0.04$& $-0.24\pm0.03$\\
 HIP 56948&8.81&8.76&8.82&8.67&8.62&8.68& $ 0.01\pm0.03$& $ 0.00\pm0.02$\\
 HIP 56960&8.95&8.89&8.85&8.71&8.67&8.65& $ 0.11\pm0.03$& $ 0.02\pm0.02$\\
 HIP 56997&8.75&8.76&8.75&8.65&8.67&8.65& $-0.02\pm0.01$& $ 0.01\pm0.01$\\
 HIP 57080&8.69&8.63&8.62&8.37&8.33&8.35& $-0.14\pm0.02$& $-0.30\pm0.01$\\
 HIP 57117&8.98&8.95&8.90&8.60&8.61&8.60& $ 0.16\pm0.02$& $-0.05\pm0.01$\\
 HIP 57300&8.71&8.68&8.67&8.45&8.43&8.45& $-0.10\pm0.01$& $-0.21\pm0.01$\\
 HIP 57349&8.81&8.75&8.74&8.57&8.53&8.54& $-0.02\pm0.02$& $-0.11\pm0.01$\\
 HIP 57443&8.69&8.69&8.68&8.54&8.54&8.55& $-0.10\pm0.01$& $-0.11\pm0.01$\\
 HIP 57450&7.92&7.80&7.90&7.71&7.59&7.67& $-0.91\pm0.05$& $-1.00\pm0.05$\\
 HIP 57532&9.01&9.02&9.02&8.90&8.92&8.92& $ 0.23\pm0.02$& $ 0.26\pm0.01$\\
 HIP 57617&8.81&8.76&8.73&8.52&8.48&8.50& $-0.02\pm0.02$& $-0.15\pm0.01$\\
 HIP 57757&9.05&9.01&8.98&8.78&8.77&8.74& $ 0.23\pm0.01$& $ 0.12\pm0.01$\\
 HIP 57939&7.99&8.06&8.15&7.81&7.87&7.94& $-0.70\pm0.08$& $-0.77\pm0.06$\\
 HIP 58171&8.90&8.84&8.82&8.77&8.72&8.72& $ 0.07\pm0.02$& $ 0.08\pm0.02$\\
 HIP 58201&8.84&8.76&8.80&8.68&8.62&8.67& $ 0.02\pm0.03$& $ 0.00\pm0.02$\\
 HIP 58229&8.42&8.36&8.30&8.14&8.09&8.08& $-0.42\pm0.04$& $-0.55\pm0.02$\\
 HIP 58331&8.79&8.76&8.73&8.44&8.45&8.45& $-0.02\pm0.01$& $-0.21\pm0.01$\\
 HIP 58576&9.10&9.10&9.05&8.99&8.99&8.95& $ 0.30\pm0.02$& $ 0.32\pm0.02$\\
 HIP 58843&8.45&8.46&8.45&8.23&8.24&8.25& $-0.33\pm0.01$& $-0.41\pm0.01$\\
 HIP 59021&9.01&8.84&8.87&8.66&8.56&8.60& $ 0.12\pm0.06$& $-0.05\pm0.04$\\
 HIP 59233&8.60&8.65&8.55&8.43&8.48&8.39& $-0.18\pm0.04$& $-0.22\pm0.04$\\
 HIP 59253&8.92&8.95&8.98&8.79&8.82&8.85& $ 0.17\pm0.04$& $ 0.17\pm0.03$\\
 HIP 59532&8.93&8.91&8.89&8.81&8.79&8.77& $ 0.13\pm0.01$& $ 0.14\pm0.01$\\
 HIP 59589&8.84&8.90&8.89&8.67&8.73&8.75& $ 0.09\pm0.04$& $ 0.06\pm0.04$\\
 HIP 59735&8.67&8.62&8.62&8.44&8.41&8.43& $-0.15\pm0.01$& $-0.23\pm0.01$\\
 HIP 59750&8.72&8.68&8.65&8.36&8.35&8.36& $-0.10\pm0.02$& $-0.30\pm0.01$\\
 HIP 60019&8.73&8.68&8.65&8.41&8.39&8.40& $-0.10\pm0.02$& $-0.25\pm0.01$\\
 HIP 60268&8.55&8.58&8.56&8.35&8.39&8.38& $-0.22\pm0.02$& $-0.28\pm0.02$\\
 HIP 60314&8.89&8.80&8.83&8.74&8.67&8.71& $ 0.06\pm0.03$& $ 0.05\pm0.02$\\
 HIP 60331&8.58&8.53&8.69&8.41&8.39&8.54& $-0.18\pm0.07$& $-0.21\pm0.07$\\
 HIP 60366&8.82&8.85&8.90&8.66&8.69&8.74& $ 0.07\pm0.04$& $ 0.04\pm0.04$\\
 HIP 60588&8.69&8.72&8.70&8.45&8.48&8.49& $-0.08\pm0.02$& $-0.18\pm0.02$\\
 HIP 60719&7.16&7.28&7.18&8.33&7.65&7.64& $-1.58\pm0.06$& $-0.78\pm0.32$\\
 HIP 60956&8.54&0.00&8.59&8.42&0.00&8.47& $-0.22\pm0.04$& $-0.21\pm0.03$\\
 HIP 61044&9.04&9.04&8.96&8.91&8.89&8.86& $ 0.23\pm0.03$& $ 0.23\pm0.02$\\
 HIP 61157&8.90&8.83&8.78&8.50&8.45&8.45& $ 0.05\pm0.04$& $-0.19\pm0.02$\\
 HIP 61264&8.54&8.50&8.46&8.21&8.19&8.18& $-0.28\pm0.02$& $-0.46\pm0.01$\\
 HIP 61272&8.94&8.91&0.00&8.74&8.74&0.00& $ 0.13\pm0.01$& $ 0.09\pm0.01$\\
 HIP 61293&8.94&8.92&8.88&8.69&8.69&8.67& $ 0.13\pm0.01$& $ 0.03\pm0.01$\\
 HIP 61317&8.71&8.69&8.69&8.52&8.51&8.53& $-0.09\pm0.01$& $-0.13\pm0.01$\\
 HIP 62039&9.02&9.00&9.00&8.88&8.86&8.87& $ 0.22\pm0.01$& $ 0.22\pm0.01$\\
 HIP 62077&8.84&8.75&8.78&8.58&8.51&8.56& $ 0.01\pm0.03$& $-0.10\pm0.03$\\
 HIP 62162&8.91&8.89&8.85&8.49&8.48&8.48& $ 0.10\pm0.01$& $-0.17\pm0.01$\\
 HIP 62175&8.84&8.90&8.84&8.71&8.76&8.72& $ 0.08\pm0.03$& $ 0.08\pm0.02$\\
 HIP 62198&8.91&8.90&8.89&8.76&8.75&8.76& $ 0.12\pm0.01$& $ 0.10\pm0.01$\\
 HIP 62240&8.56&8.56&8.52&8.35&8.35&8.36& $-0.24\pm0.01$& $-0.30\pm0.01$\\
 HIP 62307&8.94&8.88&8.83&8.52&8.49&8.49& $ 0.10\pm0.03$& $-0.15\pm0.01$\\
 HIP 62507&8.87&8.85&8.98&8.64&8.64&8.74& $ 0.12\pm0.07$& $ 0.02\pm0.05$\\
 HIP 62527&8.96&8.94&8.90&8.80&8.77&8.77& $ 0.15\pm0.01$& $ 0.13\pm0.01$\\
 HIP 62607&8.51&8.46&8.46&8.38&8.34&8.33& $-0.31\pm0.01$& $-0.30\pm0.02$\\
 HIP 62661&8.95&8.90&8.91&8.72&8.69&8.72& $ 0.14\pm0.01$& $ 0.06\pm0.01$\\
 HIP 62816&8.89&8.86&8.86&8.74&8.73&8.74& $ 0.09\pm0.01$& $ 0.08\pm0.01$\\
 HIP 62882&8.42&8.36&8.34&8.05&8.01&8.01& $-0.41\pm0.02$& $-0.63\pm0.01$\\
 HIP 63330&9.09&9.06&9.00&8.81&8.81&8.77& $ 0.27\pm0.03$& $ 0.14\pm0.02$\\
 HIP 63354&8.72&8.69&8.70&8.48&8.46&8.50& $-0.08\pm0.01$& $-0.17\pm0.02$\\
 HIP 63405&8.90&8.88&8.83&8.46&8.46&8.46& $ 0.09\pm0.02$& $-0.19\pm0.01$\\
 HIP 63881&8.95&8.95&8.91&8.81&8.80&8.79& $ 0.15\pm0.01$& $ 0.15\pm0.01$\\
 HIP 64103&8.61&8.59&8.64&8.50&8.48&8.55& $-0.17\pm0.03$& $-0.14\pm0.03$\\
 HIP 64150&8.91&8.81&8.82&8.76&8.69&8.70& $ 0.06\pm0.03$& $ 0.06\pm0.03$\\
 HIP 64241&8.99&8.89&8.78&8.59&8.53&8.48& $ 0.10\pm0.07$& $-0.12\pm0.04$\\
 HIP 64254&8.73&8.65&8.64&8.56&8.48&8.50& $-0.11\pm0.03$& $-0.14\pm0.03$\\
 HIP 64344&8.89&8.80&8.77&8.74&8.67&8.66& $ 0.04\pm0.04$& $ 0.04\pm0.03$\\
 HIP 64394&8.83&8.81&8.80&8.67&8.64&8.64& $ 0.03\pm0.01$& $-0.00\pm0.01$\\
 HIP 64407&9.09&9.00&8.97&8.64&8.58&8.60& $ 0.24\pm0.04$& $-0.05\pm0.02$\\
 HIP 64426&8.63&8.58&8.58&8.34&8.30&8.33& $-0.19\pm0.01$& $-0.33\pm0.01$\\
 HIP 64497&8.83&8.92&8.88&8.71&8.78&8.76& $ 0.09\pm0.05$& $ 0.10\pm0.03$\\
 HIP 64583&8.82&8.74&8.78&8.49&8.44&8.51& $-0.00\pm0.03$& $-0.17\pm0.03$\\
 HIP 64698&8.85&8.83&8.81&8.69&8.67&8.68& $ 0.05\pm0.01$& $ 0.03\pm0.01$\\
 HIP 64792&9.09&9.13&8.98&8.86&8.90&8.79& $ 0.28\pm0.06$& $ 0.20\pm0.04$\\
 HIP 64794&8.77&8.76&8.74&8.62&8.62&8.60& $-0.03\pm0.01$& $-0.04\pm0.01$\\
 HIP 64797&8.74&8.72&8.70&8.68&8.65&8.63& $-0.06\pm0.01$& $ 0.00\pm0.02$\\
 HIP 64924&8.78&8.76&8.74&8.66&8.65&8.64& $-0.02\pm0.01$& $-0.00\pm0.01$\\
 HIP 65049&9.07&9.09&9.09&8.94&8.95&8.95& $ 0.30\pm0.02$& $ 0.29\pm0.01$\\
 HIP 65449&8.74&0.00&8.70&8.53&0.00&8.53& $-0.07\pm0.01$& $-0.12\pm0.01$\\
 HIP 65641&8.88&8.83&8.83&8.73&8.70&8.71& $ 0.06\pm0.01$& $ 0.06\pm0.01$\\
 HIP 65708&8.94&8.92&8.96&8.72&8.72&8.78& $ 0.16\pm0.02$& $ 0.09\pm0.03$\\
 HIP 65971&8.85&8.74&8.69&8.64&8.55&8.53& $-0.02\pm0.05$& $-0.08\pm0.04$\\
 HIP 65982&8.54&8.50&8.58&8.43&8.40&8.46& $-0.24\pm0.04$& $-0.22\pm0.02$\\
 HIP 66051&8.67&8.67&8.64&8.38&8.39&8.39& $-0.12\pm0.01$& $-0.27\pm0.01$\\
 HIP 66464&8.69&8.64&8.58&8.42&8.40&8.36& $-0.15\pm0.03$& $-0.26\pm0.02$\\
 HIP 66514&8.93&8.96&8.95&8.75&8.79&8.79& $ 0.16\pm0.02$& $ 0.12\pm0.02$\\
 HIP 66860&8.90&8.83&8.81&8.56&8.53&8.54& $ 0.06\pm0.03$& $-0.11\pm0.01$\\
 HIP 66974&8.97&8.96&8.93&8.69&8.71&8.70& $ 0.17\pm0.01$& $ 0.05\pm0.01$\\
 HIP 67422&9.24&9.16&9.07&9.17&9.10&9.01& $ 0.37\pm0.06$& $ 0.44\pm0.06$\\
 HIP 67927&9.27&9.23&9.17&8.95&8.93&8.91& $ 0.45\pm0.02$& $ 0.28\pm0.01$\\
 HIP 68030&8.64&8.65&8.63&8.36&8.39&8.39& $-0.14\pm0.01$& $-0.27\pm0.02$\\
 HIP 68085&8.94&8.92&8.91&8.69&8.69&8.71& $ 0.14\pm0.01$& $ 0.04\pm0.01$\\
 HIP 68184&8.88&9.18&9.10&8.84&9.11&9.03& $ 0.27\pm0.14$& $ 0.34\pm0.12$\\
 HIP 68594&7.44&7.36&7.24&3.39&4.22&6.85& $-1.44\pm0.07$& $-3.83\pm1.48$\\
 HIP 69210&8.79&8.79&8.78&8.63&8.63&8.64& $ 0.00\pm0.01$& $-0.02\pm0.01$\\
 HIP 69232&8.42&8.45&8.53&8.24&8.27&8.37& $-0.32\pm0.06$& $-0.36\pm0.06$\\
 HIP 69535&8.96&8.90&8.86&8.64&8.59&8.58& $ 0.12\pm0.03$& $-0.05\pm0.02$\\
 HIP 69673&8.96&9.23&9.16&8.57&8.80&8.79& $ 0.35\pm0.13$& $ 0.07\pm0.11$\\
 HIP 69701&9.14&9.06&9.00&8.66&8.62&8.62& $ 0.28\pm0.04$& $-0.02\pm0.01$\\
 HIP 69972&9.09&9.28&9.41&9.05&9.22&9.34& $ 0.48\pm0.14$& $ 0.55\pm0.12$\\
 HIP 70319&8.58&8.55&8.56&8.43&8.41&8.43& $-0.22\pm0.01$& $-0.23\pm0.01$\\
 HIP 70324&8.76&8.70&8.74&8.56&8.52&8.56& $-0.05\pm0.02$& $-0.11\pm0.02$\\
 HIP 70520&8.69&8.68&8.66&8.39&8.40&8.40& $-0.11\pm0.01$& $-0.26\pm0.01$\\
 HIP 70681&8.28&8.30&8.25&8.07&8.08&8.03& $-0.51\pm0.02$& $-0.59\pm0.02$\\
 HIP 71019&8.85&8.93&8.86&8.64&8.71&8.67& $ 0.10\pm0.04$& $ 0.02\pm0.03$\\
 HIP 71076&8.71&8.69&8.62&8.42&8.40&8.39& $-0.11\pm0.03$& $-0.25\pm0.01$\\
 HIP 71193&8.83&8.86&8.82&8.68&8.71&8.70& $ 0.05\pm0.02$& $ 0.04\pm0.02$\\
 HIP 71284&8.83&8.78&8.66&8.44&8.43&8.38& $-0.03\pm0.06$& $-0.24\pm0.02$\\
 HIP 71572&8.87&8.78&8.88&8.71&8.64&8.74& $ 0.06\pm0.05$& $ 0.04\pm0.04$\\
 HIP 71681&8.83&8.88&9.02&8.78&8.83&8.96& $ 0.13\pm0.09$& $ 0.20\pm0.08$\\
 HIP 71683&8.99&9.06&8.96&8.86&8.91&8.85& $ 0.22\pm0.04$& $ 0.22\pm0.03$\\
 HIP 71819&8.87&8.79&8.82&8.64&8.59&8.63& $ 0.04\pm0.02$& $-0.03\pm0.02$\\
 HIP 72199&8.88&8.85&8.76&8.59&8.58&8.52& $ 0.05\pm0.04$& $-0.09\pm0.03$\\
 HIP 72407&8.81&8.79&8.78&8.60&8.58&8.60& $ 0.01\pm0.01$& $-0.06\pm0.01$\\
 HIP 72467&9.00&9.02&8.81&8.62&8.65&8.52& $ 0.16\pm0.09$& $-0.06\pm0.05$\\
 HIP 72604&8.95&8.90&8.90&8.74&8.71&8.72& $ 0.13\pm0.01$& $ 0.07\pm0.01$\\
 HIP 72659&8.78&8.78&8.77&8.69&8.68&8.67& $-0.01\pm0.01$& $ 0.03\pm0.01$\\
 HIP 72803&8.85&8.82&8.69&8.54&8.53&8.43& $ 0.00\pm0.06$& $-0.15\pm0.05$\\
 HIP 72835&8.69&8.60&8.62&8.38&8.34&8.37& $-0.15\pm0.03$& $-0.29\pm0.01$\\
 HIP 72848&8.72&8.84&8.86&8.66&8.77&8.78& $ 0.02\pm0.07$& $ 0.08\pm0.06$\\
 HIP 73005&8.57&8.68&8.72&8.49&8.57&8.62& $-0.13\pm0.08$& $-0.09\pm0.06$\\
 HIP 73078&8.87&8.99&8.93&8.71&8.82&8.77& $ 0.15\pm0.06$& $ 0.11\pm0.05$\\
 HIP 73385&8.08&7.94&7.97&7.69&7.58&7.61& $-0.79\pm0.05$& $-1.03\pm0.04$\\
 HIP 73440&8.76&8.74&8.74&8.49&8.48&8.50& $-0.04\pm0.01$& $-0.16\pm0.01$\\
 HIP 73695&8.67&8.63&8.61&8.48&8.45&8.46& $-0.15\pm0.01$& $-0.19\pm0.01$\\
 HIP 73768&8.74&8.80&8.83&8.40&8.46&8.52& $ 0.01\pm0.05$& $-0.19\pm0.05$\\
 HIP 73815&8.83&8.88&8.86&8.66&8.71&8.71& $ 0.07\pm0.03$& $ 0.04\pm0.03$\\
 HIP 74033&8.60&8.54&8.57&8.29&8.25&8.30& $-0.21\pm0.02$& $-0.37\pm0.02$\\
 HIP 74067&8.42&8.38&8.35&8.22&8.18&8.16& $-0.40\pm0.02$& $-0.47\pm0.02$\\
 HIP 74079&8.58&8.56&8.52&8.24&8.26&8.25& $-0.23\pm0.01$& $-0.40\pm0.01$\\
 HIP 74326&8.88&8.83&8.78&8.69&8.66&8.63& $ 0.05\pm0.03$& $ 0.01\pm0.02$\\
 HIP 74341&8.85&8.85&8.86&8.70&8.73&8.74& $ 0.07\pm0.02$& $ 0.07\pm0.02$\\
 HIP 74442&8.85&8.76&8.80&8.62&8.56&8.61& $ 0.02\pm0.03$& $-0.06\pm0.02$\\
 HIP 74443&8.53&0.00&8.57&8.44&0.00&8.46& $-0.24\pm0.03$& $-0.20\pm0.02$\\
 HIP 74933&8.78&8.81&8.74&8.50&8.55&8.52& $-0.01\pm0.03$& $-0.13\pm0.02$\\
 HIP 75206&9.16&9.07&9.02&8.74&8.67&8.67& $ 0.30\pm0.05$& $ 0.04\pm0.03$\\
 HIP 75281&8.87&8.86&8.87&8.66&8.66&8.68& $ 0.08\pm0.01$& $ 0.01\pm0.01$\\
 HIP 75370&8.67&8.62&8.65&8.52&8.48&8.53& $-0.14\pm0.02$& $-0.14\pm0.02$\\
 HIP 76219&8.94&8.94&8.91&8.71&8.74&8.73& $ 0.15\pm0.01$& $ 0.07\pm0.02$\\
 HIP 76543&8.73&8.67&8.66&8.41&8.37&8.40& $-0.10\pm0.02$& $-0.26\pm0.01$\\
 HIP 76556&9.12&9.06&9.00&8.82&8.79&8.76& $ 0.28\pm0.04$& $ 0.14\pm0.02$\\
 HIP 76899&8.84&8.80&8.83&8.60&8.58&8.62& $ 0.04\pm0.02$& $-0.05\pm0.02$\\
 HIP 76911&8.88&8.86&8.82&8.70&8.69&8.67& $ 0.07\pm0.01$& $ 0.03\pm0.01$\\
 HIP 76963&8.78&8.77&8.76&8.49&8.51&8.52& $-0.01\pm0.01$& $-0.15\pm0.02$\\
 HIP 76976&7.21&7.21&7.21&6.73&7.08&6.65& $-1.57\pm0.01$& $-1.58\pm0.05$\\
 HIP 77083&8.85&8.92&8.93&8.70&8.78&8.79& $ 0.12\pm0.05$& $ 0.10\pm0.04$\\
 HIP 77159&8.88&8.87&8.87&8.61&8.62&8.64& $ 0.09\pm0.01$& $-0.03\pm0.02$\\
 HIP 77257&8.90&8.87&8.89&8.68&8.67&8.69& $ 0.10\pm0.01$& $ 0.03\pm0.01$\\
 HIP 77358&8.94&8.87&8.86&8.82&8.76&8.76& $ 0.11\pm0.02$& $ 0.13\pm0.02$\\
 HIP 77466&8.88&8.85&8.89&8.68&8.67&8.72& $ 0.10\pm0.02$& $ 0.04\pm0.02$\\
 HIP 77655&9.01&9.19&9.05&8.81&8.98&8.88& $ 0.30\pm0.08$& $ 0.24\pm0.07$\\
 HIP 78028&8.85&8.78&8.82&8.70&8.64&8.68& $ 0.03\pm0.02$& $ 0.02\pm0.02$\\
 HIP 78030&9.03&9.17&9.05&8.88&8.99&8.90& $ 0.30\pm0.07$& $ 0.27\pm0.05$\\
 HIP 78072&8.91&8.83&8.79&8.59&8.54&8.53& $ 0.08\pm0.04$& $-0.08\pm0.02$\\
 HIP 78640&7.95&7.99&7.98&7.67&7.71&7.71& $-0.81\pm0.03$& $-0.96\pm0.02$\\
 HIP 78680&8.81&8.78&8.78&8.65&8.63&8.64& $ 0.01\pm0.01$& $-0.01\pm0.01$\\
 HIP 78747&9.16&9.16&9.01&8.69&8.69&8.61& $ 0.33\pm0.06$& $ 0.01\pm0.04$\\
 HIP 78775&8.53&8.51&8.52&8.41&8.39&8.40& $-0.26\pm0.01$& $-0.25\pm0.01$\\
 HIP 79186&8.95&8.90&8.92&8.75&8.72&8.75& $ 0.14\pm0.01$& $ 0.09\pm0.01$\\
 HIP 79190&8.70&8.62&8.76&8.64&8.55&8.68& $-0.09\pm0.06$& $-0.03\pm0.05$\\
 HIP 79276&8.84&8.84&8.80&8.69&8.69&8.68& $ 0.04\pm0.01$& $ 0.03\pm0.01$\\
 HIP 79304&8.85&8.83&8.84&8.71&8.68&8.72& $ 0.06\pm0.01$& $ 0.05\pm0.02$\\
 HIP 79448&8.74&8.81&8.74&8.57&8.62&8.59& $-0.02\pm0.04$& $-0.06\pm0.02$\\
 HIP 79545&8.74&8.69&8.72&8.43&8.40&8.46& $-0.07\pm0.02$& $-0.22\pm0.02$\\
 HIP 79672&8.82&8.88&8.84&8.68&8.73&8.71& $ 0.06\pm0.02$& $ 0.05\pm0.02$\\
 HIP 79837&8.80&8.80&8.77&8.59&8.58&8.58& $ 0.01\pm0.01$& $-0.07\pm0.01$\\
 HIP 80162&8.72&8.68&8.71&8.61&8.57&8.60& $-0.08\pm0.02$& $-0.06\pm0.01$\\
 HIP 80264&8.73&8.70&8.65&8.44&8.44&8.42& $-0.09\pm0.02$& $-0.22\pm0.01$\\
 HIP 80337&8.83&8.87&8.89&8.69&8.73&8.76& $ 0.08\pm0.04$& $ 0.07\pm0.03$\\
 HIP 80686&8.85&8.95&8.90&8.65&8.73&8.71& $ 0.12\pm0.05$& $ 0.04\pm0.04$\\
 HIP 80736&9.05&9.10&9.11&8.85&8.89&8.92& $ 0.30\pm0.04$& $ 0.23\pm0.03$\\
 HIP 80742&8.72&8.59&8.56&8.53&8.42&8.41& $-0.16\pm0.06$& $-0.20\pm0.05$\\
 HIP 80818&8.85&8.84&8.78&8.56&8.56&8.54& $ 0.04\pm0.02$& $-0.10\pm0.01$\\
 HIP 80837&8.59&8.55&8.49&8.28&8.26&8.23& $-0.24\pm0.03$& $-0.40\pm0.02$\\
 HIP 81072&8.94&8.85&8.79&8.56&8.49&8.48& $ 0.08\pm0.05$& $-0.14\pm0.03$\\
 HIP 81300&8.87&8.80&8.82&8.79&8.73&8.74& $ 0.04\pm0.02$& $ 0.10\pm0.02$\\
 HIP 81312&8.74&8.69&8.69&8.48&8.47&8.48& $-0.08\pm0.01$& $-0.18\pm0.01$\\
 HIP 81461&8.71&8.75&8.78&8.46&8.51&8.57& $-0.04\pm0.04$& $-0.14\pm0.05$\\
 HIP 81512&8.78&8.81&8.77&8.63&8.67&8.64& $ 0.00\pm0.02$& $-0.01\pm0.02$\\
 HIP 81608&9.12&9.08&9.07&8.75&8.73&8.75& $ 0.31\pm0.01$& $ 0.09\pm0.01$\\
 HIP 81681&8.82&8.82&8.81&8.62&8.62&8.63& $ 0.03\pm0.01$& $-0.03\pm0.01$\\
 HIP 81693&9.01&8.97&8.98&8.71&8.69&8.72& $ 0.20\pm0.01$& $ 0.05\pm0.01$\\
 HIP 81748&8.98&8.99&8.99&8.83&8.84&8.85& $ 0.20\pm0.02$& $ 0.19\pm0.01$\\
 HIP 82265&8.95&9.01&8.87&8.84&8.89&8.77& $ 0.16\pm0.05$& $ 0.18\pm0.05$\\
 HIP 82268&8.97&8.90&8.87&8.83&8.78&8.75& $ 0.13\pm0.03$& $ 0.13\pm0.03$\\
 HIP 82621&9.03&9.00&9.00&8.83&8.82&8.82& $ 0.23\pm0.01$& $ 0.17\pm0.01$\\
 HIP 82629&8.98&8.97&8.93&8.68&8.69&8.68& $ 0.18\pm0.01$& $ 0.03\pm0.01$\\
 HIP 82708&9.19&9.13&9.09&8.89&8.84&8.84& $ 0.35\pm0.03$& $ 0.20\pm0.02$\\
 HIP 82750&8.98&8.93&8.97&8.77&8.75&8.80& $ 0.18\pm0.02$& $ 0.12\pm0.02$\\
 HIP 82935&8.90&8.87&8.91&8.62&8.61&8.67& $ 0.11\pm0.02$& $-0.02\pm0.03$\\
 HIP 83058&9.11&9.02&9.00&8.82&8.76&8.77& $ 0.26\pm0.04$& $ 0.13\pm0.02$\\
 HIP 83069&8.87&8.79&8.85&8.60&8.55&8.60& $ 0.05\pm0.03$& $-0.07\pm0.02$\\
 HIP 83204&8.69&8.65&8.70&8.45&8.43&8.50& $-0.10\pm0.02$& $-0.19\pm0.03$\\
 HIP 83489&8.91&8.84&8.83&8.69&8.63&8.64& $ 0.08\pm0.02$& $ 0.00\pm0.02$\\
 HIP 83601&8.87&8.88&8.81&8.66&8.68&8.64& $ 0.07\pm0.02$& $ 0.01\pm0.02$\\
 HIP 84217&9.13&9.06&9.02&8.70&8.66&8.68& $ 0.29\pm0.03$& $ 0.03\pm0.01$\\
 HIP 84405&8.69&8.69&8.64&8.63&8.63&8.57& $-0.11\pm0.02$& $-0.04\pm0.03$\\
 HIP 84478&8.98&8.65&8.49&8.91&8.59&8.43& $-0.08\pm0.19$& $-0.01\pm0.20$\\
 HIP 84506&9.15&9.13&9.12&8.94&8.91&8.93& $ 0.35\pm0.01$& $ 0.27\pm0.01$\\
 HIP 84551&9.29&9.31&9.11&8.86&8.88&8.76& $ 0.45\pm0.08$& $ 0.18\pm0.05$\\
 HIP 84696&8.98&8.94&8.89&8.67&8.65&8.64& $ 0.15\pm0.02$& $ 0.00\pm0.01$\\
 HIP 84720&8.69&8.55&8.70&8.60&8.46&8.60& $-0.14\pm0.07$& $-0.10\pm0.06$\\
 HIP 84781&9.01&9.04&9.00&8.79&8.82&8.79& $ 0.23\pm0.02$& $ 0.15\pm0.02$\\
 HIP 84803&8.98&8.91&8.80&8.66&8.62&8.55& $ 0.11\pm0.06$& $-0.04\pm0.04$\\
 HIP 84824&8.79&8.79&8.78&8.59&8.60&8.60& $ 0.00\pm0.01$& $-0.06\pm0.01$\\
 HIP 84862&8.83&8.81&8.78&8.59&8.59&8.58& $ 0.03\pm0.01$& $-0.07\pm0.01$\\
 HIP 85007&8.61&8.61&8.58&8.39&8.39&8.39& $-0.18\pm0.01$& $-0.26\pm0.01$\\
 HIP 85042&8.70&8.70&8.72&8.58&8.60&8.62& $-0.08\pm0.02$& $-0.05\pm0.02$\\
 HIP 85090&9.21&9.19&9.23&8.86&8.86&8.92& $ 0.43\pm0.02$& $ 0.23\pm0.03$\\
 HIP 85235&8.51&8.49&8.40&8.42&8.40&8.31& $-0.32\pm0.04$& $-0.28\pm0.04$\\
 HIP 85378&8.88&8.85&8.78&8.59&8.57&8.54& $ 0.05\pm0.03$& $-0.09\pm0.02$\\
 HIP 85400&8.76&8.76&8.72&8.50&8.52&8.50& $-0.04\pm0.01$& $-0.15\pm0.01$\\
 HIP 85650&8.88&8.83&8.84&8.67&8.64&8.66& $ 0.07\pm0.01$& $ 0.00\pm0.01$\\
 HIP 85653&8.65&8.69&8.76&8.52&8.56&8.63& $-0.08\pm0.06$& $-0.08\pm0.05$\\
 HIP 85757&8.61&8.55&8.53&8.33&8.29&8.32& $-0.22\pm0.02$& $-0.34\pm0.01$\\
 HIP 85940&9.03&9.02&8.97&8.68&8.70&8.68& $ 0.22\pm0.02$& $ 0.03\pm0.01$\\
 HIP 85964&9.12&9.06&9.05&8.77&8.74&8.75& $ 0.29\pm0.02$& $ 0.10\pm0.01$\\
 HIP 86013&8.67&8.63&8.65&8.40&8.38&8.41& $-0.13\pm0.01$& $-0.26\pm0.01$\\
 HIP 86036&8.92&8.88&8.85&8.73&8.70&8.70& $ 0.10\pm0.02$& $ 0.06\pm0.01$\\
 HIP 86225&9.18&9.05&9.05&8.77&8.68&8.71& $ 0.31\pm0.05$& $ 0.07\pm0.03$\\
 HIP 86321&8.19&8.17&8.07&7.94&7.93&7.88& $-0.64\pm0.04$& $-0.74\pm0.02$\\
 HIP 86382&8.81&8.69&8.70&8.40&8.34&8.37& $-0.05\pm0.04$& $-0.28\pm0.02$\\
 HIP 86400&8.97&8.96&9.05&8.90&8.89&8.98& $ 0.21\pm0.05$& $ 0.27\pm0.04$\\
 HIP 86431&8.66&8.63&8.60&8.43&8.41&8.41& $-0.15\pm0.01$& $-0.24\pm0.01$\\
 HIP 86568&8.67&0.00&0.00&8.58&0.00&0.00& $-0.13\pm0.03$& $-0.08\pm0.03$\\
 HIP 86796&9.17&9.11&9.06&9.02&8.96&8.93& $ 0.33\pm0.03$& $ 0.32\pm0.03$\\
 HIP 86830&8.82&8.73&8.75&8.57&8.51&8.55& $-0.02\pm0.03$& $-0.11\pm0.02$\\
 HIP 86974&9.09&9.10&9.12&8.92&8.93&8.96& $ 0.32\pm0.02$& $ 0.28\pm0.02$\\
 HIP 87055&8.81&8.83&8.75&8.66&8.67&8.62& $ 0.01\pm0.03$& $-0.00\pm0.02$\\
 HIP 87089&8.65&0.00&8.73&8.57&0.00&8.63& $-0.10\pm0.05$& $-0.05\pm0.04$\\
 HIP 87533&8.85&8.74&8.82&8.59&8.52&8.60& $ 0.02\pm0.04$& $-0.08\pm0.03$\\
 HIP 87732&9.13&9.06&9.04&8.78&8.75&8.75& $ 0.29\pm0.03$& $ 0.11\pm0.01$\\
 HIP 88010&8.20&8.26&8.26&8.00&8.03&8.04& $-0.54\pm0.04$& $-0.63\pm0.02$\\
 HIP 88039&8.46&8.49&8.45&8.16&8.20&8.18& $-0.32\pm0.02$& $-0.47\pm0.02$\\
 HIP 88166&8.52&8.48&8.46&8.39&8.34&8.33& $-0.30\pm0.01$& $-0.30\pm0.02$\\
 HIP 88194&8.72&8.76&8.69&8.57&8.62&8.57& $-0.06\pm0.03$& $-0.07\pm0.03$\\
 HIP 88427&8.85&8.82&8.77&8.66&8.64&8.60& $ 0.03\pm0.02$& $-0.02\pm0.02$\\
 HIP 88601&8.71&8.81&8.78&8.65&8.73&8.71& $-0.02\pm0.05$& $ 0.04\pm0.04$\\
 HIP 88745&8.56&8.52&8.48&8.27&8.25&8.22& $-0.26\pm0.02$& $-0.41\pm0.02$\\
 HIP 88766&8.86&8.98&8.94&8.63&8.73&8.73& $ 0.14\pm0.06$& $ 0.04\pm0.05$\\
 HIP 88945&8.88&8.78&8.77&8.73&8.65&8.65& $ 0.03\pm0.04$& $ 0.02\pm0.03$\\
 HIP 88972&8.68&8.72&8.72&8.62&8.65&8.65& $-0.08\pm0.03$& $-0.01\pm0.02$\\
 HIP 89268&8.58&8.59&8.60&8.47&8.48&8.49& $-0.19\pm0.02$& $-0.17\pm0.01$\\
 HIP 89408&8.80&8.77&8.73&8.48&8.47&8.48& $-0.02\pm0.02$& $-0.18\pm0.01$\\
 HIP 89443&8.79&8.79&8.76&8.64&8.65&8.63& $-0.00\pm0.01$& $-0.01\pm0.01$\\
 HIP 89474&8.87&8.88&8.88&8.69&8.71&8.72& $ 0.09\pm0.02$& $ 0.05\pm0.02$\\
 HIP 89583&8.82&8.86&8.78&8.68&8.71&8.66& $ 0.04\pm0.03$& $ 0.03\pm0.02$\\
 HIP 89937&8.42&8.36&8.37&8.14&8.10&8.14& $-0.40\pm0.02$& $-0.53\pm0.02$\\
 HIP 90144&8.79&8.77&8.79&8.53&8.53&8.56& $ 0.00\pm0.01$& $-0.11\pm0.02$\\
 HIP 90539&8.77&8.72&8.74&8.65&8.61&8.64& $-0.04\pm0.01$& $-0.02\pm0.01$\\
 HIP 90542&9.02&8.96&8.98&8.81&8.77&8.80& $ 0.20\pm0.02$& $ 0.14\pm0.01$\\
 HIP 90655&9.06&9.00&8.96&8.82&8.78&8.79& $ 0.22\pm0.03$& $ 0.14\pm0.01$\\
 HIP 90745&8.89&8.80&8.82&8.61&8.54&8.59& $ 0.05\pm0.03$& $-0.07\pm0.03$\\
 HIP 90790&8.70&8.68&8.71&8.64&8.62&8.64& $-0.09\pm0.02$& $-0.02\pm0.01$\\
 HIP 90833&8.62&8.65&8.64&8.49&8.51&8.51& $-0.15\pm0.02$& $-0.15\pm0.01$\\
 HIP 91058&8.69&8.68&8.55&8.40&8.40&8.32& $-0.14\pm0.05$& $-0.28\pm0.04$\\
 HIP 91120&8.85&8.79&8.82&8.49&8.47&8.52& $ 0.04\pm0.02$& $-0.16\pm0.02$\\
 HIP 91395&8.69&8.66&8.67&8.48&8.45&8.48& $-0.11\pm0.01$& $-0.18\pm0.01$\\
 HIP 91438&8.57&8.52&8.58&8.46&8.43&8.48& $-0.23\pm0.03$& $-0.20\pm0.02$\\
 HIP 92270&8.87&8.82&8.74&8.61&8.58&8.54& $ 0.03\pm0.04$& $-0.08\pm0.02$\\
 HIP 92720&8.97&8.92&8.92&8.79&8.75&8.76& $ 0.15\pm0.01$& $ 0.11\pm0.01$\\
 HIP 93062&8.76&8.72&8.68&8.38&8.38&8.36& $-0.06\pm0.02$& $-0.28\pm0.01$\\
 HIP 93269&8.86&8.88&8.80&8.69&8.69&8.64& $ 0.06\pm0.03$& $ 0.02\pm0.02$\\
 HIP 93377&8.84&8.73&8.76&8.71&8.62&8.66& $-0.01\pm0.04$& $ 0.01\pm0.03$\\
 HIP 93827&8.72&8.74&8.70&8.43&8.45&8.44& $-0.06\pm0.02$& $-0.21\pm0.01$\\
 HIP 94129&8.94&8.87&8.83&8.71&8.67&8.65& $ 0.10\pm0.03$& $ 0.02\pm0.02$\\
 HIP 94449&8.22&8.25&8.21&7.91&7.94&7.94& $-0.56\pm0.02$& $-0.72\pm0.02$\\
 HIP 94615&9.01&8.86&8.92&8.87&8.75&8.80& $ 0.15\pm0.05$& $ 0.15\pm0.04$\\
 HIP 94842&8.82&8.86&8.96&8.69&8.73&8.83& $ 0.10\pm0.07$& $ 0.10\pm0.06$\\
 HIP 95446&8.58&8.53&8.53&8.31&8.28&8.32& $-0.24\pm0.01$& $-0.35\pm0.02$\\
 HIP 96049&8.49&8.43&8.40&8.16&8.13&8.13& $-0.34\pm0.02$& $-0.51\pm0.01$\\
 HIP 96100&8.49&8.58&8.66&8.43&8.51&8.59& $-0.21\pm0.08$& $-0.14\pm0.07$\\
 HIP 96142&8.81&8.70&8.78&8.64&8.55&8.64& $-0.02\pm0.04$& $-0.04\pm0.04$\\
 HIP 96185&8.82&8.80&8.81&8.52&8.52&8.55& $ 0.02\pm0.01$& $-0.13\pm0.01$\\
 HIP 96901&8.93&8.85&8.85&8.77&8.71&8.72& $ 0.09\pm0.03$& $ 0.08\pm0.02$\\
 HIP 96902&8.79&8.79&8.73&8.53&8.54&8.52& $-0.01\pm0.02$& $-0.12\pm0.01$\\
 HIP 96895&8.93&8.88&8.84&8.75&8.71&8.70& $ 0.12\pm0.02$& $ 0.08\pm0.01$\\
 HIP 97023&8.71&8.67&8.66&8.42&8.41&8.42& $-0.10\pm0.01$& $-0.24\pm0.01$\\
 HIP 97420&8.85&8.77&8.77&8.71&8.63&8.66& $ 0.01\pm0.03$& $ 0.01\pm0.03$\\
 HIP 97846&9.07&9.13&9.12&8.85&8.91&8.91& $ 0.32\pm0.04$& $ 0.24\pm0.03$\\
 HIP 97918&9.08&9.01&8.99&8.84&8.79&8.80& $ 0.24\pm0.03$& $ 0.16\pm0.02$\\
 HIP 98020&7.86&0.00&7.75&7.62&0.00&7.50& $-0.98\pm0.04$& $-1.09\pm0.05$\\
 HIP 98036&8.77&8.80&8.75&8.58&8.61&8.58& $-0.01\pm0.02$& $-0.06\pm0.02$\\
 HIP 98416&8.76&8.70&8.72&8.53&8.51&8.53& $-0.06\pm0.02$& $-0.13\pm0.01$\\
 HIP 98532&8.19&8.20&8.15&7.88&7.89&7.86& $-0.60\pm0.02$& $-0.78\pm0.01$\\
 HIP 98792&8.52&8.54&8.62&8.43&8.47&8.53& $-0.22\pm0.05$& $-0.18\pm0.04$\\
 HIP 98819&8.89&8.84&8.78&8.71&8.68&8.64& $ 0.05\pm0.03$& $ 0.02\pm0.02$\\
 HIP 98921&8.94&8.90&8.87&8.80&8.77&8.75& $ 0.12\pm0.02$& $ 0.12\pm0.02$\\
 HIP 99025&8.97&8.94&8.90&8.66&8.64&8.64& $ 0.15\pm0.02$& $-0.01\pm0.01$\\
 HIP 99224&8.97&8.95&8.98&8.76&8.75&8.79& $ 0.18\pm0.02$& $ 0.11\pm0.02$\\
 HIP 99240&9.14&9.20&9.16&9.03&9.09&9.05& $ 0.38\pm0.04$& $ 0.40\pm0.03$\\
 HIP 99241&8.80&8.76&8.78&8.54&8.53&8.57& $-0.00\pm0.01$& $-0.11\pm0.02$\\
 HIP 99386&8.65&8.62&8.61&8.34&8.34&8.37& $-0.16\pm0.01$& $-0.30\pm0.02$\\
 HIP 99461&8.68&8.55&8.60&8.60&8.47&8.52& $-0.17\pm0.04$& $-0.12\pm0.05$\\
 HIP 99607&8.87&8.80&8.85&8.53&8.50&8.56& $ 0.06\pm0.03$& $-0.12\pm0.02$\\
 HIP 99825&8.85&8.90&8.89&8.79&8.83&8.82& $ 0.10\pm0.03$& $ 0.16\pm0.02$\\
HIP 100017&8.72&8.70&8.69&8.55&8.54&8.54& $-0.08\pm0.01$& $-0.11\pm0.01$\\
HIP 100568&8.19&8.14&8.09&7.99&7.95&7.90& $-0.64\pm0.03$& $-0.71\pm0.03$\\
HIP 100783&8.87&8.82&8.78&8.43&8.41&8.41& $ 0.04\pm0.02$& $-0.24\pm0.01$\\
HIP 100963&8.74&8.72&8.77&8.60&8.59&8.64& $-0.04\pm0.03$& $-0.04\pm0.02$\\
HIP 100970&8.99&9.02&9.01&8.76&8.81&8.82& $ 0.22\pm0.02$& $ 0.14\pm0.03$\\
HIP 101136&8.89&8.84&8.82&8.61&8.60&8.59& $ 0.07\pm0.02$& $-0.05\pm0.01$\\
HIP 102081&9.16&9.12&9.12&8.99&8.95&8.96& $ 0.35\pm0.01$& $ 0.31\pm0.01$\\
HIP 102152&8.88&8.77&8.75&8.71&8.64&8.63& $ 0.02\pm0.04$& $ 0.01\pm0.03$\\
HIP 102379&8.64&8.53&8.58&8.33&8.26&8.34& $-0.20\pm0.04$& $-0.34\pm0.03$\\
HIP 102422&8.80&8.87&8.82&8.60&8.66&8.64& $ 0.02\pm0.04$& $-0.04\pm0.03$\\
HIP 102610&8.82&8.78&8.81&8.59&8.57&8.60& $ 0.02\pm0.02$& $-0.07\pm0.01$\\
HIP 102611&8.65&8.60&8.56&8.33&8.31&8.31& $-0.18\pm0.02$& $-0.34\pm0.01$\\
HIP 102762&8.82&8.79&8.76&8.61&8.60&8.58& $ 0.01\pm0.01$& $-0.06\pm0.01$\\
HIP 102805&8.82&8.87&8.80&8.46&8.52&8.50& $ 0.05\pm0.03$& $-0.16\pm0.03$\\
HIP 103237&8.91&8.88&8.75&8.58&8.57&8.48& $ 0.06\pm0.06$& $-0.11\pm0.04$\\
HIP 103987&8.54&8.50&8.47&8.25&8.23&8.23& $-0.28\pm0.01$& $-0.42\pm0.01$\\
HIP 104347&8.78&8.61&8.70&8.38&8.26&8.36& $-0.09\pm0.06$& $-0.32\pm0.05$\\
HIP 104421&8.79&8.78&8.72&8.49&8.51&8.48& $-0.02\pm0.02$& $-0.16\pm0.01$\\
HIP 104504&8.64&8.72&8.64&8.50&8.57&8.52& $-0.12\pm0.04$& $-0.12\pm0.03$\\
HIP 104514&8.68&8.64&8.60&8.37&8.35&8.35& $-0.14\pm0.02$& $-0.30\pm0.01$\\
HIP 104520&8.81&8.82&8.77&8.46&8.48&8.46& $ 0.02\pm0.02$& $-0.19\pm0.01$\\
HIP 104659&8.20&8.20&8.22&7.93&7.93&7.97& $-0.57\pm0.02$& $-0.70\pm0.02$\\
HIP 104660&8.61&0.00&8.60&8.31&0.00&8.34& $-0.18\pm0.01$& $-0.33\pm0.02$\\
HIP 105202&8.73&8.65&8.70&8.48&8.42&8.48& $-0.09\pm0.03$& $-0.19\pm0.03$\\
HIP 105481&9.03&8.96&8.96&8.76&8.73&8.75& $ 0.20\pm0.02$& $ 0.09\pm0.01$\\
HIP 105766&8.46&8.50&8.43&8.26&8.29&8.24& $-0.32\pm0.03$& $-0.39\pm0.02$\\
HIP 105857&8.64&8.65&8.57&8.31&8.33&8.30& $-0.16\pm0.03$& $-0.34\pm0.01$\\
HIP 105858&8.49&8.42&8.37&8.21&8.16&8.14& $-0.36\pm0.04$& $-0.48\pm0.03$\\
HIP 105969&8.97&8.91&8.91&8.69&8.65&8.66& $ 0.15\pm0.02$& $ 0.01\pm0.01$\\
HIP 106040&8.76&8.69&8.69&8.46&8.41&8.45& $-0.07\pm0.02$& $-0.21\pm0.02$\\
HIP 106122&8.72&8.74&8.80&8.62&8.63&8.70& $-0.03\pm0.05$& $-0.00\pm0.04$\\
HIP 106157&8.68&8.64&8.64&8.36&8.34&8.38& $-0.13\pm0.01$& $-0.29\pm0.02$\\
HIP 106678&9.00&9.02&8.95&8.79&8.83&8.79& $ 0.21\pm0.02$& $ 0.15\pm0.02$\\
HIP 106947&8.60&8.60&8.63&8.50&8.49&8.52& $-0.17\pm0.02$& $-0.15\pm0.01$\\
HIP 107236&8.77&8.79&8.69&8.61&8.62&8.54& $-0.03\pm0.04$& $-0.06\pm0.03$\\
HIP 107294&8.20&8.20&8.19&7.92&7.93&7.92& $-0.59\pm0.01$& $-0.73\pm0.01$\\
HIP 107350&8.86&8.81&8.79&8.67&8.65&8.64& $ 0.04\pm0.01$& $ 0.00\pm0.01$\\
HIP 107975&8.71&8.65&8.55&8.31&8.30&8.25& $-0.15\pm0.05$& $-0.37\pm0.02$\\
HIP 108056&9.13&9.03&9.01&8.93&8.86&8.86& $ 0.27\pm0.04$& $ 0.23\pm0.03$\\
HIP 108490&8.44&8.40&8.36&8.18&8.17&8.14& $-0.38\pm0.02$& $-0.49\pm0.01$\\
HIP 108514&9.39&9.30&9.11&8.86&8.79&8.68& $ 0.48\pm0.11$& $ 0.12\pm0.07$\\
HIP 108708&8.81&8.84&8.84&8.68&8.71&8.73& $ 0.05\pm0.03$& $ 0.05\pm0.02$\\
HIP 108767&8.96&8.92&8.96&8.69&8.68&8.72& $ 0.16\pm0.02$& $ 0.04\pm0.02$\\
HIP 108870&8.69&8.70&8.80&8.65&8.65&8.73& $-0.05\pm0.06$& $ 0.02\pm0.04$\\
HIP 108996&8.93&8.86&8.92&8.78&8.73&8.79& $ 0.12\pm0.03$& $ 0.11\pm0.02$\\
HIP 109067&8.54&8.58&8.56&8.38&8.41&8.40& $-0.22\pm0.03$& $-0.26\pm0.02$\\
HIP 109090&8.83&8.83&8.80&8.57&8.58&8.58& $ 0.04\pm0.01$& $-0.08\pm0.01$\\
HIP 109176&8.95&8.88&8.80&8.61&8.57&8.54& $ 0.09\pm0.05$& $-0.08\pm0.02$\\
HIP 109310&8.82&8.76&8.76&8.66&8.61&8.62& $-0.00\pm0.02$& $-0.02\pm0.02$\\
HIP 109324&8.79&8.79&8.72&8.41&8.43&8.41& $-0.02\pm0.02$& $-0.24\pm0.01$\\
HIP 109372&8.93&8.90&8.75&8.58&8.58&8.49& $ 0.08\pm0.07$& $-0.10\pm0.04$\\
HIP 109384&8.81&8.85&8.75&8.73&8.75&8.67& $ 0.02\pm0.04$& $ 0.06\pm0.03$\\
HIP 109450&8.90&8.81&8.77&8.66&8.61&8.59& $ 0.04\pm0.04$& $-0.03\pm0.02$\\
HIP 109498&8.76&8.75&8.71&8.56&8.56&8.54& $-0.04\pm0.01$& $-0.10\pm0.01$\\
HIP 109608&8.73&8.69&8.55&8.38&8.37&8.29& $-0.13\pm0.07$& $-0.31\pm0.04$\\
HIP 109677&8.99&8.97&8.83&8.64&8.64&8.55& $ 0.15\pm0.06$& $-0.04\pm0.04$\\
HIP 109771&8.69&8.58&8.66&8.35&8.27&8.36& $-0.14\pm0.04$& $-0.33\pm0.04$\\
HIP 109881&9.12&9.03&9.07&8.84&8.78&8.84& $ 0.29\pm0.03$& $ 0.17\pm0.03$\\
HIP 109931&8.88&8.88&8.86&8.73&8.74&8.73& $ 0.09\pm0.01$& $ 0.08\pm0.01$\\
HIP 109951&8.50&8.49&8.52&8.37&8.36&8.41& $-0.28\pm0.02$& $-0.27\pm0.02$\\
HIP 110016&8.81&8.74&8.74&8.50&8.46&8.48& $-0.02\pm0.02$& $-0.17\pm0.01$\\
HIP 110035&8.74&8.70&8.73&8.55&8.53&8.56& $-0.06\pm0.02$& $-0.11\pm0.01$\\
HIP 110109&8.82&8.72&8.72&8.62&8.54&8.55& $ 0.01\pm0.03$& $-0.05\pm0.03$\\
HIP 110187&8.93&8.89&8.82&8.74&8.72&8.67& $ 0.10\pm0.03$& $ 0.06\pm0.03$\\
HIP 110291&8.50&8.44&8.42&8.19&8.15&8.15& $-0.33\pm0.02$& $-0.49\pm0.01$\\
HIP 110785&9.03&8.95&8.92&8.68&8.63&8.65& $ 0.18\pm0.03$& $ 0.00\pm0.02$\\
HIP 110788&8.65&8.55&8.64&8.40&8.33&8.44& $-0.17\pm0.04$& $-0.26\pm0.04$\\
HIP 111050&8.74&8.73&8.73&8.59&8.58&8.60& $-0.05\pm0.01$& $-0.06\pm0.01$\\
HIP 111352&8.92&8.90&8.82&8.58&8.58&8.54& $ 0.10\pm0.03$& $-0.09\pm0.02$\\
HIP 111431&9.06&9.00&8.99&8.65&8.62&8.65& $ 0.23\pm0.02$& $-0.01\pm0.01$\\
HIP 111517&8.84&8.86&8.81&8.57&8.60&8.58& $ 0.05\pm0.02$& $-0.07\pm0.02$\\
HIP 111549&8.27&8.10&8.27&8.05&7.88&8.04& $-0.57\pm0.08$& $-0.66\pm0.08$\\
HIP 111723&8.74&8.71&8.70&8.52&8.52&8.52& $-0.07\pm0.01$& $-0.13\pm0.01$\\
HIP 111748&8.93&8.91&8.89&8.67&8.67&8.67& $ 0.13\pm0.01$& $ 0.02\pm0.01$\\
HIP 111796&8.65&8.60&8.54&8.27&8.25&8.25& $-0.19\pm0.03$& $-0.40\pm0.01$\\
HIP 111977&8.60&8.59&8.60&8.42&8.42&8.44& $-0.19\pm0.01$& $-0.23\pm0.01$\\
HIP 112263&9.04&9.01&9.00&8.68&8.68&8.70& $ 0.23\pm0.01$& $ 0.03\pm0.01$\\
HIP 112595&8.89&8.95&8.98&8.71&8.77&8.80& $ 0.16\pm0.05$& $ 0.11\pm0.04$\\
HIP 112666&8.80&8.71&8.70&8.69&8.60&8.60& $-0.05\pm0.03$& $-0.02\pm0.04$\\
HIP 112697&8.95&8.90&8.82&8.55&8.53&8.50& $ 0.11\pm0.04$& $-0.13\pm0.02$\\
HIP 112811&8.58&8.54&8.49&8.42&8.38&8.35& $-0.25\pm0.02$& $-0.27\pm0.02$\\
HIP 112935&8.91&8.83&8.75&8.54&8.50&8.47& $ 0.05\pm0.02$& $-0.15\pm0.01$\\
HIP 113044&9.04&8.94&8.93&8.82&8.75&8.76& $ 0.19\pm0.04$& $ 0.12\pm0.03$\\
HIP 113076&8.60&8.62&8.56&8.37&8.39&8.37& $-0.19\pm0.02$& $-0.28\pm0.01$\\
HIP 113357&8.98&9.00&8.94&8.84&8.86&8.82& $ 0.19\pm0.02$& $ 0.19\pm0.02$\\
HIP 113514&8.71&8.71&8.68&8.47&8.48&8.47& $-0.08\pm0.01$& $-0.18\pm0.01$\\
HIP 113896&8.74&8.75&8.73&8.54&8.57&8.55& $-0.04\pm0.01$& $-0.10\pm0.02$\\
HIP 113980&8.82&8.75&8.73&8.50&8.46&8.48& $-0.02\pm0.03$& $-0.17\pm0.01$\\
HIP 114034&8.95&8.95&8.87&8.59&8.61&8.58& $ 0.14\pm0.03$& $-0.06\pm0.01$\\
HIP 114210&9.01&8.93&8.92&8.66&8.59&8.62& $ 0.17\pm0.03$& $-0.03\pm0.02$\\
HIP 114354&8.70&8.67&8.67&8.41&8.41&8.43& $-0.10\pm0.01$& $-0.24\pm0.01$\\
HIP 114622&8.90&8.97&8.96&8.85&8.90&8.90& $ 0.16\pm0.04$& $ 0.23\pm0.03$\\
HIP 114729&8.80&8.66&8.69&8.48&8.39&8.44& $-0.07\pm0.05$& $-0.22\pm0.03$\\
HIP 114838&8.72&8.58&8.63&8.34&8.26&8.33& $-0.14\pm0.05$& $-0.34\pm0.03$\\
HIP 114856&8.78&8.70&8.76&8.41&8.37&8.44& $-0.04\pm0.03$& $-0.25\pm0.03$\\
HIP 114893&8.88&8.96&8.85&8.56&8.64&8.57& $ 0.11\pm0.05$& $-0.06\pm0.04$\\
HIP 114962&7.75&7.79&7.78&7.49&7.52&7.51& $-1.01\pm0.03$& $-1.15\pm0.02$\\
HIP 115012&8.84&8.84&8.80&8.63&8.66&8.64& $ 0.04\pm0.01$& $-0.01\pm0.02$\\
HIP 115066&8.97&8.89&8.91&8.83&8.77&8.79& $ 0.14\pm0.02$& $ 0.14\pm0.02$\\
HIP 115220&8.84&8.83&8.77&8.51&8.52&8.50& $ 0.03\pm0.02$& $-0.14\pm0.01$\\
HIP 115359&8.81&8.84&8.78&8.59&8.63&8.59& $ 0.03\pm0.02$& $-0.05\pm0.02$\\
HIP 115370&8.96&8.90&8.96&8.75&8.71&8.78& $ 0.16\pm0.03$& $ 0.09\pm0.03$\\
HIP 115604&8.93&8.91&8.88&8.78&8.76&8.75& $ 0.12\pm0.01$& $ 0.11\pm0.01$\\
HIP 115704&7.78&7.73&0.00&7.41&7.36&0.00& $-1.03\pm0.01$& $-1.27\pm0.02$\\
HIP 115714&8.85&8.85&8.75&8.60&8.60&8.55& $ 0.03\pm0.04$& $-0.07\pm0.02$\\
HIP 115721&8.78&8.71&8.79&8.51&8.47&8.55& $-0.02\pm0.04$& $-0.14\pm0.03$\\
HIP 115761&8.92&8.87&8.84&8.55&8.53&8.55& $ 0.09\pm0.02$& $-0.11\pm0.01$\\
HIP 116106&8.62&8.61&8.59&8.40&8.42&8.40& $-0.18\pm0.01$& $-0.25\pm0.01$\\
HIP 116421&8.79&8.77&8.75&8.53&8.53&8.52& $-0.01\pm0.01$& $-0.13\pm0.01$\\
HIP 116478&8.89&8.85&8.80&8.73&8.72&8.69& $ 0.08\pm0.02$& $ 0.07\pm0.01$\\
HIP 116616&8.80&8.82&8.79&8.55&8.59&8.59& $ 0.02\pm0.02$& $-0.08\pm0.02$\\
HIP 116727&8.91&9.01&9.06&8.72&8.82&8.88& $ 0.21\pm0.07$& $ 0.15\pm0.07$\\
HIP 116771&8.92&8.89&8.83&8.60&8.60&8.58& $ 0.10\pm0.03$& $-0.06\pm0.01$\\
HIP 117029&8.66&8.69&8.63&8.37&8.41&8.39& $-0.14\pm0.01$& $-0.27\pm0.02$\\
HIP 117484&8.97&8.94&8.83&8.64&8.63&8.57& $ 0.13\pm0.05$& $-0.04\pm0.03$\\
HIP 117582&8.70&8.65&8.63&8.42&8.39&8.40& $-0.12\pm0.02$& $-0.25\pm0.01$\\
HIP 117762&8.83&8.82&8.81&8.48&8.49&8.52& $ 0.04\pm0.01$& $-0.16\pm0.02$\\
HIP 117776&8.63&8.59&8.54&8.29&8.27&8.26& $-0.20\pm0.02$& $-0.38\pm0.01$\\
HIP 118010&8.85&8.85&8.83&8.65&8.65&8.64& $ 0.06\pm0.01$& $-0.01\pm0.01$\\
HIP 118115&8.84&8.83&8.79&8.66&8.66&8.64& $ 0.04\pm0.01$& $ 0.00\pm0.01$\\
HIP 118159&8.76&8.73&8.77&8.61&8.59&8.64& $-0.03\pm0.02$& $-0.04\pm0.02$\\
HIP 118162&8.71&8.78&8.78&8.59&8.65&8.66& $-0.03\pm0.04$& $-0.02\pm0.04$\\
HIP 118225&9.05&9.00&9.00&8.84&8.80&8.84& $ 0.23\pm0.01$& $ 0.17\pm0.02$\\

